Replication-proof Bandit Mechanism Design with Bayesian Agents

We study the problem of designing replication-proof bandit mechanisms when agents strategically register or replicate their own arms to maximize their payoff. Specifically, we consider Bayesian agents who only know the distribution from which their own arms' mean rewards are sampled, unlike the original setting of by Shin et al. 2022. Interestingly, with Bayesian agents in stark contrast to the previous work, analyzing the replication-proofness of an algorithm becomes significantly complicated even in a single-agent setting. We provide sufficient and necessary conditions for an algorithm to be replication-proof in the single-agent setting, and present an algorithm that satisfies these properties. These results center around several analytical theorems that focus on \emph{comparing the expected regret of multiple bandit instances}, and therefore might be of independent interest since they have not been studied before to the best of our knowledge. We expand this result to the multi-agent setting, and provide a replication-proof algorithm for any problem instance. We finalize our result by proving its sublinear regret upper bound which matches that of Shin et al. 2022.

==> ETC.tex <==
\section{Attempt - Stochastic Permutation Free}

The above theorem characterizes the sufficient condition for an algorithm to be replication-proof for any number of agents.
These characterizations allow us to deeply understand which types of properties suffice to make an algorithm replication-proof, however, it is often not easy to see that
Indeed, as we will see in the following section, it is tricky to check whether an algorithm satisfy SPF or not, since it requires us to compare all the tail probabilities of multiple bandit instances with different parameters.
Thus, in what follows, we directly prove that the combination of ETC and ETC in $\hbb$ admits the replication-proofness.

\begin{theorem}
	Let $\alg_1$ be ETC with arbitrary exploration parameter $M \ge m(\sum_{i=1}^l l_i)$, and $\alg_2$ be ETC with exploration parameter $m = \frac{2}{\Delta^2} (\max_il_i) \ln (2T)$.
	Then, $\hbb$ with $\alg_1$ and $\alg_2$ is replication-proof for any number of agents.
\end{theorem}
\begin{proof}
	We focus our attention to agent $i$.
	Index agent $i$'s arms by $1,2,\ldots, l$.
	We borrow the notations in the proof of Theorem~\ref{thm:spf_rp}.
	As per equation~\eqref{eq:04271244}, the conditional expected regret given permutation $\sigma$ and the realization $v$ can be written as follows.
	\begin{align}
		\sum_{\sigma \in S_l} 
		\CEx{U_i(\cS)}{\sigma, v}
		&=
		\parans{
		\sum_{\sigma \in S_l}
		\Ex{\Gamma_i^{\cS}(M,v)}
		}
		+
		\Ex{\Gamma_i^{\cS}(T-Mn,v)}
		\int_{0}^1
		p_i^{\cS}(y,v)
		\parans{
		\sum_{\sigma \in S_l}
		q_i^{\cS}(y,\sigma(v))
		}dy.\label{eq:05082043}
	\end{align}
	Note that it suffices to prove that $\sum_{\sigma \in S_l} 
		\CEx{U_i(\cO)}{\sigma, v} \ge \sum_{\sigma \in S_l} 
		\CEx{U_i(\cS)}{\sigma, v}$ for any strategy $\cS$.
	
	Let $\cS$ be agent $i$'s strategy with replication vector $r = (r_1,r_2,\ldots, r_l)$, with at least one coordinate being strictly positive.
	Without loss of generality, suppose $r_1 \ge r_2 \ge \ldots \ge r_l$, then we have $r_1 \ge 1$.
	This indeed brings no difference since the expected payoff is marginalized over all the possible permutations, as we see thus far.
	Let $\Omega_1$ be a set of permutation $\sigma \in S_l$ such that arm $\sigma(1) = 1$, \ie the best arm is replicated the most times, and define $\Omega_2 = S_l \setminus \Omega_1$.
	We handle case $\omega \in \Omega_1$ and $\omega \in \Omega_2$ separately.
	
	With the truthful strategy $\cO$, the last term $q_i^{\cO}(y,\sigma(v))$ in equation~\eqref{eq:05082043} can be written as follow.
	\begin{align*}
		q_i^{\cO}(y,\sigma(v))
		&=
		\Pr{\sum_{i=1}^l \Gamma_i^\cO(M,\sigma(v))}
	\end{align*}

\end{proof}


\section{ETC}
\paragraph{Note:} The algorithm assumes knowledge of the minimum gap between the arms $\min_{i \in [k]} \Delta_i$. 

\paragraph{Note:} Any algorithm which assumes knowledge of the minimum gap must also imply that the prior over the means is over a discrete support. For example, the prior has non-zero probability only over the set  over $\{0,0.2,0.4,0.6,0.8,1.0\} \subset [0,1]$. If that is not the case and we deal with continuous distributions instead, then it is possible in general to have two means such that the gap between them is arbitrarily small. 

Let $r$ be a realization of the means of the $l_i$ arms that have been samples from $D_i$. For this realization $r$, let $\Delta_r$ be the minimum gap between an optimal arm and a sub-optimal arm. Then define $\Delta=\min_{r \sim D_i} \Delta_r$. In words $\Delta$ is the minimum possible gap over all realizations. In the above example where the support of the distribution is $\{0,0.2,0.4,0.6,0.8,1.0\}$ then clearly $\Delta=0.2$. 


For now, we just do regret analysis for the following ETC algorithm:
\begin{algorithm}
Play each arm once for $m$ rounds.\\
Play the arm with the highest empirical mean for all remaining rounds. 
\caption{\textsc{ETC}}\label{alg:ETC}
\end{algorithm}

Let $n_i(T)$ be the total number of pulls for sub-optimal arm $i$, then we have the following theorem:
\begin{theorem}\label{th:ETC_main_th}
If $m=\frac{2}{\Delta^2} \ln{2T}$, then for a sub-optimal arm we have:
\begin{align}
\expect{n_i(T)} \leq m+1 = 1 + \frac{2}{\Delta^2} \ln{(2T)}
\end{align}
Further, the regret is upper bounded by:
\begin{align}
    R(T) \leq \sum_{i:\Delta_i>0} (m+1) \Delta_i \leq \sum_{i:\Delta_i>0} \Big( \frac{2 \ln{(2T)}}{\Delta^2} + 1 \Big)
\end{align}
\end{theorem}
\begin{proof}
For a sub-optimal arm $i$ we have: 
\begin{align*}
    \expect{n_i(T)} \leq m + (T-mk) \Pr{\hat{\mu}_i(m) \ge \hat{\mu}_{i^*}(m)} 
\end{align*}
Now we focus on upper bounding $\Pr{\hat{\mu}_i(m) \ge \hat{\mu}_{i^*}(m)}$: 
\begin{align}
    \Pr{\hat{\mu}_i(m) \ge \hat{\mu}_{i^*}(m)} &= \Pr{(\hat{\mu}_i(m) -\mu_i) + (\mu_{i^*} - \hat{\mu}_{i^*}(m)) \ge \Delta_i} \\ 
    & \leq \Pr{(\hat{\mu}_i(m) -\mu_i) \ge \frac{\Delta_i}{2}} + \Pr{(\mu_{i^*} - \hat{\mu}_{i^*}(m)) \ge \frac{\Delta_i}{2}} \\ 
    & \leq 2 \exp(- \frac{\Delta_i^2}{4} \frac{1}{2} \frac{1}{\frac{1}{4m}}) \ \ \ \ \  \text{(using sub-Gaussian tail concentration with $\sigma=\frac{1}{2}$ since rewards are in $[0,1]$)} \\
    & \leq 2\exp(- \frac{\Delta_i^2 m}{2})
\end{align}
Set $m=\frac{2}{\Delta^2} \ln{\frac{T}{c}}$ where $c$ is a constant to be determined. Now let us go back to upper bounding $\expect{n_i(T)}$: 
\begin{align}
       \expect{n_i(T)} & \leq m + (T-mk) \Pr{\hat{\mu}_i(m) \ge \hat{\mu}_{i^*}(m)} \\ 
       & \leq m + T (2)\exp(- \frac{\Delta_i^2 m}{2}) \\
       & \leq m + 2T  \exp(- \Big(\frac{\Delta_i}{\Delta}\Big)^2 \ln{\Big(\frac{T}{c}\Big)}) \\
       & \leq m+ 2T  \exp(- \ln{\Big(\frac{T}{c}\Big)}) \ \ \ \text{(since $\frac{\Delta_i}{\Delta} \ge 1$)} \\
       & = m + 2T \frac{c}{T} \\
       & = m + 1 \ \ \ \text{(by setting $c=\frac{1}{2}$)}
\end{align}
\note{Seyed: In the above we chose $c=\frac{1}{2}$, this was done out of convenience. }
\\ 
This proves the upper bound on $\expect{n_i(T)}$, now we prove the regret upper bound: 
\begin{align*}
    R(T) & \leq \sum_{i:\Delta_i>0} (m+1) \Delta_i \\ 
    & = \sum_{i:\Delta_i>0} (\frac{2}{\Delta^2} \ln{2T}+1) \Delta_i \\ 
    & \leq \sum_{i:\Delta_i>0} ( \frac{2\Delta_i}{\Delta^2} \ln{2T} + \Delta_i) \\ 
    & \leq \sum_{i:\Delta_i>0} ( \frac{2}{\Delta^2} \ln{2T} +1) \ \ \ \text{(since the rewards are in $[0,1]$, we have $\Delta_i\leq 1$)} 
\end{align*}
\end{proof} 


\subsection{The original conjecture using ETC}
Consider the following instances where $\mu_1 >\mu_2$ and the distributions can be random (not deterministic): 
\begin{enumerate}
    \item A: run ETC with instance $(\mu_1, \mu_2)$
    \item B: run ETC with instance $(\mu_1, \mu_2, \mu_1)$
    \item C: run ETC with instance $(\mu_1, \mu_2, \mu_2)$
\end{enumerate}

What we want to prove as stronger version of conjecture:
For any $x \in [0,T]$ ,
\begin{align*}
    \Pr{R_A < x} \le \frac{\Pr{R_B < x} + \Pr{R_C < x}}{2}
\end{align*}

\begin{theorem}
    Using the above ETC algorithm then we have $R_A \leq \frac{R_B+R_C}{2}$ if the horizon $T\ge 2$. 
    \note{Seyed: the horizon must always have at least two rounds so this is not restrictive at all.}
\end{theorem}
\begin{proof}
Using Theorem \ref{th:ETC_main_th} we clearly have: 
\begin{align}
    R_A \leq (m+1) \Delta_2 = m\Delta_2 + \Delta_2 
\end{align}
Since the algorithm always does $m$ many exploration rounds per arm we immediately have:
\begin{align}
    & R_B \ge m \Delta_2  \\
    & R_C \ge 2 m \Delta_2 
\end{align}
\end{proof}
This implies that: 
\begin{align}
    \frac{R_B+R_C}{2} \ge \frac{3}{2} m \Delta_2 = m\Delta_2 + \frac{1}{2} m\Delta_2 \ge  m\Delta_2 + \Delta_2  \ge R_A
\end{align}
where $m\Delta_2 + \frac{1}{2} m\Delta_2 \ge  m\Delta_2 + \Delta_2$ holds if $m\ge 2$. Since $m=2 \ln(2T)$ and we have at least two rounds $T\ge 2$, then $m\ge 2$. 

\paragraph{Note:} What made the above result easy to obtain is that ETC has a deterministic sub-process where each arm is always pulled $m$ times during exploration. Further, the above version of ETC has $m$ without any dependence on the number of existing arms $k$. 


==> aaai2025/reproduce.tex <==
\section*{Reproducibility Checklist}
Below we give the answers to the reproducibility checklist for this paper. 
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced: \textcolor{blue}{Yes}
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results:\textcolor{blue}{Yes}
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper: \textcolor{blue}{Yes}
    \item Does this paper make theoretical contributions? \textcolor{blue}{Yes}
    \item All assumptions and restrictions are stated clearly and formally. \textcolor{blue}{Yes}
    \item All novel claims are stated formally (e.g., in theorem statements). \textcolor{blue}{Yes}
    \item Proofs of all novel claims are included. \textcolor{blue}{Yes}
    \item Proof sketches or intuitions are given for complex and/or novel results. \textcolor{blue}{Yes}
    \item Appropriate citations to theoretical tools used are given. \textcolor{blue}{Yes}
    \item All theoretical claims are demonstrated empirically to hold. \textcolor{blue}{No}
    \item All experimental code used to eliminate or disprove claims is included. \textcolor{blue}{NA}
    \item Does this paper rely on one or more datasets? \textcolor{blue}{No}
    \item Does this paper include computational experiments? \textcolor{blue}{No}
\end{itemize}

==> abstract.tex <==
%Revised version
We study a problem of designing replication-proof bandit mechanisms when agents strategically register or replicate their own arms to maximize their payoff. 
We consider Bayesian agents who are unaware of ex-post realization of their own arms' mean rewards, which is the first to study Bayesian extension of~\cite{shin2022multi}. 
This extension presents significant challenges in analyzing equilibrium, in contrast to the fully-informed setting by~\cite{shin2022multi} under which the problem simply reduces to a case where each agent only has a single arm.
With Bayesian agents, even in a single-agent setting, analyzing the replication-proofness of an algorithm becomes complicated.
Remarkably, we first show that the algorithm proposed by~\cite{shin2022multi}, defined H-UCB, is no longer replication-proof for any exploration parameters.
Then, we provide sufficient and necessary conditions for an algorithm to be replication-proof in the single-agent setting.
These results centers around several analytical results in comparing the expected regret of multiple bandit instances, which might be of independent interest. 
We further prove that exploration-then-commit (ETC) algorithm satisfies these properties, whereas UCB does not, which in fact leads to the failure of being replication-proof.
We expand this result to multi-agent setting, and provide a replication-proof algorithm for any problem instance.
The proof mainly relies on the single-agent result, as well as some structural properties of ETC and the novel introduction of a restarting round, which largely simplifies the analysis while maintaining the regret unchanged (up to polylogarithmic factor).
We finalize our result by proving its sublinear regret upper bound, which matches that of H-UCB.


%%%% Seyed Edits 
%We study the problem of designing replication-proof bandit mechanisms when agents strategically register, or even replicate, their own arms to maximize payoff.
%We consider Bayesian agents who is oblivious to the ex-post realization of their own arms, which is the first to study Bayesian extension of \cite{shin2022multi}.
%%This extension
%%Compared to the fully informed agent of \cite{shin2022multi}, the Bayesian agent cannot cherrypick its own best arm, but instead computes the expected rewards over the realization of rewards, and plays a strategy that maximizes ex-ante payoff \note{Seyed - previous sentence could be improved, maybe keep it high-level}.
%This extension introduces significant challenges in analyzing replication-proof algorithms, compared to the single-agent setting under which the problem simply reduces to the case where each agent only has a single arm.
%% \note{Seyed- change to something like even the single agent case in the Bayesian setting is not trivial as the problem cannot be reduced to to the case where each agent only has a single arm}
%Notably, analyzing the replication-proofness of an algorithm is not straightforward even in a single-agent setting.
%We first show that, surprisingly, H-UCB proposed by \cite{shin2022multi} is no longer replication-proof.
%On the positive side, we first provide sufficient conditions under which an algorithm is replication-proof for a single-agent setting, and further prove that exploration-then-commit (ETC) satisfies these properties.
%At the heart of this analysis, we provide several analytical results in comparing the expected regret of multiple bandit instances, which might be of independent interest.
%For the multi-agent setting, we introduce a variant of H-UCB, named \textsc{Hierarchy with Restart}, and prove its replication-proofness.
%Our proof is based on the algebraic properties of ETC as well as the introduction of restarting round which largely simplifies the analysis by removing the correlation between the rounds.
%
%For the multi-agent setting, we present a slightly stronger condition that makes it sufficient for any algorithm to be replication-proof, once it runs as a sub-module of a two-stage hierarchical algorithms with first-stage being ETC. \note{Seyed - previous sentence: I think that part (b) would effect thi sentence. I think it might be best to remove it.}
%We further show that such a hierarchical algorithm equipped with ETC and ETC essentially satisfies replication-proof, while maintaining sublinear regret. \note{Seyed - previous sentence: (1) I think you should give an idea of what hierarchical means. Say something like a Bandit alg is applied over the arms of each aget and another over the agents with the rewards of all of their pulled arms aggregated. (2) ``ETC and ETC'': I think it's not clear, maybe something like both levels of the heirachcal algorithm use ETC.}

%%%%% Original abstract 
% We study a problem of designing replication-proof bandit mechanism when agents strategically register, or even replicate, their own arms to maximize payoff, where each agent is oblivious the ex-post realization of its own arms' parameters.
% Compared to the fully informed agent of \cite{shin2022multi}, the Bayesian agent cannot cherrypick its own best arm, but instead computes the expected rewards over the realization of rewards, and plays a strategy that maximizes ex-ante payoff.
% This introduces significant challenges in analyzing replication-proof algorithm, compared to the single-agent setting under which the problem simply reduces to the case where each agent only has a single arm.
% Notably, analyzing a replication-proofness of an algorithm is not straightforward even in a single-agent setting.
% We first show that, surprisingly, H-UCB (and RH-UCB) proposed by \cite{shin2022multi} is no more replication-proof, due to UCB's deterministic and adaptive exploration, based on the observation that UCB is not replication-proof even in the single agent setting.
% On positive sides, we first provide sufficient conditions under which an algorithm is replication-proof for a single-agent setting, and further prove that exploration-then-commit (ETC) satisfies these properties.
% For the multi-agent setting, we present a slightly stronger condition that makes sufficient for an algorithm replication-proof, once it runs as a submodule of a two-stage hierarchical algorithms with first-stage being ETC.
% We further show that such a hierarchical algorithm equipped with ETC and ETC essentially satisfies replication-proof, while maintaining sublinear regret.
% At the heart of our analysis, we provide several analytical results in comparing the expected regret of multiple bandit instances, which might be of independent interest.





==> approach.tex <==
\section{Some notes on the analysis}
\suho{below are some approaches that we've tried, most of which are not working.}

\suho{it basically is very hard to directly dealing with failure probability of algorithm equipped with ETH style submodule.}
Currently, what we are thinking of is to compare two strategies. one of which is to register all arms without any replications; and the other is to register all arms and also register a random replicated arm.

In order to do so, we have to compare the reward we get in exploitation phase of these two strategies (expected reward in exploration phase is clear). In exploitation phase, we always take the arm that has given us the best sum of rewards in the exploration phase. Since we take each arm exactly $N$ times in exploration, and we assume that rewards come from Bernoulli distributions, then the sum of rewards come from a Binomial distribution. So we have several Binomial random variables and our goal is to analyze the \textbf{argmax} of these variables.

\begin{observation}
if we have $k$ i.i.d random variables $X_1, X_2, ..., X_k$ as our Binomial random variables ($X_i \sim \text{Binomial}(\mu_i, N)$), then the probability that $X_i$ is the maximum of all those random variables is equal to:
$$
\sum_{x=0}^N \mathbb{P}\left[X_i=x\right] \prod_{j\neq i} \mathbb{F}_{X_j}(x)
$$
\end{observation}

Finding exact probabilities is hard. In order to compare those two strategies, we need find both upper-bounds and lower-bounds on the probability that each arm is chosen as the maximum arm. So, we need to have a lower-bound and an upper-bound for this value:
$$
\text{LB} \leq \prod_x \mathbb{F}_{X_i}(x) \leq \text{UB}.
$$

based on this
\href{https://math.stackexchange.com/questions/2673745/bounding-the-probability-of-one-binomial-r-v-greater-than-another?noredirect=1&lq=1}{link},
we can find an upper-bound on the probability that $X_i$ is bigger than $X_{*}$ (random variable corresponds to optimal $\mu_{*}$). Therefore, we can find an upper-bound on the probability that $X_i$ is the maximum among all random variables.
\begin{observation}
The probability that the sub-optimal r.v. $X_i$ is taken as the maximum r.v. is bounded by:
$$\mathbb{P}\left[X_i\ \text{is the maximum r.v.}\right] \leq e^{-\frac{N (\mu_{*} - \mu_i)^2}{2}}$$
\end{observation}

This bound is not tight :(



==> attempt-nonadaptiveexploration.tex <==
\section{Attempt - Permutation-free}

To this end, we first introduce a stochastic ordering between a random variable, which will play a crucial role in analyzing replication-proofness of an algorithm.
We write $\Z_0$ and $\R_0$ to denote the set of nonnegative integers and real numbers, respectively.
\begin{definition}[Stochastic dominance]
	For any two random variable, we define a version of (first-order) stochastic dominance as follows: for any two nonnegative random variables $X$ and $Y$, we write $X \succ_{sd} Y$ if $\Pr{X < x} < \Pr{Y < x}$ for any $x \in \R_0$.\footnote{Note that this slightly different from the standard definition of first-order stochastic dominance.}
\end{definition}

\begin{definition}[Group-wise Stochastic dominance]
	For any two set of random variables $\cX = \{X_1,\ldots, X_n\}$ and $\cY = \{Y_1,\ldots, Y_m\}$, we say that $\cX$ is group-wise stochastic dominant over $\cY$, $\cX \succ_{gsd} \cY$, if $\sum_{i=1}^n\Pr{X_i < x}/n < \sum_{i=1}^n \Pr{Y_i < x}/m$ for any $x \in R_0$.
\end{definition}


Stochastic ordering effectively allows us to reasonable compare two random variables, and will shed light on the construction of a replication-proof algorithm.
Note that this is more strict notion of ordering compared to the dominance with respect to the expectation of the random variables.



We now introduce the following notion of permutation-freeness, which will be the core of our analysis.
\begin{definition}[Permutation-free]
	Consider a standard bandit instance $\cI$ with mean rewards $\mu_1 \ge \ldots \ge \mu_l$.
	For any $x=(x_1,\ldots, x_l)\in \Z_0^l$, let $\cI_x$ be a bandit instance such that arm $i$ is replicated $x_i$ times for $i \in [l]$ from $\cI$.
	Then, a regret of an algorithm is \emph{stochastically schur-concave} if for any $x,y\in \Z_0^l$ such that $x \prec y$, the algorithm satisfies the following properties for any $T \ge 1$.
	\begin{align}\label{eq:spf}
		\{\reg_{\cI_{\sigma(x)}}\}_{\sigma \in S_l}
		\prec_{gsd}
		\{\reg_{\cI_{\sigma(y)}}\}_{\sigma \in S_l},
	\end{align}
	where $\sigma:[l] \mapsto [l]$ denotes a permutation and $S_l$ denotes the set of all permutations.
	If it satisfies
	\begin{align}
		\sum_{\sigma \in S_l}\reg_{\cI_{\sigma(x)}}/|S_l| \le \sum_{\sigma \in S_l}\reg_{\cI_{\sigma(y)}}/|S_l|,
	\end{align}
	then we say that the algorithm is \emph{schur-concave}.

\end{definition}


\section{Attempt - Deriving Permutation-free Algorithms}

\note{Possible further contents: (i) lower bound. (i) approximate equilibrium some corresponding trivial solutions}

\begin{theorem}
	$\eps_t$-greedy is stochastically schur-concave in the deterministic setting.
\end{theorem}
\begin{proof}
	\note{TBD - Compare strategy $v_1$ and $v_2$ with hamming distance $1$, and applies robin-hood operation to prove its schur-concavity.}
\end{proof}

\begin{conjecture}
	$\eps_t$-greedy is stochastically schur-concave.
\end{conjecture}
\begin{proof}
	\note{No clear idea yet, but sth similar to induction argument above may apply}	
\end{proof}

\begin{theorem}
	ETC is schur-concave.	
\end{theorem}

\begin{conjecture}
	ETC is stochastically schur-concave.	
\end{conjecture}


\section{Attempt - Non-adaptive Exploration}


\paragraph{Beyond exploration-then-commit}
TBD...



\begin{conjecture}
	Any UCB-like (deterministic, adaptively exploring) algorithm is not replication-proof.
\end{conjecture}
\begin{proof}
	\note{I feel that this is correct, but it seems not easy to formalize - not quite sure whether it would be worth pursuing.}
\end{proof}


\begin{definition}[Exploration and exploitation round]
	A round $t$ is exploration round if the action $a_t$ and feedback $r_t$ at this round is used by the algorithm in the future rounds, and the choice of action $a_t$ does not depend on the reward history $r_{t'}$ for $t' < t$.
	If a round is not exploration round, then we call it an exploitation round.
\end{definition}

\begin{definition}[Non-adaptive exploration, \cite{slivkins2019introduction}]
	A (possibly randomized) algorithm has \emph{non-adaptive exploration} if the set of all exploration rounds and corresponding algorithm's decision is fixed in advance, given the random bits of the algorithm, 
\end{definition}

Representative examples of algorithms with non-adaptive exploration are $\eps$-greedy and exploration-then-commit (ETC).
ETC consists of two phases where in the first phase the algorithm explores all the arms for some given number of times, in a round-robin or randomly permuted manner.
Then, it computes the empirically best arm, and enters the exploitation phase which always pull the chosen arm with the highest empirical average reward during the exploration phase.
On the other hand, $\eps$-greedy tosses a biased coin with parameter $\eps$, and if it outputs head with probability $\eps$, then it explores an arm in an equally like manner, otherwise if it realizes head, then it exploits by selecting an empirically best arm computed thus far.
It is easy to check that both algorithms have non-adaptive exploration structure.

\begin{definition}[Monotone]
	An algorithm is monotone if it selects the arm with the highest empirical average reward in the exploitation phase, unless it has unexplored arms, where it chooses those arms.
\end{definition}

Now we introduce a slightly stronger version of SPF, defined as follows.
\begin{definition}[Uniformly SPF]
	We say that an algorithm is uniformly stochastic permutation-free if \note{TBD - permutation-freeness holds for round-wise manner.}
\end{definition}



\begin{theorem}
	Let $\alg_1$ be monotone algorithm with non-adaptive exploration, and $\alg_2$ be uniformly SPF.
	Then, running $\hbb$ with $\alg_1$ and $\alg_2$ satisfies replication-proofness.
\end{theorem}
\begin{proof}
	We again start with the following expressions in \eqref{eq:04262152}.
	\begin{align*}
		u^{\cS_i}_i(T)
		=
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 \le v_1}\ldots \int_{\mu_k = v_l\le v_{l-1}} 
		\sum_{\sigma \in S_l}\Ex{U^{\cS_i}_i(T) \ |\ \sigma(v)_1,\ldots, \sigma(v)_l}g(v)dv.
	\end{align*}
	We simply write $\CEx{U^{\cS_i}_i(T) }{\sigma, v}$ to denote the term inside the summation
%	, and overwrite $u_i(T)$ and $U_i(\cS ,T)$ to denote the ex-ante and ex-post utility of agent playing $\cS$ given the time horizon $T$.
	Overall, we will prove that given a fixed realization $v$, we have
	\begin{align*}
		\sum_{\sigma \in S_l}\CEx{U^{\cO_i}_i(T)}{\sigma, v}
		\ge
		\sum_{\sigma \in S_l}\CEx{U^{\cS_i}_i(T)}{\sigma, v},
	\end{align*}
	for any strategy $\cS$ and time horizon $T$.
	Our proof will be based on the induction technique with respect to $T$.
	
	\paragraph{Base case $T = 1$}
	\note{TBD - Easy}
	
	\paragraph{Induction step}
	Suppose $u^{\cO_i}_i(T) \ge u^{\cS_i}_i(T)$ for any strategy $\cS_i$ for some given $T$.
	We will prove that $u^{\cO_i}_i(T+1) \ge u^{\cO_i}_i(T+1)$.
	We write $\gamma_i(\cS_i, t)$ to denote the reward of agent $i$ at round $t$, and $N_i(\cS, t)$ to denote the number of rounds that agent $i$ is selected after the round $t$ ends.
	We also write $\muhat^{\cS_i}_i(t)$ to denote agent $i$'s empirical average reward after round $t$ ends.
	We can expand
	\begin{align*}
		u^{\cS_i}_i(T+1)
		&=
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 \le v_1}\ldots \int_{\mu_k = v_l\le v_{l-1}} 
		\sum_{\sigma \in S_l}\Ex{U^{\cS_i}_i(T+1)\ |\ \sigma(v)_1,\ldots, \sigma(v)_l}g(v)dv
		\\
		&=
		u^{\cS_i}_i(T) + \int_{\mu_1 = v_1} \int_{\mu_2 = v_2 \le v_1}\ldots \int_{\mu_k = v_l\le v_{l-1}} 
		\sum_{\sigma \in S_l}\Ex{\gamma^{\cS_i}_i(T+1)\ |\ \sigma(v)_1,\ldots, \sigma(v)_l}g(v)dv
	\end{align*}
	We focus on the latter part in RHS.
	We can decompose the term inside the summation as follows.
	\begin{align*}
		\CEx{\gamma^{\cS_i}_i(T+1)}{\sigma, v}
		&=
		\sum_{x \in \N_0}\CEx{\gamma^{\cS_i}_i(T+1)}{\sigma, v, N^{\cS_i}_i(T) = x}\CPr{N^{\cS_i}_i(T) = x}{\sigma, v}.
	\end{align*}
	Thus, we can obtain
	\begin{align*}
		\sum_{\sigma \in S_l}\Ex{\gamma^{\cS_i}_i(T+1)\ |\ \sigma(v)_1,\ldots, \sigma(v)_l}
		&=
		\sum_{\sigma \in S_l}
		\sum_{x \in \N_0}\CEx{\gamma^{\cS_i}_i(T+1)}{\sigma, v, N^{\cS_i}_i(T) = x}\CPr{N^{\cS_i}_i(T) = x}{\sigma, v}
		\\
		&=
		\sum_{x \in \N_0}
		\sum_{\sigma \in S_l}\CEx{\gamma^{\cS_i}_i(T+1)}{\sigma, v, N^{\cS_i}_i(T) = x}\CPr{N^{\cS_i}_i(T) = x}{\sigma, v}
	\end{align*}

	
	We first prove the following claim.
	\begin{claim}\label{cl:number_dom}
		Fix any realization of the arms' parameters $v$ of agent $i$.
		For any strategy $\cS_i$, the random variable $N_i(\cO, t)$ group-wise stochastically dominates $\{N_i(\cS,t) | \sigma\}_{\sigma \in S_l}$, \ie
		\begin{align*}
			\sum_{\sigma \in S_l}\CPr{N^{\cO_i}_i(t) \ge x}{\sigma, v}
			\ge
			\sum_{\sigma \in S_l}\CPr{N^{\cS_i}_i(t) \ge x}{\sigma, v}.
		\end{align*}
	\end{claim}
	\begin{proof}
		\note{SHOULD CONSIDER PERMUTATION!!}
		We again proceed by induction argument.
		If $t=1$, regardless of whether it is exploration or exploitation phase in $\alg_1$, it chooses the agent given some tie-breaking rule (or initialization rule).
		Hence, it simply implies $N_i(\cO_i, 1) = N_i(\cS_i, 1)$.
		
		Suppose that $N^{\cO_i}_i(t-1) \succ  N^{\cS_i}_i(t-1)$ for some $t \ge 2$.
		If round $t$ is exploration phase in $\alg_1$, then the probability that $\alg_1$ chooses agent $i$ remains the same for any strategy of agent $i$ since the agent selection process is independent from the history of the agent, but only depends on the configuration of the agent-wise bandit instance, \ie the number of agents and their indices.
		Now suppose that round $t$ is exploitation phase.
		Note that the random variable $N^{\cS_i}_i(t)$ can be decomposed as follows.
		\begin{align*}
			\CPr{N^{\cS_i}_i(t) \ge x}{\sigma, v}
			&=
			\sum_{y=1}^{t-1}\CPr{N^{\cS_i}_i(t) \ge y}{N^{\cS_i}_i(t-1) = y, \sigma, v} \CPr{N^{\cS_i}_i(t-1) = y}{\sigma, v}
			\nonumber
			\\
			&=
			\sum_{y=x-1}^{t-1}
			\CPr{N^{\cS_i}_i(t) \ge x}{N_i(\cS_i,t-1) = y, \sigma, v} \CPr{N^{\cS_i}_i(t-1) = y}{\sigma, v}
			\nonumber
		\end{align*}
		where the second equality follows from the fact that if $y \le x-2$, then $N_i(\cS_i, t) \ge x$ cannot hold.
		Note that the RHS can be further decomposed as follows.
		\begin{align}
			\underbrace{\CPr{\hat{i}_t = i}{N^{\cS_i}_i( t-1) = x-1, \sigma, v}\CPr{N^{\cS_i}_i(t-1)=x-1}{\sigma, v}}_{A_i^{\cS_i}}
			+
			\sum_{y=x}^{t-1}\CPr{N^{\cS_i}_i(t-1) = y}{\sigma, v},
			\label{eq:05022158}	
		\end{align}

		Now we focus on the first term in RHS, which we denote by $A_i^{\cS_i}(t)$.
		For simplicity, we write $\Pru{x-1}{X}$ to denote $\CPr{X}{N^{\cS_i}_i(t-1) = x-1,\sigma, v}$ for any random variable $X$.
		Then, we can further obtain
		\begin{align*}
			A_i^{\cS_i}(t)
			&=
			\parans{\int_{z \in [0,1]}\Pru{x-1}{\muhat^{\cS_i}_i(t-1) \ge z}\Pru{x-1}{\max_{\cN \ni j \neq i}\muhat_j(\cS_j, t-1) = z}dz}
			\Pr{N_i(\cS_i, t-1) = x-1}.
		\end{align*}
		Note that in fact we have
		\begin{align*}
			\Pru{x-1}{\muhat_i(\cS_i, t-1) \ge z} 
			&= 
			\Pru{x-1}{\muhat_i(\cS_i, t-1)(x-1) \ge z(x-1)}
			\\
			&=
			\CPr{U_i(\cS_i, t-1) \ge z(x-1)}{N_i(\cS_i, t-1) = x-1}.
		\end{align*}
		Observe that the distribution of $U^{\cS_i}_i(t-1)$ conditioned on the realization of $N^{\cS_i}_i(t-1) = x$ is exactly the same as the distribution of agent $i$'s utility under the single agent setting with time horizon $x$.
		\note{correct?.. seems not! there is correlation between $N_i$ and $U_i$, which needs to be handled. }
		Hence, from the fact that $\alg_2$ satisfies SPF, we obtain the following inequality
		\begin{align*}
			\CPr{U_i(\cO_i, t-1) \ge z(x-1)}{N_i(\cS_i, t) = x-1}
			\ge
			\sum_{\sigma \in S_{l_i}}\CPr{U_i(\cS_i, t-1) \ge z(x-1)}{N_i(\cS_i, t) = x-1} / |S_{l_i}|
		\end{align*}

		
		we know that $U_i(\cS_i, t)$ conditioned on the specific value of $N_i(\cS_i, t)$ is stochastically dominated by $U_i(\cO_i, t)$ conditioned on the same event.
		This implies that
		\begin{align*}
			\Pru{x-1}{\muhat_i(\cS_i, t-1) \ge z}
			\ge
			\Pru{x-1}{\muhat_i(\cS_i, t-1) \ge z},
		\end{align*}
		for any strategy $\cS_i$.
		Note also that $\Pru{x-1}{\max_{\cN \ni j \neq i}\muhat_j(\cS_j, t-1) = z}$ in $A_i^{\cS_i}(t)$ remains the same regardless of the strategy $\cS_i$.
		Combined with our induction assumption, we conclude that $A_i^{\cO_i}(t) \ge A_i^{\cS_i}(t)$ for any $t$ and $\cS_i$.
		\note{expand more on this.}
		Again due to the induction assumption, we also have
		\begin{align*}
			\sum_{y=x}^{t-1}\Pr{N_i(\cO_i,t-1) = y} 
			&=
			\Pr{N_i(\cO_i,t-1) \ge x} 
			\\
			&\ge
			\Pr{N_i(\cS_i,t-1) \ge x} 
			\\
			&=
			\sum_{y=x}^{t-1}\Pr{N_i(\cS_i,t-1) = y}.
		\end{align*}
		Putting back to \eqref{eq:05022158}, we finish the proof.
	\end{proof}
	Due to the claim above, it suffices to show that
	\begin{align*}
		\sum_{x \in \N_0}\underbrace{\CEx{\gamma_i(\cO_i, T+1)}{\sigma, v, N_i(\cS_i, T) = x}}_{(a)}
		\ge
		\sum_{x \in \N_0}\CEx{\gamma_i(\cS_i, T+1)}{\sigma, v, N_i(\cS_i, T) = x},
	\end{align*}
	for any $\cS_i$ and $T$.
	Note further that the quantity inside the summation, (a), can be decomposed as follows
	\begin{align*}
		(a)
		&=
		\CEx{\gamma_i(\cO_i, T+1)}{\sigma, v, N_i(\cS_i, T) = x, \text{$i$ is selected at $T+1$}}\cdot \Pr{\text{$i$ is selected at $T+1$}}
		\\
		&+
		\CEx{\gamma_i(\cO_i, T+1)}{\sigma, v, N_i(\cS_i, T) = x, \text{$i$ is not selected at $T+1$}}\cdot \Pr{\text{$i$ is not selected at $T+1$}}
		\\
		&=
		\underbrace{\CEx{\gamma_i(\cO_i, T+1)}{\sigma, v, N_i(\cS_i, T) = x, \text{$i$ is selected at $T+1$}}}_{(b)}\cdot \underbrace{\Pr{\text{$i$ is selected at $T+1$}}}_{(c)},
	\end{align*}
	since if $i$ is not selected then its instant reward will be zero.
	
	For the probability $(c)$, we can rewrite
	\begin{align*}
		(c) 
		= 
		\parans{\int_{z \in [0,1]}\Pru{x-1}{\muhat_i(\cS_i, T) \ge z}\Pru{x-1}{\max_{\cN \ni j \neq i}\muhat_j(\cS_j, T) = z}dz},
	\end{align*}
	and similar to the proof of Claim~\ref{cl:number_dom}, we can conclude that $(c)$ under $\cO$ is at least that under $\cS$.
	
	Furthermore, for the conditional expectation $(a)$, we proceed with the following claim.
	\begin{claim}
		Consider a single agent	setting with agent $i$.
		For any round $t\ge 1$, Agent $i$'s expected reward at that round under $\cO_i$ is at least the average of expected reward that under $\cS_i$.
	\end{claim}
	\begin{proof}
		\note{Due to the definition of uniformly SPF}
	\end{proof}
	Observe that the quantity $(c)$ is exactly the same with the expected reward at round $T+1$ under the single agent setting with agent $i$.
	Hence, by the above claim and our observation on $(c)$, we conclude that 



%	Note however that this quantity is exactly the total reward of the single-agent problem when the arms have parameters $\sigma(v)_1, \sigma(v)_2, \ldots, \sigma(v)_l$ under the algorithm $\alg_2$ due to our hierarchical nature of $\hbb$.
\end{proof}


	
%	
%	Note that $p_i^{\cS'}(y,v)$ is monotone decreasing over $y$ and $\sum_{\sigma \in S_l}
%		q_i^{\cS'}(y,v)$ is monotone increasing over $y$ since each element $q_i^{\cS'}(y,v)$ is monotone increasing over $y$.
%	Namely, $p_i^{\cS'}(y,v)$ and $\sum_{\sigma \in S_l}
%		q_i^{\cS'}(y,v)$ are negatively correlated.
%	Now we use the following correlation inequality, called \emph{Fortuin-Kasteleyn-Ginibre} (FKG) inequality.
%	\begin{lemma}[\cite{alon2016probabilistic}]
%		Let $\nu_1, \ldots, \nu_n$ be a probability measure on $\R$.
%		If functions $f,g: \R^n \mapsto [0,1]$ are monotone decreasing and increasing functions over $\nu$, respectively, then $\Exu{\nu}{f \cdot g} \le \Exu{\nu}{f}\Exu{\nu}{g}$.
%	\end{lemma}
%	Using FKG inequality, we can further expand \eqref{eq:04271244} as follows.
%	\begin{align*}
%		\CEx{U_i(\cS')}{\sigma, v}
%		&\le
%		\parans{
%		\sum_{\sigma \in S_l}
%		\Ex{\Gamma_i^{\cS'}(M,v)}
%		}
%		+
%		\Ex{\Gamma_i^{\cS'}(T-Mn,v)}
%		\parans{
%		\sum_{y \in [0,1]}
%		p_i^{\cS'}(y,v)
%		}
%		\parans{
%		\sum_{y \in [0,1]}
%		\sum_{\sigma \in S_l}
%		q_i^{\cS'}(y,v)
%		}.
%	\end{align*}
%	Note that $\sum_{y \in [0,1]}q_i(y) = \int_{y}\Pr{\muhat_i(M) \ge y}dF_y(y) = \Ex{\Gamma_i(M)}$.
%	Recall that we have fixed $v = (v_1,\ldots, v_l)$ to obtain the results so far.
%	
%	Now, to cope with the exact value of expected utility, we again write $\Gamma_i^{v}(M), p_i^v(y), q_i^v(y)$ to denote the values obtained so far, assuming that agent $i$'s arms' parameters are fixed to be $v$.
%	Then, putting back to equation~\eqref{eq:04262152}, we finally obtain
%	\begin{align*}
%		u_i(\cS)
%		&=
%		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 \le v_1}\ldots \int_{\mu_k = v_l\le v_{l-1}} 
%		\sum_{\sigma \in S_l}\Ex{U_i(\cS)\ |\ \sigma(v)_1,\ldots, \sigma(v)_l}g(v)dv
%		\\
%		&\le
%		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 \le v_1}\ldots \int_{\mu_k = v_l\le v_{l-1}} 
%		\sum_{\sigma \in S_l}\parans{\Ex{\Gamma_i^v(M)} + \sum_{y \in [0,1]}p_i(y) \Ex{\Gamma_i^v(M)}}g(v)dv
%		\\
%		&\le
%		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 \le v_1}\ldots \int_{\mu_k = v_l\le v_{l-1}} 
%		\sum_{\sigma \in S_l}\parans{\Ex{\Gamma_i^v(M)} + \sum_{y \in [0,1]}p_i(y) \Ex{\Gamma_i^v(M)}}g(v)dv
%	\end{align*}







%	
%	\begin{align*}
%		u_i(\cS) 
%		&=
%		\Ex{v_i(\cS)}
%		\\
%		&=
%		\sum_{j \in \cN}\sum_{x \in [0,1]}\CEx{v_i(\cS)}{i^* = j , \muhat_i(M) = x}\Pr{i^* = j,\muhat_i(M) = x}
%		\\
%		&=
%		\sum_{j \in \cN}\sum_{x \in [0,1]}\CEx{v_i(\cS)}{i^* = j , \muhat_i(M) = x}\Pr{i^* = j,\muhat_i(M) = x}
%		\\
%		&=
%		\CEx{v_i(\cS)}{i^* = i}\Pr{i^* = i} + \sum_{\cS \ni j \neq i}\CEx{v_i(\cS)}{i^* = j}\Pr{i^* = j}
%		\\
%		&=
%		\CEx{v_i(\cS)}{i^* = i}\Pr{i^* = i} + \sum_{\cS \ni j \neq i}\CEx{v_i(\cS)}{i^* = j}\Pr{i^* = j}
%	\end{align*}



%
%
%
%\begin{definition}[Mean-based monotone algorithm]
%	A bandit algorithm is \emph{mean-based monotone} if  at each round, it selects an arm $a$ based on its empirical average $\hat{\mu}_a$ and the number of times that it is pulled $n_a$, and for any $t \in [T]$, $\Pr{a_t = a}$ is nondecreasing on $\mu_a$ where $a_t$ denotes the arm selected at round $t$.
%\end{definition}
%
%\note{Mohammad: merge into a big single theorem/proof, instead of decomposing it.}
%\begin{theorem}
%	Given any (possibly randomized) mean-based monotone $\alg_1$ and permutation free $\alg_2$, H-BlackBox with $\alg_1$ and $\alg_2$ is replication-proof.
%\end{theorem}
%\begin{proof}
%	Let $\cS_0$ be the truthful strategy and $\cS$ be any strategy with replication.
%	\note{this is not a single random variable}
%	\begin{claim}
%		\begin{align*}
%			\Pr{R^{\cS}_T(i) \ge x | N_T^{\cS}(i) = t}
%			\ge
%			\Pr{R^{\cS'}_T(i) \ge x | N_T^{\cS'}(i) = t}	
%		\end{align*}
%		\note{This will be based on schur-concavity, similar to single-agent case.}
%	\end{claim}
%
%	\begin{claim}
%		$\Pr{N^{\cS}_t(i) \ge x} \ge \Pr{N^{\cS'}_t(i) \ge x}$ for any rounds $t \in [T]$ and any $x \in \N_0$.
%		\note{this will essentially builds upon the previous claim, and the nature of Phase 1.}
%	\end{claim}
%	
%	\begin{claim}
%		We also have
%		\begin{align*}
%			\Ex{R^{\cS}_T(i) | N_T^{\cS}(i) = t}
%			\ge
%			\Ex{R^{\cS'}_T(i) | N_T^{\cS'}(i) = t}
%		\end{align*}
%		\note{This will be a corollary of Claim 4.10}
%	\end{claim}
%
%	
%	\begin{claim}
%		We can finally decompose
%		\begin{align*}
%			\Ex{R^{\cS}_T(i)}
%			=	
%			\sum_{i=t}^T\Ex{R^{\cS}_T(i) | N_T^{\cS}(i) = t}\Pr{N_T^{\cS}(i) = t},
%		\end{align*}
%		and it completes the proof by the above claims, combined with some algebraic manipulations.
%	\end{claim}
%
%\end{proof}


% \subsection{Beyond the permutation-freeness}
% \note{I think the above notion of permutation-freeness is sufficient for replication-proofness. But, it will be of independent interest if we can prove more general properties of schur-concavity as below.}
% Next, we introduce a partial ordering over a set of multi-dimensional vectors, and present the notion of schur-concavity of an algorithm.
% \begin{definition}[Majorization]
% 	For two $l$-dimensional real vectors $x,y \in \R^l$, $x$ majorizes $y$ if $\sum_{i=1}^s x_{(i)} \ge \sum_{i=1}^s y_{(i)}$ for $s \in [l]$, where $x_{(i)}$ denotes the $i$-th largest element in $x$, and denote by $x \succ_m y$.
% \end{definition}

% \begin{definition}[Schur-concavity]
% %	Let $x,y$ be any two $k$-dimensional vectors such that $x \succ y$.
% 	Consider a standard bandit instance $\cI$ with mean rewards $\mu_1 \ge \ldots \ge \mu_l$.
% 	For any $x=(x_1,\ldots, x_l)\in \Z_0^l$, let $\cI_x$ be a bandit instance such that arm $i$ is replicated $x_i$ times for $i \in [l]$ from $\cI$.
% 	Then, a regret of an algorithm is \emph{schur-concave} if for any $x,y \in \Z_0^l$ with $y \succ_m x$, the algorithm satisfies the following for any $T \ge 1$,
% 	\begin{align}\label{eq:schur}
% 		\{\reg_{\cI_{\sigma(x)}}\}_{\sigma \in S_k}
% 		\prec_{gsd}
% 		\{\reg_{\cI_{\sigma(y)}}\}_{\sigma \in S_k},
% 	\end{align}
%         \note{$l$ instead of $k$}
% 	where $\sigma:[l] \mapsto [l]$ denotes a permutation and $S_l$ denotes the set of all permutations.
% \end{definition}


==> attempt_reward_desired.tex <==



\section{Attempt: Reward Desired Behaviour} 
\begin{algorithm}
  \SetAlgoLined
  Parameter $N_0$; \\
  \For{$i=1,\ldots, K$}{
        For each agent $i$, pull his arms $N_0$ times in a cyclical manner; (total of $N_0$ pulls per agent) \\
  } 
  Pull each agent $i$ for a number of rounds equal to $N_i=\max_{j \in \set{S}_i} n_j$ where $n_j$ is the pulls received by arm $j$ in the exploration phase. \\
  Select empirically best arm (\textcolor{blue}{according to the exploration phase if it has been explored enough}) and pull it for the remaining rounds
 \caption{Agentwise-Exploration-then-Commit-with-Rewards}\label{alg:agent_explore_comm}
\end{algorithm}

In the algorithm the agent would not benefit by giving more than $N_0$ explorations since the reward in line (4) depends on the total number of pulls which is reduced by registering more arms. 

\begin{fact}
$N_i=\ceil{\frac{N_0}{|\set{S}_i|}}\leq N_0$. 
\end{fact}

\textcolor{blue}{1-Even if all agents only contribute $\ell_i$ arms, how do we set $N_0$. All of the versions I had seen would require knowing the total number of arms, we only know the number of agents.} 

\textcolor{blue}{2-We don't to incentivize contributing less than $\ell_i$ to maximize $N_i$ rewards.} 

\subsection{$\epsilon$-Greedy}
Consider Bernoulli arms.
\begin{enumerate}
    \item A: run UCB with instance $(0.1, 0.3)$
    \item B: run UCB with instance $(0.1, 0.3, 0.3)$
    \item C: run UCB with instance $(0.1, 0.1, 0.3)$
\end{enumerate}
Consider the deterministic case. Then the regret will only come from the exploration rounds. Clearly, we have:
\begin{align}
    R_A = (0.2) \frac{1}{2} T_R \\ 
    R_B = (0.2) \frac{1}{3} T_R \\ 
    R_C = (0.2) \frac{2}{3} T_R  
\end{align}
Therefore, $R_B + R_C = (0.2) T_R = 2 R_A$. 

\subsection{$\epsilon$-Greedy: Resolving the Conjecture for Deterministic Distributions}
%\textcolor{red}{\textbf{(NOT FINISHED YET)}} \\ 
Following the work of \cite{auer2002finite}, the $\epsilon$-greedy algorithm is the following: 
\begin{algorithm}
Play each arm once for the first $k$ rounds.\\
In a given round $t>k$:  \\
\ \ (1) Sample a Bernoulli random variable $s_t$ from $Bern(\epsilon_t)$. \\
\ \ (2) If $s_t=1$, then a pick an arm uniformly at random. \\
\ \ (3) If $s_t=0$, then sample an arm uniformly at random from the set of arms with maximum empirical mean. 
\caption{\textsc{$\epsilon$-Greedy}}\label{alg:eps_greedy}
\end{algorithm}
In \cite{auer2002finite} $\epsilon_t = \epsilon_t(\Delta,k,T)=\min \{1,\frac{c k}{d^2 T}\}$ where $c>10$ and $d<\Delta$. Note that $\Delta = \min_{i \in [k]} \Delta_i$. We note tha following: 
\begin{align}
    T = T^k_R + T_E 
\end{align}
where $T^k_R$ is the number of exploration rounds where a random arm is picked (the superscript $k$ is added to indicate dependence on the number of arms $k$) and $T_E$ is the number of exploitation rounds. Clearly we have: 
\begin{align}
    \expect{T^k_R} = \sum_{t=1}^T  \epsilon_t
\end{align}

\paragraph{Instance Details:} We consider an agent with two arms $a_1$ and $a_2$ of deterministic distributions of means $\mu_1 > \mu_2$ and $\Delta=\mu_1 - \mu_2$. The contributed arms will could be of means: (1) A: $(\mu_1,\mu_2)$ or (2) B: $(\mu_1,\mu_2,\mu_1)$ or C: $(\mu_1,\mu_2,\mu_2)$. 

\begin{theorem}
$R_A \leq \frac{R_B+R_C}{2}$ for $\epsilon$-greedy. 
\end{theorem}
\begin{proof}
\begin{fact}
If the constant $c$ in $\epsilon_t$ is always the same regardless of the number of arms, then $\expect{T^{k'}_R} > \expect{T^{k}_R}$ if $k'>k$. 
\end{fact}
\begin{proof}
This follows since $\epsilon_t(\Delta,k',T) = \min \{1,\frac{c k'}{d^2 T}\} \ge \min \{1,\frac{c k}{d^2 T}\} =\epsilon_t(\Delta,k,T)$. Therefore,  $\expect{T^{k'}_R}= \sum_{t=1}^T  \epsilon_t(\Delta,k',T) \ge \sum_{t=1}^T  \epsilon_t(\Delta,k,T)= \expect{T^k_R}$. 
\end{proof}
\begin{fact}
For $A,B,$ or $C$, no arm of mean $\mu_2$ will be pulled after the first $k$ rounds in an exploitation round. 
\end{fact}
\begin{proof}
    This follows since the distributions are deterministic and thus the arm of mean $\mu_1$ will always have a higher mean and will always be pulled in an exploitation round. 
\end{proof}

\begin{lemma}
For any case $A,B,$ or $C$, the regret can be expressed in the following form: 
\begin{align}
    R(T)= \Delta |A_2| + \Delta \frac{|A_2|}{k} \expect{T^k_R}
\end{align}
where $A_2$ is the set of arms of mean $\mu_2$. 
\end{lemma}
\begin{proof}
This follows since arms of mean $\mu_2$ will be pulled once each in the first $k$ rounds, then afterwards an arm is pulled in an exploration round with probability $\frac{1}{k}$.   
\end{proof}
From the above lemma we have the following regret calculations: 
\begin{enumerate}
    \item $A:(\mu_1,\mu_2) \xrightarrow{} R_A = \Delta + \frac{1}{2} \Delta \expect{T^2_R}$.
    \item $B:(\mu_1,\mu_2,\mu_1) \xrightarrow{} R_B = \Delta + \frac{1}{3} \Delta \expect{T^3_R}$.
    \item $C:(\mu_1,\mu_2,\mu_2) \xrightarrow{} R_C = 2 \Delta + \frac{2}{3} \Delta \expect{T^3_R}$.
\end{enumerate}
Clearly we have $\frac{R_B+R_C}{2}=\frac{3}{2} \Delta + \frac{1}{2} \Delta \expect{T^3_R} > \Delta + \frac{1}{2} \Delta \expect{T^3_R} > \Delta + \frac{1}{2} \Delta \expect{T^2_R} = R_A$, i.e. we have $\frac{R_B+R_C}{2} > R_A$. 
\end{proof}


\section{Successive Elimination} 
\paragraph{Original Arms} The original arms are one of the $l_i$ samples in the $\set{O}_i$ set.    

\paragraph{Submitted Arms} The arms submitted by the agent (the set $\set{S}_i$). 

\paragraph{Clone Arms} Arms $i$ and $j$ are called clones, if $i$ is a replica of $j$, or $j$ is a replica of $i$, or there exists an arm $r$ such that both $i$ and $j$ are replicas of $r$. Clone arms not only have the same mean but also the same exact distribution.  

\paragraph{Assumption} In the below instances $\mu_2 > \mu_1$. 

\begin{enumerate}
    \item $A:(\mu_1,\mu_2)$
    \item $B:(\mu_1,\mu_2,\mu_1)$ 
    \item $C:(\mu_1,\mu_2,\mu_2)$
\end{enumerate}

Below is the pseudo-code for successive elimination (Slivkins' Book has full derivation in chapter 1). 
\begin{algorithm}
Play each arm once for the first $k$ rounds.\\
Loop:  \\
\ \ (1) Play each active arm once. \\
\ \ (2) Deactivate all arms $a$ such that $UCB_t(a) < LCB_t(a')$ where $a'$ is another arm. 
\caption{\textsc{Successive Elimination}}\label{alg:succ_elemination}
\end{algorithm}

Suppose we follow this modified version of successive elimination instead: 
\begin{algorithm}
Play each arm once for the first $k$ rounds.\\
Loop:  \\
\ \ (1) Play each arm $a$ once unless $\exists a': UCB_t(a) < LCB_t(a')$.  
\caption{\textsc{Modified Successive Elimination}}\label{alg:succ_elemination}
\end{algorithm}
The difference is this modified does not deactivate arms and instead pulls them all in a given ``loop'' unless their $UCB$ value is found to be smaller then the $LCB$ of some other arm. This algorithm feels like UCB1 but is different since it consists of ``loops'' where it pulls all arms sequentially. I am not sure but the following seems reasonable: 
\begin{conjecture}
Modified Successive Elimination has sublinear regret. Actually probably $O(\log n)$ regret.
\end{conjecture}
From the general formula for regret: 
\begin{align*}
    R(n) = \sum_{i:\Delta_i>0} \Delta_i \expect{T_i(n)}   \\
    \expect{T_i(n)} = n -\expect{T^c_i(n)}
\end{align*}
where $T^c_i(n)$ is the total number of rounds where arm $i$ is not pulled. Therefore if we show that $\expect{T^c_i(n)}\leq L$, then $\expect{T_i(n)}=n-\expect{T^c_i(n)}\ge n-L$ which would upper bound the regret. \\

Let $\tau$ denote a loop index, let $I^{X}_{\tau}(i)=0$ be the event that arm $i$ is not pulled at loop index $\tau$ for instance $X$ where the instance is from the above mentioned instances (either instance $A$ with 2 arms, or $B$ and $C$ which have three arms), consider the following calculations:
\begin{align}
    \textbf{A:}\ \ \ \Pr{I^A_{\tau}(1)=0} = \Pr{UCB^A_{\tau}(a_1) < LCB^A_{\tau}(a_2)} \\ \nonumber \\ 
\end{align} 

To upper bound the regret of $B$ and $C$ we can upper the probability that sub-optimal arms are not pulled: 
\begin{align}
   \textbf{B:}\ \ \  \Pr{I^B_{\tau}(1)=0}  & = \Pr{UCB^B_{\tau}(a_1) < LCB^B_{\tau}(a_2) \text{ OR } UCB^B_{\tau}(a_1) < LCB^B_{\tau}(a_3)} \\ 
     & = \Pr{UCB^B_{\tau}(a_1) < LCB^B_{\tau}(a_2)} + \Pr{UCB^B_{\tau}(a_1) < LCB^B_{\tau}(a_3)} \\ 
     & - \Pr{UCB^B_{\tau}(a_1) < LCB^B_{\tau}(a_2) \text{ AND } UCB^B_{\tau}(a_1) < LCB^B_{\tau}(a_3)} \\ 
     & \leq \Pr{UCB^B_{\tau}(a_1) < LCB^B_{\tau}(a_2)} + \Pr{UCB^B_{\tau}(a_1) < LCB^B_{\tau}(a_3)}
\end{align}
By symmetry the following seems correct, it relates \textbf{A} and \textbf{B}: 
\begin{align}
    \Pr{UCB^B_{\tau}(a_1) < LCB^B_{\tau}(a_2)} = \Pr{UCB^A_{\tau}(a_1) < LCB^A_{\tau}(a_2)} = \Pr{I^A_{\tau}(1)=0} 
\end{align}
\textcolor{red}{But it is actually is not correct:} The issue has to do with the fact that in instance $B$ we also have arm $a_3$ and because of this there is a probability that it would block arm $a_2$ if $LCB_3 > UCB_2$ but this is a low probability event and there must be a way to factor that in the calculation.  


The following for \textbf{B} also seem correct: 
\begin{align}
    \Pr{UCB^B_{\tau}(a_1) < LCB^B_{\tau}(a_3)} = \text{small value, maybe something like $O(\frac{1}{T^2})$}   
\end{align}
The above would follow since arms $a_1$ and $a_3$ are clones and the algorithm is symmetric in terms of arm index. 

\textcolor{red}{Assume the above facts are correct:} This would imply that $R_B \ge 2R_A$ and therefore $\frac{R_B+R_C}{2} \ge \frac{R_B+0}{2} \ge R_A$. 


The following should hold since arms $a_1$ and $a_3$ are clones: 
\begin{align}
    \Pr{I^B_{\tau}(1)=0} = \Pr{I^B_{\tau}(3)=0}
\end{align}

The following are calculation for \textbf{C}: 
\begin{align}
   \textbf{C:}\ \ \  \Pr{I^C_{\tau}(1)=0}  & = \Pr{UCB^C_{\tau}(a_1) < LCB^C_{\tau}(a_2) \text{ OR } UCB^C_{\tau}(a_1) < LCB^C_{\tau}(a_3)}\\ & \leq \Pr{UCB^C_{\tau}(a_1) < LCB^C_{\tau}(a_2)} + \Pr{UCB^C_{\tau}(a_1) < LCB^C_{\tau}(a_3)} \\ 
   & = 2 \Pr{UCB^C_{\tau}(a_1) < LCB^C_{\tau}(a_2)}
\end{align}
where the last line follows since $a_2$ and $a_3$ are clones in instance \textbf{C}. 






==> bck.tex <==
\section{ETC regret}
Fix a permutation $\sigma$ and realization $v$, and we can further decompose the agent's conditional utility as follows.
	\begin{align*}
		\CEx{U_i(\cS)}{\sigma, v}
		&=
		\sum_{j \in \cN}\sum_{x \in [0,1]}\CEx{U_i(\cS)}{i^* = j , \muhat_i(M) = x,\sigma, v}\CPr{i^* = j,\muhat_i(M) = x}{\sigma,v}
		\\
		&=
		\sum_{j \in \cN}\sum_{x \in [0,1]}\CEx{U_i(\cS)}{i^* = j , \muhat_i(M) = x,\sigma,v}\CPr{i^* = j}{\muhat_i(M) = x,\sigma,v}\CPr{\muhat_i(M) = x}{\sigma,v}
		\\
		&=
		\sum_{j \in \cN}\sum_{x \in [0,1]}\phi_i(x,j,\sigma),
	\end{align*}
	where we write the function inside the summation $\phi(\cdot)$ for simplicity.
	Further, we write $\Gamma_i(t)$ to denote agent $i$'s utility when he is selected $t$ times under the single agent setting with $\alg_2$ where only agent $i$ exists.
	Now, we consider the case when $j = i$ and $j \neq i$ separately.
	
	If $j=i$, then we have
	\begin{align*}
		\phi_i(x,i,\sigma)
		&=
		\CEx{U_i(\cS)}{i^* = i , \muhat_i(M) = x,\sigma}\CPr{i^* = i}{\muhat_i(M) = x,\sigma}\CPr{\muhat_i(M) = x}{\sigma}
		\\
		&\overset{(a)}{=}
		\parans{xM + \CEx{\Gamma_i(T-Mn)}{i^* = i , \muhat_i(M) = x,\sigma}}\CPr{i^* = i}{\muhat_i(M) = x,\sigma}\CPr{\muhat_i(M) = x}{\sigma}
		\\
		&\overset{(b)}{=}
		\parans{xM + \Ex{\Gamma_i(T-Mn)}}\CPr{i^* = i}{\muhat_i(M) = x,\sigma}\CPr{\muhat_i(M) = x}{\sigma}.
	\end{align*}
	Note that equation $(a)$ follows from the fact that agent $i$'s utility can be decomposed to (i) exploration phase rewards and (ii) exploitation phase rewards.
	For (i), since the expectation is conditioned over the event $\muhat_i(M) = x$, this simply reduces to $xM$ given the agent-wise exploration length $M$.
	For (ii), observe that the rewards from the exploitation phase are entirely independent from what happens in the exploration phase.
	Thus, we can essentially reduce the rewards from this phase to be $\Gamma_i(T-Mn)$, given the length of exploration phase $T-Mn$.
	
	Otherwise if $j \neq i$, we have
	\begin{align*}
		\phi_i(x,j,\sigma)
		&=
		\CEx{U_i(\cS)}{i^* = j , \muhat_i(M) = x,\sigma}\CPr{i^* = j}{\muhat_i(M) = x,\sigma}\CPr{\muhat_i(M) = x}{\sigma}
		\\
		&=
		xM \cdot \CPr{i^* = j}{\muhat_i(M) = x,\sigma}\CPr{\muhat_i(M) = x}{\sigma},
	\end{align*}
	where the second equation holds since agent $i$ is only selected at the exploration phase $M$ times.
	This further implies that
	\begin{align*}
		\sum_{j \neq i}\phi_i(x,j,\sigma)
		&=
		\sum_{j \neq i}xM \cdot \CPr{i^* = j}{\muhat_i(M) = x,\sigma}\CPr{\muhat_i(M) = x}{\sigma}
		\\
		&=
		xM\cdot \CPr{\muhat_i(M) = x}{\sigma} \parans{\sum_{j \neq i}\CPr{i^* = j}{\muhat_i(M) = x,\sigma}}
		\\
		&=
		xM\cdot \CPr{\muhat_i(M) = x}{\sigma} \parans{1 - \CPr{i^* = i}{\muhat_i(M) = x, \sigma}}
	\end{align*}

	
	Thus, we can rewrite $\CEx{U_i(\cS)}{\sigma}$ as follows.
	\begin{align*}
		\CEx{U_i(\cS)}{\sigma}
		&=
		\sum_{j \in \cN}\sum_{x \in [0,1]}\phi_i(x,j,\sigma)
		\\
		&=
		\sum_{x \in [0,1]}\sum_{j \in \cN}\phi_i(x,j,\sigma)
		\\
		&=
		\sum_{x \in [0,1]}
		\CPr{\muhat_i(M) = x}{\sigma}
		\cdot 
		\parans{xM+ \Ex{\Gamma_i(T-Mn)}\cdot \CPr{i^* = i}{\muhat_i(M) = x, \sigma}}
		\\
		&=
		\sum_{x \in [0,1]}
		xM
		\CPr{\muhat_i(M) = x}{\sigma}
		+
		\sum_{x \in [0,1]}
		\CPr{\muhat_i(M) = x}{\sigma}
		\Ex{\Gamma_i(T-Mn)} \CPr{i^* = i}{\muhat_i(M) = x, \sigma}.
	\end{align*}
	Denote the first and second term by $A,B$, respectively.
	Note that the first term is simply $A = \Ex{\Gamma_i(M)}$.
	For $B$, we rewrite it as follows.
	\begin{align*}
		B 
		&= 
		\sum_{x \in [0,1]}
		\CPr{\muhat_i(M) = x}{\sigma}
		\Ex{\Gamma_i(T-Mn)} \CPr{i^* = i}{\muhat_i(M) = x, \sigma}
		\\
		&=
		\Ex{\Gamma_i(T-Mn)} 
		\cdot
		\sum_{x \in [0,1]}
		\CPr{\muhat_i(M) = x}{\sigma}
		\CPr{i^* = i}{\muhat_i(M) = x, \sigma}
		\\
		&=
		\Ex{\Gamma_i(T-Mn)} 
		\cdot
		\CPr{i^* = i}{\sigma}.
	\end{align*}
	For ease of exposition, we assume that the reward distribution of an arm does not have discontinuity.\footnote{}
	
	Then, we can further expand the latter part as \note{change it to be integral}
	\begin{align*}
		\CPr{i^* = i}{\sigma}
		&=
		\sum_{y \in [0,1]}
		\CPr{\muhat_i(M) \ge y, C_i(y)}{\sigma}
		\\
		&=
		\int_{0}^1
		\CPr{\muhat_i(M) \ge y}{\sigma}\cdot p_i(y)dy,
	\end{align*}
	where the last equation follows from the fact that the exploration phase runs independently for each agent $i$.\note{steps above are quite redundant. Make it concise}
	
	Define $q_i(y) = \CPr{\muhat_i(M) \ge y}{\sigma}$, and we obtain
	\begin{align*}
		\CEx{U_i(\cS)}{\sigma}
		&=
		\Ex{\Gamma_i(M)} + \Ex{\Gamma_i(T-Mn)} \int_0^1p_i(y)q_i(y)dy.
	\end{align*}
	Recall that we have fixed $v = (v_1,\ldots, v_l)$ to obtain the results so far.
	Now, to cope with the exact value of expected utility, we again write $\Gamma_i^{\cS}(M, v), p_i^{\cS}(y, v), q_i^{\cS}(y, v)$ to denote the values obtained so far, assuming that agent $i$'s arms' parameters are fixed to be $v$.
	\note{change the notation... throughout the proof...}
	
	Then, we can rewrite \note{notations need to be revised}
	\begin{align*}
		\CEx{U_i(\cS)}{\sigma, v}
		&=
		\Ex{\Gamma_i^{\cS}(M,\sigma(v))} + \Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))} \int_0^1p_i^{\cS}(y,\sigma(v))q_i^{\cS}(y,\sigma(v))dy.
	\end{align*}
	This completes the proof of the claim.
	
	
\section{Removed proofs}
%\section{Proof of Proposition~\ref{prop:subset}}\label{app:subset}
%
%\begin{proof}
%	Suppose that an algorithm achieves sublinear regret in any problem instance.
%	Given a truthful strategy $\cO_i$ of agent $i$, let a partial replication $\cS_i \subset \cO_i$ such that $\cS_i \neq \cO_i$ be a dominant strategy.
%	Suppose without loss of generality that $\cS$ does not include arm $(i,1)$.
%	Since the agent has no information regarding others, $\cS$ has to be also the dominant strategy when any other agent $j \neq i$ has prior distribution supported on a singleton $\{0\}$.
%	Consider a realization of $l_i$ arms, $v = (v_1,v_2,\ldots, v_{l_i})$ where $v_j \in [0,1]$ for $j \in [l_i]$.
%	Let $E_1$ be the event that $v_1 = \max_{j \in [l_i]} v_j$ and $v_1 \neq \max_{[l_i] \ni j \neq i} v_j$.
%	Let the latter quantity be $v_{(2)}$.
%	Note that this happens with strictly positive probability since agent $i$'s prior distribution has at least two points with positive measure.
%	Since the algorithm achieves sublinear regret, by playing $\cO_i$ agent $i$ can achieve regret of $o(T)$.
%	Thus, under event $E_1$, agent $i$'s expected utility will be $\max_{j \in [l_i]}v_j T - o(T) = v_1T - o(T)$, whereas by playing $\cS_i$ the agent obtains at most $v_2T$.
%\end{proof}


%\section{Pseudocode of H-UCB and ETC}\label{app:h-ucb}


%\begin{algorithm} 
%\SetAlgoLined
%%$i \in \set{N}$, $\set{S} = \cup_{i \in \set{N}} \set{S}_i$\\
%
%Initialize $R(i), N(i), r(a)$ and $n(a)$ at zero  
%for all $i \in \set{N}$ and $a\in \cup_{i \in \set{N}} \set{S}_i$;
%
%%Initialize $r(a) = n(a) = R(i)=N(i)=0$~$\forall a, i$;
%
%
% \For{$t=1,2,\ldots$}{
%  \tcp{Phase 1 - agent selection}
%  
%  \eIf{Unexplored agent exists}{ 
%    %\tcp{Agent initialization}
%    Pick an unexplored $\hat{i}\in \{i \in \set{N}: N(i) = 0\} $; % an unexplored agent ;
%  }{
%    % $i^\star = \argmax_{i} \{R_i + \sqrt{2\ln t / N_i}\}$
%    Pick $\hat{i} = \argmax_{i \in \set{N}} \left\{R(i) + \sqrt{\frac{f(t)}{N(i)}} \right\}$;
%  }
%  
%  \tcp{Phase 2 - arm selection}
%  \eIf{Unexplored arm exists}{ 
%    %\tcp{Agent initialization}
%    Pick an unexplored $\hat{a}\in \{a \in \set{S}_i: n(a) = 0\} $; % an unexplored agent ;
%  }{
%    Pick $\hat{a} = \argmax_{a \in \set{S}_i} \left\{r(a) + \sqrt{\frac{g(N(i))}{n(a)}} \right\}$;
%  }
%%  
%%  If $N(i) \le 1/2T^{1/3} \log(T)^{1/3}$, round-robin exploration of arms in $\set{S}_i$;\\
%%  Else, commit $\hat{a} = \argmax_{a \in \set{S}_{\hat{i}}} 
%%    \left\{r(a) \right\}$
%  Play $A_t = \hat{a}$ and receive reward $R_t$; \\
%  Update statistics:
%  $r(\hat{a}) \leftarrow \tfrac{r(\hat{a})n(\hat{a}) + R_t}{n(\hat{a})+1}; ~~
%  R(\hat{i}) \leftarrow \tfrac{R(\hat{i})N(\hat{i}) + R_t}{N(\hat{i})+1};$
%  
%  $n(\hat{a}) \leftarrow n(\hat{a}) + 1; ~~ N(\hat{i}) \leftarrow N(\hat{i}) + 1;$
% }
% \caption{H-UCB [\cite{shin2022multi}]\label{alg:hucb}}
%\end{algorithm}

\section{Proof of Theorem~\ref{thm:ucb_negative}}
\begin{proof}
	Denote the exploration parameter by function $f(t):\N \mapsto \R_{\ge 0}$.
	Consider a single agent with two arms indexed by $1$ and $2$ from distribution $D$ in which each arm's mean reward is $1$ with probability $1/2$ and $0$ with probability $1/2$.
	Consider a truthful strategy $\set{O}$ and strategy $\set{S}$ that replicates arm $1$.
	There exists four possible cases regarding the realization of the arms parameters: (i) both the arms have mean reward $1$, (ii) only arm $1$ has mean reward $1$, (iii) only arm $2$ has mean reward $1$, and (iv) both the arms have mean reward $0$.
	Denote each cases by $X_i$ for $i =1,2,3,4$.
%	
%	\begin{lemma}[Ex-post to ex-ante dominance]
%		For any two strategies $\set{S}$ and $\set{S}'$, suppose that agent $i$'s ex-post utility under $\set{S}$ is larger than or equal to that under $\set{S}'$ for any measurable set $E_i$ of agent $i$'s arms' realization.
%		Then, $\set{S}$ is dominant strategy over $\set{S}'$.
%		Furthermore, if the equality does not hold for some measurable $E_i$ with strictly positive probability, then $\set{S}$ is strictly dominant strategy over $\set{S}'$.
%	\end{lemma}
%	\begin{proof}
%		\note{Suho - TBD - straightforward but will spell it out}
%	\end{proof}
	For $X_1$ and $X_4$, note that there exists no difference in the agent's ex-post utility.
	For $X_2$ and $X_3$, we show that there exists a time horizon $T$ such that the average ex-post regret is minimized for strategy $\set{S}$.
	
	Consider the following list of bandit problem instances with Bernoulli arms.
	\begin{itemize}
		\item Let $A$ be a bandit instance with $\cI_A = (1,0)$.
		\item Let $B$ be a bandit instance with $\cI_B = (1,1',0)$.
		\item Let $C$ be a bandit instance with $\cI_C = (1,0,0')$.
	\end{itemize}
	Each element in $\cI$ denotes the sequence of mean reward of Bernoulli arms, where we write $1'$ and $0'$ to distinguish the arms with same mean.
	Importantly, observe that $A$ denotes the ex-post problem instance that the algorithm faces against strategy $\set{O}$ under $X_2$ or $X_3$.
	Furthermore, $B$ denotes the ex-post problem instance against $\set{S}$ under $X_2$, and $C$ denotes that against $\set{S}$ under $X_3$.
	
	We now show the following claim.
	\begin{claim}\label{cl:neg_ucb}
		Suppose that we run UCB with exploration parameter $f(\cdot)$ for all the problem instances $A,B$, and $C$.
		Then, there exists a time horizon $T$ such that $\reg_A(T) > \nicefrac{(\reg_B(T) + \reg_C(T))}{2}$.
	\end{claim}
	\begin{proof}[Proof of the claim]
		
	
	For any integer $i \ge 2$, let $s_i$ denote the minimum integer satisfying
	\begin{align*}
		1 + \sqrt{\frac{f(s_i + i)}{s_i}} 
		< 0 + \sqrt{\frac{f(s_i + i)}{i}}.
	\end{align*}
	Define $s_1 = 1$.
	Such $s_i$ exists for any $i \ge 2$ since LHS is a decreasing function of $s_i$ and RHS is an increasing function of $s_i$ and putting $s_i = i$ yields LHS is larger than RHS.
	It is obvious that $s_i > s_j$ if $i > j$ and $s_i \ge i$.
	
	Due to our construction of the sequence $s_i$, in $A$, arm with mean $1$ is selected exactly $s_i$ times and then arm with mean $0$ is selected for a single round, and it repeats for $i=1,2,\ldots$.
	Thus, the bandit process in $A$ can be described as
	\begin{align*}
		(1:s_1, 0:1, 1:s_2, 0:1, 1:s_3, 0:1, \ldots),
	\end{align*}
	where in each element of $x:y$ denotes that arm with mean $x$ is selected $y$ times.
	Likewise, in $B$, we have
	\begin{align*}
		(1:s_1, 1':s_1, 0:1, [1:s_2, 1':s_2], 0:1, [1:s_3, 1':s_3], 0:1, \ldots),
	\end{align*}
	where for each element in $[\cdot]$, we ignore the orders how $1$ and $1'$ are selected, but aggregate them to only present the total number of times each one is selected before getting to the arm $0$.
	For $C$, we have
	\begin{align*}
		(1:s_1, [0:1, 0':1], 1:s_2, [0:1, 0':1], 1:s_3, [0:1, 0':1], \ldots).
	\end{align*}
	Set $T = s_1 + 2 + s_2$.
	Given $T$, in $A$, the arm $0$ is selected twice.
	In $B$, the arm $0$ is selected once.
	In $C$, the arm $0$ is selected once, and also $0'$ is selected once.
	Hence, at round $t=T$, $\reg_A(T) = 2 > \frac{1+ 2}{2} = \frac{\reg_B(T) + \reg_C(T)}{2}$,
	and it completes the proof.
	\end{proof}
	Set $T$ as defined in the claim above.
	% In the single-agent setting, given any realization $E = (\mu_1, \mu_2)$ with $\mu_1 \ge \mu_2$, note that an agent's ex-ante utility can be easily derived from his ex-post regret as follows.
	% \begin{align*}
	% 	U(\set{S};E) = \mu_1 N_1(T) + \mu_2 N_2(T) = 
	% 	\mu_1 T - (\mu_1 - \mu_2)N_2(T) =  \max_{a \in E}\mu_a \cdot T - \reg_E(T).
	% \end{align*}
	Finally, we can decompose the agent's ex-ante utility as follows.
	\begin{align*}
		u(\set{O}) 
		= 
		\frac{1}{4}\parans{\sum_{i=1}^4U(\set{O};E_i)}
		&=
		\frac{1}{4}\parans{\sum_{i=1,4}U(\set{O};E_i)} + \frac{1}{4}\parans{\sum_{i=2,3}U(\set{S};E_i)}
		\\
		&=
		\frac{1}{4}\parans{\sum_{i=1,4} \parans{\max_{a \in E_i}\mu_a \cdot T - \reg_{E_i}(T)}}
		+
		\frac{1}{4}\parans{\sum_{i=2,3} \parans{\max_{a \in E_i}\mu_a \cdot T - \reg_{E_i}(T)}}
		\\
		&=
            \frac{T - \reg_A(T)}{2}
		\\
		&<
		\frac{T - (\reg_B(T) + \reg_C(T))/2}{2}
		\\
		&=
		\frac{1}{4}\parans{\sum_{i=1,4}U(\set{S};E_i)} + \frac{1}{4}\parans{\sum_{i=2,3}U(\set{S};E_i)}
		\\
		&= u(\set{S}),
	\end{align*}
	and thus $\set{S}$ yields the strictly larger ex-ante utility, and it concludes the proof.
\end{proof}

\section{Proof of Theorem~\ref{thm:hucb_negative}}
\begin{proof}
	If there exists only a single agent, it is easy to see that the dynamics of the algorithm reduces to standard UCB with exploration parameter $g(\cdot)$.
	Thus, by Theorem~\ref{thm:ucb_negative}, H-UCB is not replication-proof.
	Now we consider multiple agents with $n \ge 2$.
	We only show for the case $n=2$ since it easily extends to the cases with $n \ge 3$.
	Without loss of generality, we assume that the algorithm breaks tie uniformly at random in both phases $1$ and $2$.
	Suppose that agent $1$ has two deterministic arms sampled from $D$ in which the mean reward is $c \in [0,1]$ with probability $0.5$, and $0$ otherwise, for some $c>0$.
	We further assume that agent $2$ is equipped with a deterministic prior $D_i$ supported on $\mu$, and the arm also deterministically outputs reward $\mu$, where the exact quantity $\mu$ will be determined later.
	Note that the bandit process is deterministic for any realization of the arms' parameters.
	
	We consider a truthful strategy $\cO$ of registering both arms, and another strategy $\cS$ of replicating only a single arm, and focus on the difference on the agent's expected utility between two strategies.
	If the agent samples $c$ or $0$ both the arms, then the rewards of the bandit process and the agent's ex-post utility therein will be indifferent.
	Thus, we only focus on the remaining case.
	Suppose that agent $1$ samples $c$ for one arm and $0$ for the other, which occurs with probability $1/2$.
	Similar to the proof of Claim~\ref{cl:neg_ucb}, we consnider the following list of bandit problem instances with deterministic arms.
	\begin{itemize}
		\item Let $A$ be a bandit instance with $\cI_A = (c,0)$.
		\item Let $B$ be a bandit instance with $\cI_B = (c,c',0)$.
		\item Let $C$ be a bandit instance with $\cI_C = (c,0,0')$.
	\end{itemize}
	% \note{Some figure may help}
	Each element in $\cI$ denotes the sequence of mean reward of Bernoulli arms, where we write $c'$ and $0'$ to distinguish the arms with same mean.
	We simply say arm $c$ and arm $0$ to denote the arm with the corresponding parameter $c$ and $0$, respectively.
	Then, the realization of the agent $1$'s arms in playing strategy $\cS$ corresponds to either of bandit instance $B$ or $C$, and strategy $\cO$ corresponds to the bandit instance $A$.
	Let us abuse the notation of $s_1,s_2,\ldots$ defined in the proof of Claim~\ref{cl:neg_ucb}, so that it denotes the number of rounds that arm $c$ is selected consecutively before arm $0$ is sampled $i$-th time, in problem instance $A$.
	Also, we use $R_t(i)$ and $N_t(i)$ to denote the quantity of $R(i)$ and $N(i)$ at round $t$.
	
	Given the random bits of the tie-breaking rule used by the algorithm, let $\tau^{i}_1,\tau^i_2,\ldots, \tau^i_{k}, \ldots$ be the rounds that agent $1$ is sampled $k$ times when the mean rewards of the agent $1$'s arms are realized to be $i= A,B,C$.
	It is straightforward to check that $\tau^{B}_t \le \tau^{A}_t \le \tau^{C}_t$\footnote{This can  be shown using the coupling technique introduced in \cite{shin2022multi}.}.
	Let $k = s_1+s_2+2$, and following the argument of Claim~\ref{cl:neg_ucb}, we observe that at round $\tau^{B}_k$, agent $1$'s empirical mean rewards by playing $\cS$ will be either of (i) $\frac{c(s_1+s_2)}{s_1+s_2+2}$ or (ii) $\frac{c(s_1+s_2+1)}{s_1+s_2+2}$ based on whether the arms are realized to be instance $B$ or $C$.
	By playing $\cO$, agent $1$ simply has empirical mean reward of $\frac{c(s_1+s_2)}{s_1+s_2+2}$ at round $\tau^{A}_k$.
	Furthermore, if $\tau^{B}_k < \tau^{A}_k$, then in problem instance $A$, it means that the agents' parameters at round $\tau^{B}_k$ satisfy
	\begin{align*}
		R_{\tau^B_k}(1) + \sqrt{\frac{f(t)}{k-1}}
		<
		R_{\tau^B_k}(2) + \sqrt{\frac{f(t)}{\tau^B_k - k}},
	\end{align*}
	where $R_t(i)$ denotes the empirical average reward of agent $i$ at round $t$,  $R_{\tau^B_k}(1) = \frac{c(s_1+s_2)}{s_1+s_2+2}$ and $R_{\tau^B_k}(2) = \mu$.
	However, from our construction of the variables and the fact that H-UCB selects agent $1$ at round $\tau^{B}_k$ in $B$, we know that
	\begin{align*}
		\frac{c(s_1+s_2)}{s_1+s_2+2} + \sqrt{\frac{f(t)}{k-1}}
		\ge
		\mu + \sqrt{\frac{f(t)}{\tau^B_k - k}},
	\end{align*}
	and thus $\tau^A_k$ and $\tau^B_k$ needs to be exactly equivalent.
	Similarly, for instance $C$, since arm $c$ and $c'$ are selected the same number of times at the beginning of round $\tau^B_k$, we conclude that $\tau^i_k$ are equivalent for $i=A,B,C$.
	
	Now define $C = \sqrt{\frac{f(t)}{k}} - \sqrt{\frac{f(t)}{\tau^B_k-k}}$ and we pick any $\mu \in (\frac{c(s_1+s_2)}{s_1+s_2+2} + C,\frac{c(s_1+s_2+1)}{s_1+s_2+2} + C)$.
%	We claim that there exists a choice of parameters $c$ that such $\mu$ always exist.
%	\begin{claim}
%		There exists  $c>0$ such that the interval $\mu \in (\frac{c(s_1+s_2)}{s_1+s_2+2} + C_1,\frac{c(s_1+s_2+1)}{s_1+s_2+2} + C_2)$ is well-defined.
%	\end{claim}
%	\begin{proof}
%		It suffices to show that 
%		\begin{align*}
%			\sqrt{\frac{f(t)}{k-1}} - \sqrt{\frac{f(t)}{k}} < \frac{c}{s_1+s_2+2}.
%		\end{align*}
%		Note that all $k = s_1+s_2+2$,$s_1$ and $s_2$ are in fact functions of $c$.
%		Define $s = s_1+s_2$ and rearrange the inequality, we obtain 
%		\begin{align*}
%			\sqrt{f(t)}\parans{\frac{\sqrt{s+2} - \sqrt{s+1}}{\sqrt{(s+1)(s+2)}}}
%			<
%			\frac{c}{s+2}.
%		\end{align*}
%		Define $x = \sqrt{s+1}$ and rearrange again, it suffices to show that
%		\begin{align*}
%			\sqrt{f(t)}\parans{x+\frac{1}{x}-1} \le c,
%		\end{align*}
%		for some $c$.
%		Since LHS is at most 
%		
%
%
%		
%		When we increase the value of $c$, it is easy to see that  
%		
%		By making $c$ sufficiently large, we
%
%	\end{proof}

	
	Then, at round $\tau^B_k+1$, for bandit instance $A$ and $C$, we observe that agent $2$ will be selected since
	\begin{align*}
		R_{\tau^B_k+1}(2) + \sqrt{\frac{f(t)}{N_{\tau^B_k}(2)}}
		&=
		\mu + \sqrt{\frac{f(t)}{\tau^B_k - k}}
		\\
		&>
		\frac{s_1+s_2}{s_1+s_2+2} + C + \sqrt{\frac{f(t)}{\tau^B_k - k}}
		\\
		&=
		\frac{s_1+s_2}{s_1+s_2+2} + \sqrt{\frac{f(t)}{k}}
		= 
		R_{\tau^B_k+1}(1) + \sqrt{\frac{f(t)}{N_{\tau^B_k}(1)}}.
	\end{align*}
	For bandit instance $C$, however, observe that
	\begin{align*}
		R_{\tau^C_k+1}(2) + \sqrt{\frac{f(t)}{N_{\tau^C_k}(2)}}
		&=
		\mu + \sqrt{\frac{f(t)}{\tau^C_k - k}}
		\\
		&<
		\frac{s_1+s_2+1}{s_1+s_2+2} + C + \sqrt{\frac{f(t)}{\tau^C_k - k}}
		\\
		&=
		\frac{s_1+s_2+1}{s_1+s_2+2} + \sqrt{\frac{f(t)}{k}} 
		=
		R_{\tau^C_k+1}(1) + \sqrt{\frac{f(t)}{N_{\tau^C_k}(1)}},
	\end{align*}
	and thus arm $1$ is selected.
	This essentially implies that by setting $T = \tau_k^A+1$, agent $1$ is selected at round $T$ with probability $1/4$ if he plays $\cS$, is never selected if he plays $\cO$, where the probability $1/4$ comes from the fact that problem instance $C$ is realized with probability $1/4$.
	Thus, agent $1$'s expected utility becomes larger for such $T$ by replicating one of its arm, and we finish the proof.
%
%
%	
%	Note that each $\tau_i$ depends on agent $2$'s reward $\mu$.
%	Define the sequence $s_1,s_2,\ldots$ and the problem instance $A,B$, and $C$ as we did in the proof of Claim~\ref{cl:neg_ucb}.
%	Following the argument of Claim~\ref{cl:neg_ucb}, we observe that at round $\tau_i$ with $i = s_1+2+s_2$, agent $1$'s ex-post regret is strictly larger on problem instance $A$, compared to the average of that of $B$ and $C$.
%	This essentially implies that at round $\tau_i$, agent $1$'s empirical mean reward becomes exactly larger in strategy $\cS'$.
%	
%	Now we pick any $\mu \in (\frac{s_1+s_2}{s_1+s_2+2},\frac{s_1+s_2+1}{s_1+s_2+2})$.
%	Then, in problem instance $A$, at round $\tau$
	
%	
%	\note{Suho - TBD - need to be fixed}
%	
%	Consider two symmetric agents $a$ and $b$ with two deterministic arms of $1$ and $\eps$.
%	Denote the agent $a$'s arm by $1_a$ and $\eps_a$, and similarly for agent $b$.
%	Let $(s_i)_{i\in \N}$ be the sequence defined in the proof of Theorem~\ref{thm:ucb_negative}.
%	Set $T = 2(s_1+2+s_2) + 1$.
%	Suppose that both the agents truthfully register.
%	Up to round $t=T-1$, due to the deterministic nature of the arms, both agents are selected $s_1+2+s_2$ times, and their agent-wise average rewards are $R(a) = R(b) = 1 - \frac{2\eps}{s_1+2+s_2}$.
%	Thus, at round $t=T$, the selected agent will be based on the tie-breaking rule of H-UCB.
%	On the other hand, suppose that agent $a$ replicates one of the arms randomly.
%	Then, by the observation in the proof of Theorem~\ref{thm:ucb_negative}, the average reward of agent $a$ at round $t=T-1$ will be $R(a) = 1 - \frac{\eps}{s_1+2+s_2}$ if arm $1$ is replicated.
%	Otherwise if arm $\eps$ is replicated, then $R(a) = 1 - \frac{2\eps}{s_1+2+s_2}$.
%	In the former case, agent $a$ will be deterministically selected as it satisfies $R(a) > R(b)$.
%	In the latter case, the tie-breaking rule determines whom to select.
%	This implies that the average reward of replicating both arms is larger, and thus $H-UCB$ is not replication-proof.
	\end{proof}
	
	
\section{Proof of Theorem~\ref{thm:single_pf_rp}}
\begin{proof}
	Let $\fA$ be an algorithm with symmetry and TRP.
	Given a single agent problem instance $\cI$ with original set $\cO$ with $l$ arms, let $\cS$ be a truthful strategy that registers $\cO$.
	Consider any non-truthful strategy $\cS$ such that it replicates $r_i \in \Z_0$ times for arm $a$ for $a \in [l]$, where $\Z_0 =  \{0,1,2,\ldots\}$ denotes the set of nonnegative integers.
	Note that since $\cS$ is non-truthful strategy, at least one $r_a$ has to be strictly positive for some $a \in [l]$.
	We abuse $r_a=0$ to say that arm $a$ is only registered once without any replication, and write $r = (r_1,\ldots, r_l)$.
	For $v = (v_1,\ldots, v_l) \in \R_{\ge 0}^l$, we write $g(v)$ to denote the density of the mean rewards of arms having $v$, \ie $g(v) = \prod_{a=1}^l f(v_a)$, where $\R_{\ge 0}^l$ denotes the set of $l$-dimensional nonnegative real vectors.
	For simplicity, we assume that the prior distribution $D$ of the agent does not have any point mass.\footnote{This assumption is for ease of exposition, and does not restrict any of our results. \note{expand why (we can essentially unionize two arms with same mean rewards)}}
	We further write $dv$ to denote $dv_1 dv_2 \ldots dv_l$.
	We use $\reg_{v, r}$ to denote the regret of problem instance such that the arms' mean rewards are realized to be $v$ and each arm $i$ is replicated $r_i$ times.
	We finally write $\sigma(v)$ to the permuted vector given a permutation $\sigma \in S^l$, and $\sigma(v)_i$ to denote $i$-coordinate of $\sigma(v)$.
	
%	The following claim easily follows from our definition of permutation-freeness.
	
	Observe that the expected utility in playing the strategy $\cS$ can be written as follows.
	\begin{align*}
		u(\cS) 
		&= 
		\int_{\mu_1 = v_1}\ldots \int_{\mu_l = v_l} \Ex{U(\cS)\ |\ v_1,\ldots, v_l}g(v)dv		
		\\
		&=
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 < v_1}\ldots \int_{\mu_k = v_l< v_{l-1}} 
		\sum_{\sigma \in S_l}\Ex{U(\cS)\ |\ \sigma(v)_1,\ldots, \sigma(v)_l}g(v)dv
		\\
		&=
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 < v_1}\ldots \int_{\mu_k = v_l< v_{l-1}} 
		\sum_{\sigma \in S_l}\Ex{v_1T - \reg_{\sigma(v),r}(T) \ |\ \sigma(v)_1,\ldots, \sigma(v)_l}g(v)dv.
	\end{align*}
	Due to the symmetry of the algorithm, we can further expand it to be
	\begin{align}
		u(\cS)
		&=
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 <v_1}\ldots \int_{\mu_l = v_l< v_{l-1}} 
		\sum_{\sigma \in S_l}\Ex{v_1T - \reg_{v,\sigma(r)}(T) \ |\ v_1, \ldots, v_l}g(v)dv,
		\label{ineq:05131256}
	\end{align}
	where $\vec{0}_l$ denotes the $l$-dimensional zero vector, and the inequality easily follows from the fact that $(0,0,\ldots,0) \prec_m r$ and the algorithm is TRP.
	We now prove the following claim.
	\begin{claim}
		For any $v \in R_{\ge 0}^l$ and $\sigma \in S_l$, we have
		\begin{align*}
			\sum_{\sigma \in S_l}\Ex{\reg_{v,\sigma(\vec{0}_l)}(T)} 
			\le 
			\sum_{\sigma \in S_l}
			\Ex{\reg_{v,\sigma(\vec{0}_l)}(T)}.
		\end{align*}
	\end{claim}
	\begin{proof}
		This directly follows from our definition of TRP.
		More formally,
		\begin{align*}
			\sum_{\sigma \in S_l}\Ex{\reg_{v,\sigma(\vec{0}_l)}(T)} 
			\tag{def. of RP-Regtret}
			&=
			\frac{\rpreg(\fA,T;\cO) }{|S_l|}
			\\
			&\le
			\frac{\rpreg(\fA,T;\cS) }{|S_l|}
			\tag{since $\fA$ is TRP}
			\\
			&=
			\sum_{\sigma \in S_l}
			\Ex{\reg_{v,\sigma(\vec{0}_l)}(T)}.
			\tag{def. of RP-Regret}
		\end{align*}
		It completes the proof.
	\end{proof}
	By the claim, we can further expand from \eqref{ineq:05131256} as follows.
	\begin{align*}
		u(\cS)
		&\le
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 < v_1}\ldots \int_{\mu_l = v_l< v_{l-1}} 
		\sum_{\sigma \in S_l}\Ex{v_1T - \reg_{v,\sigma(\vec{0}_l)}(T) \ |\ v_1,\ldots, v_l}g(v)dv,	
	\end{align*}

	

	Since $\reg_{v, \sigma(\vec{0}_l)}$ is equivalent to the regret of the truthful strategy $\cO$ given the ex-post realization $v$, we obtain
	\begin{align*}
		u(\cS)
		&\le
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 < v_1}\ldots \int_{\mu_l = v_l< v_{l-1}} 
		\sum_{\sigma \in S_l}\Ex{v_1T - \reg_{\cI}(T) \ |\ v_1,v_2,\ldots, v_l}g(v)dv
		\\
		&=
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 }\ldots \int_{\mu_l = v_l} 
		\Ex{U(\cO)\ |\ v_1,\ldots, v_l}g(v)dv
		\\
		&=
%		\int_{\mu_1 = v_1}\ldots \int_{\mu_l = v_l} \Ex{U(\cO)\ |\ v_1,\ldots, v_l}g(v)dv		
%		=
		u(\set{O}),
	\end{align*}
	and thus the truthful registration $\set{O}$ is a dominant strategy.
\end{proof}


\section{Proof of Theorem~\ref{thm:single_rp}}
\begin{proof}
	We will deal with a single agent.
	Consider a bandit instance $\cI$ in which there exists $l$ arms with parameters $v_1 \ge v_2 \ge \ldots \ge v_l$, and the time horizon is $T$.
	Let $n_a(t)$ be the number of rounds that arm $a$ is pulled and $\muhat_a(t)$ be the empirical average reward, at the end of round $t$, and define $\delta_a = v_1 - v_a$ for $a \in [l]$.
	
	Our proof mainly relies on the following lemma.
	\begin{lemma}\label{th:ETC_main_th}
		Suppose that the realization of the arms's mean rewards is given, and let $a^*$ be the arm the largest mean reward.
		If $m \ge \frac{2 l}{\Delta^2} \ln{2T}$, then for a sub-optimal arm we have:
		\begin{align*}
			\Ex{n_a(T)} \leq m+1.
		\end{align*}
		Especially for $m = \frac{2}{\Delta^2} l \ln (2T)$, the expected regret is upper bounded by:
		\begin{align*}
    		\reg(T) 
    		\leq 
    		\sum_{a\in [l]} (m+1) \Delta_i 
    		\leq 
    		\sum_{a\in [l]} \Big( \frac{2\delta_a l\ln{(2T)}}{\Delta^2} + 1 \Big).
		\end{align*}	
	\end{lemma}
	\begin{proof}[Proof of the lemma]
		Due to the structural nature of ETC, for any sub-optimal arm $a$ we have
		\begin{align*}
    		\Ex{n_a(T)} \leq m + (T-mk) \Pr{\hat{\mu}_a(m) \ge \hat{\mu}_{a^*}(m)} 
    	\end{align*}
    	Now we focus on upper bounding $\Pr{\hat{\mu}_a(m) \ge \hat{\mu}_{a^*}(m)}$.
    	\begin{claim}\label{cl:concen}
    		For any arm $a \neq a^*$, the following holds.
    		\begin{align*}
    			\Pr{\hat{\mu}_a(m) \ge \hat{\mu}_{a^*}(m)} 
    			\le 
    			2\exp(-\frac{\delta_a^2 m}{2})
    		\end{align*}
    	\end{claim}
    	\begin{proof}[Proof of the claim]
    		We can expand the inequality as follows.
    		\begin{align*}
    			\Pr{\hat{\mu}_a(m) \ge \hat{\mu}_{a^*}(m)} &= \Pr{(\hat{\mu}_a(m) -v_i) + (v_{a^*} - \hat{\mu}_{a^*}(m)) \ge \delta_i}
    			\\ 
    	    	&\leq 
    	    	\Pr{(\hat{\mu}_a(m) -v_i) \ge \frac{\delta_a}{2}} + \Pr{(v_{a^*} - \hat{\mu}_{a^*}(m)) \ge \frac{\delta_a}{2}}
    	    	\\ 
    	    	&\leq 
    	    	2 \exp(- \frac{\delta_a^2}{4} \frac{1}{2} \frac{1}{\frac{1}{4m}}) \tag{Hoeffding's inequality} \\
    	    	& \leq 2\exp(- \frac{\delta_i^2 m}{2}),
			\end{align*}
			where we use the following type of concentration inequality.
			\begin{theorem}
				Let $X_1,\ldots, X_n$ be independent random variables such that $a_i \le X_i \le b_i$ almost surely.
				Define $S_n = X_1 + \ldots X_n$.
				For any $t >0$,
				\begin{align*}
					\Pr{|S_n - \Ex{S_n}| \ge t}
					\le 
					2\exp\parans{-\frac{2t^2}{\sum_{i=1}^n (b_i - a_i)^2}}.	
				\end{align*}
			\end{theorem}
			We finish the proof of the claim.
    	\end{proof}
		Using the claim above, we can further expand,
		\begin{align*}
       		\Ex{n_a(T)} 
       		&\leq
       		m + (T-mk) \Pr{\hat{\mu}_a(m) \ge \hat{\mu}_{a^*}(m)} 
       		\\
       		&\leq 
       		m + 2T\exp(- \frac{\delta_i^2 m}{2})
       		\tag{Claim~\ref{cl:concen} $\&$ $T-mk \le T$}
      		\\
       		&\leq
       		m + 2T  \exp(- \Big(\frac{\delta_a}{\Delta}\Big)^2 \ln{2T})
       		\tag{$m\ge 2/\Delta^2 \ln(2T)$}
       		\\
       		&\leq 
       		m+ 2T  \exp(- \ln{2T})
       		\tag{Since $\frac{\delta_a}{\Delta} \ge 1$} 
       		\\
       		&=
       		m + 1.
		\end{align*}
		This proves the upper bound on $\Ex{n_a(T)}$.
		To obtain the upper bound on the regret, one can use the following well-known regret decomposition lemma.
		\begin{lemma}[Regret decomposition]
			The regret can be writtten as
			$\reg(T) = \sum_{a \in [l]} \Ex{n_i(T)\delta_a}$.
		\end{lemma}

		From this, the regret bound easily follows as below
		\begin{align*}
    		\reg(T)
    		&\leq 
    		\sum_{a\in [l]} (m+1) \delta_a 
    		\\
    		&= 
    		\sum_{a\in [l]} (\frac{2l}{\Delta^2} \ln{2T}+1) \delta_a 
    		\\ 
    		&\leq 
    		\sum_{a\in [l]} ( \frac{2l\delta_a}{\Delta^2} \ln{2T} +1).
    		\tag{Since $\Delta_a\leq 1$} 
		\end{align*}
		This completes the proof.
	\end{proof}
	
	Now, consider a strategy $\cS \neq \cO$ of which the replication vector is $r = (r_1,\ldots, r_l)$ (as defined in the proof of Theorem~\ref{thm:single_pf_rp}), and at least one coordinate being strictly positive.
	Consider a realization $v \in \R_{\ge 0}^l$, and a permutation $\sigma(v)$.
	Let $\cI_{\sigma}$ be a bandit instance in which the arms are permuted by $\sigma$ from $\cI$.

	
	
	Given $v_1 \ge \ldots \ge v_l$, let $\cI_{\sigma,v}$ be the instance in which $i$-th arm has mean reward $v_{\sigma(i)}$ for $i \in [l]$.
	Denote the expected regret under $\cI_{\sigma,v}$ by $\reg_{I_{\sigma,v}}$.
	
	From the regret decomposition lemma, we have
	\begin{align*}
		\reg_{I_{\sigma,v}}(T) = \sum_{a\in [l]}	\Ex{n_{\sigma(a),t}}\delta_{\sigma(a)} \parans{r_a + 1}.
	\end{align*}
	Due to the initial exploration phase of ETC, obviously $\Ex{n_{\sigma(a),t}} \ge m$.
	Hence we obtain
	\begin{align*}
		\reg_{I_{\sigma,v}}(T) 
		&\ge
		\sum_{a\in [l]} m \cdot \delta_{\sigma(a)}(r_a + 1).
	\end{align*}
	Now, RHS in the random permutation regret \eqref{eq:epf} can be written as follows.
	\begin{align}
		\sum_{\sigma \in S_l}\reg(\cI_{\sigma,v})/|S_l|
		&\geq
		\frac{\sum_{\sigma \in S_l}\sum_{a\in [l]} m \cdot \delta_{\sigma(a)}(r_a + 1)}{l!}
		\nonumber
		\\
		&\geq
		\frac{\sum_{a\in [l]} \sum_{\sigma \in S_l} m \cdot \delta_{\sigma(a)}(r_a + 1)}{l!}
		\nonumber
		\tag{Change order of summation}
		\\
		&=
		\frac{\sum_{a\in [l]} \sum_{\sigma \in S_l} m \cdot \delta_{a}(r_{\sigma(a)} + 1)}{l!}
		\nonumber
		\tag{Sum over $\sigma$ equals that over $\sigma^{-1}$}
		\\
		&=
		\frac{\sum_{a\in [l]} m \cdot \delta_a(l-1)!\sum_{j=1}^l (r_{j}+1)}{l!}
		\nonumber
		\tag{fix $\sigma(a) = j$ and sum over $\sigma \in S_l$	}
		\\
		&=
		\frac{\sum_{a\in [l]} m \cdot \delta_a (\norm{r}_1+l)}{l}\label{ineq:05090221}
	\end{align}
	Due to our construction of $r$, we have $\norm{r}_1 \ge 1$, and finally we obtain
	\begin{align}
		\reg(\cI) 
		&\le
		\sum_{a\in [l]} (m+1) \delta_a 
		\label{ineq:05090222}
		\\
		&\le
		\sum_{a\in [l]} m\delta_a \frac{l+1}{l},
		\nonumber
		\tag{$m = \frac{2l}{\Delta^2}\ln 2T \ge l$}
		\\
		&\le
		\frac{\sum_{a\in [l]} m \cdot \delta_a\sum_{j=1}^l (r_{j}+1)}{l}
		\tag{$\norm{r}_1 \ge 1$}
		\nonumber
		\\
		&\le
		\sum_{\sigma \in S_l}\reg(\cI_{\sigma,v})/|S_l|,
		\nonumber
	\end{align}
	where the last inequality follows from inequality~\eqref{ineq:05090221}.
	Note further that $\reg(\cI)$ is $\rpreg$ of truthful strategy $\cO$ given the realization $v$, and RHS denotes that of a strategy $\cS$ whose replication vector is $r$.
	Thus,
	\begin{align*}
		\rpreg(\fA, T, \cO) \le \rpreg(\fA, T, \cS),	
	\end{align*}
	for $\fA$ being ETC, and it concludes that ETC is TRP.
\end{proof}


\section{Proof of Theorem~\ref{thm:multi_rp_uniform}}
\begin{proof}
	Let $\set{S}_i$ be the strategy of agent $i$.
	Define $\Gamma_i(\set{S}_i)$ be the agent $i$'s utility under the single-agent setting with agent $i$, \ie when there are no other agents other than $i$.
	Due to the uniformly random selection nature of $\alg_1$, the expected utility of any agent $i$ can be simply written $u_i(\cS_i, \cS_{-i}) = \nicefrac{\Gamma_i(\set{S}_i)}{n}$.
	Note that the dynamic of $\hbb$ reduces to the dynamic of $\alg_2$ if there's only a single agent.
	Hence, by Theorem~\ref{thm:single_pf_rp} and due to the TRP and symmetry of $\alg_2$, we conclude that truthful registration is a dominant strategy for any agent $i$, and it completes the proof.
\end{proof}

\section{Proof of Theorem~\ref{thm:spf_rp}}
\begin{proof}
    \note{proofread again, and structurize}
	First, note that our $\hbb$ is well-defined since our choice of $M$ and $m$ ensures that the exploitation phase of $\alg_1$ starts after the exploitation of $\alg_2$ ends.
	Pick an agent $i$ with arms $\{o_{i,1}, \ldots, o_{i,l}\}$, let $\cS_i$ be agent $i$'s arbitrary strategy which replicates arm $o_{i,j}$ of $r_{i,j} \in \N_0$ times for each $j \in [l_i]$.
	Let $r_i = (r_{i,1},\ldots, r_{i,l_i})$.
	Fix strategies of all the other agents $j \neq i$, by $\cS_{-i}$
	We use $i^*$ to denote the agent selected at the exploitation phase of $\alg_1$, and $l_i$ to denote agent $i$'s number of arms.
	We further write $\muhat_i(M)$ to denote the empirical average reward of agent $i$ when he is selected $M$ times in total,
	and $\muhat_{i,a}(m)$ to denote the empirical average reward of agent $i$'s arm $a$ when it's selected $m$ times in total.
	
	
	Similar to the proof of Theorem~\ref{thm:single_pf_rp}, we first write agent $i$'s expected utility as follows.
	\begin{align}
		u_i(\cS_i)
		=
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 < v_1}\ldots \int_{\mu_k = v_l< v_{l-1}} 
		\sum_{\sigma \in S_{l_i}}\Ex{U_i(\cS_i)\ |\ \sigma, v}g(v)dv.\label{eq:04262152}
	\end{align}
%	Now, we fix a realization of agent $i$'s arms' parameters to be $v = (v_1,v_2,\ldots, v_l)$, and focus on the integrand.
%	Since we fix the realization of the parameters, we simply write $\sigma(v)$ to denote the event $\{\mu_1 = \sigma(v)_1,\ldots, \mu_l = \sigma(v)_l\}$, \ie
%	\begin{align*}
%		\Ex{U_i(\cS)\ |\ \sigma(v)_1,\ldots, \sigma(v)_l}
%		=
%		\CEx{U(\cS)}{\sigma(v)},
%	\end{align*}
%	unless confusion arises.
	
	We first characterize the expected utility of agent $i$ based on its single agent utility.
	To this end, we introduce several notations.
	Write $\Gamma_i(t, \sigma(v))$ to denote agent $i$'s utility when he is selected $t$ times under the single agent setting with $\alg_2$ where only agent $i$ exists and his arms' mean rewards are realized to be $\sigma(v)$, and he plays strategy $\cS$.
	Given $M$ and $m$, denote the event $\{\max_{\cN \ni j\neq i}\parans{\muhat_j(M) = y} \ | \ \sigma, v\}$ by $C_i(y,\sigma(v))$.
	Define $p_i(y, \sigma(v)) = \CPr{C_i(y)}{\sigma,v}$ and $q_i(y,\sigma(v)) = \CPr{\muhat_i(M) \ge y}{\sigma,v}$.

	The following claim essentially characterizes the expected utility of agent $i$ under strategy $\cS$.
	\begin{claim}
		Agent $i$'s expected utility can be written as follows.
		\begin{align}
			\CEx{U_i(\cS)}{\sigma, v}
			&=
			\Ex{\Gamma_i^{\cS}(M,\sigma(v))} + \Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))} \int_0^1p_i^{\cS}(y,\sigma(v))q_i^{\cS}(y,\sigma(v))dy.\label{eq:04271231}	
		\end{align}
	\end{claim}
	\begin{proof}[Proof of the claim]
		Since $\hbb$ is running with Phase 1 ETC, the expected utility of agent $i$ can be decomposed as (i) expected utility in the exploration phase and (ii) expected utility in the exploitation phase.
		Note that (i) essentially coincides with the expectation of $\Gamma_i^\cS(M, \sigma(v))$ since it chooses agent $i$ exactly $M$ times regardless of the random rewards.
		Moreover, due to our restarting at time $\tau = Mn$, when the exploitation phase of $\alg_1$ starts, all the parameters of $\alg_2$ is initialized.
		Thus, conditioned on the event that agent $i$ has the largest empirical average reward at round $\tau = Mn$, its expected utility in the exploitation phase again coincides with the single agent case expected utility $\Gamma_i^{\cS}(T-Mn, \sigma(v))$.
		Otherwise, if agent $i$ has not been selected as the empirically best agent, then its conditional expected utility is simply zero.
		Since the probability of agent $i$ being the empirically best agent can be written as follows,\footnote{To be precise, we need to take account for the tie-breaking rule and the event that tie happens, but we omit the detail as it can be easily handled and is beyond of our interest.}
		\begin{align*}
			\Pr{\text{agent $i$ is the empirically best agent at round $\tau = Mn$}}
			&=
			\int_{0}^1 \Pr{\muhat_i(M) \ge y}\Pr{C_i(y)}
			\\
			&=
			\int_0^1p_i^{\cS}(y,\sigma(v))q_i^{\cS}(y,\sigma(v))dy,
		\end{align*}
		and it completes the proof.
	\end{proof}
	Using the claim above, for any strategy $\cS$, we can further expand its conditional expected utility as follows.
	\begin{align}
		\sum_{\sigma \in S_{l_i}} 
		\CEx{U_i(\cS)}{\sigma, v}
		&=
		\sum_{\sigma \in S_{l_i}}
		\parans{
		\Ex{\Gamma_i^{\cS}(M,\sigma(v))} + \Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))} \int_0^1p_i^{\cS}(y,\sigma(v))q_i^{\cS}(y,\sigma(v))dy
		}
		\nonumber
		\\
		&=
		\parans{
		\sum_{\sigma \in S_{l_i}}
		\Ex{\Gamma_i^{\cS}(M,\sigma(v))}
		}
		+
		\sum_{\sigma \in S_{l_i}}
		\parans{
		\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		\int_{0}^1p_i^{\cS}(y,\sigma(v))q_i^{\cS}(y,\sigma(v))dy
		}
		\nonumber
		\\
		&=
		\parans{
		\sum_{\sigma \in S_{l_i}}
		\Ex{\Gamma_i^{\cS}(M,\sigma(v))}
		}
		+
		\int_{0}^1
		\parans{\sum_{\sigma \in S_{l_i}}
		\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		p_i^{\cS}(y,\sigma(v))q_i^{\cS}(y,\sigma(v))}dy
		\nonumber
		\\
		&=
		\parans{
		\sum_{\sigma \in S_{l_i}}
		\Ex{\Gamma_i^{\cS}(M,\sigma(v))}
		}
		+
		\int_{0}^1
		p_i^{\cS}(y,\sigma(v))
		\parans{
		\sum_{\sigma \in S_{l_i}}
		\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		q_i^{\cS}(y,\sigma(v))
		}dy,\label{eq:04271244}
	\end{align}
	where the third equality follows from Fubini's theorem, and the last inequality holds since $p_i^{\cS}(y,\sigma(v))$ is independent from $\sigma$.
	
	In case of the truthful strategy $\cO$, since any permutation $\sigma$ yields the same problem instance, all the terms inside \eqref{eq:04271244} remains the same.
	Thus,
	\begin{align}
		\sum_{\sigma \in S_{l_i}} 
		\CEx{U_i(\cS)}{\sigma, v}
		&=
		|S_l| 
		\parans{
		\Ex{\Gamma_i^{\cO}(M,v)}
		+
		\Ex{\Gamma_i^{\cO}(T-Mn,v)}
		\int_{0}^1p_i^{\cO}(y,v)q_i^{\cO}(y,v)dy
		}.\label{eq:05082325}
	\end{align}
	Now it suffices to prove that the RHS of \eqref{eq:05082325} is at least that of \eqref{eq:04271244}.
	
	We first observe that the first term can effectively compared based on our result on the single-agent setting.
	\begin{claim}\label{cl:reduc_to_single}
		For any strategy $\cS$, we have
		\begin{align*}
			\sum_{\sigma \in S_{l_i}}\Ex{\Gamma_i^{\cO}(M, \sigma(v))}	
			\ge
			\sum_{\sigma \in S_{l_i}}\Ex{\Gamma_i^{\cS}(M, \sigma(v))}.
		\end{align*}
	\end{claim}
	\begin{proof}
		Note that $\Gamma_i^{\cO}(M, \sigma(v))$ denotes the agent $i$'s utility at round $M$ under the single agent setting.
		Thus, the claim directly follows from Theorem~\ref{thm:single_rp} since we run ETC with $m = 2l/\Delta^2 \ln (2T)$ as Phase 2 algorithm.
	\end{proof}
	Thus, it remains to compare the latter term that involves the integral.
	
	Given $v \in \R_{\ge 0}^{l_i}$, for $a \in [l_i]$, write $Y_{i,a}$ to denote the event that the arm with mean $v_a$ is selected in the exploitation rounds of $\alg_2$ for agent $i$.
	Let $Z_{i,a}$ denote the event that arm with mean $v_a$ has empirical average reward is the largest at the end of the exploration rounds in $\alg_2$.
	
	Similar to the definition of $\Gamma_i^\cS(\cdot, \cdot)$, define $\Gamma_{i,a}^{\cS}(\cdot, \cdot)$ by the random cumulative rewards when there exists only agent $i$ and only arm $a$, when we're running ETC.
	That is, $\Gamma_{i,a}^{\cS}(t, \sigma(v))$ is just a summation of $t$ random variables where each random variable has expectation $\sigma(v)_a$.
	Note that our construction in equation~\eqref{eq:04262152} verifies that $v_1 \ge v_2 \ge \ldots \ge v_{l_i}$.
	Define $\delta_{i,a} = v_1 - v_a$.
	
	We now construct a lower bound of $q_i^\cO(y,\sigma(v))$ in the following.
	\begin{claim}\label{cl:tail_lower}
		For any $y \in [0,1]$, and $\sigma \in S_{l_i}$, consider arbitrary $v \in [0,1]^l$ such that $v_1 \ge v_2 \ge \ldots \ge v_{l_i}$.
		 Then, we have
		\begin{align*}
			q_i^{\cO}(y, \sigma(v))
			\ge
			\Pr{\Gamma_{i,1}^\cO(M,v) \ge y} \parans{1 - 2\sum_{a=2}^l \exp(-\frac{\delta_{i,a}^2 m }{2})}
		\end{align*}

	\end{claim}
	\begin{proof}[Proof of the claim]
		Due to the independence of rewards from arm $a$ at exploitation phase and the random variable $\Ind{Y_{i,a}}$, we can rewrite $q_i^{\cO}(y,\sigma(v))$ as follows.
		\begin{align}
			q_i^{\cO}(y,\sigma(v))
			=
			q_i^{\cO}(y,v)
			&=
			\Pr{
			\sum_{a=1}^{l_i}
			\parans{
			\Gamma_{i,a}^\cO(m,v)
			+
			\Ind{Y_{i,a}}\Gamma_{i,a}^{\cO}(M-lm, v)
			}
			\ge y
			}
			\nonumber
			\\
			&=
			\sum_{a=1}^{l_i}
			\CPr{
			\sum_{a=1}^{l_i} 
			\parans{
			\Gamma_{i,a}^\cO(m,v)
			+
			\Ind{Y_{i,a}}\Gamma_{i,a}^{\cO}(M-lm, v)
			}
			\ge y
			}{Z_{i,a}}\Pr{Z_{i,a}}
			\nonumber
			\\
			&=
			\sum_{a=1}^{l_i}
			\CPr{
			\Gamma_{i,a}^\cO(M,v) \ge y
			}{Z_{i,a}}\Pr{Z_{i,a}}
			\tag{Definition of $\Gamma_{i,a}^{\cO}$}
			\\
			&=
			\sum_{a=1}^{l_i}
			\Pr{
			\Gamma_{i,a}^\cO(M,v) \ge y
			}\Pr{Z_{i,a}}
			\tag{Independence of $\Gamma_{i,a}^{\cO}$ and $Z_{i,a}$}
			\\
			&\ge
			\Pr{\Gamma_{i,1}^\cO(M,v) \ge y}\Pr{Z_{i,a}},
			\label{ineq:05090246}
		\end{align}
		where the last inequality follows from stochastic dominance between the arms.
		
		Since $Z_{i,1}$ is the complement of $\cup_{a=2}^l Z_{i,a}$, observe that
		\begin{align*}
			\Pr{Z_{i,1}^c}
			&=
			\Pr{\cup_{a=2}^l Z_{i,a}}
			\\
			&\le
			\sum_{a=2}^l\Pr{Z_{i,a}}
			\tag{Union bound}
			\\
			&\le
			\sum_{a=2}^l\Pr{\muhat_{i,1}(m) \le \muhat_{1,a}(m)}
			\tag{Definition of $Z_{i,a}$}
			\\
			&\le
			\sum_{a=2}^l 2\exp(-\frac{\delta_{i,a}^2 m}{2}).
			\tag{Claim~\ref{cl:concen}}
		\end{align*}
		Hence, we obtain
		\begin{align*}
			q_i^{\cO}(y,\sigma(v))
			\ge
			\Pr{\Gamma_{i,1}^\cO(M,v) \ge y} \parans{1 - 2\sum_{a=2}^l \exp(-\frac{\delta_{i,a}^2 m }{2})},
		\end{align*}
		and it proves the claim.
	\end{proof}
	
	To lower bound the difference between $q_i^\cO(y,\sigma(v))$ and $q_i^\cS(y,\sigma(v))$, we use the following rough uper bound for $q_i^\cS(y,\sigma(v))$.
	\begin{claim}\label{cl:tail_upper}
		For any strategy $\cS_i$, $\sigma \in S_{l_i}$, $y \in [0,1]$ and $v \in [0,1]^{l_i}$, we have 
		\begin{align*}
			q_i^{\cS_i}(y, \sigma(v))	 
			\le 
			\Pr{\Gamma_{i,1}^{\cS}(y,\sigma(v)) \ge y}
			=
			\Pr{\Gamma_{i,1}^{\cO}(y,\sigma(v)) \ge y}
		\end{align*}
	\end{claim}
	\begin{proof}[Proof of the claim]
		We can expand
		\begin{align*}
			q_i^{\cS}(y,\sigma(v))
			&=
			\Pr{
			\sum_{a=1}^{l_i}
			\parans{
			\Gamma_{i,a}^\cS(m,\sigma(v))
			+
			\Ind{Y_{i,a}}\Gamma_{i,a}^{\cS}(M-lm, \sigma(v))
			}
			\ge y
			}
			\\
			&=
			\sum_{a=1}^{l_i}
			\CPr{
			\Gamma_{i,a}^\cS(M,\sigma(v)) \ge y
			}{Z_{i,a}}\Pr{Z_{i,a}}
			\\
			&=
			\sum_{a=1}^{l_i}
			\Pr{
			\Gamma_{i,a}^\cS(M,\sigma(v)) \ge y
			}\Pr{Z_{i,a}}.
		\end{align*}
		Note further that $\Pr{\Gamma_{i,a}^\cS(M,\sigma(v)) \ge y} \le \Pr{\Gamma_{i,1}^\cS(M,\sigma(v)) \ge y}$ due to the stochastic dominance of the arm with mean $v_1$ over the arm with mean $v_a$, for any $a \in [l_i]$.
		Thus, we have
		\begin{align*}
			q_i^{\cS}(y,\sigma(v))
			&\le
			\sum_{a=1}^{l_i}
			\Pr{
			\Gamma_{i,1}^\cS(M,\sigma(v)) \ge y
			}\Pr{Z_{i,a}}
			\\
			&=
			\Pr{\Gamma_{i,1}^\cS(M,\sigma(v)) \ge y},
		\end{align*}
		and it completes the proof of the claim.
		Note that 
		\begin{align*}
			\Pr{\Gamma_{i,1}^{\cS}(y,\sigma(v)) \ge y}
			=
			\Pr{\Gamma_{i,1}^{\cO}(y,\sigma(v)) \ge y}	
		\end{align*}
		follows from the fact that $\Gamma_{i,1}^{\cS}(y,\sigma(v)) = \Gamma_{i,1}^{\cO}(y,\sigma(v))$ since both are random rewards when there is only arm with mean rewards $v_1$ of agent $i$.
	\end{proof}

	Now, combining Claim~\ref{cl:tail_lower} and~\ref{cl:tail_upper}, we obtain
	\begin{align}
		q_i^{\cO}(y, \sigma(v)) - q_i^{\cS}(y,\sigma(v))
		&\ge
		-2\Pr{\Gamma_{i,1}^\cO(M,\sigma(v)) \ge y}
		\parans{\sum_{a=2}^{l_i} \exp(-\frac{\delta_{i,a}^2 m }{2})}
		\nonumber
		\\
		&\ge
		-2l_i \Pr{\Gamma_{i,1}^\cO(M,\sigma(v)) \ge y}
		\parans{\exp(-\frac{\Delta^2 m }{2})}
		\tag{Due to $\delta_{i,a} \ge \Delta$}
		\\
		&\ge
		-2l_i \cdot \frac{q_i^{\cO}(y, v)}{\Pr{Z_{i,1}}} \cdot
		\parans{\exp(-\frac{\Delta^2 m }{2})}\tag{Due to ineq. \eqref{ineq:05090246}}
		\\
		&\ge
		-2l_i \cdot \frac{q_i^{\cO}(y, v)}{1 - \sum_{a=2}^{l_i} 2\exp(-\frac{\delta_i^2 m}{2})} \cdot
		\parans{\exp(-\frac{\Delta^2 m }{2})}
		\nonumber
		\\
		&\ge
		-2l_i
		\cdot 
		\frac{q_i^{\cO}(y, v)}{1 - 2l_i\exp(-\frac{\Delta^2 m}{2})} \cdot
		\parans{\exp(-\frac{\Delta^2 m }{2})},
		\label{ineq:05090213}
	\end{align}
	where the fourth inequality follows from the concentration on $Z_{i,1}$ in the proof of Claim~\ref{cl:tail_lower}.

	Now we consider two cases regarding $\sigma$: (i) when $\sigma(1) = 1$ and (ii) otherwise.
	
%	\paragraph{case (i): $\sigma(1) = 1$}
%	This means that there exists a suboptimal arm with at least one replication.
%	In this case, as per the proof of 
%	
%	\paragraph{case (ii): $\sigma(1) \neq 1$}
	
	Recall that it suffices to prove that the RHS of \eqref{eq:05082325} is at least that of \eqref{eq:04271244}.
	Due to Claim~\ref{cl:reduc_to_single}, it suffices to prove the following inequality.
	\begin{align}
		\int_{0}^1
		&p_i^{\cS}(y,\sigma(v))
		\parans{
		\sum_{\sigma \in S_l}\underbrace{\paranm{\Ex{\Gamma_i^{\cO}(T-Mn,\sigma(v))}
		q_i^{\cO}(y,\sigma(v))
		-
		\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		q_i^{\cS}(y,\sigma(v))}}_{\Theta(\sigma, v)}
		}dy 
		\ge 
		0.
		\label{eq:05090205}
	\end{align}
%	Now we prove the following positive correlation.
%	\begin{claim}
%		For any $\sigma_1,\sigma_2 \in S_l$, 
%		it satisfies $q_i^{\cS}(y,\sigma_1(v)) \ge 	q_i^{\cS}(y,\sigma_2(v))$ iff the following holds.
%		\begin{align*}
%			\Ex{\Gamma_i^{\cS}(T-Mn,\sigma_1(v))} \ge \Ex{\Gamma_i^{\cS}(T-Mn,\sigma_2(v))}	
%		\end{align*}
%	\end{claim}
%	\begin{proof}
%		\note{TBD - Intuitive}
%	\end{proof}
%	Thus, by Chebyshev's sum inequality, we have
%	
%
%
%
%	
%	=========2nd=========
	
	
	Note that the term inside the summation can be decomposed as follows.
	\begin{align*}
		\Theta(v)
		=
		\paranm{\Ex{\Gamma_i^{\cO}(T-Mn,\sigma(v))} - \Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}}q_i^{\cO}(y,\sigma(v))
		\\
		+
		\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		\paranm{q_i^\cO(y,\sigma(v)) - q_i^{\cS}(y,\sigma(v))}.
	\end{align*}
	
	Due to \eqref{ineq:05090213}, we further obtain
	\begin{align*}
		\Theta(\sigma, v) 
		&\ge 
		\underbrace{\paranm{\Ex{\Gamma_i^{\cO}(T-Mn,\sigma(v))} - \Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}}q_i^{\cO}(y,\sigma(v))}_{\Theta_1(\sigma, v)}
		\\
		&-
		\underbrace{2\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		\cdot l_i\cdot \frac{q_i^{\cO}(y, v)}{1 - 2l_i\exp(-\frac{\Delta^2 m}{2})} \cdot
		\parans{\exp(-\frac{\Delta^2 m }{2})}}_{\Theta_{2}(\sigma, v)} 
		.
	\end{align*}
	By summing over $\sigma \in S_{l_i}$, for $\Theta_1(\sigma, v)$, we have
	\begin{align*}
		\sum_{\sigma \in S_l} \Theta_1(\sigma, v)	
		&=
		\sum_{\sigma \in S_l}\paranm{\Ex{\Gamma_i^{\cO}(T-Mn,\sigma(v))} - \Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}}q_i^{\cO}(y,\sigma(v))
		\\
		&=
		q_i^{\cO}(y,\sigma(v)) \cdot \sum_{\sigma \in S_{l_i}}\paranm{\Ex{\Gamma_i^{\cO}(T-Mn,\sigma(v))} - \Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}}
	\end{align*}
	
	From inequality~\eqref{ineq:05090221} and \eqref{ineq:05090222} we know that
	\begin{align*}
		\sum_{\sigma \in S_{l_i}}\paranm{\Ex{\Gamma_i^{\cO}(T-Mn,\sigma(v))} - \Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}}
		&\ge
		\sum_{a \in [l_i]} \delta_{i,a} (\frac{m}{l_i} - 1)
		\\
		&\ge
		\sum_{a \in [l_i]} \delta_{i,a} (\frac{2l_i \ln 2T / \Delta^2}{l_i} - 1)
		\\
		&= 
		\sum_{a \in [l_i]} \delta_{i,a} (\frac{\ln 2T}{\Delta^2} - 1),
	\end{align*}
	which implies
	\begin{align*}
		\sum_{\sigma \in S_l} \Theta_1(\sigma, v)
		&\ge
		q_i^{\cO}(y,\sigma(v)) 
		\cdot \sum_{i \in [l]} \delta_{i,a} (\frac{\ln 2T}{\Delta^2} - 1).
	\end{align*}
	
	Putting $m = 4 \cdot \frac{2}{\Delta^2} (\max_i l_i) \ln(2T)$, observe that the following holds.
	\begin{align*}
		\exp(-\frac{\Delta^2 m}{2}) \le \frac{1}{4l_iT}	
	\end{align*}

	Hence, for $\Theta_2(\sigma,v)$, we further obtain
	\begin{align*}
		\sum_{\sigma \in S_{l_i}}\Theta_2(\sigma,v)
		&=
		2\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		\cdot l_i\cdot \frac{q_i^{\cO}(y, v)}{1 - 2l_i\exp(-\frac{\Delta^2 m}{2})} \cdot
		\parans{\exp(-\frac{\Delta^2 m }{2})}
		\\
		&\le
		4\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		\cdot l_i\cdot q_i^\cO(y,v)\cdot \frac{1}{4l_iT}
		\\
		&=
		\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		 q_i^\cO(y,v)\frac{1}{4T}
		\\
		&\le
		\frac{q_i^{\cO}(y,v)}{4}\tag{Since $\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))} \le T$}
	\end{align*}
	
	Combining the above observations, for $\Theta(\sigma, v)$, we obtain
	\begin{align*}
		\sum_{\sigma \in S_{l_i}}\Theta(\sigma, v)
		&\ge
		q_i^{\cO}(y,v)
		\parans{
		\sum_{a \in [l_i]} \delta_{i,a} (\frac{\ln 2T}{\Delta^2} - 1)
		-
		\frac{1}{4}
		}
		\\
		&\ge
		q_i^{\cO}(y,v)
		\parans{
		\sum_{a \in [l_i]}  (\frac{\ln 2T}{\Delta} - 1)
		-
		\frac{1}{4}
		}
		\\
		&=
		q_i^{\cO}(y,v)\parans{l_i \cdot \ln(2T) - l_i -\frac{1}{4}} 
		\\
		&\ge 0,
	\end{align*}
	where the last inequality follows from $T \ge 1$ and $q_i^\cO(y,v) \ge 0$.
	Thus, inequality \eqref{eq:05090205} is true, and it finishes the proof.

	
%	===========	===========	===========	===========	===========	===========
%
%	
%	Let $\cS$ be agent $i$'s strategy with replication vector $r = (r_1,r_2,\ldots, r_l)$, with at least one coordinate being strictly positive.
%	Without loss of generality, suppose $r_1 \ge r_2 \ge \ldots \ge r_l$, then we have $r_1 \ge 1$.
%	This indeed brings no difference since the expected payoff is marginalized over all the possible permutations, as we see thus far.
%	Let $\Omega_1$ be a set of permutation $\sigma \in S_l$ such that arm $\sigma(1) = 1$, \ie the best arm is replicated the most times, and define $\Omega_2 = S_l \setminus \Omega_1$.
%	We handle case $\omega \in \Omega_1$ and $\omega \in \Omega_2$ separately.
	
	

%
%	
%	Since our $alg_2$ is stochastically schur-concave, if two strategies $\cS$ and $\cS'$ with replication vector $r$ and $r'$ satisfy $r' \succ r$, then we can obtain
%	\begin{align*}
%		\sum_{\sigma \in S_l}
%		q_i^{\cS}(y,\sigma(v))
%		\ge
%		\sum_{\sigma \in S_l}
%		q_i^{\cS'}(y,\sigma(v)).
%	\end{align*}
%	Furthermore, the following easily follows from the fact that $\alg_2$ is SPF.
%	\begin{claim}
%		Given that $\alg_2$ is SPF, for any $v$ and $t$, we have $\Ex{\Gamma_i^{\cS}(t,v)}\ge \Ex{\Gamma_i^{\cS'}(t,v)}$.
%	\end{claim}
%	\begin{proof}
%		It is easy to check that SPF implies EPF.
%		Then, the claim directly follows from the single-agent characterization in  Theorem~\ref{thm:single_pf_rp}.
%	\end{proof}
%	
%	Combining the above facts, we can obtain
%	\begin{align*}
%		\sum_{\sigma \in S_l} 
%		\CEx{U_i(\cS)}{\sigma, v}
%		\ge
%		\sum_{\sigma \in S_l} 
%		\CEx{U_i(\cS')}{\sigma, v}.
%	\end{align*}

%	Thus, putting back to \eqref{eq:04262152} completes the proof.
%
%	
\end{proof}


==> conclusion.tex <==
\section{Conclusion}
We study bandit mechanism design problem to disincentivize replication of arms, which is the first to study Bayesian extension of \cite{shin2022multi}.
Our extension brings significant challenges in analyzing equilibrium, even in the single-agent setting.
We first prove that H-UCB of \cite{shin2022multi} does not work.
We then characterize sufficient conditions for an algorithm to be replication-proof in the single-agent setting.
A special case of our analysis boils down to identify whether a bandit algorithm is robust against an adversary who replicates some arms uniformly-at-random given a bandit instance, which might be of independent interest.
Based on the single-agent result, we obtain the existence of replication-proof algorithm with sublinear regret, by introducing a restarting round and exploiting the structural property of exploration-then-commit algorithm.
We further provide a regret analysis of our replication-proof algorithm, which matches the regret of H-UCB.
Obtaining a lower bound of any replication-proof algorithm, improving the regret upper bound using more sophisticated algorithm possibly with adaptive exploration, and further investigating which algorithms satisfy truthfulness under random permutation remain as major open problems.


==> discussion.tex <==
\section{Discussions}
\subsection{algorithm}

\begin{algorithm} 
\SetAlgoLined
%$i \in \set{N}$, $\set{S} = \cup_{i \in \set{N}} \set{S}_i$\\

Initialize $R(i), N(i), r(a)$ and $n(a)$ at zero  
for all $i \in \set{N}$ and $a\in \cup_{i \in \set{N}} \set{S}_i$;

%Initialize $r(a) = n(a) = R(i)=N(i)=0$~$\forall a, i$;


 \For{$t=1,2,\ldots$}{
  \tcp{Phase 1 - agent selection}
  \eIf{Unexplored agent exists}{ 
    %\tcp{Agent initialization}
    Pick an unexplored $\hat{i}\in \{i \in \set{N}: N(i) = 0\} $; % an unexplored agent ;
  }{
    % $i^\star = \argmax_{i} \{R_i + \sqrt{2\ln t / N_i}\}$
    Pick $\hat{i} = \argmax_{i \in \set{N}} \left\{R(i) + \sqrt{\frac{2 \sqrt{t}}{N(i)}} \right\}$;
  }
  
  \tcp{Phase 2 - arm selection}
  \eIf{Unexplored arm exists in $\set{S}_{\hat{i}}$}{
    %\tcp{Arm initialization}
    Pick an unexplored $\hat{a} \in \{a \in \set{S}_{\hat{i}}: n(a) = 0\} $; % an unexplored agent
  }{
    % $a^\star = \argmax_{a \in \set{S}_{i^\star}} \{r(a) + \sqrt{2 \ln N_i / n(a)}\}$
    Pick $\hat{a} = \argmax_{a \in \set{S}_{\hat{i}}} 
    \left\{r(a) + \sqrt{\frac{2 \ln N(i)}{n(a)}} \right\}$;
  }
  
  Play $A_t = \hat{a}$ and receive reward $R_t$; \\
  Update statistics:
  $r(\hat{a}) \leftarrow \tfrac{r(\hat{a})n(\hat{a}) + R_t}{n(\hat{a})+1}; ~~
  R(\hat{i}) \leftarrow \tfrac{R(\hat{i})N(\hat{i}) + R_t}{N(\hat{i})+1};$
  
  $n(\hat{a}) \leftarrow n(\hat{a}) + 1; ~~ N(\hat{i}) \leftarrow N(\hat{i}) + 1;$
 }
 \caption{Hierarchical UCB (H-UCB) \label{alg:hucb}}
\end{algorithm}

The major bottleneck in analyzing incentive compatibility in Bayesian setting is that it is hard to show the following fact.
\begin{conjecture}
Consider Bernoulli arms.
\begin{enumerate}
    \item A: run UCB with instance $(0.1, 0.3)$
    \item B: run UCB with instance $(0.1, 0.3, 0.3)$
    \item C: run UCB with instance $(0.1, 0.1, 0.3)$
\end{enumerate}
Note that $0.1, 0.3$ can be replaced with any two different numbers.
Definitely in terms of regret, regret of $C > A > B$ (this can be easily proved using coupling technique of ~\cite{shin2022multi}).
Main question is, then, how can we prove that (average regret of B,C) is larger than (regret of A)?
I personally think that we should prove stochastic dominance of regret random variables, rather than comparison between expected regret, i.e., $R_B + R_C >= 2R_A$ where $>=$ is (first-order) stochastic dominance.
\end{conjecture}
This conjecture basically implies, although it needs to be generalized, that replicating one arm randomly does not give any incentive to the agent, in case of H-UCB in \cite{shin2022multi}.
To briefly see why, phase 2 is running UCB, and by conjecture, replicating arm only increases expected regret, however the agent should maximize the expected regret in phase 2 to be selected more in phase 1.

This was not happened in complete information setting, since complete information setting reduces to the single-arm-per-agent case which significantly simplifies the analysis of incentive compatibility.

\paragraph{ETC style algorithm}
Using exploration-then-commit (ETC) style of algorithm, we can directly compute the regret, as depicted by the failure probability in exploitation phase.
In this context, we've tried Algorithm~\ref{alg:agent_explore_comm} which we believed to be incentive compatible.

\begin{algorithm}
  \SetAlgoLined
  Parameter $N_0$; \\
  \For{$i=1,\ldots, K$}{
    Uniform randomly sort the arms of agent $i$; \\
  	Explore the arms total $N_0$ times in round-robin manner; \\
  } 
  Select empirically best arm and pull it for the remaining rounds
 \caption{Agentwise-Exploration-then-Commit}\label{alg:agent_explore_comm}
\end{algorithm}

However, suppose that there is an agent with only $0$ reward arm.
If this agent replicates as much as possible, so that during the entire exploration phase each replicated arm will be selected a single time, then it is hard to distinguish that this agent's arm is indeed bad.
This definitely gives incentive for this agent to replicate, which yields that this does not have DSIC.

\paragraph{hierarchical algorithm}
Next, we thought about hierarchical algorithm with phase 2 changed to ETC, as described by Algorithm~\ref{alg:hucb}.
For simplicity, I denote $0.1'$ the replicated arm of $0.1$.
In this case, we can at least (roughly) prove that  submitting $0.1,0.3,0.1',0.3'$ is worse than submitting $0.1,0.3$.
This is because in order to be selected more in phase 1, the agent should make the algorithm find arm with $0.3$ with higher probability.
Submitting more $0.1$ and $0.3$ only reduces this probability.
To see why, let the length of exploration phase be $4N$.
In the replicated case, call it an instance $X$, each $0.1,0.3,0.1',0.3'$ will be sampled $N$ times in the exploration phase.
In the truthful case, call it an instance $Y$, each $0.1,0.3$ will be sampled $2N$ times.
Suppose that the infinite tape of $0.1$ and infinite tape of $0.1'$ till round $t$ in problem $X$ is coupled to the infinite tape of $0.1$ till round $2t$ in problem $Y$ for any $t \in [T]$.
For example, at even round, $0.1$ in $Y$ is coupled with $0.1'$ in $X$, and at odd round, it is coupled with $0.1$ in $X$.
In such a coupling, joint probability measure over $N$ random variables of $0.1$ and $0.1'$ in problem $X$ exactly corresponds to probability measure over $2N$ random variables in problem $Y$, thus we can just compare the statistics in $X,Y$ by assuming that their random incidences are coupled in this manner.
Then, we can conclude, followed by some probability calculations, that the probability of false exploitation is higher for the replicated case.


Note however that in order for this argument to be held, the length of exploration phase should be some multiplies of the registered arm.
What even worse is that we cannot handle the case of single replication using these coupling techniques.
For example, if agent with two original arms replicate only one arm, there are two possible cases: when better arm is replicated and when worse arm is replicated. Hence, this strategy's payoff will be average of this one.
Indeed, the payoff exactly corresponds to the average regret of B,C in Conjecture 1.
Proving this conjecture seems not easy, so it will be interesting if one can prove this conjecture with some nice algorithms.

Secondly, we should derive a lower bound for any incentive-compatible algorithm.
Recall that Algorithm~\ref{alg:agent_explore_comm} does not work.
This gave us some general intuitions that some kinds of hierarchy is essential to make algorithm incentive-compatible.
Combined with the fact that Algorithm~\ref{alg:agent_explore_comm} has regret of $T^{2/3}$, we conjecture that any incentive-compatible algorithm suffers regret lower bound of $O(T^{3/4})$.


\paragraph{SPA style algorithm}
See~\cite{braverman2019multi}.
The analysis seems to again reduce to Conjecture 1.


% \subsection{lower bound}
% Known results: any non-adaptive exploration algorithm has regret lower bound of $T^{2/3}$.

% \todo{priority 2: Regret lower bound of any incentive-compatible algorithm is $T^{2/3}$.}

% \todo{conjecture: if the algorithm explores adaptively, then it has regret lower bound of $O(T^{3/4})$, then since non-adaptive exploration has lower bound of $O(T^{2/3})$, the proof will be done.}
% \suho{This does not work}




\begin{algorithm} 
\SetAlgoLined
%$i \in \set{N}$, $\set{S} = \cup_{i \in \set{N}} \set{S}_i$\\

Initialize $R(i), N(i), r(a)$ and $n(a)$ at zero  
for all $i \in \set{N}$ and $a\in \cup_{i \in \set{N}} \set{S}_i$;

%Initialize $r(a) = n(a) = R(i)=N(i)=0$~$\forall a, i$;


 \For{$t=1,2,\ldots$}{
  \tcp{Phase 1 - agent selection}
  
  \eIf{Unexplored agent exists}{ 
    %\tcp{Agent initialization}
    Pick an unexplored $\hat{i}\in \{i \in \set{N}: N(i) = 0\} $; % an unexplored agent ;
  }{
    % $i^\star = \argmax_{i} \{R_i + \sqrt{2\ln t / N_i}\}$
    Pick $\hat{i} = \argmax_{i \in \set{N}} \left\{R(i) + \sqrt{\frac{2 \sqrt{t}}{N(i)}} \right\}$;
  }
  
  \tcp{Phase 2 - arm selection}
  If $N(i) \le 1/2T^{1/3} \log(T)^{1/3}$, round-robin exploration of arms in $\set{S}_i$;\\
  Else, commit $\hat{a} = \argmax_{a \in \set{S}_{\hat{i}}} 
    \left\{r(a) \right\}$
  Play $A_t = \hat{a}$ and receive reward $R_t$; \\
  Update statistics:
  $r(\hat{a}) \leftarrow \tfrac{r(\hat{a})n(\hat{a}) + R_t}{n(\hat{a})+1}; ~~
  R(\hat{i}) \leftarrow \tfrac{R(\hat{i})N(\hat{i}) + R_t}{N(\hat{i})+1};$
  
  $n(\hat{a}) \leftarrow n(\hat{a}) + 1; ~~ N(\hat{i}) \leftarrow N(\hat{i}) + 1;$
 }
 \caption{Hierarchy(UCB, Exploration-then-Commit) \label{alg:hucb}}
\end{algorithm}




\section{Byproducts in some trials}
	\note{Below - attempt to show it with sth between EPF and SPF.}
	\begin{assumption}
		For any strategy $\cS$, we have $\Ex{\Gamma_i^{\cO}\Ind{\Gamma_i^{\cO} \le x}} \le \Ex{\Gamma_i^{\cS}\Ind{\Gamma_i^{\cS} \le x}}$ for any $x \in [0,1]$. 	
	\end{assumption}
	
	\begin{claim}
		Let $p= (p_i)_{i \in [l]}$, $q = (q_i)_{i \in [l]}$ and $q' = (q'_i)_{i \in [l]}$ be sequences of real values such that $p$ is monotone increasing, $q$ and $q'$ are monotone decreasing, and $q$ majorizes $q'$ in an inverse order, \ie $\sum_{i=1}^k q_{n-i+1} \ge \sum_{i=1}^k q'_{n-i+1}$ for any $k \in [n]$.
		Then, we have $\sum_{i \in [l]}p_iq_i \ge \sum_{i \in [l]}p_iq'_i$.
	\end{claim}
	\begin{proof}
		Some algebra
	\end{proof}
	
	By assumption we have
	\begin{align*}
		\sum_{y \le x}\sum_{\sigma \in S_l} q_i^{\cS'}(y,v)	
		\ge
		\sum_{y \le x}\sum_{\sigma \in S_l} q_i^{\cS'}(y,v),
	\end{align*}
	for any $x \in [0,1]$.
	Hence, by the claim we obtain
	\begin{align*}
		\sum_{y \in [0,1]}
		p_i^{\cO}(y,v)
		\parans{
		\sum_{\sigma \in S_l}
		q_i^{\cO}(y,v)
		}
		\ge
		\sum_{y \in [0,1]}
		p_i^{\cS}(y,v)
		\parans{
		\sum_{\sigma \in S_l}
		q_i^{\cS}(y,v)
		},
	\end{align*}
	and it completes the proof.


==> dynamic.tex <==
\section{Dynamic Setting with Online Arrivals}\label{sec:dynamic}
\note{Not quite sure to add this section or not.}
In this section, we discuss how our model and corresponding results can be extended to beyond the simultaneous game setup.
We mainly discuss that our model accommodates a \emph{dynamic game} version of interpretation.
Instead of considering simultaneous game between the agents, we consider an online arrival of agents.
At each time step $t$,

suppose that at each time step $t$, an agent $t$ with $\cO_t$ arrives and decide which (sub)set of arms to register in the platform.
\note{Make it more formal}
The arms registered in the system are cumulated over the rounds, and the algorithm runs from the initial round with no contents.
The agents may have partial information on the other arms exist in the system, \eg by observing some statistics of the system or directly exploring the contents, or may have no information at all.
In any case, our notion of dominant strategy effectively allows us to guarantee an \emph{anytime truthfulness} of our algorithm, \ie regardless of arrival time, own prior distribution and information on other agents, any agent will play truthful strategy.
We will discuss this more formally in Section~\ref{sec:dynamic}.


==> intro.tex <==
\section{Introduction}\label{sec:intro}
Multi-armed bandit (MAB) algorithms are an important paradigm for interactive learning that focuses on quantifying the trade-off between exploration and exploitation \citep{slivkins2019introduction}. They are used to model various practical applications where there is a set of actions (arms) to be selected (pulled) over a collection of rounds. Pulling an arm yields a reward sampled from its distribution which is generally different from the other arms' distributions. The objective is to maximize the sum of rewards accumulated through the rounds or equivalently minimize the \emph{regret} with respect to the optimal clairvoyant arm choice. The main difficulty of the problem stems from the fact that the distributions are unknown and have to be learned by pulling the arms over a collection of rounds. Due to its significant usefulness, the MAB model has been used in various applications such as recommender systems  \citep{barraza2020introduction,tang2014ensemble}, dynamic pricing by \citep{badanidiyuru2018bandits,badanidiyuru2014resourceful}, and clinical trials by \citep{djallel2019survey} to name a few.
%Clearly, algorithms with low regret (good performance) minimize the pulls of all sub-optimal arms. 

In deploying MAB algorithms in real-world applications, however, the rewards are often not coming from stochastic distributions, but from a collection of rational individuals (agents) who seek to maximize their own payoff.
Consequently, there has been a surge of interest in bandit mechanism design, which studies MAB algorithms which induces a good outcome with respect to agents' strategic behavior, while maintaining its efficiency.
Examples of such settings include two-sided matching markets, where agents learn their preferences through sequential interactions \citep{liu2021bandit,liu2020competing}, and learning in environments where agents can strategically modify the realized rewards of their arms \citep{braverman2019multi,feng2020intrinsic}.
%In the meantime, MAB algorithms are being exceedingly applied in game theoretic settings where there are a collection of individuals (agents) interested in maximizing their utility, and thus there has been a surge of interest in bandit mechanism design. In words, MAB algorithms that take agents' incentives into account and achieve good performance. Examples include two-sided matching markets where agents learn their preferences thorugh sequential interactions \citep{liu2021bandit,liu2020competing} and learning in settings where agents can strategically modify the realized rewards of their arms \citep{braverman2019multi,feng2020intrinsic}. 

Recently, \cite{shin2022multi} considered a problem where agents register arms to a platform that uses a MAB algorithm to minimize regret. 
Each agent has an original set of arms, and the mean reward of each arm is known to him a priori, \ie agents are \emph{fully-informed}.
Each agent receives a fixed constant portion of the reward whenever its arm is pulled, and tries to maximize cumulative reward.
Importantly, each agent can potentially register the same arm \emph{more than once} (replication), which possibly ruins the exploration-exploitation balance of the bandit algorithm, where the replicated arm has exactly the same are with the original arm.
Indeed, \cite{shin2022multi} show that ``ordinary'' algorithms such as upper-confidence-bound (UCB) or $\eps$-greedy induce rational agents to replicate infinitely many times, and thus the algorithm suffers linear regret.
To address this problem, \cite{shin2022multi} introduce a novel problem of designing \emph{replication-proof} bandit mechanism where any agents' dominant strategy is to not replicate.
They propose a hierarchical algorithm that consists of two phases, where the first phase determines agent and the second one decides the arm to select within the selected agent.

Although the replication-proof mechanism of \cite{shin2022multi} is remarkable, the assumptions that each agent is fully informed about its own arms is very strong, both in terms of theoretical and practical perspective.
Intuitively, if an agent knows all of its own arms' mean rewards, there exists no reason for the agent to consider suboptimal arms.
Indeed, this assumption significantly simplifies the equilibrium analysis so that the problem simply reduces to the case under which each agent only has a \emph{single arm}.
Then, it is straightforward to check that any bandit algorithm is replication-proof under a single-agent setting, and their contribution lies on introducing a hierarchical structure to maintain replication-proofness with multiple agents.
Moreover, in practice, it is more reasonable to assume that each agent only has partial information regarding its own arm.
For instance, in an online content platform, each content provider usually does not know the quality of each content that has not been posted yet, but only can guess its outcome, based on the data possibly acquired from the previous contents he/she may have.

In this context, we study a \emph{Bayesian extension}\footnote{We remark that our notion of Bayesian differs from that of Bayesian mechanism design or Bayesian game in the literature. In those settings, each agent usually computes ex-interim payoff given the \emph{incomplete} information regarding others' types. In this paper, however, we aim to develop an \emph{incentive-compatible} mechanism under which each agent truthfully register all the arms without regard to others' actions, when he/she faces uncertainty on their own arms and computes ex-ante payoff over such uncertainty.} of the replication-proof bandit mechanism design problem, where each agent only knows such a distribution from which its own arm's mean reward is sampled.\footnote{To practically motivate our problem setup, in creator economy like Youtube, a content creator typically does exactly know about each content's quality in advance, but only has some historical information on the qualities of his/her previous content. Historical information can be thought of as a prior distribution of the agent in our setting. The setting by Shin et al. can be interpreted as a scenario in which all the agents know the exact quality of their contents. In this case, the agent does not have any ambiguity in registering/replicating which arms, since he/she knows own best arm, which might be a bit impractical.}
Given the prior distribution, each agent computes its own ex-ante payoff by taking expectation over all the possible realization of its own arms, and commits to a strategy that maximizes the payoff.
Importantly, we aim to obtain an \emph{dominant strategy incentive-compatible} (DSIC) mechanism such that each agent has no incentive to deviate from its truthful strategy, \ie submitting all the original arms without any replication, regardless of the others' strategies.

Our extension brings significant challenges in analyzing an algorithm's equilibrium compared to the fully-informed agent setting.
Notably, even in a single-agent case, it is not trivial to obtain a replication-proof algorithm.
This is in stark contrast to fully-informed setting by~\cite{shin2022multi} under which any bandit algorithm trivially satisfies replication-proofness.
The question of designing replication-proofness in the single-agent setting spawns an intriguing question of \emph{comparing expected regret of multiple bandit instances}, which we will elaborate more shortly.

\paragraph{Outline of the paper}
In the two subsequent subsections, we present our main contributions and related works.
Section~\ref{sec:model} introduces formal problem setup and preliminary.
The failure of H-UCB and its implication is provided in Section~\ref{sec:fail}.
Section~\ref{sec:single} develops our main intuition on constructing replication-proof algorithm by investigating single-agent setting, and Section~\ref{sec:multi} extends this result and provide our main result on the replication-proof algorithm with sublinear regret.

\subsection{Contributions and techniques}
Overall, our main results towards replication-proof algorithms are presented in a step-by-step manner.
We start with investigating the previous algorithm suggested by~\cite{shin2022multi}, which mainly builds upon standard UCB\footnote{We focus our attention on a structured class of UCB algorithms with index $\muhat_a + f(t,n_a)$ where $\muhat_a$ denotes empirical average reward, $t$ is current round, and $n_a$ denotes the number of pulls of arm $a$. Note that standard UCB1~\cite{auer2002finite} has a form of $f(t,n_a) = \sqrt{\log(t)/n_a}$.} along with the idea of hierarchical structure.
Unlike from the fully-informed setting under which any bandit algorithm is replication-proof in the single-agent setting, we reveal that the standard UCB algorithm fails to be replication-proof even with single-agent, regardless of the exploration parameter $f$.
Mainly, we show that UCB does not satisfy a property called \emph{truthful under random permutation} which will be elaborated shortly, via construction of worst-case problem instance that exploits structural properties of UCB which adaptively and deterministically (up to tie-break) select the arms.
This phenomenon carries over to the multi-agent setting, so that UCB equipped with hierarchical structure, namely H-UCB by~\cite{shin2022multi}, fails to be replication-proof, regardless of the number of agents.

To tackle this challenge, we first thoroughly investigate the single-agent setting, and characterize necessary and sufficient conditions for an algorithm to be replication-proof.
Let us provide a simple example to explain the main technical challenges one would face in analyzing equilibriums.
\begin{example}
	Consider a single agent whose prior distribution is $Bern(0.5)$. 
	The agent has two original arms, say arm $a$ and $b$.
	There exist three cases in terms of the pair of realized rewards $(\mu_a, \mu_b)$: (i) $(1,1)$ with probability (w.p.) $0.25$ (ii) $(1,0)$ w.p. $0.25$, (iii) $(0,1)$ w.p. $0.25$, (iv) $(0,0)$ w.p. $0.25$.
	Suppose that the agent decides replicate only arm $a$, without observing the ex-post realization of the mean rewards, say the replicated arm $a'$.
	For cases (i) and (iv), the replicated arm has no effect since all the arms have the same mean rewards, \ie pulling any arm yields the same expected reward, so let's focus on case (ii) and (iii).
	In case (ii), the resulting bandit instance from the agent's strategy will be $\cI_A: (\mu_a, \mu_{a'},\mu_b) = (1,1,0)$ whereas in case (iii), it will be $\cI_B: (1,0,0)$
	Hence, compared to the strategy with no replication, the agent's gain from replicating arm $a$ is equal to the gain from the average of expected payoff in case (ii) and (iii), compared to the case in which the algorithm runs with bandit instance $\cI_O: (1,0)$.
	Hence, if the agent has no incentive to replicate arm $a$ once, the expected regret under $\cI_O$ should be at most the average of that under $\cI_A$ and $\cI_B$.
\end{example}
%
%We observe that the problem of designing a replication-proof algorithm even under this simple case (single agent, Bernoulli arms) boils down to the following question.
%\begin{example}
%    Consider a bandit instance $\cI_A$ with two Bernoulli arms with mean rewards $0.1$ and $0.5$. Consider Bernoulli bandit instances $\cI_B$ and $\cI_C$ each equipped with three Bernoulli arms such that $B$'s arms have mean rewards $0.1, 0.1$ and $0.5$ and $\cI_C$'s arms have $0.1, 0.5$ and $0.5$. 
%    Given some standard bandit algorithms, would the expected regret under $\cI_A$ be larger than the average of expected regret under $\cI_B$ and $\cI_C$?
%\end{example}
Even under simplistic and standard algorithms such as UCB, it is not straightforward to answer the above question.
Intuitively, instance $\cI_A$ will incur smaller regret as the number of optimal arm increases, but the instance $\cI_B$ will have larger regret due to more suboptimal arms with mean reward $0.1$.\footnote{Note that this can be shown using a coupling-like argument between random reward tapes of the arms, combined with a regret decomposition lemma. See~\cite{shin2022multi} for more details.}
Thus, the question is whether the loss from $\cI_B$ will be larger than the gain from $\cI_A$ in average, compared to $\cI_O$.

More formally, we can refine the above observation as the following fundamental question in comparing the expected regret of multiple bandit instances.
\begin{center}
	\emph{Given an arbitrary stochastic bandit problem, consider an adversary who uniformly randomly selects an arm and replicates. Which bandit algorithms guarantee that the regret does not increase against the adversary? What if it randomly replicates multiple arms possibly at different times?}
\end{center}
We affirmatively answer this question by proving that, there exists an algorithm that satisfies the above questions for \emph{any} bandit instance under some mild assumptions.
To this end, we introduce a notion of \emph{random-permutation regret}, which captures the average regret of an agent's strategy with replication without observing the ex-post realization.
We show that if an algorithm satisfies that the random-permutation regret does not increase with respect to replication (called, truthfulness under random permutation - TRP), and is permutation invariant between the arm indices, then it is replication-proof under single-agent setting.
We refer to Section~\ref{sec:single} for precise definitions.
We further prove that the conditions presented above are indeed necessary for any algorithm to be replication-proof.
In fact, the failure of UCB comes from violating TRP.
Meanwhile, we prove that exploration-then-commit (henceforth ETC) satisfies these properties, thus replication-proof in the single-agent setting.

With the goal of designing a replication-proof algorithm for any number of agents, we combine several techniques upon the observation above.
First, we borrow the hierarchical structure of~\cite{shin2022multi}, and analyze hierarchical algorithm with each phase running ETC, which effectively decomposes each agent's payoff from each other.
Moreover, our analysis heavily depends on the non-adaptivity and decoupled nature of ETC.
It remains as a major open problem whether it is necessary for the algorithm to have non-adaptive exploration structure in order to satisfy TRP.
In addition, we introduce a restarting round in the second phase at the beginning of the exploitation rounds in the first rounds.
This largely simplifies the analysis of the selected agent in the exploitation rounds in the first phase, since the second phase simply reduces to the single-agent case with that selected agent with the highest empirical average reward.
We cement our result by proving that our algorithm has sublinear regret, thereby achieving both of robustness and efficiency.


%%Then, we extend it to replication-proof algorithm in the multi-agent setting by adopting the hierarchical structure of \cite{shin2022multi} while introducing a novel device of \emph{restarting} and largely exploiting the \emph{non-adaptive} and \emph{decoupled} structural nature of ETC algorithm.
%We cement our result by proving that our algorithm has sublinear regret, thereby achieving both of robustness and efficiency.


%
%We develop a replication-proof algorithm based on this single-agent analysis, which captures the both rabbits of efficiency and robustness.
%To this end, we begin with analyzing H-UCB presented by \cite{shin2022multi}.
%Surprisingly, however, we observe that it is no more replication-proof with Bayesian agents.
%This mainly stems from the fact that UCB itself is \emph{not replication-proof} even in the single-agent setting, and thereby H-UCB is \emph{not replication-proof} in the multi-agent setting.
%Thus, UCB is not the algorithm that answers the above question positively.
%To overcome the limitation of H-UCB, we first thoroughly investigate the single-agent setting, and characterize \emph{sufficient conditions} under which an algorithm becomes replication-proof.
%This analysis eventually spawns the question presented above, which might be of independent interest in \emph{comparing regrets of multiple bandit instances}.
%Notably, we prove that exploration-then-commit (henceforth ETC) satisfies these properties, thus replication-proof in the single-agent setting.
%Then, we extend it to replication-proof algorithm in the multi-agent setting by adopting the hierarchical structure of \cite{shin2022multi} while introducing a novel device of \emph{restarting} and largely exploiting the \emph{non-adaptive} and \emph{decoupled} structural nature of ETC algorithm.
%We cement our result by proving that our algorithm has sublinear regret, thereby achieving both of robustness and efficiency.
%
%
%
%
%
%We reveal that 
% and show that it fails to be replication-proof even in the single-agent setting.
%Subsequently, we characterize necessary and sufficient conditions for an algorithm to be replication in the single-agent setting, and prove that exploration-then-commit (ETC) satisfies this property, whereas UCB does not.
%Built upon it, we present a hierarchical algorithm with ETC, equipped with a restarting technique that re-initializes every parameters in the second phase (arm selection phase), and analyze its replication-proofness.
%We complement this result by providing its sublinear regret upper bound, thereby capturing the both rabbits of robustness and efficiency.
%
%
%As noted thus far, our main result starts with the failure of H-UCB.
%
%Indeed, we observe that the analysis of designing a replication-proof algorithm even under a very simple case (two Bernoulli arms, single agent) boils down to the following question.
%\begin{example}
%    Consider a Bernoulli bandit instance $\cI_A$ with two arms with mean rewards $0.1$ and $0.5$. Consider Bernoulli bandit instances $\cI_B$ and $\cI_C$ each equipped with three arms such that $B$'s arms have mean rewards $0.1, 0.1$ and $0.5$ and $\cI_C$'s arms have $0.1, 0.5$ and $0.5$. 
%    Given some standard bandit algorithms, would the expected regret under $\cI_A$ be larger than the average of expected regret under $\cI_B$ and $\cI_C$?
%\end{example}
%Even under simplistic and standard algorithms such as exploration-then-commit (ETC) or UCB, it is not straightforward to answer the above question.
%Obviously, instance $C$ will incur smaller regret, but the instance will have larger regret.\footnote{Note that this can be shown using a coupling-like argument between random reward tapes of the arms, combined with a regret decomposition lemma. See~\cite{shin2022multi} for more details.}
%Thus, the question is whether the loss from $B$ will be larger than the gain from $C$, compared to $A$ respectively.
%
%More formally, in its simplest form, a single-agent analysis case of our objective to construct replication-proof algorithm spawns to the fundamental question of comparing the expected regret of multiple bandit instances, presented as follows.
%\begin{center}
%	\emph{Given an arbitrary stochastic bandit problem, consider an adversary who uniformly randomly selects an arm and replicates. Which bandit algorithms guarantee that the regret does not increase against the adversary? What if it randomly replicates multiple arms possibly at different times?}
%\end{center}
%We affirmatively answer this question by proving that, there exists an algorithm that satisfies the above questions for \emph{any} bandit instance under some mild assumptions.
%We develop a replication-proof algorithm based on this single-agent analysis, which captures the both rabbits of efficiency and robustness.
%To this end, we begin with analyzing H-UCB presented by \cite{shin2022multi}.
%Surprisingly, however, we observe that it is no more replication-proof with Bayesian agents.
%This mainly stems from the fact that UCB itself is \emph{not replication-proof} even in the single-agent setting, and thereby H-UCB is \emph{not replication-proof} in the multi-agent setting.
%Thus, UCB is not the algorithm that answers the above question positively.
%To overcome the limitation of H-UCB, we first thoroughly investigate the single-agent setting, and characterize \emph{sufficient conditions} under which an algorithm becomes replication-proof.
%This analysis eventually spawns the question presented above, which might be of independent interest in \emph{comparing regrets of multiple bandit instances}.
%Notably, we prove that exploration-then-commit (henceforth ETC) satisfies these properties, thus replication-proof in the single-agent setting.
%Then, we extend it to replication-proof algorithm in the multi-agent setting by adopting the hierarchical structure of \cite{shin2022multi} while introducing a novel device of \emph{restarting} and largely exploiting the \emph{non-adaptive} and \emph{decoupled} structural nature of ETC algorithm.
%We cement our result by proving that our algorithm has sublinear regret, thereby achieving both of robustness and efficiency.


% In Section~\ref{sec:model}, we introduce our model and further preliminaries.
% We then provide negative result of UCB and H-UCB in Section~\ref{sec:fail}.
% Positive results for the single-agent setting is presented in Section~\ref{sec:single}.
% Finally in Section~\ref{sec:multi}, we present our main results of replication-proof algorithm along with its regret analysis.
% All the proofs are deferred to the appendix due to space constraints.

%In this context, we study a Bayesian extension of \cite{shin2022multi}, where each agent only knows such a distribution.

%it is inadequate to apply in various applications where --more realistically-- an agent's knowledge about the means of his arms is imperfect. Specifically, an agent in general does not know the mean of each arm but rather has a Bayesian prior over the mean of the arm, e.g. an arm may have mean $0.7$ with probability $\frac{1}{4}$ and $0.3$ with probability $\frac{3}{4}$. 
%
%
%This Bayesian modification of the setting holds for many real life applications. For example, consider an online video sharing platform such as YouTube. An agent can have a collection of videos which he may be able to upload more than once, however he may only posses uncertain knowledge (Bayesian prior) about the quality (mean reward) of a video before it is registered to the platform and viewed by the users. Similarly, one can consider an e-commerce website such a eBay or Airbnb \note{Seyed - the issue with both of these is that unlike a video the resource can be consumed, i.e. if someone rents a place you cannot replicate it, similarly if someone wants to buy an item you cannot replicate it as well}   
%
%While the modification to the model is simple it introduces non-trivial implications. Specifically, we show that \note{text needs to flow better with what is before and after}   

%
%\subsection{Our contributions and techniques}
%Our negative result on H-UCB of \cite{shin2022multi} mainly relies on the deterministic nature of UCB along with its adaptive exploration.
%This
%
%
%\note{Emphasize that our problem basically  boils down to the problem of comparing the expected regret of multiple bandit instances.}
%
%\note{Also emphasize that our results directly carry over to the dynamic setting in which at each round an agent arrives with some arms and try to register their contents, since we are essentially dealing with "incentive-compatible".}



\subsection{Related work}
There exists a growing literature at the intersection of multi-armed bandits and game theory. The work of \cite{braverman2019multi} considers a setting where the arms are agents. When an arm (agent) is pulled a reward is realized. The agent can take part of the reward and only report the remaining reward to the principal. The paper's major contribution is showing that there exists instances where the agents can engage in collusion and deliver only a sublinear amount of cumulative rewards to the principle. The work of \cite{feng2020intrinsic} is closely related to \cite{braverman2019multi} in that the agents are still arms that can modify their rewards. However, in \cite{feng2020intrinsic} an agent's utility equals the total number of pulls and are not related to the rewards. Further, the reward modifications are not real but rather fake and not adding to the principal's utility. Their main contribution is showing that under such a setting standard MAB algorithms like UCB and $\eps$-greedy can still achieve sublinear regret if the modifications are sublinear. 
\cite{esmaeili2023robust} introduce a further extension of~\cite{braverman2019multi} in which the agent can either take the rewards or increase the rewards at costly efforts.
\cite{ghosh2013learning} consider a setting where each arm (agent) gains higher utility with more pulls. The arm can increase its mean at some cost and they show that if the horizon is large enough, then a Nash equilibrium exists where all agents contribute the highest possible mean. 
\cite{hajiaghayi2023regret} study a bandit variant of the delegated choice problem by~\cite{kleinberg2018delegated} where a strategic agent decides which arm to commit while the principal can either accept or reject based on its reward afterward.
While the above works share some connections to our model in their perspective of \emph{bandit mechanism design against strategic agents}, the problem setups are very different from ours.

Initiated by \cite{kremer2014implementing} and \cite{che2018recommender}, there exists a line of works studying \emph{incentivized exploration} to design a mechanism that incentivizes myopic agents to explore the arms.
At each round, a myopic agent arrives and select an arm based on the signal sent by the bandit algorithm.
If the signaling scheme is not incentive-compatible, the agent will not follow the algorithm's recommendation, but rather exploits the empirically best arm.
Thus, the principal needs to design a mechanism to induce myopic agents to explore the arms.
To this end, the principal may exploit the information asymmetry arises from the principal's information design scheme~\citep{mansour2015bayesian, immorlica2018incentivizing, sellke2021price} or may compensate the myopic users~\citep{frazier2014incentivizing, han2015incentivizing, chen2018incentivizing}.
These works, however, focus on agents who are delegated to \emph{select} the arms based on the information available at hand, whereas our problem focuses on agents who are delegated to \emph{design} the bandit instance by selecting which arms to register in the system.
A long line of works \citep{banerjee1992simple, bala1998learning, smith2000pathological, lazer2007network, banihashem2023bandit} has been asking a similar question of \emph{learning dynamics} under a presence of myopic agents pulling the arms. Since these works mostly aim to characterize regimes under which the social learning succeeds or fail, \ie not in a mechanism design perspective, so we do not discuss more in details.


% There also exists a growing literature at the intersection of matching and multi-armed bandits where the agents preferences are learned through sequential interactions in centralized \citep{liu2020competing,jagadeesan2021learning} as well as decentralized settings \citep{liu2021bandit,basu2021beyond}. 
% \suho{we can add SODA paper, and some more papers, if we will discuss matching and bandit. But not quite sure whether this topic is worth discussing}
% \suho{explain a bit about bandit algorithm against infinite number of arms, refer to SHIN.}
% \suho{discuss incentivized exploration literature as well}

% While the above works share some connections to our work in their perspective of bandit mechanism design against strategic agents, the models are very different from ours. 
Most closely related to this paper is the work of \cite{shin2022multi}. 
In particular, similar to our work agents have a collection of arms which they can register to the platform and are capable of replicating an unbounded number of times. 
The main contribution is to construct an incentive-compatible mechanism, named hierarchical UCB (H-UCB), under which each agent does not replicate, but registers only the arm with the highest mean.
Their equilibrium analysis is relatively simple due to the fact that the agents are aware of the ex-post realization of their own arms' mean rewards, \ie \emph{fully informed}.
% The main contribution is showing that a hierarchical UCB algorithm (H-UCB) that leads to an incentive-compatible mechanism where each agent's dominant strategy is to only register the arm with the highest mean. 
Despite the close connection to our work, in our setting the agent's knowledge of the arms' means is not complete (deterministic) but rather imperfect and modelled by Bayesian priors. 
While the modification itself looks simple, its consequences are challenging. In fact, we show that H-UCB fails in this setting. 
Further, while our solution shares some features with \cite{shin2022multi} in that we still use a hierarchical structure, the details of our solution differ greatly and require new ideas and analysis.

Finally, a number of works~\citep{manyarmed:berry, manyarmed:carpentier, manyarmed:wang, manyarmed:zhu} study a bandit algorithm when there exists infinite number of arms in the system or the arms arrive over the time. 
While these works focus on designing a robust algorithm to adapt to infinite number of arms with some structural assumptions on the proportion of optimal arms or their arrival time, our work takes a perspective of algorithmic scheme to \emph{prevent} such many arms in advance.
We remark that preventing such an overload in advance is typically more desirable, \eg  saving computational resources.


==> model.tex <==
% !TEX root =  main.tex
\section{Model}\label{sec:model}
% We consider a mechanism design approach for the standard stochastic bandit problem in which the set of arms registered in the bandit instance are determined by the algorithm itself.
We consider a simultaneous game between a set of agents $[n] = \{1,2,\ldots, n\}$ and a principal.
Each agent $i \in \set{N}$ has a set of original arms $\set{O}_i = \{o_{i,1},\ldots, o_{i,l_i}\}$ given a constant $l_i \in \N$.
Each agent $i$ is equipped with a cumulative distribution $F_i$ from which each original arm $o_{i,k}$'s mean reward $\mu(o_{i,k})$ is sampled for $k \in [l_i]$.
Each arm $o_{i,k}$ further follows a reward distribution $G_{i,k}$ with the mean reward sampled as noted above.
We use $f_i$ and $g_{i,k}$ to denote the density function of $F_i$ and $G_{i,k}$,\footnote{We assume the existence of density function for ease of exposition, but all the results will easily be generalized.} and we assume that all the distributions are supported on $[0,1]$.
%Each arm $o_{i,k}$ has a 
%Let $f_i$ denotes the density function of $F_i$,\footnote{We assume that $f_i$ exists for ease of exposition, but all the results will easily be generalized.} and we assume it has bounded support on $[0,1]$.
We further assume that $F_i$ is independent from $F_j$ for $i \neq j \in [n]$.
For instance, $F_i$ might be a uniform distribution over $[0,1]$, and each arm $a \in \cO_i$ has a Bernoulli reward distribution with the mean sampled from $F_i$.
%Precisely, arm $a \in \set{O}_i$ is parameterized by its mean reward $\mu(a)$, which is sampled from the cumulative distribution $F_i$ with density function $f_i$ supported on $[0,1]$.
%We assume $F_i$ is independent between the agents $i \in [n]$.
%For instance, $\cF_i$ can be a family of Bernoulli distributions with mean rewards sampled from $[0,1]$, or even simply can be a family of distributions having a singleton support on the mean reward.
%We assume that this sampling of mean reward is independent across the agents.
%This assumption is innocuous because a creation of contents (arms) is usually independent of what other content providers are creating simultaneously.
We often deal with a \emph{single agent} setting with $n=1$.

\paragraph{Bayesian agents}
Importantly, we consider a \emph{Bayesian scenario} in which each agent is only aware of its own distribution $F_i$, but not the exact realization of $\mu_a$ for $a \in \set{O}_i$.
We note that such assumption is indeed practical since content providers (agents) in contents platform typically only have a partial information on how much their contents may attract the users, \eg based on his/her previous contents and outcomes therein.
This is in stark contrast to the setting of~\cite{shin2022multi} in which they assume \emph{fully-informed} agents such that any strategic agent does not have any incentive to register the arms except the best one reducing the problem into the single-arm case, which is not practical in many real-world scenarios.
We highlight that the equilibrium analysis in the fully-informed setting simply boils down to the case under which each agent only has a single original arm and decides how much to replicate that unique arm, whereas our extension significantly complicates the analysis of equilibrium, as will be elaborated shortly.
%Compared to their model, our setting of Bayesian agents brings a substantial amount of technical challenges in both designing and analyzing equilibrium of algorithms, where we elaborate more in subsequent sections.

%\paragraph{Agent's strategy}
\paragraph{Agent's strategy and mechainsm procedure}
Given the prior distribution $F_i$, the set of original $O_{i,k}$ and the principal's algorithm $\fA$, each agent $i$ decides how many times to replicate arm $k$, including $0$ of no replication, for each $k \in [l_i]$.
Precisely, agent $i$ commits to a set $\set{S}_i = \{s_{i,k}^{(c)}:c \in [c_{i,k}], k \in [l_i]\}$ in a strategic manner, where $c_{i,k}$ denotes the total number of replica for arm $o_{i,k}$.
The replicated arm $s_{i,k}^{(c)}$ has the same mean reward to the original arm, \ie $\mu(s_{i,k}^{(c)}) = \mu(o_{i,k})$ for any $i \in [n]$ and $k \in [l_i]$.
We often use $s_{i,k}^{(0)}$ to denote $o_{i,k}$ for simplicity.
Define $\cS = (\cS_1, \ldots, \cS_n)$ and $\cO = (\cO_1, \ldots, \cO_n)$.
Given all the agents' strategies $\set{S}$, the bandit algorithm $\fA$ runs and corresponding rewards are realized.
%Importantly, we assume that a constant portion $\alpha \in (0,1)$, which is exogenous to the mechanism, of the rewards are transferred from to each agent whenever the agent's arm is selected.

The overall mechanism proceeds as follows: (i) The principal commits to a bandit algorithm (mechanism), (ii) Each agent $i \in \set{N}$  decides an action $\set{S}_i$ to register given $\mathfrak{A}$ to maximize own payoff, (iii) The mean rewards $\mu_a$ for each $a \in \set{O}$ are sampled, (iv) The bandit algorithm $\mathfrak{A}$ runs and rewards are realized, (v) The principal and the agent realize their own utility.\footnote{Note that if all the agents do not strategize and simply register $\set{O}_i$ in step (ii), our problem reduces to the standard stochastic multi-armed bandit problem, where standard bandit algorithms would work well.}
% \begin{enumerate}[(i)]
% \item The principal commits to a bandit algorithm $\mathfrak{A}$.
% \item Each agent $i \in \set{N}$  decides an action $\set{S}_i$ to register given $\mathfrak{A}$ to maximize own payoff.
% \item The mean rewards $\mu_a$ for each $a \in \set{O}$ are sampled.
% \item The bandit algorithm $\mathfrak{A}$ runs and rewards are realized.
% \item The principal and the agent realize their own utility.
% \end{enumerate} 


\paragraph{Agent's payoff}
%The most remarkable difference from the perfect information model is that the exact mean reward in $\set{S}_i$ is determined after the selection of the strategy.
%Therefore, each agent should basically select the strategy set in ex-ante manner so that its expected payoff becomes larger in regards of the randomness in realization of $\mu_a$ for $a \in \set{O}_i$.
%Alternatively, this procedure can be interpreted as (i) sampling $\mu_a$ for $a \in \set{O}_i$ from $D_i$ and then (ii) randomly permuting the realized mean reward over the set of arms $o_{i,1},\ldots, o_{i,l(i)}$.
%This interpretation will particularly be useful in defining the expected payoff of each agent.
%\note{Suho - TBD - No need to interpret like this here. Just present the expectation, and later provide some intuitions when we define replication proof or results.}
Once an arm is selected by $\fA$, a fixed portion $\alpha \in (0,1)$ of the reward is paid to the agent who registers the arm.
We write $\muvec_i$ to denote $(\mu_{i,1}, \mu_{i,2}, \ldots, \mu_{i,l_i})$, \ie the vector of agent $i$'s (realized) mean rewards of the arms.
Let $E_{i}(\muvec_i)$ be an event that the mean reward of agent $i$'s arms are realized to be $\muvec_{i}$.
Recall that $E_i(\cdot)$ are mutually independent for for $i \in [n]$.
We often abuse $E_{i}$ to denote $E_i(\muvec_i)$ if the realization $\muvec_i$ is clear from the context.
% and write $E_{-i}(\muvec_{-i})$ to denote the realization of the other agents' mean rewards of the arms, \ie an event that for $\cN \ni j \neq i$, agent $j$'s arms' mean rewards are sampled to be $\muvec_j$.
We also write $\cS_{-i}$ to denote $(\cS_1, \ldots, \cS_{i-1}, \cS_{i+1}, \ldots, \cS_n)$, and $E(\muvec)$ for $\muvec = (\muvec_1,\muvec_2, \ldots, \muvec_n)$ to denote the event such that $\cap_{i \in [n]}E_i(\muvec_i)$.

We further introduce some notations given the principal's algorithm $\fA$.
Conditioned on the $E_{i}(\muvec_i)$, agent $i$'s \emph{ex-post payoff} of selecting strategy $\set{S}_i$ given the others' strategies is defined as
\begin{align*}
U_i(\set{S}_i, \set{S}_{-i} ;E(\muvec)) = \alpha \sum_{t=1}^T R_t\Ind{I^{(t)} \in \set{S}_i},
\end{align*}
where  $R_t$ refers to the reward at round $t$ and $I_t$ denotes the arm selected at round $t$.

Given the ex-post utility, each agent computes its \emph{ex-ante payoff} by marginalizing over the realization of its own arms' mean rewards, defined as follows
\begin{align*}
	u_i(\set{S}_i, \set{S}_{-i}) = \Ex{U_i(\set{S}_i, \set{S}_{-i};E(\muvec))},
\end{align*}
where the randomness in the expectation comes from $E(\muvec)$, i.e. the realization of the mean rewards, and possibly from the random bits of the algorithm $\fA$.
In words, each agent is rational \emph{expected utility maximizer} who maximizes its expected payoff.
%We denote $U_i(\set{S}_i, \set{S}_{-i};E_{i})$ by \emph{ex-post} utility, and $u_i(\set{S}_i, \set{S}_{-i})$ by \emph{ex-ante} utility.
% We often overwrite $u_i(\set{S}_i, \set{S}_{-i})$ by $u_i(\set{S}_i)$ when $\set{S}_{-i}$ is clear from the context.

\paragraph{Information and desiderata}
We now describe the information structure of the mechanism, and how each agent decides its own strategy based on its ex-ante payoff.
We first assume that the principal does not have any information regarding the agents' distributions, nor the number of original arms.
This is often called \emph{prior-independent mechanism} in the mechanism design, \cf \cite{hartline2013bayesian}.
In addition, we assume that the agent does not have any information regarding the others.
Instead, our objective is to construct a \emph{incentive-compatible} mechanism such that each agent's \emph{dominant strategy} is to register the arms without any replication, without regard to what others may have proposed.
To this end, we first define a dominant strategy as follows.
\begin{definition}[Dominant Strategy]
Agent $i$'s strategy $\set{S}_i$ is dominant strategy if $u_i(\cS_i \cup \set{S}_{-i}) \ge  u_i(\set{S}'_i \cup \cS_{-i})$ for any $\set{S}'_i$ and $\set{S}_{-i}$.
\end{definition}
Correspondingly, we introduce the following notion of \emph{dominant strategy equilibrium}.
\begin{definition}[Equilibrium]
An algorithm $\mathfrak{A}$ has dominant strategy equilibrium	(DSE) if there exists a set of agent strategies $\set{S} = \{\set{S}_i\}_{i \in [n]}$ such that $\set{S}_i$ is dominant strategy for any agent $i \in [n]$.
\end{definition}
As per the definition, the total ordering of the agent's payoff with respect to its own strategy should remain the same regardless of the others' strategies $\cS_{-i}$.
Thus, we often omit the parameter $\cS_{-i}$ in denoting agent $i$'s payoff, \eg $u_i(\cS_i)$ instead of $u_i(\cS_i, \cS_{-i})$.
Note, however, that the realization of the other agents' mean rewards may affect the actual quantity of $u_i(\cS_i)$, although it does not affect which strategy agent $i$ will eventually commit to.
Since we are interested only in how the agents will "behave", the absolute amount of the payoff is beyond our interest, and thus it does not lose any generality.

We finally introduce incentive compatibility of an algorithm as follows.
\begin{definition}[Replication-proof]
An algorithm $\mathfrak{A}$ is \emph{replication-proof} if it has a dominant strategy equilibrium $\{\set{O}_i\}_{i \in [n]}$ for any $T \in \N$.
\end{definition}
Replication-proofness is desirable as the agents are not motivated to replicate their own arms, thereby reducing the number of arms that a bandit algorithm faces.
Since the regret upper bound of a standard bandit algorithm usually depends on the number of arms, maintaining a smaller number of suboptimal arms in the system affects the eventual learning efficiency of the algorithm.
% it narrows down a set of identical arms into a single arm, therefore reduces the exploration burden in which the algorithm should have faced to identify that they indeed are equal arms.
We often say that the algorithm is \emph{incentive-compatible} or \emph{truthful} to denote the replication-proofness, as in the literature, \cf \cite{nisan2007algorithmic}.

%In short, our objective is to construct a \emph{prior-independent} \emph{incentive-compatible} mechanism.



%Importantly, we do not impose any assumption on the information structure of an agent regarding others, \ie each agent does not know about the realization of the others' mean rewards nor their prior distributions.
%This allows some agents to be aware of other agents' prior distributions so that they may strategize over such a knowledge, while also admitting other agents to be fully oblivious to others' information.
%
%Instead, the principal's objective here is to construct an \emph{dominant-strategy incentive-compatible mechanism} under which each agent has no incentive to deviate from its truthful strategy, with "no" regards to what others do.
%\begin{definition}[Dominant Strategy]
%Agent $i$'s strategy $\set{S}_i$ is dominant strategy if $u_i(\cS_i \cup \set{S}_{-i}) \ge  u_i(\set{S}'_i \cup \cS_{-i})$ for any $\set{S}'_i$ and $\set{S}_{-i}$.
%\end{definition}
%
%Correspondingly, we introduce the following notion of \emph{dominant strategy equilibrium}.
%\begin{definition}[Equilibrium]
%An algorithm $\mathfrak{A}$ has dominant strategy equilibrium	(DSE) if there exists a set of agent strategies $\set{S} = \{\set{S}_i\}_{i \in [n]}$ such that $\set{S}_i$ is dominant strategy for any agent $i \in [n]$.
%\end{definition}
%
%We emphasize that such a mechanism with dominant strategy equilibrium indeed allows each agent to have arbitrary information regarding other agents in deciding its own strategy, since the inequality above holds for any choice of $\cS_{-i}$.
%Hence, with focus on obtaining dominant strategy, we can simply write $u_i(\cS_i)$ to denote $u_i(\cS_i, \cS_{-i})$.
%Note, however, that the realization of the other agents' mean rewards may affect the actual quantity of $u_i(\cS_i)$, although it does not affect what agent $i$ will eventually "choose" as a strategy.
%Since we are interested only in how the agents will "behave", the absolute amount of the payoff is beyond our interest, and thus it does not lose any generality.
%
%Finally, we assume that the principal has no information on the agents' prior distributions.
%This is often called \emph{prior-independent mechanism} in the mechanism design (\cite{hartline2013bayesian}).

%For example, given two agents $a$ and $b$, suppose that agent $a$ has an incomplete information and thus knows the prior distribution of agent $b$ and its number of arms, and agent $b$ has no information regarding $a$ at all.
%In this case, agent $a$ may decide its own strategy based on marginalizing all the possible outcomes of $\muvec$, while assuming that agent $b$ will play
%On the contrary, agent $b$ may play maxmin strategy,


%Then, we can define agent $i$'s \emph{expected payoff} of choosing action $\set{S}$ to be
%\begin{align*}
%u_i(\set{S}_i, \set{S}_{-i}) = \Exu{\mu_{\set{O}_i}}{\Ex{v_i(\set{S}_i, \set{S}_{-i};\mu_{\set{O}_i})} | \mu_{\set{O}_i}},	
%\end{align*}
%
%This is mainly because each agent does not know the realization of the rewards $\mu_a$ for own arm $a \in \set{O}_i$, the strategy itself may include a randomness arisen from choosing which arms to replicate or register.
%For example, suppose that agent $i$ decides to register only a single arm among $\set{O}_i = \{o_{i,1},o_{i,2}\}$ where $\mu_{o_{i,1}} > \mu_{o_{i,2}}$.
%Since he does not know the exact realization of the mean rewards $\mu_{o_{i,1}}$ and $\mu_{o_{i,2}}$, the only possible action would be to choose any single arm and register it, which yields the probability $50\%$ of registering high-reward arm and another $50\%$ of registering low-reward arm.
%Alternatively, this procedure can be interpreted as (i) given the prior distribution $D_i$, agent $i$ selects own action


%Importantly, we consider a \emph{Bayesian information} of agents in which each agent $i$ only has a partial information on its own arms $\set{O}_i$.
%More precisely, each agent $i$ only knows a distribution $D_i$ with support on $[0,1]$ from which the expected reward of arm $a$ is drawn independently and identically for the original arms $a \in \set{O}_i$.




%\paragraph{Learning efficiency}
On top of designing \emph{prior-independent} \emph{incentive-compatible} mechanism, we are also interested in a learning efficiency, \ie learning the reward distribution in a sample-efficient manner.
In the online learning and bandit literature, this is usually described as a notion of cumulative regret, defined as follows.
\begin{definition}[Regret]
	Given time horizon $T$, strategy $\set{S}$ and the event $E(\muvec)$, the ex-post regret of algorithm $\mathfrak{A}$ is 
	\[\reg(\mathfrak{A}, T ; \set{S}, E(\muvec)) = \parans{\max_{a \in \cup_{i \in \cN} \cO_i}\sum_{t=1}^T \mu(a)} -\sum_{t=1}^T \mu(I_t),\]
	where $I_t$ denotes the arm selected by $\mathfrak{A}$ at round $t$.
\end{definition}
\sscomment{Clarify ex-post, but its expected regret, and define it w.r.t. expectation, and expand as above}
We emphasize that the optimal benchmark is selected from $\cup_{i \in \set{N}}\set{O}_i$, not from the registered set of arms $\cup_{i \in \set{S}}\set{S}_i$.
This benchmark is indeed important since the principal should incentivize the agents to decide an action that contains own best arm to maintain larger utility.
For example, if an algorithm motivates an agent to not register all the arms, then there might be a constant probability that the omitted arm has the largest mean reward, which essentially yields sublinear regret with respect to the regret defined above.
More formally, our notion of regret implicitly implies that any sublinear regret algorithm incentivizes all the agents to register all their original arms at least once.
%Note that this definition of regret is based on the ex-post realization of the arms' parameters.
%We can also define a version of Bayesian regret by marginalizing over the realization of the arms' parameters, but we will focus on obtaining a good performance based on our definition presented above.
%Note that any analysis of the regret upper bound based on our definition easily carries over to the Bayesian regret by simply marginalizing over the priors.
We also remark that although the arms' mean rewards are sampled from prior distributions, which is often referred to Bayesian bandits (\eg see Ch.3 of \cite{slivkins2019introduction}), we deal with ex-post regret, \eg as does in \cite{agrawal2012analysis} which analyzes the ex-post regret of Thompson Sampling in Bayesian bandits.
Obviously, ex-post regret upper bound \emph{implies} the Bayesian regret upper bound by simply taking an expectation over the prior distributions.
%We also emphasize that the optimal benchmark $a^\star$ is selected from $\cup_{i \in \set{N}}\set{O}_i$, not from the registered set of arms $\cup_{i \in \set{S}}\set{S}_i$.
%This benchmark is indeed important since the principal should incentivize the agents to decide an action that contains own best arm to maintain larger utility.



%\paragraph{Negative result for standard algorithms}
%Note, however, that it is not obvious how much the algorithm could be worsen even if it does not satisfy replication-proofness.
%This is because even though an algorithm is not replication-proof, if it only allows a small number of replication, then the standard algorithm would still enjoy sublinear regret assuming that the agents only replicate sublinear number of times.
%In \cite{shin2022multi}, the authors define the following notion of replication-proneness to show that the standard algorithms indeed incurs a bad outcome.
%\begin{definition}[Replication-prone]
%An algorithm $\mathfrak{A}$ is replication-prone (RP) if for any strategy $\set{S}_i$ of agent $i$, there exists a strategy $\set{S}'_i$ such that $\set{S}_i \subset \set{S}'_i$ and $u_i(\set{S}_i \cup \set{S}_{-i}) < u_i(\set{S}'_i \cup \set{S}_{-i})$ for any $\set{S}_{-i}$.
%\end{definition}
%They formally prove that the standard algorithm such as UCB suffers replication-proneness based on a coupling technique.
%This essentially implies that the number of arms registered in the system can be arbitrarily large if the agents behavior in a strategic manner.
%Since our model accommodates the setup of \cite{shin2022multi} as a special case with prior distributions having singleton support, since their model is essentially reduced to each agent having a single arm, this negative result carries over to our model as well.
%\begin{proposition}
%	UCB suffers replication-proneness.
%\end{proposition}
%
%This would be the worst possible property that any algorithm may have, since any rational agent under such algorithm would infinitely replicate its own arms to maximize the expected payoff, and thus the it cannot guarantee the sublinear regret anymore since UCB has regret of $O(\sqrt{KT\log T})$ in the worst case where $K\to \infty$ denotes the number of arms registered in the system.
%
%\paragraph{Precluding partial replication}
%Finally, we note that it is always bad strategy for agent $i$ to register only a proper subset of $\cO$.
%Suppose that agent $i$ plays $\cS_i \subset \cO_i$ and $\cS_i \neq \cO_i$.
%Then, there exists an arm $a \in \cO_i$ which is not contained in $\cS_i$.
%Due to the nature of sampling process of arms' mean rewards, with constant probability of at least $1/|\cO_i|$, arm $a$ has the largest (or equal) mean reward.
%In this realization, excluding $a$ always induce linear regret of $\Theta(t)$ in terms of agent $i$'s utility until agent $i$ is selected $t$ rounds, and thus incurs constant probability times $\Theta(t)$ regret in expectation.
%Therefore, we only consider a strategy $\cO_i \subset \cS_i$ without loss of generality.
%This can be formalized as follows, where the proof is deferred to Appendix~\ref{app:subset}.
%\begin{proposition}\label{prop:subset}
%	For any algorithm that achieves sublinear-regret in any problem instance, for any $T$ and agent $i \in [n]$, playing $\cS_i \subset \cO_i$ such that $\cS_i \neq \cO_i$ is not dominant strategy, unless agent $i$'s distribution only has a strictly positive measure on a singleton support.
%\end{proposition}

%
%\subsection{Preliminary}
%We now discuss 
%
%\note{Suho - TBD - discuss previous algorithms/analysis, and discuss why bayesian setting makes it challenging}
%
%\note{It might be good to motivate both the single/multi agent setting.}
%
%\note{Also, briefly argue that if the agent excludes some arms, then it is always bad strategy, so without loss of generality, we only consider a strategy that replicates some arms from $\cO$.}


==> multi-agent.tex <==
\section{Towards Replication-proof Algorithm}\label{sec:multi}

%
%In the proof of Theorem~\ref{thm:hucb_negative} for the multiple agent case, we essentially observe that agent $i$ will play a strategy that maintains the random variable $R(i)$ as large as possible at every round in order to maximize the change of being selected.
%In this context, for an algorithm to be intuitively replication-proof given the hierarchical structure, we need to construct an algorithm such that truthful registration yields the random variable $R(i)$ largest possible for each agent $i$, regardless of the others' strategies.
%
%=========================
%
Now we turn our attention to the more general setting with multiple agents.
Basically, we start by reusing the machinery of \emph{hierarchical structure} by \cite{shin2022multi} 

%This effectively separates Phase 2 from each agent and motivates the agents to increase their chance of being selected in Phase 1, which will in turn imply the replication-proofness equipped with some good choices of $\alg_1$ and $\alg_2$.

% \vspace{-1mm}
\begin{algorithm} 
\SetAlgoLined
%$i \in \set{N}$, $\set{S} = \cup_{i \in \set{N}} \set{S}_i$\\
\textbf{Input}: Tie-breaking rule, agent set $\cN$, arm set $\cS_i$ for $i \in \cN$, restarting round $\tau \in [T]$\\
Let $\muhat_i \gets 0$, $n_i\gets 0$, $\muhat_{i,a} \gets 0$, $n_{i,a} \gets 0$ for $i \in \cN$ and $a \in \cS_i$\\


 \For{$t=1,2,\ldots,M$}{
  \If{$t = \tau+1$}
  {
  $\muhat_{i,a} \gets 0; ~ n_{i,a} \gets 0$ for $\forall a \in \cS_i$, $\forall i \in \cN$
  }
  \If{$n_i < M$ for some $i \in \cN$}
  {
  	$\hat{i} \gets i$
  }
  \Else{$\hat{i} \gets \argmax_{i \in \cN}\muhat_{i}$}
  
  \If{$n_{\hat{i},a} < m$ for some $a \in \cS_{\hat{i}}$}
  {
  	$\hat{a} \gets a$
  }
  \Else{$\hat{a} \gets \argmax_{a \in \cS_{\hat{i}}}\muhat_{\hat{i},a}$}  
%  If $N(i) \le 1/2T^{1/3} \log(T)^{1/3}$, round-robin exploration of arms in $\set{S}_i$;\\
%  Else, commit $\hat{a} = \argmax_{a \in \set{S}_{\hat{i}}} 
%    \left\{r(a) \right\}$
  Pull $\hat{a}$ of agent $\hat{i}$ and obtain reward $R_t$\\
  Update statistics:
  $\muhat_{\hat{i},\hat{a}} \leftarrow \tfrac{\muhat_{\hat{i},\hat{a}}n_{\hat{i}, \hat{a}} + R_t}{n_{\hat{i}, \hat{a}}+1}; ~
  \muhat_{\hat{i}} \leftarrow \tfrac{\muhat_{\hat{i}}n_{\hat{i}} + R_t}{n_{\hat{i}}+1};~ n_{\hat{i}, \hat{a}} \leftarrow n_{\hat{i}, \hat{a}} + 1; ~~ n_{\hat{i}} \leftarrow n_{\hat{i}} + 1;$
 }
 \caption{Hierarchical ETC with Restarting ($\hbb$)\label{alg:hbb}}
\end{algorithm}
% \vspace{-1mm}

A direct implication of Theorem~\ref{thm:single_pf_rp} is that if we run a variant of H-UCB such that the first phase runs a simple uniform-random selection algorithm, and the second phase runs some arbitrary TRP and PI algorithms, then the resulting algorithm is replication-proof.
To formally see this why, let $\set{S}_i$ be the strategy of agent $i$.
Define $\Gamma_i(\set{S}_i)$ be the agent $i$'s utility under the single-agent setting with agent $i$, \ie when there are no other agents other than $i$.
Due to the uniformly random selection nature in the first phase, the expected utility of any agent $i$ can be simply written $u_i(\cS_i, \cS_{-i}) = {\Gamma_i(\set{S}_i)}/{n}$.
Note that the dynamic of the algorithm purely reduces to the dynamic of the second phase algorithm if there's only a single agent.
Hence, by Theorem~\ref{thm:single_pf_rp} and due to the TRP and PI of the second phase algorithm, we conclude that truthful registration is a dominant strategy for any agent $i$, and thus the result follows.
%\begin{theorem}\label{thm:multi_rp_uniform}
%	The algorithm constructed as above is replication-proof
%\end{theorem}
%\begin{proof}
%	Let $\set{S}_i$ be the strategy of agent $i$.
%	Define $\Gamma_i(\set{S}_i)$ be the agent $i$'s utility under the single-agent setting with agent $i$, \ie when there are no other agents other than $i$.
%	Due to the uniformly random selection nature of $\alg_1$, the expected utility of any agent $i$ can be simply written $u_i(\cS_i, \cS_{-i}) = \nicefrac{\Gamma_i(\set{S}_i)}{n}$.
%	Note that the dynamic of $\hbb$ reduces to the dynamic of $\alg_2$ if there's only a single agent.
%	Hence, by Theorem~\ref{thm:single_pf_rp} and due to the TRP and PI of $\alg_2$, we conclude that truthful registration is a dominant strategy for any agent $i$, and it completes the proof.
%\end{proof}
%Note, however, that
%The main takeaway of Theorem~\ref{thm:multi_rp_uniform} is that the use of hierarchical structure effectively decouples the agent-wise exploration.
Note, however, that if we deploy uniform random selection algorithm in $\alg_1$, it essentially suffers \emph{linear regret} since it always choose any suboptimal agent with constant probability at every rounds.



To capture the both rabbits of sublinear regret and replication-proofness, we need more carefully tailored algorithm with sublinear regret in the first phase.
To this end, we present $\hbb$ presented in Algorithm~\ref{alg:hbb}, which adopts ETC in both phases along with additional device of \emph{restarting round}.
Similar to H-UCB, this consists of two phases each running ETC agent-wise and arm-wise manner, respectively.
To analyze the replication-proofness, we pose a minor assumption on the arms.
We say that the set of arms belong to \emph{stochastically ordered family} if two arms $a$ and $b$ satisfy $\mu_a \ge \mu_b$, then the reward distribution of arm $a$ is (first-order) stochastic dominant over that of $b$, \ie $\Pr{r_a \ge x} \ge \Pr{r_b \ge x}$ for any $x\ge 0$, where $r_i$ denotes arm $i$'s reward random variable.\footnote{Note that Bernoulli arms and Gaussian arms parameterized by mean rewards, belongs to this family. We also refer to~\cite{yu2009stochastic} for more examples in exponential family.}
Further, define $L = \max_{i \in [n]}l_i$.
Then, our main result can be presented as follows.
\begin{theorem}\label{thm:spf_rp}
	Consider a stochastically ordered family of arms, and discrete support of prior distributions.
	Consider $\hbb$ with $M \ge mL$ and $m = \frac{2}{\Delta^2} L\ln (2T)$, and $\tau = Mn$
	Then, $\hbb$ is replication-proof under any number of agents.\footnote{Similar to what we discussed in Theorem~\ref{thm:single-refine1}, we can refine this results and make the algorithm truly prior-independent, at the cost of some other assumptions. We omit these details as it goes beyond our main interest/takeaway.}
\end{theorem}
We provide a brief proof sketch.
\sscomment{revise sketches}
The proof mainly relies on the single-agent result in Theorem~\ref{thm:single_pf_rp} along with a number of algebraic manipulations which heavily relies on the nature of ETC and the restarting round.
Let us focus on agent $i$.
We can decompose agent $i$'s total expected utility to be (i) exploitation phase utility and (ii) exploration phase utility.
In terms of the infinite reward tapes, remark that the utility from (i) and (ii) is independent due to the nature of ETC.
Since (i) simply reduces to running single-agent ETC for each agent, we can compare (i) of two strategies using the single-agent result, thus truthful strategy is at least better for (i).

For (ii), if agent $i$ is not selected in the exploitation phase, it is simply zero, so we can only focus on the case when agent $i$ is selected in the exploitation phase.
Thus, its expected utility from (ii) can be written as multiplication of (a) probability that agent $i$ has the largest empirical average reward and (b) the expected utility by being pulled over the exploitation rounds.
For (b), since our choice of $\tau$ \emph{restarts} Phase 2 for any agent exactly at the beginning of exploitation phase of Phase 1, the expected utility therein simply reduces to the expected utility of single-agent setting with agent $i$ given the time horizon $T-Mn$.
Thus, again by our single-agent result of Theorem~\ref{thm:single_pf_rp}, the truthful strategy yields larger (or equal) quantity for (b) as well.
Finally, by carefully using a series of concentration inequalities, we bound the difference from (a) between the truthful strategy and any other strategy is relatively smaller and by doing so, loss from (a) cannot make up the gains from (b) and (i), which eventually implies the dominance of truthful strategy.

% To accommodate the case under which the algorithm does not know $l_i$ for $i \in [n]$, one can effectively replace each $l_i$ with some superconstant function on $T$, \eg $\log T$, and run the same algorithm.
% This will eventually incur the same regret bound (up to polylogarithmic factor) assuming that $l(i) = O(1)$ for $i \in [n]$.
% The detailed analysis of this technique have been presented in \cite{shin2022multi}.


We finalize our results by presenting regret upper bound of the $\hbb$ with ETC and ETC,  which concludes that it achieves sublinear regret as well as replication-proofness.
\begin{theorem}\label{thm:regret}
	Set $\alg_1$ be ETC with $M = \max(mL, \sqrt{T\ln T})$, and $\alg_2$ be ETC with $m =\nicefrac{2}{\Delta^2}\cdot L\ln(2T)$.
	Then, $\hbb$ has expected regret of $O(\frac{nL^3\sqrt{T \ln T}}{\Delta^3})$.
\end{theorem}
The regret analysis is based on a construction of clean event on each agent under which the agent's empirical average reward becomes close enough to his own optimal arm's mean reward.
The deviation probability of this clean event can be obtained using tail bounds along with the regret analysis of ETC, which essentially implies the necessity of having $\alg_1$'s exploration length polynomial.
The regret bound then easily follows from obtaining the probability that all the clean event holds.
The full proof for the regret analysis is deferred to Appendix~\ref{apd:thm:regret}.

\sscomment{discussion 1: obtaining instance-independent regret bound}

\sscomment{discussion 2: comparing the regret bound to Shin et al.}

Finally, we remark that the algorithm's dependency on the problem parameters can be weakened analogous to Theorem~\ref{thm:single-refine1}, but we omit the details as it goes beyond our interest.

\subsection{Proof of Theorem~\ref{thm:spf_rp}}
\begin{proof}
	\sscomment{proofread again, and structurize}
	First, note that our $\hbb$ is well-defined since our choice of $M$ and $m$ ensures that the exploitation phase of the first phase starts after the exploitation of the second phase ends.
	For simplicity, denote the first phase ETC by $\alg_1$ and the second phase ETC by $\alg_2$.
	Pick an agent $i$ with arms $\{o_{i,1}, \ldots, o_{i,l}\}$, let $\cS_i$ be agent $i$'s arbitrary strategy which replicates arm $o_{i,j}$ of $r_{i,j} \in \N_0$ times for each $j \in [l_i]$.
	Let $r_i = (r_{i,1},\ldots, r_{i,l_i})$, and denote by $v_i = (v_{i,1}, \ldots, v_{i,l_i})$ the realization of agent $i$'s original arms' mean rewards.
	Fix strategies of all the other agents $j \neq i$ by $\cS_{-i}$, and fix a realization $v_{-i}$ of all the other agents' arms' mean rewards.
	Henceforth, we will omit $\cS_{-i}$ and $v_{-i}$ from the arguments in the notations presented hereafter, unless confusion arises.
	In addition, we assume that all the prior distributions do not have point mass for simplicity, but it can easily be generalized as discussed in the proof of Theorem~\ref{thm:single_pf_rp}.
	
	Let $i^*$ denote the agent selected at the exploitation phase of $\alg_1$, and $l_i$ to denote agent $i$'s number of arms.
	We further write $\muhat_i(M)$ to denote the empirical average reward of agent $i$ when agent $i$ is selected $M$ times,
	and $\muhat_{i,a}(m)$ to denote the empirical average reward of agent $i$'s arm $a$ when it's selected $m$ times.
	Then, given $v_i$ and $r_i$, recall that the bandit instance agent $i$ submits can be presented as $\bigtimes_{i \in [l]}(v_a: r_a)$.
	
	Now, similar to the proof of Theorem~\ref{thm:single_pf_rp}, we first write agent $i$'s expected utility as follows.
	\begin{align}
		u_i(\cS_i)
		=
		\int_{\mu_{i,1} = v_{i,1}} \int_{\mu_{i,2} = v_{i,2} < v_{i,1}}\ldots \int_{\mu_{i,l_i} = v_{i,l_i}< v_{i,l_i-1}} 
		\sum_{\sigma \in \cP_{l_i}}\Ex{U_i(\cS_i)\ |\ \bigtimes_{a \in [l_i]}(v_{i,\sigma(a)}: r_{i,a})}g(v_i)dv_i.\label{eq:04262152}
	\end{align}
%	Now, we fix a realization of agent $i$'s arms' parameters to be $v = (v_1,v_2,\ldots, v_l)$, and focus on the integrand.
%	Since we fix the realization of the parameters, we simply write $\sigma(v)$ to denote the event $\{\mu_1 = \sigma(v)_1,\ldots, \mu_l = \sigma(v)_l\}$, \ie
%	\begin{align*}
%		\Ex{U_i(\cS)\ |\ \sigma(v)_1,\ldots, \sigma(v)_l}
%		=
%		\CEx{U(\cS)}{\sigma(v)},
%	\end{align*}
%	unless confusion arises.
	
	We first characterize the expected utility of agent $i$ based on its utility under the single agent setting with agent $i$.
	To this end, we introduce several notations.
	Write $\Gamma_i^{\cS_i}(t, \sigma(v_i))$ to denote agent $i$'s utility when he is selected $t$ times under the single agent setting in $\alg_2$ when its arms' mean rewards are realized to be $\sigma(v_i)$, and he plays strategy $\cS_i$ with replication vector $r_i$.
	Given $M$, $m$, and $\cS_i$, define an event
	\[
	C^{\cS_i}_i(y,\sigma(v)) = \{\max_{\cN \ni j\neq i}\parans{\muhat_j(M) }= y \ | \ \bigtimes_{a \in [l_i]}(v_{i, \sigma(a)}:r_{i,a})\},
	\]
	\ie the event that agents other than $i$ have maximal agent-wise empirical average reward $y$ at the end of the exploration phase in $\alg_1$.
	Again given $M$, $m$, and $\cS_i$, we further define following two quantities:
	\begin{align*}
		p^{\cS_i}_i(y, \sigma(v_i)) &= \CPr{C_i(y)}{\bigtimes_{a \in [l_i]}(v_{i, \sigma(a)}:r_{i,a})}
		\\
		q^{\cS_i}_i(y,\sigma(v_i)) &= \CPr{\muhat_i(M) \ge y}{\bigtimes_{a \in [l_i]}(v_{i, \sigma(a)}:r_{i,a})}.
	\end{align*}
	Remark that all the quantities above are conditioned on the event that $v_{-i}$ is realized and the other agents are playing $\cS_{-i}$.

	The following claim essentially characterizes the expected utility of agent $i$ under strategy $\cS$.
	\begin{claim}
		Agent $i$'s expected utility can be written as follows.
		\begin{align}
			\CEx{U_i(\cS_i)}{\bigtimes_{a \in [l_i]}(v_{i, \sigma(a)}:r_{i,a}}
			&=
			\Ex{\Gamma_i^{\cS_i}(M,\sigma(v_i))}  \nonumber
			\\
			&~~~+ \Ex{\Gamma_i^{\cS_i}(T-Mn,\sigma(v_i))} \int_0^1p_i^{\cS_i}(y,\sigma(v_i))q_i^{\cS_i}(y,\sigma(v_i))dy.\label{eq:04271231}	
		\end{align}
	\end{claim}
	\begin{proof}[Proof of the claim]
		Since $\hbb$ is running with the first phase being ETC, the expected utility of agent $i$ can be decomposed as (i) expected utility in the exploration phase and (ii) expected utility in the exploitation phase.
		Note that (i) essentially coincides with the expectation of $\Gamma_i^{\cS_i}(M, \sigma(v_i))$ since it chooses agent $i$ exactly $M$ times regardless of the random rewards.
		Moreover, due to our restarting at time $\tau = Mn$, when the exploitation phase of $\alg_1$ starts, all the parameters of $\alg_2$ is initialized.
		Thus, conditioned on the event that agent $i$ has the largest empirical average reward at round $\tau = Mn$, its expected utility in the exploitation phase again coincides with the single agent case expected utility $\Gamma_i^{\cS_i}(T-Mn, \sigma(v_i))$.
		Otherwise, if agent $i$ has not been selected as the empirically best agent, then its conditional expected utility is simply zero.
		Note that the probability of agent $i$ being the empirically best agent can be written as follows,\footnote{To be precise, we need to take account for the tie-breaking rule and the event that tie happens, but we omit the detail as it can be easily handled and is beyond of our interest.}
		\begin{align*}
			\Pr{\text{agent $i$ is the empirically best agent at round $\tau = Mn$}}
			&=
			\int_{0}^1 \Pr{\muhat_i(M) \ge y}\Pr{C_i(y)}
			\\
			&=
			\int_0^1p_i^{\cS_i}(y,\sigma(v_i))q_i^{\cS_i}(y,\sigma(v_i))dy,
		\end{align*}
		and we finish the proof of the claim.
	\end{proof}
	Using the claim above, for any strategy $\cS_i$, we can further expand its conditional expected utility $\sum_{\sigma \in \cP_{l_i}} \CEx{u_i(\cS_i)}{\bigtimes_{a \in [l_i]}(v_{i, \sigma(a)}:r_{i,a})}$ as follows.
	\begin{align}
		\sum_{\sigma \in \cP_{l_i}}
		& 
		\CEx{U_i(\cS_i)}{\bigtimes_{a \in [l_i]}(v_{i, \sigma(a)}:r_{i,a})}\nonumber
		\\
		&=
		\sum_{\sigma \in \cP_{l_i}}
		\parans{
		\Ex{\Gamma_i^{\cS_i}(M,\sigma(v_i))} + \Ex{\Gamma_i^{\cS_i}(T-Mn,\sigma(v_i))} \int_0^1p_i^{\cS_i}(y,\sigma(v))q_i^{\cS_i}(y,\sigma(v_i))dy
		}
		\nonumber
		\\
		&=
		\parans{
		\sum_{\sigma \in \cP_{l_i}}
		\Ex{\Gamma_i^{\cS}(M,\sigma(v_i))}
		}
		+
		\sum_{\sigma \in \cP_{l_i}}
		\parans{
		\Ex{\Gamma_i^{\cS_i}(T-Mn,\sigma(v_i))}
		\int_{0}^1p_i^{\cS_i}(y,\sigma(v_i))q_i^{\cS_i}(y,\sigma(v_i))dy
		}
		\nonumber
		\\
		&=
		\parans{
		\sum_{\sigma \in \cP_{l_i}}
		\Ex{\Gamma_i^{\cS_i}(M,\sigma(v_i))}
		}
		+
		\int_{0}^1
		\parans{\sum_{\sigma \in \cP_{l_i}}
		\Ex{\Gamma_i^{\cS_i}(T-Mn,\sigma(v_i))}
		p_i^{\cS_i}(y,\sigma(v_i))q_i^{\cS_i}(y,\sigma(v_i))}dy
		\nonumber
		\\
		&=
		\parans{
		\sum_{\sigma \in \cP_{l_i}}
		\Ex{\Gamma_i^{\cS_i}(M,\sigma(v_i))}
		}
		+
		\int_{0}^1
		p_i^{\cS_i}(y,\sigma(v_i))
		\parans{
		\sum_{\sigma \in \cP_{l_i}}
		\Ex{\Gamma_i^{\cS_i}(T-Mn,\sigma(v_i))}
		q_i^{\cS_i}(y,\sigma(v_i))
		}dy,\label{eq:04271244}
	\end{align}
	where the third equality follows from Fubini's theorem, and the last inequality holds since $p_i^{\cS_i}(y,\sigma(v_i))$ is independent from $\sigma$.
	
	In case of the truthful strategy $\cO_i$, since any permutation $\sigma$ yields the same problem instance, all the terms inside \eqref{eq:04271244} remains the same.
	Thus,
	\begin{align}
		\sum_{\sigma \in \cP_{l_i}} &
		\CEx{U_i(\cO_i)}{\bigtimes_{a \in [l_i]}(v_{i, \sigma(a)}:r_{i,a})}\nonumber
		\\
		&~~~~~~=
		|\cP_{l_i}| 
		\parans{
		\Ex{\Gamma_i^{\cO_i}(M,
		v_i)}
		+
		\Ex{\Gamma_i^{\cO_i}(T-Mn,v_i)}
		\int_{0}^1p_i^{\cO_i}(y,v_i)q_i^{\cO_i}(y,v_i)dy
		}.\label{eq:05082325}
	\end{align}
	Now it suffices to prove that the RHS of \eqref{eq:05082325} is at least that of \eqref{eq:04271244}.
	
	We first observe that the first term can effectively compared based on our result on the single-agent setting.
	\begin{claim}\label{cl:reduc_to_single}
		For any strategy $\cS_i$, we have
		\begin{align*}
			\sum_{\sigma \in \cP_{l_i}}\Ex{\Gamma_i^{\cO_i}(M, \sigma(v_i))}	
			\ge
			\sum_{\sigma \in \cP_{l_i}}\Ex{\Gamma_i^{\cS_i}(M, \sigma(v_i))}.
		\end{align*}
	\end{claim}
	\begin{proof}
		Note that $\Gamma_i^{\cO_i}(M, \sigma(v_i))$ denotes the agent $i$'s utility at round $M$ under the single agent setting.
		Thus, the claim directly follows from Theorem~\ref{thm:single_rp} since we run ETC with $m = 2l/\Delta^2 \ln (2T)$ as Phase 2 algorithm.
	\end{proof}
	Thus, it remains to compare the latter term that involves the integral.
	Given $v_i \in \R_{\ge 0}^{l_i}$, for $a \in [l_i]$, write $Y_{i,a}$ to denote the event that the arm with mean $v_a$ of agent $i$ is selected in the exploitation rounds of $\alg_2$ for agent $i$, \ie having the largest empirical average reward at the end of the exploration rounds in $\alg_2$ for agent $i$.
%	Let $Z_{i,a}$ denote the event that arm with mean $v_a$ in agent $i$ has the largest empirical average reward at the end of the exploration rounds in $\alg_2$.
	
	\sscomment{Proofread}
	Further, similar to the definition of $\Gamma_i^{\cS_i}(\cdot, \cdot)$, we analogously define $\Gamma_{i,a}^{\cS_i}(\cdot, \cdot)$ to be the random cumulative rewards when there exists only agent $i$ and only arm $a$ under $\alg_2$.
	That is, $\Gamma_{i,a}^{\cS_i}(t, \sigma(v_i))$ is just a summation of $t$ random variables where each random variable follows the agent $i$'s arm's reward distribution parameterized by the mean reward $\sigma(v_i)$.
	Note that our construction in equation~\eqref{eq:04262152} verifies $v_{i,1} \ge v_{i,2} \ge \ldots \ge v_{i,l_i}$.
	Define $\delta_{i,a} = v_{i,1} - v_{i,a}$ for $a \in [l_i]$.
	
	We now construct a lower bound of $q_i^{\cO_i}(y,v_i)$ in the following. \sscomment{$o_i$ and $o$ are both used. Also, make consistent $\sigma(v)$ or $v$.}
	\begin{claim}\label{cl:tail_lower}
		For any $y \in [0,1]$, and $\sigma \in \cP_{l_i}$, consider arbitrary $v_i \in [0,1]^{l_i}$ such that $v_{i,1} \ge v_{i,2} \ge \ldots \ge v_{i,l_i}$.
		 Then, we have
		\begin{align*}
			q_i^{\cO_i}(y, v_i)
			\ge
			\Pr{\Gamma_{i,1}^{\cO_i}(M,v_i) \ge My} \parans{1 - 2\sum_{a=2}^{l_i} \exp(-\frac{\delta_{i,a}^2 m }{2})}
		\end{align*}

	\end{claim}
	\begin{proof}[Proof of the claim]
		Due to the independence of rewards from arm $a$ at exploitation phase and the random variable $\Ind{Y_{i,a}}$, we can rewrite $q_i^{\cO}(y,\sigma(v))$ as follows.
		\sscomment{FIXING...}
		\begin{align}
%			q_i^{\cO}(y,\sigma(v))
%			=
			q_i^{\cO_i}(y,v_i)
			&=
			\Pr{
			\sum_{a=1}^{l_i}
			\parans{
			\Gamma_{i,a}^{\cO_i}(m,v)
			+
			\Ind{Y_{i,a}}\Gamma_{i,a}^{\cO_i}(M-l_im, v_i)
			}
			\ge My
			}
			\nonumber
			\\
			&=
			\sum_{a=1}^{l_i}
			\CPr{
			\sum_{a=1}^{l_i} 
			\parans{
			\Gamma_{i,a}^\cO(m,v)
			+
			\Ind{Y_{i,a}}\Gamma_{i,a}^{\cO}(M-l_im, v)
			}
			\ge My
			}{Y_{i,a}}\Pr{Y_{i,a}}
			\nonumber
			\\
			&=
			\sum_{a=1}^{l_i}
			\CPr{
			\parans{
			\sum_{a=1}^{l_i} 
			\Gamma_{i,a}^\cO(m,v)
			}
			+
			\Gamma_{i,a}^{\cO}(M-l_im, v)
			\ge My
			}{Y_{i,a}}\Pr{Y_{i,a}}
			\nonumber
			\\
			&\ge
			\CPr{
			\parans{
			\sum_{a=1}^{l_i} 
			\Gamma_{i,1}^\cO(m,v)
			}
			+
			\Gamma_{i,1}^{\cO}(M-l_im, v)
			\ge My
			}{Y_{i,1}}\Pr{Y_{i,1}}
%			\nonumber
%			\\
%			&=
%			\sum_{a=1}^{l_i}
%			\CPr{
%			\Gamma_{i,a}^\cO(M,v) \ge l_iMy
%			}{Z_{i,a}}\Pr{Z_{i,a}}
%			\tag{Definition of $\Gamma_{i,a}^{\cO}$}
%			\\
%			&=
%			\sum_{a=1}^{l_i}
%			\Pr{
%			\Gamma_{i,a}^\cO(M,v) \ge l_iMy
%			}\Pr{Z_{i,a}}
%			\tag{Independence of $\Gamma_{i,a}^{\cO}$ and $Z_{i,a}$}
%			\\
%			&\ge
%			\Pr{\Gamma_{i,1}^\cO(M,v) \ge l_iMy}\Pr{Z_{i,a}},
%			\label{ineq:05090246}
			\nonumber
		\end{align}
		
		Note further that due to the positive correlation between the event $Y_{i,1}$ and the tail event, it follows that
		\begin{align*}
			\CPr{
			\parans{
			\sum_{a=1}^{l_i} 
			\Gamma_{i,1}^{\cO_i}(m,v)
			}
			+
			\Gamma_{i,1}^{\cO_i}(M-l_im, v)
			\ge My
			}{Y_{i,1}}
			\ge
			\Pr{
			\parans{
			\sum_{a=1}^{l_i} 
			\Gamma_{i,1}^{\cO_i}(m,v)
			}
			+
			\Gamma_{i,1}^{\cO_i}(M-l_im, v)
			\ge My
			}.
		\end{align*}
		
		Let us write
		\begin{align*}
			\psi_i(M, y, v) 
			= \Pr{
			\parans{
			\sum_{a=1}^{l_i} 
			\Gamma_{i,1}^{\cO_i}(m,v)
			}
			+
			\Gamma_{i,1}^{\cO_i}(M-l_im, v)
			\ge My
			},
		\end{align*}
		then we have
		\begin{align}
			q_i^{\cO_i}(y,v_i) \ge \psi_i(M, y,v)\Pr{Y_{i,1}}
			\label{ineq:05090246}
		\end{align}
		
		Since $Z_{i,1}$ is the complement of $\cup_{a=2}^l Z_{i,a}$, observe that
		\begin{align*}
			\Pr{Z_{i,1}^c}
			&=
			\Pr{\cup_{a=2}^l Z_{i,a}}
			\\
			&\le
			\sum_{a=2}^l\Pr{Z_{i,a}}
			\tag{Union bound}
			\\
			&\le
			\sum_{a=2}^l\Pr{\muhat_{i,1}(m) \le \muhat_{1,a}(m)}
			\tag{Definition of $Z_{i,a}$}
			\\
			&\le
			\sum_{a=2}^l 2\exp(-\frac{\delta_{i,a}^2 m}{2}).
			\tag{Claim~\ref{cl:concen}}
		\end{align*}
		
		Hence, we obtain
		\begin{align*}
			q_i^{\cO}(y,\sigma(v))
			\ge
			\psi_i(M, y, v)  \parans{1 - 2\sum_{a=2}^l \exp(-\frac{\delta_{i,a}^2 m }{2})},
		\end{align*}
		and it proves the claim.
	\end{proof}
	
%	\begin{lemma}
%		Let $X_1,X_2,\ldots, X_n$ be random variables supported on $ S\subset\R_{\ge 0}$ such that $X_i$ stochastically dominates $X_j$ for $i,j \in [n]$ such that $i \le j$.
%		Then, the following holds for any $x \in \R_{\ge 0}$ and $i < j$:
%		\begin{align*}
%			\Pr{\sum_{k \in [n]}X_k \ge x, X_i = \max_{k \in [n]}X_k} \ge \Pr{\sum_{k \in [n]}X_k \ge x, X_j = \max_{k \in [n]}X_k}.
%		\end{align*}
%	\end{lemma}
%	\begin{proof}[Proof of the lemma]
%		Let the random variables be discrete random variables with finite support for simplicity. Note that the arguments easily extend to the continuous case.
%		Write $S = \{s_1,s_2,\ldots, s_m\}$ and $X_{-i,-j}$ to denote the vector of random variables $X_k$ or $k \in [n]$ such that $k \neq i,j$, \ie
%		\begin{align*}
%			X_{-i,-j} = (X_1,\ldots, X_{i-1},X_{i+1}, \ldots, X_{j-1},X_{j+1}, \ldots, X_n).
%		\end{align*}
%		Note that LHS can be decomposed as follows.
%		\begin{align}
%			\Pr{\sum_{k \in [n]}X_k \ge x, X_i = \max_{k \in [n]}X_k}
%			&= \sum_{z \in S^{n-2}}\Pr{\sum_{k \in [n]}X_k \ge x, X_i = \max_{k \in [n]}X_k, X_{-i,-j} = z}.\label{eq:12231632}
%		\end{align}
%		Fix any realization $z \in S^{n-2}$ of $X_{-i,-j}$, and we can rewrite each term in RHS as follows.
%		\begin{align*}
%			\Pr{\sum_{k \in [n]}X_k \ge x, X_i = \max_{k \in [n]}X_k, X_{-i,-j} = z}
%			&= \Pr{X_i + X_j \ge x - \abs{z}_1, X_i \ge \max(\abs{z}_{\infty}, X_j)}\Pr{X_{-i,-j} = z},
%		\end{align*}
%		where $\abs{\cdot}_1$ and $\abs{\cdot}_\infty$ denote $\ell_1$ and $\ell_{\infty}$ norm respectively.
%		We can further expand
%		\begin{align*}
%			\Pr{X_i + X_j \ge x - \abs{z}_1, X_i \ge \max(\abs{z}_{\infty}, X_j)} = \sum_{k \in [m]}\Pr{ X_i \ge \max(x - \abs{z}_1 - s_k,\abs{z}_{\infty}, s_k)}\Pr{X_j = s_k}.
%		\end{align*}
%		Given $z$, define $f_k = \max(x-\abs{z}_1 - s_k, \abs{z}_\infty, s_k)$, then RHS can be written as
%		\begin{align*}
%			\sum_{k \in [m]}\Pr{X_i \ge f_k}\Pr{X_j = s_k}.	
%		\end{align*}
%		Note that $f_k$ is monotone increasing over $k$.
%		By Abel's transformation
%		\begin{align*}
%			\sum_{k \in [m]}\Pr{X_i \ge f_k}\Pr{X_j = s_k}
%			&= \Pr{X_i = f_m} - \sum_{k=1}^{m-1}\Pr{X_j \le s_k}\Pr{X_i = f_{k+1}} \\
%			&\ge \Pr{X_i = f_m} - \sum_{k=1}^{m-1}\Pr{X_i \le s_k}\Pr{X_i = f_{k+1}} \\
%			&= \sum_{k \in [m]}\Pr{X_i \ge f_k}\Pr{X_i = s_k} \\
%			&\ge \sum_{k \in [m]}\Pr{X_j \ge f_k}\Pr{X_i = s_k}.
%		\end{align*}
%		Hence we obtain
%		\begin{align*}
%			\Pr{\sum_{k \in [n]}X_k \ge x, X_i = \max_{k \in [n]}X_k, X_{-i,-j} = z}
%			&= \sum_{k \in [m]}\Pr{X_i \ge f_k}\Pr{X_j = s_k} \\
%			&\ge \sum_{k \in [m]}\Pr{X_j \ge f_k}\Pr{X_i = s_k} \\
%			&= \Pr{\sum_{k \in [n]}X_k \ge x, X_j = \max_{k \in [n]}X_k, X_{-i,-j} = z}.
%		\end{align*}
%		Plugging into~\eqref{eq:12231632} we finish the proof.
%	\end{proof}
%	\begin{lemma}
%		Let $X_1,X_2,\ldots, X_n$ be random variables supported on $ S\subset\R_{\ge 0}$ such that $X_i$ stochastically dominates $X_j$ for $i,j \in [n]$ such that $i \le j$.
%		Then, the following holds for any $x \in \R_{\ge 0}$:
%		\begin{align*}
%			\CPr{\sum_{k \in [n]}X_k \ge x}{X_1 = \max_{k \in [n]}X_k} \ge \Pr{\sum_{k \in [n]}X_k \ge x}
%		\end{align*}
%	\end{lemma}
%	\begin{proof}
%		Note that
%		\begin{align*}
%			\Pr{\sum_{k \in [n]}X_k \ge x} 
%			&= \sum_{i \in [n]}\Pr{\sum_{k \in [n]}X_k \ge x, X_i = \max_{k \in [n]}X_k} \\
%			&\le n\cdot\Pr{\sum_{k \in [n]}X_k \ge x, X_1 = \max_{k \in [n]}X_k}
%		\end{align*}
%	
%	\end{proof}
%
%
%	
%	To lower bound the difference between $q_i^\cO(y,\sigma(v))$ and $q_i^\cS(y,\sigma(v))$, we use the following rough upper bound for $q_i^\cS(y,\sigma(v))$.
%	\begin{claim}\label{cl:tail_upper}[New Claim]
%		For any strategy $\cS_i$, $\sigma \in S_{l_i}$, $y \in [0,1]$ and $v \in [0,1]^{l_i}$, we have 
%		\begin{align*}
%			q_i^{\cS_i}(y, \sigma(v))	 
%			\le 
%			\CPr{asd \ge y}{Y_{i,1}}\Pr{Y_{i,1}} + 1-\Pr{Y_{i,1}}.
%		\end{align*}
%	\end{claim}
	\begin{claim}\label{cl:tail_upper}
		For any strategy $\cS_i$, $\sigma \in S_{l_i}$, $y \in [0,1]$ and $v \in [0,1]^{l_i}$, we have 
		\begin{align*}
			q_i^{\cS_i}(y, \sigma(v))	 
			\le 
			\psi_i(M, y, v)
%			\Pr{\Gamma_{i,1}^{\cS}(M,\sigma(v)) \ge y}
%			=
%			\Pr{\Gamma_{i,1}^{\cO}(M,\sigma(v)) \ge y}
		\end{align*}
	\end{claim}
	\begin{proof}[Proof of the claim]
		This easily follows from the fact that in the probability $\psi(M,y,v)$, the exploration phase runs with the original $l_i$ arms for $m$ times each and then the exploration phase runs with the optimal arm $(i,1)$, whereas in the probability $q_i^{\cS_i}(y, \sigma(v))$, the exploration runs with the original $l_i$ arms upon the replicated arm for $m$ times each, and then exploitation runs with the empirically best arm.
		That is, we can couple the first $l_i \cdot m$ rounds for the exploration phase of the original $l_i$ arms, and then the exploitation is dominant for $\psi(M,y,v)$ due to the stochastic dominance of the arm $(i,1)$ over the other arms.
		
%		We can expand
%		\begin{align*}
%			q_i^{\cS}(y,\sigma(v))
%			&=
%			\Pr{
%			\sum_{a=1}^{l_i}
%			\parans{
%			\Gamma_{i,a}^\cS(m,\sigma(v))
%			+
%			\Ind{Y_{i,a}}\Gamma_{i,a}^{\cS}(M-lm, \sigma(v))
%			}
%			\ge y
%			}
%			\\
%			&=
%			\sum_{a=1}^{l_i}
%			\CPr{
%			\Gamma_{i,a}^\cS(M,\sigma(v)) \ge y
%			}{Z_{i,a}}\Pr{Z_{i,a}}
%			\\
%			&=
%			\sum_{a=1}^{l_i}
%			\Pr{
%			\Gamma_{i,a}^\cS(M,\sigma(v)) \ge y
%			}\Pr{Z_{i,a}}.
%		\end{align*}
%		Note further that $\Pr{\Gamma_{i,a}^\cS(M,\sigma(v)) \ge y} \le \Pr{\Gamma_{i,1}^\cS(M,\sigma(v)) \ge y}$ due to the stochastic dominance of the arm with mean $v_1$ over the arm with mean $v_a$, for any $a \in [l_i]$.
%		Thus, we have
%		\begin{align*}
%			q_i^{\cS}(y,\sigma(v))
%			&\le
%			\sum_{a=1}^{l_i}
%			\Pr{
%			\Gamma_{i,1}^\cS(M,\sigma(v)) \ge y
%			}\Pr{Z_{i,a}}
%			\\
%			&=
%			\Pr{\Gamma_{i,1}^\cS(M,\sigma(v)) \ge y}.
%		\end{align*}
%		In addition, observe that 
%		\begin{align*}
%			\Pr{\Gamma_{i,1}^{\cS}(y,\sigma(v)) \ge y}
%			=
%			\Pr{\Gamma_{i,1}^{\cO}(y,\sigma(v)) \ge y}	
%		\end{align*}
%		follows from the fact that $\Gamma_{i,1}^{\cS}(y,\sigma(v)) = \Gamma_{i,1}^{\cO}(y,\sigma(v))$ since both are random rewards when there is only arm with mean rewards $v_1$ of agent $i$.
	\end{proof}

	Now, combining Claim~\ref{cl:tail_lower} and~\ref{cl:tail_upper}, we obtain
	\begin{align}
		q_i^{\cO}(y, \sigma(v)) - q_i^{\cS}(y,\sigma(v))
		&\ge
		-2
		\psi_i(M, y, v)
%		\Pr{\Gamma_{i,1}^\cO(M,\sigma(v)) \ge y}
		\parans{\sum_{a=2}^{l_i} \exp(-\frac{\delta_{i,a}^2 m }{2})}
		\nonumber
		\\
		&\ge
		-2l_i 
		\psi_i(M, y, v)
%		\Pr{\Gamma_{i,1}^\cO(M,\sigma(v)) \ge y}
		\parans{\exp(-\frac{\Delta^2 m }{2})}
		\tag{Due to $\delta_{i,a} \ge \Delta$}
		\\
		&\ge
		-2l_i \cdot \frac{q_i^{\cO}(y, v)}{\Pr{Y_{i,1}}} \cdot
		\parans{\exp(-\frac{\Delta^2 m }{2})}\tag{Due to ineq. \eqref{ineq:05090246}}
		\\
		&\ge
		-2l_i \cdot \frac{q_i^{\cO}(y, v)}{1 - \sum_{a=2}^{l_i} 2\exp(-\frac{\delta_i^2 m}{2})} \cdot
		\parans{\exp(-\frac{\Delta^2 m }{2})}
		\nonumber
		\\
		&\ge
		-2l_i
		\cdot 
		\frac{q_i^{\cO}(y, v)}{1 - 2l_i\exp(-\frac{\Delta^2 m}{2})} \cdot
		\parans{\exp(-\frac{\Delta^2 m }{2})},
		\label{ineq:05090213}
	\end{align}
	where the fourth inequality follows from the concentration on $Z_{i,1}$ in the proof of Claim~\ref{cl:tail_lower}.

	Now we consider two cases regarding $\sigma$: (i) when $\sigma(1) = 1$ and (ii) otherwise.
	
%	\paragraph{case (i): $\sigma(1) = 1$}
%	This means that there exists a suboptimal arm with at least one replication.
%	In this case, as per the proof of 
%	
%	\paragraph{case (ii): $\sigma(1) \neq 1$}
	
	Recall that it suffices to prove that the RHS of \eqref{eq:05082325} is at least that of \eqref{eq:04271244}.
	Due to Claim~\ref{cl:reduc_to_single}, it suffices to prove the following inequality.
	\begin{align}
		\int_{0}^1
		&p_i^{\cS}(y,\sigma(v))
		\parans{
		\sum_{\sigma \in S_l}\underbrace{\paranm{\Ex{\Gamma_i^{\cO}(T-Mn,\sigma(v))}
		q_i^{\cO}(y,\sigma(v))
		-
		\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		q_i^{\cS}(y,\sigma(v))}}_{\Theta(\sigma, v)}
		}dy 
		\ge 
		0.
		\label{eq:05090205}
	\end{align}
%	Now we prove the following positive correlation.
%	\begin{claim}
%		For any $\sigma_1,\sigma_2 \in S_l$, 
%		it satisfies $q_i^{\cS}(y,\sigma_1(v)) \ge 	q_i^{\cS}(y,\sigma_2(v))$ iff the following holds.
%		\begin{align*}
%			\Ex{\Gamma_i^{\cS}(T-Mn,\sigma_1(v))} \ge \Ex{\Gamma_i^{\cS}(T-Mn,\sigma_2(v))}	
%		\end{align*}
%	\end{claim}
%	\begin{proof}
%		\note{TBD - Intuitive}
%	\end{proof}
%	Thus, by Chebyshev's sum inequality, we have
%	
%
%
%
%	
%	=========2nd=========
	
	
	Note that the term inside the summation can be decomposed as follows.
	\begin{align*}
		\Theta(\sigma, v)
		=
		\paranm{\Ex{\Gamma_i^{\cO}(T-Mn,\sigma(v))} - \Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}}q_i^{\cO}(y,\sigma(v))
		\\
		+
		\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		\paranm{q_i^\cO(y,\sigma(v)) - q_i^{\cS}(y,\sigma(v))}.
	\end{align*}
	
	Due to \eqref{ineq:05090213}, we further obtain
	\begin{align*}
		\Theta(\sigma, v) 
		&\ge 
		\underbrace{\paranm{\Ex{\Gamma_i^{\cO}(T-Mn,\sigma(v))} - \Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}}q_i^{\cO}(y,\sigma(v))}_{\Theta_1(\sigma, v)}
		\\
		&-
		\underbrace{2\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		\cdot l_i\cdot \frac{q_i^{\cO}(y, v)}{1 - 2l_i\exp(-\frac{\Delta^2 m}{2})} \cdot
		\parans{\exp(-\frac{\Delta^2 m }{2})}}_{\Theta_{2}(\sigma, v)} 
		.
	\end{align*}
	By summing over $\sigma \in S_{l_i}$, for $\Theta_1(\sigma, v)$, we have
	\begin{align*}
		\sum_{\sigma \in S_l} \Theta_1(\sigma, v)	
		&=
		\sum_{\sigma \in S_l}\paranm{\Ex{\Gamma_i^{\cO}(T-Mn,\sigma(v))} - \Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}}q_i^{\cO}(y,\sigma(v))
		\\
		&=
		q_i^{\cO}(y,\sigma(v)) \cdot \sum_{\sigma \in S_{l_i}}\paranm{\Ex{\Gamma_i^{\cO}(T-Mn,\sigma(v))} - \Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}}
	\end{align*}
	
	From inequality~\eqref{ineq:05090221} and \eqref{ineq:05090222} we know that
	\begin{align*}
		\sum_{\sigma \in S_{l_i}}\paranm{\Ex{\Gamma_i^{\cO}(T-Mn,\sigma(v))} - \Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}}
		&\ge
		\sum_{a \in [l_i]} \delta_{i,a} (\frac{m}{l_i} - 1)
		\\
		&\ge
		\sum_{a \in [l_i]} \delta_{i,a} (\frac{2l_i \ln 2T / \Delta^2}{l_i} - 1)
		\\
		&= 
		\sum_{a \in [l_i]} \delta_{i,a} (\frac{\ln 2T}{\Delta^2} - 1),
	\end{align*}
	which implies
	\begin{align*}
		\sum_{\sigma \in S_l} \Theta_1(\sigma, v)
		&\ge
		q_i^{\cO}(y,\sigma(v)) 
		\cdot \sum_{i \in [l]} \delta_{i,a} (\frac{\ln 2T}{\Delta^2} - 1).
	\end{align*}
	
	Putting $m = 4 \cdot \frac{2}{\Delta^2} (\max_i l_i) \ln(2T)$, observe that the following holds.
	\begin{align*}
		\exp(-\frac{\Delta^2 m}{2}) \le \frac{1}{4l_iT}	
	\end{align*}

	Hence, for $\Theta_2(\sigma,v)$, we further obtain
	\begin{align*}
		\sum_{\sigma \in S_{l_i}}\Theta_2(\sigma,v)
		&=
		2\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		\cdot l_i\cdot \frac{q_i^{\cO}(y, v)}{1 - 2l_i\exp(-\frac{\Delta^2 m}{2})} \cdot
		\parans{\exp(-\frac{\Delta^2 m }{2})}
		\\
		&\le
		4\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		\cdot l_i\cdot q_i^\cO(y,v)\cdot \frac{1}{4l_iT}
		\\
		&=
		\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		 q_i^\cO(y,v)\frac{1}{4T}
		\\
		&\le
		\frac{q_i^{\cO}(y,v)}{4}\tag{Since $\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))} \le T$}
	\end{align*}
	
	Combining the above observations, for $\Theta(\sigma, v)$, we obtain
	\begin{align*}
		\sum_{\sigma \in S_{l_i}}\Theta(\sigma, v)
		&\ge
		q_i^{\cO}(y,v)
		\parans{
		\sum_{a \in [l_i]} \delta_{i,a} (\frac{\ln 2T}{\Delta^2} - 1)
		-
		\frac{1}{4}
		}
		\\
		&\ge
		q_i^{\cO}(y,v)
		\parans{
		\sum_{a \in [l_i]}  (\frac{\ln 2T}{\Delta} - 1)
		-
		\frac{1}{4}
		}
		\\
		&=
		q_i^{\cO}(y,v)\parans{l_i \cdot \ln(2T) - l_i -\frac{1}{4}} 
		\\
		&\ge 0,
	\end{align*}
	where the last inequality follows from $T \ge 1$ and $q_i^\cO(y,v) \ge 0$.
	Thus, inequality \eqref{eq:05090205} is true, and it finishes the proof.

	
%	===========	===========	===========	===========	===========	===========
%
%	
%	Let $\cS$ be agent $i$'s strategy with replication vector $r = (r_1,r_2,\ldots, r_l)$, with at least one coordinate being strictly positive.
%	Without loss of generality, suppose $r_1 \ge r_2 \ge \ldots \ge r_l$, then we have $r_1 \ge 1$.
%	This indeed brings no difference since the expected payoff is marginalized over all the possible permutations, as we see thus far.
%	Let $\Omega_1$ be a set of permutation $\sigma \in S_l$ such that arm $\sigma(1) = 1$, \ie the best arm is replicated the most times, and define $\Omega_2 = S_l \setminus \Omega_1$.
%	We handle case $\omega \in \Omega_1$ and $\omega \in \Omega_2$ separately.
	
	

%
%	
%	Since our $alg_2$ is stochastically schur-concave, if two strategies $\cS$ and $\cS'$ with replication vector $r$ and $r'$ satisfy $r' \succ r$, then we can obtain
%	\begin{align*}
%		\sum_{\sigma \in S_l}
%		q_i^{\cS}(y,\sigma(v))
%		\ge
%		\sum_{\sigma \in S_l}
%		q_i^{\cS'}(y,\sigma(v)).
%	\end{align*}
%	Furthermore, the following easily follows from the fact that $\alg_2$ is SPF.
%	\begin{claim}
%		Given that $\alg_2$ is SPF, for any $v$ and $t$, we have $\Ex{\Gamma_i^{\cS}(t,v)}\ge \Ex{\Gamma_i^{\cS'}(t,v)}$.
%	\end{claim}
%	\begin{proof}
%		It is easy to check that SPF implies EPF.
%		Then, the claim directly follows from the single-agent characterization in  Theorem~\ref{thm:single_pf_rp}.
%	\end{proof}
%	
%	Combining the above facts, we can obtain
%	\begin{align*}
%		\sum_{\sigma \in S_l} 
%		\CEx{U_i(\cS)}{\sigma, v}
%		\ge
%		\sum_{\sigma \in S_l} 
%		\CEx{U_i(\cS')}{\sigma, v}.
%	\end{align*}

%	Thus, putting back to \eqref{eq:04262152} completes the proof.	
\end{proof}





==> neurips2024/neurips-checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 2, 3, and 4 justifies it.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 2,3,4, and the appendix include discussions on the limitations.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 3,4, and the appendix includes all details.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: It is respected.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This is a theoretical extension of existing problem.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> normal_bandit_analysis.tex <==
\section{Warm-up for normal bandits}
Let us consider a set-up where for each agent we have a distribution of means $O$ and each arm has a distribution $\cN(\mu, f(\mu))$ where $\mu$ is sampled from $O$. We will further assume that $P(O \in [0,1]) = 1$ and $f(\mu)$ is continuous with a maximum in $\frac{1}{2}$ and $f(0) = f(1) = 0$ that is what happens in the Bernoulli setting.
\subsection{Comparing normals}
Suppose that we have two arms $A_1$ and $A_2$ that have sampled (independently) $\mu$ and $\mu^*$ respectively with $\mu < \mu^*$. We want test (independently) each arm $N$ times and we want to know the probability that the sum of $A_1$ is lower than the sum of $A_2$, this is $B = P(S(A_1)<S(A_2))$. Recall that $\cN(\mu_1, \sigma_1^2) + \cN(\mu_2, \sigma_2^2) = \cN(\mu_1+\mu_2, \sigma_1^2+\sigma_2^2)$ if they are independent. Then $$P(S(A_1)<S(A_2)) = P(\cN(N\mu, Nf(\mu)) < \cN(N\mu^*, Nf(\mu^*))) =$$ $$ = P(\cN(\mu, f(\mu)/N) < \cN(\mu^*, f(\mu^*)/N)) = P(\cN(\mu, f(\mu)/N) - \cN(\mu^*, f(\mu^*)/N) < 0) = $$ $$ =  P(\cN(\mu-\mu^*, (f(\mu)+f(\mu^*))/N) < 0) $$
Since $\mu - \mu^* < 0$ we can bound the previous quantity by $P(\cN(\mu-\mu^*, 2f(1/2)/N) < 0) $. If we call $\Delta\mu = \mu^* - \mu > 0$ we have $B \leq P(\cN(0, 1) \leq \Delta\mu \sqrt{N} / \sqrt{2f(1/2)})$. Using \href{https://www.johndcook.com/blog/norm-dist-bounds/}{this} we can bound $B \leq P(Z \leq \Delta\mu \sqrt{N} / \sqrt{2f(1/2)}) = 1 - P(Z > \Delta\mu \sqrt{N} / \sqrt{2f(1/2)}) \leq 1 - \frac{t}{(t^2+1)\sqrt{2\pi}}e^{-t^2/2} $ where $t = \Delta\mu\sqrt{N}/\sqrt{2f(1/2)}$. This bound approaches $1$ approximately as $1/\sqrt{N}e^N \to 0$.\\
In the other hand suppose $f(\mu^*) \leq f(\mu)$ then we can set a lower bound in $B$ with $P(\cN(-\Delta\mu, 2f(\mu^*)/N) < 0)$ and then $B \geq 1 - P(Z > \Delta\mu \sqrt{N} / \sqrt{2f(\mu^*)}) \geq 1 - e^{-t'^2/2}\frac{1}{t'\sqrt{2\pi}}$ where $t' = \frac{\Delta\mu \sqrt{N}}{\sqrt{2f(\mu^*)}}$ that approaches $1$ at the same rate as before.
\subsection{The 3 arms scenario}
Suppose that we draw 3 arms from $O$ with $\mu_1, \mu_2 < \mu^*$ and test them $N$ times. We want to give some bounds to the probability $G = P(S(\mu^*) \geq \max_{i=1,2}{S(\mu_i)})$. $G \leq P(S^* \geq S_i)$.

Suppose that $O = U([0,1])$ and $f(\mu) = \mu(1-\mu)$. Then I think we can make the calculations explicit (maybe there is a difficult integral with exponential that needs to be bounded). I will work on it.

==> positive_lemma.tex <==
\section{Towards Replication-Proof Mechanism}
The following notation will play a crucial role in analyzing replication-proofness of an algorithm.
\begin{definition}[Permutation-free]
	Consider any single-agent bandit instance $\cI$ with mean rewards $\mu_1\ge \mu_2 \ge \ldots \ge \mu_k$.
	Let $\cI_i$ be a bandit instance in which arm $i$ is replicated once from $\cI$.
	We say that an algorithm is permutation-free if the following holds for any $T \ge 1$,
	\begin{align*}
		\reg_{\cI}(T) \le \frac{\sum_{i=1}^k\reg_{\cI_i}(T)}{k}.
	\end{align*}
\end{definition}

\begin{theorem}[Permutation-free yields replication-proof under a single agent]\label{thm:single_pf_rp}
	Under a single-agent setting, if an algorithm is permutation-free, then it is replication-proof.
\end{theorem}
\begin{proof}
	
	\begin{lemma}
		Consider a permutation-free algorithm $\alg$ under a single-agent instance $\cI$ with mean rewards $\mu_1 \ge \mu_2 \ge \ldots \ge \mu_k$.
		Let $R$ be a random variable that chooses $l$ indices from $[k]$ uniformly at random, allowing the repetition.
		Let $\cI'$ be any bandit instance in which the corresponding $l$ arms are selected according to the index sampled from $R$.
		Then, the following holds for any $T \ge 1$,
		\begin{align*}
			\reg_{\cI}(T) \le \reg_{\cI'}(T).
		\end{align*}
	\end{lemma}
	\begin{proof}[Proof of the lemma]
	\note{Suho - TBD}
	\end{proof}
	
	\begin{lemma}
		Given two strategies
		Let $R_{\alg}(i)$ be the agent-wise random variable of agent $i$ under $\alg$, and $R_{\alg'}(i)$ be that under $\alg'$.
		
	\end{lemma}
	\note{Suho - TBD}
\end{proof}



\begin{algorithm} 
\SetAlgoLined
%$i \in \set{N}$, $\set{S} = \cup_{i \in \set{N}} \set{S}_i$\\
Parameter $\alg_1$, $\alg_2$
;\\
Initialize $R(i), N(i), r(a)$ and $n(a)$ at zero  
for all $i \in \set{N}$ and $a\in \cup_{i \in \set{N}} \set{S}_i$;


 \For{$t=1,2,\ldots$}{
  \tcp{Phase 1 - agent selection}
  Run $\alg_1$ with agent-wise parameters $R(i)$, $N(i)$, and round index $t$;\\
  Let $\hat{i}$ be the selected agent;\\
  \tcp{Phase 2 - arm selection}
  Run $\alg_2$ within agent $\hat{i}$ with parameters $r(a)$, $n(a)$, and round index $N(i)$ for $a \in \set{S}_i$;\\
  Let $\hat{a}$ be the selected arm;\\
%  
%  If $N(i) \le 1/2T^{1/3} \log(T)^{1/3}$, round-robin exploration of arms in $\set{S}_i$;\\
%  Else, commit $\hat{a} = \argmax_{a \in \set{S}_{\hat{i}}} 
%    \left\{r(a) \right\}$
  Play $A_t = \hat{a}$ and receive reward $R_t$; \\
  Update statistics:
  $r(\hat{a}) \leftarrow \tfrac{r(\hat{a})n(\hat{a}) + R_t}{n(\hat{a})+1}; ~~
  R(\hat{i}) \leftarrow \tfrac{R(\hat{i})N(\hat{i}) + R_t}{N(\hat{i})+1};$
  
  $n(\hat{a}) \leftarrow n(\hat{a}) + 1; ~~ N(\hat{i}) \leftarrow N(\hat{i}) + 1;$
 }
 \caption{\hbb\label{alg:hbb}}
\end{algorithm}

A direct implication of Theorem~\ref{thm:single_pf_rp} is that H-BlackBox with a simple of $\alg_1$ and $\alg_2$ yields 
\begin{theorem}
	Let $\alg_1$ denote a uniform random selection algorithm.
	Then, for any permutation-free  $\alg_2$, $\hbb$ with $\alg_1$ and $\alg_2$ is replication-proof.
\end{theorem}
\begin{proof}
	\note{Suho - TBD - Easily follow, but make it formal}	
\end{proof}

Together with Theorem [That shows permutation-free example], the above theorem implies the existence of the replication-proof algorithm.
Note however that if we deploy uniform random selection algorithm in $\alg_1$, it essentially suffers linear regret since it always choose any suboptimal agent with constant probability at every rounds.
To capture the both rabbits of sublinear regret and replication-proofness, we need more carefully tailored algorithm with sublinear regret in $\alg_1$.

\begin{conjecture}[Hierarchical algorithm with permutation free submodule suffices]
	Given permutation-free algorithms $\alg_1$ and $\alg_2$, suppose that $\alg_1$ satisfies STH.
	Then,
	H-BlackBox $\alg_1$ and $\alg_2$ is replication-proof.
	\note{What should be STH? - Thompson sampling would be a natural choice, since each choice prob. is naturally proportional to the mean empirical reward of the agent.}
\end{conjecture}


==> regret-analysis.tex <==


%
%\begin{definition}[Permutation-free]
%	\note{"permutation"?}
%	Consider any single-agent bandit instance $\cI$ with mean rewards $\mu_1\ge \mu_2 \ge \ldots \ge \mu_k$.
%	Let $\cI_i$ be a bandit instance in which arm $i$ is replicated once from $\cI$.
%	We say that an algorithm is permutation-free if the following holds for any $T \ge 1$,
%	\begin{align*}
%		\reg_{\cI}(T) \preceq \frac{\sum_{i=1}^k\reg_{\cI_i}(T)}{k}.
%	\end{align*}
%\end{definition}
%
%In the following, we prove that any permutation-free algorithm yields replication-proofness in a single agent setting.
%This fact nicely works as a stepping stone to construct a replication-proof algorithm in the general setting.
%
%\begin{theorem}[Permutation-free yields replication-proof under a single agent]\label{thm:single_pf_rp}
%	Under a single-agent setting, if an algorithm is permutation-free, then it is replication-proof.
%\end{theorem}
%\begin{proof}
%	We start with the following lemma which states the transitivity of the permutation-freeness.
%	\begin{lemma}
%		Consider a permutation-free algorithm $\alg$ under a single-agent instance $\cI$ with mean rewards $\mu_1 \ge \mu_2 \ge \ldots \ge \mu_k$.
%		Given a vector $v\in (\N\cup \{0\})^k$ of nonnegative integer, consider a random permutation $\sigma(v)$ over the set of all feasible permutations, where each permutation is equally likely selected.
%		Let $\cI_{\sigma(v)}$ be a bandit instance in which arm $K$ is replicated $\sigma(v)_i$ times.
%		Then, for any $v\in (\N\cup \{0\})^k$ and any time horizon $T$, the following holds,
%		\begin{align*}
%			\reg_{\cI}(T) \preceq \Exu{\sigma}{\reg_{\cI_{\sigma(v)}}(T)}.
%		\end{align*}
%	\end{lemma}
%	\begin{proof}[Proof of the lemma]
%		For $j \in [k]$, define $\cI^{(j)}$ be a bandit instance in which the arm $j$ is replicated once from $\cI$.
%		Then, by the definition of permutation-free algorithm, we have
%		\begin{align*}
%			\reg_{\cI^{(j)}}(T) 
%			\preceq 
%			\frac{\sum_{i=1}^{k+1} \reg_{\cI_i^{(j)}}(T)}{k+1},
%	\end{align*}
%	for $j \in [k]$.
%	Let $v_1 = $...
%	Summing up over $j$, we obtain
%	\begin{align*}
%		asd
%		=
%		\sum_{j \in [k]}\reg_{\cI^{(j)}}(T)
%		\preceq 
%		\sum_{j \in [k]}\frac{\sum_{i=1}^{k+1} \reg_{\cI_i^{(j)}}(T)}{k+1} 
%	\end{align*}
%	
%
%
%	\note{Suho - TBD}
%	\end{proof}
%	\note{Suho - TBD}
%\end{proof}




==> single-agent.tex <==
\section{Warm-up: Single-agent Setting}\label{sec:single}
As noted thus far, UCB is not replication-proof even in the single agent setting.
Indeed, as per Theorem~\ref{thm:ucb_negative}, it is not obvious to verify which algorithm would satisfy replication-proofness even in the single-agent setting.
%Inferring from the worst-case problem instance we present in Theorem~\ref{thm:ucb_negative}, one can essentially observe that an algorithm should \emph{necessarily} be robust to partial replication.
%Indeed, it is not easy to verify which algorithms would satisfy replication-proofness even in the single agent setting.
In this section, we step towards in constructing replication-proof algorithm, by carefully investigating the single-agent setting first.
We present a set of conditions which is sufficient for an algorithm to be replication-proof in the single-agent setting, and then, as an example, will prove that exploration-then-commit (ETC) will satisfy these properties.
As we restrict our attention to single-agent setting in this section, we often omit the agent index $i$ in the notations.

To this end, we first introduce several notations.
For any natural number $l$, let $\cP_l$ be a set of all possible permutations $\sigma:[l] \mapsto [l]$.
Now we introduce a dictionary form of bandit instance $\cI$.
Given the realization of the arms' mean rewards, suppose that the set of mean rewards constitute a sorted sequence $\{1 \ge \mu_1 > \mu_2 > \ldots > \mu_l  > 0\}$, where some arms may share the same mean reward.
For each $\mu_a$ for $a \in [l]$, we count the number of arms which have mean reward $\mu_a$, and denote the count by $c_a$.
Then, our bandit instance $\cI$ can essentially presented as tuples of the mappings $\bigtimes_{a\in[l]}(\mu_a:c_a)$, which we say dictionary form of the bandit instance $\cI$.

Suppose that we have a standard multi-armed bandit instance $\cI$ with dictionary form $(\mu_a:c_a)_{a \in [l]}$.
Then, we define a \emph{permuted bandit instance} $\cI_\sigma$ to be a bandit instance with dictionary form of $\bigtimes_{a\in[l]}(\mu_a: c_{\sigma(a)})$, \ie arms with mean reward $\mu_i$ appears $c_{\sigma(a)}$ times.
For instance, given the original bandit instance $\cI = (0.5: 1, 0.7: 2)$, consider a permutation $\sigma$ such that $\sigma(1) = 2$ and $\sigma(2)=1$ correspondingly.
Then, one can easily verify that $\cI_\sigma = (0.5:2, 0.7:1)$.


Now, we introduce the following refinement of the standard regret.
\begin{definition}[Random permutation regret]
	Given a single-agent bandit instance $\cI$ with $l$ arms, we define an algorithm $\fA$'s \emph{random permutation regret} (RP-Regret) as follows.
	\begin{align}
		\rpreg(\fA, T) 
		&= 
		\Exu{\sigma \in \cP_l}{\reg_{I_{\sigma}}(\fA, T)}
		\nonumber
		\\
		&=
		\frac{1}{|\cP_l|} \cdot \parans{\sum_{\sigma \in \cP_l}\reg_{I_{\sigma}}(\fA, T)}.\label{eq:epf}
	\end{align}
\end{definition}
Given the random permutation regret, we define the following property of algorithm, which will play an essential role in obtaining truthful algorithm in the single-agent setting.
\begin{definition}[Truthful under random permutation]
	Given an arbitrary single-agent bandit instance $\cI$ with $l$ arms,
	consider a truthful strategy $\cO$ and arbitrary strategy $\cS$.
	We say that an algorithm $\fA$ is \emph{truthful under random permutation} (TRP) if
	\begin{align*}
		\rpreg(\fA,T;\cO) 
		\le 	
		\rpreg(\fA,T;\cS).
	\end{align*}
\end{definition}
Note that TRP requires the inequality to holds for arbitrary bandit instance $\cI$.
The foundation of these notions essentially builds upon the observation from our counterexample provided in Theorem~\ref{thm:ucb_negative}.
To elaborate more, 
consider a strategy $\cS$ that only replicates the first arm given a bandit instance $\mu_1\ge \mu_2 \ge \ldots \ge \mu_l$.
Then, we can observe that any permutation $\sigma \in \cP_l$ results in a bandit instance that belongs to the following family of bandit instances: define $\cI^* = \cup_{i \in [l]}\cI_i$ such that
\begin{align*}
    \cI_1 = \{\underbrace{\mu_1, \mu_1}_{replicated}, \mu_2, \mu_3, \ldots, \mu_l\}, \cI_2 = \{\mu_1, \underbrace{\mu_2,\mu_2}_{replicated}, \mu_3, \ldots, \mu_l\}, \ldots,  \cI_l = \{\mu_1, \underbrace{\mu_2,\mu_2}_{replicated}, \mu_3, \ldots, \mu_l\}
\end{align*}
% \begin{itemize}
% 	\item $\cI_1 = \{\underbrace{\mu_1, \mu_1}_{replicated}, \mu_2, \mu_3, \ldots, \mu_l\}, \cI_2 = \{\mu_1, \underbrace{\mu_2,\mu_2}_{replicated}, \mu_3, \ldots, \mu_l\}, \cI_2 = \{\mu_1, \underbrace{\mu_2,\mu_2}_{replicated}, \mu_3, \ldots, \mu_l\}$
% 	\item $\cI_2 = \{\mu_1, \underbrace{\mu_2,\mu_2}_{replicated}, \mu_3, \ldots, \mu_l\}$
% 	\\ $\vdots$\\
% 	\item $\cI_l = \{\mu_1, \mu_2, \mu_3, \ldots, \underbrace{\mu_l, \mu_l}_{replicated}\}$.
% \end{itemize}
In words, $\cI_i$ denotes the case that the strategy $\cS$ replicates the arm with $i$-th highest reward.
For example, suppose that $\sigma \in \cP_l$ satisfies $\sigma(1) = i$ for some $i \in [l]$.
Since $\cS$ replicates the first arm, under the permutation $\sigma$, the arm with parameter $\mu_i$ is replicated, and thus it corresponds to $\cI_i$.
Then, our notion of TRP essentialy asks what is an algorithm that makes the expected regret of $\cI$ smaller than (or equal to) the average of expected regret of $\cI_1,\dots, \cI_l$.
Put it differently, TRP essentially asks the following fundamental question, which corresponds to the one that we discuss in Section~\ref{sec:intro}.
\begin{center}
	\emph{Given a bandit instance, does ``uniform randomly'' replicate one arm increase the expected regret?}
\end{center}
This foundation of truthfulness under random permutation will play an essential role in constructing replication-proof algorithm in both the single-agent and the multi-agent setting, as can be seen shortly.
Indeed, one can verify that UCB does not satisfy the above question, and thus fails to be replication-proof, from our proof of Theorem~\ref{thm:ucb_negative}.


We finally introduce a permutation invariant of a bandit algorithm.
\begin{definition}[Permutation invariance]
	An algorithm is \emph{permutation invariant} (PI) if given the random bits of the algorithm and the arms, the choice of which arms to pull remains the same (up to tie-breaking) when the index of the arms are permuted.
\end{definition}
Note that the permutation-invariance essentially requires the algorithm to be agnostic to the index of the arms, \ie does not use the arm index to choose the arm, possibly except the tie-breaking case.
One can easily verify that it holds for a broad class canonical algorithms including the ETC, UCB, $\eps$-greedy, etc.

Our main result on the single-agent setting can be presented as follows.

\begin{theorem}\label{thm:single_pf_rp}
	Under the single-agent setting, if an algorithm is truthful under random permutation and permutation-invariant, then it is replication-proof.
\end{theorem}
The proof essentially follows from the observation that the algorithm's ex-ante regret can be partitioned into a disjoint set of random permutation regret, with respect to the ex-post realization of the mean rewards.
Based on this disjoint partition, we can effectively marginalize over the priors while maintaining the partition, and thus conclude that the dominance over the partition yields the overall dominance, where each partition corresponds to a set of randomly permuted bandit instances.
\begin{proof}[Proof of Theorem~\ref{thm:single_pf_rp}]
	Let $\fA$ be an algorithm with symmetry and TRP.
	Given a single agent problem instance $\cI$ with original set $\cO$ with $l$ arms, let $\cS$ be a truthful strategy that registers $\cO$.
	Consider any non-truthful strategy $\cS$ such that it replicates $r_i \in \Z_0$ times for arm $a$ for $a \in [l]$, where $\Z_0 =  \{0,1,2,\ldots\}$ denotes the set of nonnegative integers.
	Note that since $\cS$ is non-truthful strategy, at least one $r_a$ has to be strictly positive for some $a \in [l]$.
	We abuse $r_a=0$ to say that arm $a$ is only registered once without any replication, and write $r = (r_1,\ldots, r_l)$.
	For $v = (v_1,\ldots, v_l) \in \R_{\ge 0}^l$, we write $g(v)$ to denote the density of the mean rewards of arms having $v$, \ie $g(v) = \prod_{a=1}^l f(v_a)$, where $\R_{\ge 0}^l$ denotes the set of $l$-dimensional nonnegative real vectors.
	For simplicity, we assume that the prior distribution of the agent has probability density function, and does not have any point mass.\footnote{This assumption is for ease of exposition, and does not restrict any of our results. For instance, if there exists point mass so that two arms may realize the same mean reward with strictly positive probability, then we can essentially unionize those two arms and consider it as a single arm. In this way, one can verify that all the analysis carry over.}
	We further write $dv$ to denote $dv_1 dv_2 \ldots dv_l$.
	We use $\reg_{v, r}$ to denote the regret of problem instance such that the arms' mean rewards are realized to be $v$ and each arm $i$ is replicated $r_i$ times.
	We finally write $\sigma(v)$ to the permuted vector given a permutation $\sigma \in S^l$, and $\sigma(v)_i$ to denote $i$-coordinate of $\sigma(v)$.
	
%	The following claim easily follows from our definition of permutation-freeness.
	
	Observe that the expected utility in playing the strategy $\cS$ can be written as follows.
	\begin{align*}
		u(\cS) 
		&= 
%		\int_{\mu_1 = v_1}\ldots \int_{\mu_l = v_l} \Ex{U(\cS)\ |\ v_1,\ldots, v_l}g(v)dv
		\int_{\mu_1 = v_1}\ldots \int_{\mu_l = v_l} \Ex{U(\cS)\ |\ \bigtimes_{i \in [l]}(v_a: r_a)}g(v)dv
		\\
		&=
%		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 < v_1}\ldots \int_{\mu_k = v_l< v_{l-1}} 
%		\sum_{\sigma \in \cP_l}\Ex{U(\cS)\ |\ \sigma(v)_1,\ldots, \sigma(v)_l}g(v)dv
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 < v_1}\ldots \int_{\mu_k = v_l< v_{l-1}} 
		\sum_{\sigma \in \cP_l}\Ex{U(\cS)\ |\ \bigtimes_{i \in [l]}(v_{\sigma(a)}: r_a)}g(v)dv
		\\
		&=
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 < v_1}\ldots \int_{\mu_k = v_l< v_{l-1}} 
%		\sum_{\sigma \in \cP_l}\Ex{v_1T - \reg_{\sigma(v),r}(T) \ |\ \sigma(v)_1,\ldots, \sigma(v)_l}g(v)dv.
		\sum_{\sigma \in \cP_l}\Ex{v_1T - \reg_{\sigma(v),r}(T) \ |\ \bigtimes_{i \in [l]}(v_a: r_a)}g(v)dv,
	\end{align*}
	where in the last equation, we condition on $\bigtimes_{i \in [n]}(v_i:r_i)$ since $\reg_{\sigma(v),r}(T)$ already accounts for the permuted bandit instance.
	Further, due to the permutation invariance of the algorithm, applying $\sigma^{-1}$ to all the arm indices does not change the expected regret, and thus we can further expand it to be
	\begin{align}
		u(\cS)
		&=
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 <v_1}\ldots \int_{\mu_l = v_l< v_{l-1}} 
%		\sum_{\sigma \in \cP_l}\Ex{v_1T - \reg_{v,\sigma(r)}(T) \ |\ v_1, \ldots, v_l}g(v)dv.
		\sum_{\sigma \in \cP_l}\Ex{v_1T - \reg_{v,\sigma(r)}(T) \ |\ \bigtimes_{a \in [l]}(v_a: r_a)}g(v)dv.
		\label{ineq:05131256}
	\end{align}
	Let $\vec{0}_l$ denote the $l$-dimensional zero vector.
%	, and the inequality easily follows from the fact that $(0,0,\ldots,0) \prec_m r$ and the algorithm is TRP.
	We now prove the following claim.
	\begin{claim}
		For any $v \in R_{\ge 0}^l$, $\sigma \in \cP_l$, and $r \in \Z_{\ge 0}^l$, we have
		\begin{align*}
			\sum_{\sigma \in \cP_l}\Ex{\reg_{v,\sigma(\vec{0}_l)}(T)} 
			\le 
			\sum_{\sigma \in \cP_l}
			\Ex{\reg_{v,\sigma(r)}(T)}.
		\end{align*}
	\end{claim}
	\begin{proof}
		This directly follows from our definition of TRP.
		More formally,
		\begin{align*}
			\sum_{\sigma \in \cP_l}\Ex{\reg_{v,\sigma(\vec{0}_l)}(T)} 
			\tag{def. of RP-Regtret}
			&=
			\frac{\rpreg(\fA,T;\cO)}{|\cP_l|}
			\\
			&\le
			\frac{\rpreg(\fA,T;\cS) }{|\cP_l|}
			\tag{since $\fA$ is TRP}
			\\
			&=
			\sum_{\sigma \in \cP_l}
			\Ex{\reg_{v,\sigma(r)}(T)}.
			\tag{def. of RP-Regret}
		\end{align*}
		It completes the proof.
	\end{proof}
	By the claim, we can further expand from \eqref{ineq:05131256} as follows.
	\begin{align*}
		u(\cS)
		&\le
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 < v_1}\ldots \int_{\mu_l = v_l< v_{l-1}} 
		\sum_{\sigma \in \cP_l}\Ex{v_1T - \reg_{v,\sigma(\vec{0}_l)}(T) \ |\ \bigtimes_{a \in [l]}(v_a: r_a)}g(v)dv,	
	\end{align*}

	

	Since $\reg_{v, \sigma(\vec{0}_l)}$ is equivalent to the regret of the truthful strategy $\cO$ given the ex-post realization $v$, we obtain
	\begin{align*}
		u(\cS)
		&\le
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 < v_1}\ldots \int_{\mu_l = v_l< v_{l-1}} 
		\sum_{\sigma \in \cP_l}\Ex{v_1T - \reg_{\cI}(T) \ |\ \bigtimes_{a \in [l]}(v_a: r_a)}g(v)dv
		\\
		&=
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 }\ldots \int_{\mu_l = v_l} 
		\Ex{U(\cO)\ |\ \bigtimes_{a \in [l]}(v_a: r_a)}g(v)dv
		\\
		&=
%		\int_{\mu_1 = v_1}\ldots \int_{\mu_l = v_l} \Ex{U(\cO)\ |\ v_1,\ldots, v_l}g(v)dv		
%		=
		u(\set{O}),
	\end{align*}
	and thus the truthful registration $\set{O}$ is a dominant strategy.
\end{proof}

Furthermore, we observe that TRP is indeed a necessary condition for an algorithm to be replication-proof in the single-agent setting.
\begin{theorem}
	If an algorithm is not truthful under random permutation, then it is not replication-proof.
\end{theorem}
\begin{proof}
	Consider a single-agent setting.
	Since the algorithm $\fA$ does not satisfy TRP, there exists a problem instance with original arms $\cO$ and the agent's strategy $\cS$, time horizon $T$ such that 
	\begin{align*}
		\rpreg(\fA,T;\cO) 
		\le 	
		\rpreg(\fA,T;\cS).
	\end{align*}
	As observed in the proof of Theorem~\ref{thm:single_pf_rp}, the expected utility of the strategies $\cO$ and $\cS$ can be compared using $\rpreg(\fA,T;\cO)$ and $\rpreg(\fA,T;\cS)$, so the result follows.
    \sscomment{double check}
\end{proof}

\begin{discussion}
	One may wonder if PI can be violated for any replication-proof algorithm.
	This is indeed true.
	For example, one can consider a black-box algorithm that first randomly selects an agent, and runs a bandit algorithm within the agent.
	Further consider a very artificial agent-selection process which does not uniform randomly select the agents, but asymmetrically favors some agent indices with higher probability.
	Such an algorithm indeed is not permutation invariant, since the permutation of agent index would lead to a different outcome given the bandit instance.
	In perspective of the agents, however, each agent only needs to care about the secondary arm selection phase after the agent selection since they cannot change the probability to be selected in the agent selection phase.
	Using these observations, one can observe that such an algorithm is indeed replication-proof, but not permutation invariant.
	One may refine the notion of PI to be restricted within each agent, but we do not argue any more details as it is beyond of our interest and main takeaway.
\end{discussion}



\paragraph{Constructing TRP algorithm}
We now present an algorithm that satisfies TRP.
In what follows, we mainly prove that exploration-then-commit (ETC) satisfies TRP once equipped with a proper parameter.
Its pseudocode is presented in Algorithm~\ref{alg:ETC} for completeness.
We suppose that the algorithm breaks tie in a uniform random manner.\footnote{As can be seen in the proof, any tie-breaking rule does not hurt our analysis.}
ETC essentially decouples the exploration phase and the exploitation phase very explicitly, and thus brings a significant advantage in comparing its expected regret under several problem instances.


\begin{algorithm}
\textbf{Input}: exploration length $m$, tie-breaking rule\\
Play each arm for $m$ rounds.\\
Play the arm with the highest empirical mean for all remaining rounds
\caption{\textsc{ETC}}\label{alg:ETC}
\end{algorithm}

For analytical tractability, we pose some \emph{assumptions} on the support of the prior distributions.
Namely, for any agent $i$, $F_i$ has a discrete support over $[0,1]$ for $i \in \cN$.
Further, we define $\Delta_i$ be the minimum gap between any two possible outcomes from $F_i$, and let $\Delta = \min_{i \in \cN}\Delta$.
Furthermore, the algorithm knows this gap $\Delta$.
\begin{discussion}
	We discuss how one can weaken these assumptions at the end of Section~\ref{sec:single}, possibly at the cost of polylogarithmic blowup in the regret rate or another assumptions.
	We also remark that such assumptions, especially that the algorithm knows the minimum gap, often appear in the literature, \cf \cite{auer2002finite,audibert2010best,garivier2016explore}.
	Moreover, in practice, we believe that it is quite plausible in real-world applications. 
	For example in content platforms, suppose that a content creator comes up with several contents and is about to register. 
	Assume the reward of each content is just the number of views. 
	Typically, the content creator does not exactly know the reward of each content but has historical data on its previous contents. 
	The historical data can be used to structure a prior distribution of the quality of his/her contents. 
	In this case, since usually each content creator has a very small number of original contents compared to the recommendation algorithm's time scale (one for each traffic), this prior distribution may consist of a fairly limited number of samples, thereby having discrete support with a few number of points.
\end{discussion}


Then, our main result in the single-agent setting can be written as follows.
\begin{theorem}\label{thm:single_rp}
	ETC with exploration length $m \ge \frac{2}{\Delta^2} l \ln (2T)$ is TRP in the single-agent setting.
        Further, it has regret of
        \begin{align*}
            \sum_{a\in [l]} \Big( \frac{2\delta_a l\ln{(2T)}}{\Delta^2} + 1 \Big),
        \end{align*}
        where $l$ denotes the number of arms and $\delta_a$ denotes the gap of the mean rewards between optimal arm and arm $a$, of the single agent.
\end{theorem}
The proof essentially follows from the standard regret analysis of ETC along with carefully chosen $m$.
By setting $m$ sufficiently large, we can essentially decrease the probability that a suboptimal arm is chosen to be $o(1/T)$.
This will guarantee that the expected number of rounds the suboptimal arm is chosen is smaller than $1$, whereas any replicating strategy incurs a simple regret lower bound larger than this quantity.
Together with Theorem~\ref{thm:single_pf_rp} and the fact that ETC is permutation invariant (which is straightforward to verify), it follows that ETC is replication-proof in the single-agent setting.

\begin{proof}[Proof of Theorem~\ref{thm:single_rp}]
	Recall that we will deal with a single agent.
	Consider a bandit instance $\cI$ in which there exists $l$ arms with parameters $v_1 \ge v_2 \ge \ldots \ge v_l$, and the time horizon is $T$.
	Let $n_a(t)$ be the number of rounds that arm $a$ is pulled and $\muhat_a(t)$ be the empirical average reward, at the end of round $t$, and define $\delta_a = v_1 - v_a$ for $a \in [l]$.
	
	Our proof mainly relies on the following lemma.
	\begin{lemma}\label{th:ETC_main_th}
		Suppose that the realization of the arms's mean rewards is given, and let $a^*$ be the arm the largest mean reward.
		If $m \ge \frac{2 l}{\Delta^2} \ln{2T}$, then for a sub-optimal arm we have:
		\begin{align*}
			\Ex{n_a(T)} \leq m+1.
		\end{align*}
		Especially for $m = \frac{2}{\Delta^2} l \ln (2T)$, the expected regret is upper bounded by:
		\begin{align*}
    		\reg(T) 
    		\leq 
    		\sum_{a\in [l]} (m+1) \Delta_i 
    		\leq 
    		\sum_{a\in [l]} \Big( \frac{2\delta_a l\ln{(2T)}}{\Delta^2} + 1 \Big).
		\end{align*}	
	\end{lemma}
	\begin{proof}[Proof of the lemma]
		Due to the structural nature of ETC, for any sub-optimal arm $a$ we have
		\begin{align*}
    		\Ex{n_a(T)} \leq m + (T-mk) \Pr{\hat{\mu}_a(m) \ge \hat{\mu}_{a^*}(m)} 
    	\end{align*}
    	Now we focus on upper bounding $\Pr{\hat{\mu}_a(m) \ge \hat{\mu}_{a^*}(m)}$.
    	\begin{claim}\label{cl:concen}
    		For any arm $a \neq a^*$, the following holds.
    		\begin{align*}
    			\Pr{\hat{\mu}_a(m) \ge \hat{\mu}_{a^*}(m)} 
    			\le 
    			2\exp(-\frac{\delta_a^2 m}{2})
    		\end{align*}
    	\end{claim}
    	\begin{proof}[Proof of the claim]
    		We can expand the inequality as follows.
    		\begin{align*}
    			\Pr{\hat{\mu}_a(m) \ge \hat{\mu}_{a^*}(m)} &= \Pr{(\hat{\mu}_a(m) -v_a) + (v_{a^*} - \hat{\mu}_{a^*}(m)) \ge \delta_a}
    			\\ 
    	    	&\leq 
    	    	\Pr{(\hat{\mu}_a(m) -v_a) \ge \frac{\delta_a}{2}} + \Pr{(v_{a^*} - \hat{\mu}_{a^*}(m)) \ge \frac{\delta_a}{2}}
    	    	\\ 
    	    	&\leq 
    	    	2 \exp(- \frac{\delta_a^2}{4} \frac{1}{2} \frac{1}{\frac{1}{4m}}) \tag{Hoeffding's inequality} \\
    	    	& \leq 2\exp(- \frac{\delta_a^2 m}{2}),
			\end{align*}
			which finishes the proof.
			Note that we use the following well-known type of Hoeffding's inequality.
			\begin{theorem}
				Let $X_1,\ldots, X_n$ be independent random variables such that $a_i \le X_i \le b_i$ almost surely.
				Define $S_n = X_1 + \ldots X_n$.
				For any $t >0$,
				\begin{align*}
					\Pr{|S_n - \Ex{S_n}| \ge t}
					\le 
					2\exp\parans{-\frac{2t^2}{\sum_{i=1}^n (b_i - a_i)^2}}.	
				\end{align*}
			\end{theorem}
    	\end{proof}
		Using the claim above, we can further expand,
		\begin{align*}
       		\Ex{n_a(T)} 
       		&\leq
       		m + (T-mk) \Pr{\hat{\mu}_a(m) \ge \hat{\mu}_{a^*}(m)} 
       		\\
       		&\leq 
       		m + 2T\exp(- \frac{\delta_a^2 m}{2})
       		\tag{Claim~\ref{cl:concen} $\&$ $T-mk \le T$}
      		\\
       		&\leq
       		m + 2T  \exp(- \Big(\frac{\delta_a}{\Delta}\Big)^2 \ln{2T})
       		\tag{$m\ge 2/\Delta^2 \ln(2T)$}
       		\\
       		&\leq 
       		m+ 2T  \exp(- \ln{2T})
       		\tag{Since $\frac{\delta_a}{\Delta} \ge 1$} 
       		\\
       		&=
       		m + 1.
		\end{align*}
		This proves the upper bound on $\Ex{n_a(T)}$.
		To obtain the upper bound on the regret, one can use the following well-known regret decomposition lemma.
		\begin{lemma}[Regret decomposition]
			The regret can be writtten as
			$\reg(T) = \sum_{a \in [l]} \Ex{n_i(T)\delta_a}$.
		\end{lemma}

		From this, the regret bound easily follows as below
		\begin{align*}
    		\reg(T)
    		&\leq 
    		\sum_{a\in [l]} (m+1) \delta_a 
    		\\
    		&= 
    		\sum_{a\in [l]} (\frac{2l}{\Delta^2} \ln{2T}+1) \delta_a 
    		\\ 
    		&\leq 
    		\sum_{a\in [l]} ( \frac{2l\delta_a}{\Delta^2} \ln{2T} +1).
    		\tag{Since $\Delta_a\leq 1$} 
		\end{align*}
		This completes the proof.
	\end{proof}
	
	Now, consider a strategy $\cS \neq \cO$ of which the replication vector is $r = (r_1,\ldots, r_l)$ (as defined in the proof of Theorem~\ref{thm:single_pf_rp}), and at least one coordinate being strictly positive.
	Consider a realization $v \in \R_{\ge 0}^l$, and a permutation $\sigma(v)$.
	Let $\cI_{\sigma}$ be a bandit instance in which the arms are permuted by $\sigma$ from $\cI$.

	
	
	Given $v_1 \ge \ldots \ge v_l$, let $\cI_{\sigma,v}$ be the instance in which $i$-th arm has mean reward $v_{\sigma(a)}$ for $a \in [l]$, \ie $\cI_{\sigma, v} = \bigtimes_{a \in [l]}(v_{\sigma(a)}: r_a)$.
	Denote the expected regret under $\cI_{\sigma,v}$ by $\reg_{I_{\sigma,v}}$.
	
	From the regret decomposition lemma, we have
	\begin{align*}
		\reg_{I_{\sigma,v}}(T) = \sum_{a\in [l]}	\Ex{n_{\sigma(a),t}}\delta_{\sigma(a)} \parans{r_a + 1}.
	\end{align*}
	Due to the initial exploration phase of ETC, obviously $\Ex{n_{\sigma(a),t}} \ge m$.
	Hence we obtain
	\begin{align*}
		\reg_{I_{\sigma,v}}(T) 
		&\ge
		\sum_{a\in [l]} m \cdot \delta_{\sigma(a)}(r_a + 1).
	\end{align*}
%	\note{Notation for $reg$ suddenly changes}
	Now, RHS in the random permutation regret \eqref{eq:epf} can be written as follows.
	\begin{align}
		\sum_{\sigma \in \cP_l}\reg_{\cI_{\sigma,v}}(T)/|\cP_l|
		&\geq
		\frac{\sum_{\sigma \in \cP_l}\sum_{a\in [l]} m \cdot \delta_{\sigma(a)}(r_a + 1)}{l!}
		\nonumber
		\\
		&\geq
		\frac{\sum_{a\in [l]} \sum_{\sigma \in \cP_l} m \cdot \delta_{\sigma(a)}(r_a + 1)}{l!}
		\nonumber
		\tag{Change order of summation}
		\\
		&=
		\frac{\sum_{a\in [l]} \sum_{\sigma \in \cP_l} m \cdot \delta_{a}(r_{\sigma(a)} + 1)}{l!}
		\nonumber
		\tag{Sum over $\sigma$ equals that over $\sigma^{-1}$}
		\\
		&=
		\frac{\sum_{a\in [l]} m \cdot \delta_a(l-1)!\sum_{j=1}^l (r_{j}+1)}{l!}
		\nonumber
		\tag{fix $\sigma(a) = j$ and sum over $\sigma \in \cP_l$	}
		\\
		&=
		\frac{\sum_{a\in [l]} m \cdot \delta_a (\norm{r}_1+l)}{l}\label{ineq:05090221}
	\end{align}
	Due to our construction of $r$, we have $\norm{r}_1 \ge 1$, and finally we obtain
	\begin{align}
		\reg_\cI(T) 
		&\le
		\sum_{a\in [l]} (m+1) \delta_a 
		\label{ineq:05090222}
		\\
		&\le
		\sum_{a\in [l]} m\delta_a \frac{l+1}{l},
		\nonumber
		\tag{$m = \frac{2l}{\Delta^2}\ln 2T \ge l$}
		\\
		&\le
		\frac{\sum_{a\in [l]} m \cdot \delta_a\sum_{j=1}^l (r_{j}+1)}{l}
		\tag{$\norm{r}_1 \ge 1$}
		\nonumber
		\\
		&\le
		\sum_{\sigma \in \cP_l}\reg_{\cI_{\sigma,v}}(T)/|\cP_l|,
		\nonumber
	\end{align}
	where the last inequality follows from the inequality~\eqref{ineq:05090221}.
	Note further that $\reg_\cI(T)$ is $\rpreg$ of truthful strategy $\cO$ given the realization $v$, and RHS denotes that of a strategy $\cS$ whose replication vector is $r$.
	Thus,
	\begin{align*}
		\rpreg(\fA, T, \cO) \le \rpreg(\fA, T, \cS),	
	\end{align*}
	for $\fA$ being ETC, and it concludes that ETC is TRP.
\end{proof}


%\begin{discussion}
Note that the proof of Theorem~\ref{thm:single_rp} heavily relies on the fact that the algorithm can observe $\Delta$ in advance and set the exploration length correspondingly.
Thus, despite we aim to obtain a \emph{prior-independent} algorithm that does not require any knowledge in the agent's prior distributions, it is not \emph{truly} prior-independent in an algorithmic manner since it requires some problem parameters to operate the algorithm.
We discuss several ways to refine such restrictions, thereby suggesting a road for truly prior-independent algorithm.
First, assume $\Delta$ is constant but not known to the algorithm.
In this case, one may replace $\Delta$ in the algorithm to be some increasing functions $f(T) = \omega(1)$, and it is straightforward to verify that Theorem~\ref{thm:single_rp} still holds, but in an asymptotical regime.
Similarly, one can effectively wipe out the dependency on the total number of original arms $l$ by assuming that $l = O(1)$ and replacing it with some increasing functions.
Furthermore, the knowledge on $T$ can be wiped out by the standard doubling trick, \cf see Chapter 1 in ~\cite{slivkins2019introduction}, without sacrificing any other guarantees on the truthfulness.
In short, the guarantees can remain the same even without knowing the problem parameters, with sacrifice on the analysis being held only in an asymptotic manner.
Remark that all these refinements only introduce polylogarithmic blowup in the regret upper bound.
%We do not provide more formal discussions as this goes beyond our main takeaway.
%\end{discussion}
The following theorem spells out these arguments, whose formal proof is deferred to Appendix~\ref{apd:thm:single-refine1}.
\begin{theorem}\label{thm:single-refine1}
	Assume $l = O(1),\Delta = \Omega(1)$.
	Then, there is a prior-independent algorithm, which does not require any information on problem parameters, satisfying TRP and PI in the single-agent setting for sufficiently large $T$.
\end{theorem}

\begin{discussion}
	One may ask if we can fully remove the assumption on $\Delta$ without sacrificing regret at all.
	This, in fact, is impossible using a variant of ETC as discussed by~\cite{garivier2016explore}.
	Instead, \cite{garivier2016explore} propose a variant of ETC via considering a best arm identification algorithm in the exploration phase, in the two-armed bandit setting.
	This approach indeed wipes out the dependency of $\Delta$ in the algorithm description, however, such successive elimination style of algorithms, that shrinks the set of active arms gradually based on some stopping rules, significantly complicates the analysis of truthfulness.
	This is because we need to account for every probability that a single arm is deactivated at certain rounds, and this event is highly correlated with the reward tape of the other arms as well as its own.
	The non-adaptive structure of ETC largely simplifies such an analysis as we observe, and it remains as major open problems whether any adaptively exploring algorithm can be made replication-proof in the single-agent setting.
\end{discussion}

%Now that we obtain truly prior-independent algorithm, this is still not satisfactory since the assumption that all the prior distributions have discrete support and $\Delta = O(1)$ may look restrictive.
%Indeed, the assumption of $\Delta$ being constant, however, is more crucial.
%For example, if $\Delta$ can be arbitrarily small, \eg $\Delta = 1/\sqrt{T}$, then our theorem statement specifies that exploration length needs to be set $O(T \ln T)$, which obviously yields a linear regret.
%Indeed, our proof essentially relies on the inequality~\eqref{ineq:05090222},\footnote{This in fact can be loosened by $\reg(\cI) \le \sum_{a \in [l]} (m+m/l)\delta_a$, but it does not change our arguments thereafter.} and this cannot be made true if $\Delta$ is not sufficiently large.
%For example, if $\Delta$ is very small, \eg $O(1/\sqrt{T})$, the quantity $n_a(T)$ in Lemma~\ref{th:ETC_main_th} cannot be upper bounded by $m+c$ for some positive constant $c$.
%
%Instead, one can tackle this assumption as what we describe follows so that our argument carries over even to prior distributions with continuous support.
%Take a sufficiently small positive real number $d$.
%For any two different arms $a \neq a' \in \cO$, define an event $\clean_{a,a'}$ such that the realized quantities $\mu_{a}$ and $\mu_{a'}$ satisfies $|\mu_{a} - \mu_{a'}| \ge d$.
%Further define $\clean = \cap_{a\neq a' \in \cO} \clean_{a,a'}$, and one can compute the deviation probability such that $\clean$ does not occur.
%In upper bounding the number of pulls for suboptimal arms, we can decompose $\Ex{n_a(T)}$ as follows.
%\begin{align*}
%	\Ex{n_a(T)} = \CEx{n_a(T)}{\clean}\Pr{\clean} + \CEx{n_a(T)}{\clean^c}\Pr{\clean^c}.
%\end{align*}
%The first term can be analogously upper bounded to the proof of Theorem~\ref{thm:single_rp}.
%For the latter term, note that $\Pr{\clean^c}$ can equivalently presented as $\Pr{\min_{a \neq a' \in \cO} |\mu_a - \mu_{a'}| < d}$.
%Therefore, if one can essentially compute $\Ex{\min_{a \neq a' \in \cO} |\mu_a - \mu_{a'}|}$, one may upper bound the latter term using some concentration inequalities using a proper amount of deviation.
%Hence, we may only need some reasonable assumptions on  the quantity $\Ex{\min_{a \neq a' \in \cO} |\mu_a - \mu_{a'}|}$.
%Formalizing this argument, we obtain the following theorem.
%\begin{theorem}\label{thm:single-refine2}
%	Let $Z:= \min_{a \neq a' \in \cO} |\mu_a - \mu_{a'}|$.
%\end{theorem}
%
%Remark that
%\begin{theorem}\label{thm:single-refine2}
%	Suppose that $F_i(x) = x$ for $x \in [0,1]$, \ie all the prior distributions	follow $U[0,1]$.
%	Then, there exists an algorithm satisfying TRP and PI in the single-agent setting.
%\end{theorem}

%\note{discuss that this can be further generalized}
%
%\note{discuss why it is hard to fully remove the assumption on $\Delta$}
%
%\note{See also Double Explore-then-Commit: Asymptotic Optimality and Beyond}
%
%\note{See also Garivier, and see if we can remove this assumption. This also argued that if gap is unknown, fixed-interval ETC cannot have logarithmic regret.}

% and for the latter term, one can essentially use some anti-concentration arguments to obtain a upper bound.
%More detailedly, we need to compute a deviation probability
%
%This anti-concentration argument, however, entails a computation of
%
%We provide a formal 



%Next, we tackle the assumption that $\Delta$ is constant, which further requires that all the prior distributions have discrete support.



% \begin{corollary}
% 	ETC is replication-proof in the single agent setting.
% \end{corollary}


%\paragraph{Note:} The algorithm assumes knowledge of the minimum gap between the arms $\min_{i \in [k]} \Delta_i$. 

%\paragraph{Note:} Any algorithm which assumes knowledge of the minimum gap must also imply that the prior over the means is over a discrete support. For example, the prior has non-zero probability only over the set  over $\{0,0.2,0.4,0.6,0.8,1.0\} \subset [0,1]$. If that is not the case and we deal with continuous distributions instead, then it is possible in general to have two means such that the gap between them is arbitrarily small. 


==> temp/icml-ETC.tex <==
\section{Attempt - Stochastic Permutation Free}

The above theorem characterizes the sufficient condition for an algorithm to be replication-proof for any number of agents.
These characterizations allow us to deeply understand which types of properties suffice to make an algorithm replication-proof, however, it is often not easy to see that
Indeed, as we will see in the following section, it is tricky to check whether an algorithm satisfy SPF or not, since it requires us to compare all the tail probabilities of multiple bandit instances with different parameters.
Thus, in what follows, we directly prove that the combination of ETC and ETC in $\hbb$ admits the replication-proofness.

\begin{theorem}
	Let $\alg_1$ be ETC with arbitrary exploration parameter $M \ge m(\sum_{i=1}^l l_i)$, and $\alg_2$ be ETC with exploration parameter $m = \frac{2}{\Delta^2} (\max_il_i) \ln (2T)$.
	Then, $\hbb$ with $\alg_1$ and $\alg_2$ is replication-proof for any number of agents.
\end{theorem}
\begin{proof}
	We focus our attention to agent $i$.
	Index agent $i$'s arms by $1,2,\ldots, l$.
	We borrow the notations in the proof of Theorem~\ref{thm:spf_rp}.
	As per equation~\eqref{eq:04271244}, the conditional expected regret given permutation $\sigma$ and the realization $v$ can be written as follows.
	\begin{align}
		\sum_{\sigma \in S_l} 
		\CEx{U_i(\cS)}{\sigma, v}
		&=
		\parans{
		\sum_{\sigma \in S_l}
		\Ex{\Gamma_i^{\cS}(M,v)}
		}
		+
		\Ex{\Gamma_i^{\cS}(T-Mn,v)}
		\int_{0}^1
		p_i^{\cS}(y,v)
		\parans{
		\sum_{\sigma \in S_l}
		q_i^{\cS}(y,\sigma(v))
		}dy.\label{eq:05082043}
	\end{align}
	Note that it suffices to prove that $\sum_{\sigma \in S_l} 
		\CEx{U_i(\cO)}{\sigma, v} \ge \sum_{\sigma \in S_l} 
		\CEx{U_i(\cS)}{\sigma, v}$ for any strategy $\cS$.
	
	Let $\cS$ be agent $i$'s strategy with replication vector $r = (r_1,r_2,\ldots, r_l)$, with at least one coordinate being strictly positive.
	Without loss of generality, suppose $r_1 \ge r_2 \ge \ldots \ge r_l$, then we have $r_1 \ge 1$.
	This indeed brings no difference since the expected payoff is marginalized over all the possible permutations, as we see thus far.
	Let $\Omega_1$ be a set of permutation $\sigma \in S_l$ such that arm $\sigma(1) = 1$, \ie the best arm is replicated the most times, and define $\Omega_2 = S_l \setminus \Omega_1$.
	We handle case $\omega \in \Omega_1$ and $\omega \in \Omega_2$ separately.
	
	With the truthful strategy $\cO$, the last term $q_i^{\cO}(y,\sigma(v))$ in equation~\eqref{eq:05082043} can be written as follow.
	\begin{align*}
		q_i^{\cO}(y,\sigma(v))
		&=
		\Pr{\sum_{i=1}^l \Gamma_i^\cO(M,\sigma(v))}
	\end{align*}

\end{proof}


\section{ETC}
\paragraph{Note:} The algorithm assumes knowledge of the minimum gap between the arms $\min_{i \in [k]} \Delta_i$. 

\paragraph{Note:} Any algorithm which assumes knowledge of the minimum gap must also imply that the prior over the means is over a discrete support. For example, the prior has non-zero probability only over the set  over $\{0,0.2,0.4,0.6,0.8,1.0\} \subset [0,1]$. If that is not the case and we deal with continuous distributions instead, then it is possible in general to have two means such that the gap between them is arbitrarily small. 

Let $r$ be a realization of the means of the $l_i$ arms that have been samples from $D_i$. For this realization $r$, let $\Delta_r$ be the minimum gap between an optimal arm and a sub-optimal arm. Then define $\Delta=\min_{r \sim D_i} \Delta_r$. In words $\Delta$ is the minimum possible gap over all realizations. In the above example where the support of the distribution is $\{0,0.2,0.4,0.6,0.8,1.0\}$ then clearly $\Delta=0.2$. 


For now, we just do regret analysis for the following ETC algorithm:
\begin{algorithm}
Play each arm once for $m$ rounds.\\
Play the arm with the highest empirical mean for all remaining rounds. 
\caption{\textsc{ETC}}\label{alg:ETC}
\end{algorithm}

Let $n_i(T)$ be the total number of pulls for sub-optimal arm $i$, then we have the following theorem:
\begin{theorem}\label{th:ETC_main_th}
If $m=\frac{2}{\Delta^2} \ln{2T}$, then for a sub-optimal arm we have:
\begin{align}
\expect{n_i(T)} \leq m+1 = 1 + \frac{2}{\Delta^2} \ln{(2T)}
\end{align}
Further, the regret is upper bounded by:
\begin{align}
    R(T) \leq \sum_{i:\Delta_i>0} (m+1) \Delta_i \leq \sum_{i:\Delta_i>0} \Big( \frac{2 \ln{(2T)}}{\Delta^2} + 1 \Big)
\end{align}
\end{theorem}
\begin{proof}
For a sub-optimal arm $i$ we have: 
\begin{align*}
    \expect{n_i(T)} \leq m + (T-mk) \Pr{\hat{\mu}_i(m) \ge \hat{\mu}_{i^*}(m)} 
\end{align*}
Now we focus on upper bounding $\Pr{\hat{\mu}_i(m) \ge \hat{\mu}_{i^*}(m)}$: 
\begin{align}
    \Pr{\hat{\mu}_i(m) \ge \hat{\mu}_{i^*}(m)} &= \Pr{(\hat{\mu}_i(m) -\mu_i) + (\mu_{i^*} - \hat{\mu}_{i^*}(m)) \ge \Delta_i} \\ 
    & \leq \Pr{(\hat{\mu}_i(m) -\mu_i) \ge \frac{\Delta_i}{2}} + \Pr{(\mu_{i^*} - \hat{\mu}_{i^*}(m)) \ge \frac{\Delta_i}{2}} \\ 
    & \leq 2 \exp(- \frac{\Delta_i^2}{4} \frac{1}{2} \frac{1}{\frac{1}{4m}}) \ \ \ \ \  \text{(using sub-Gaussian tail concentration with $\sigma=\frac{1}{2}$ since rewards are in $[0,1]$)} \\
    & \leq 2\exp(- \frac{\Delta_i^2 m}{2})
\end{align}
Set $m=\frac{2}{\Delta^2} \ln{\frac{T}{c}}$ where $c$ is a constant to be determined. Now let us go back to upper bounding $\expect{n_i(T)}$: 
\begin{align}
       \expect{n_i(T)} & \leq m + (T-mk) \Pr{\hat{\mu}_i(m) \ge \hat{\mu}_{i^*}(m)} \\ 
       & \leq m + T (2)\exp(- \frac{\Delta_i^2 m}{2}) \\
       & \leq m + 2T  \exp(- \Big(\frac{\Delta_i}{\Delta}\Big)^2 \ln{\Big(\frac{T}{c}\Big)}) \\
       & \leq m+ 2T  \exp(- \ln{\Big(\frac{T}{c}\Big)}) \ \ \ \text{(since $\frac{\Delta_i}{\Delta} \ge 1$)} \\
       & = m + 2T \frac{c}{T} \\
       & = m + 1 \ \ \ \text{(by setting $c=\frac{1}{2}$)}
\end{align}
\note{Seyed: In the above we chose $c=\frac{1}{2}$, this was done out of convenience. }
\\ 
This proves the upper bound on $\expect{n_i(T)}$, now we prove the regret upper bound: 
\begin{align*}
    R(T) & \leq \sum_{i:\Delta_i>0} (m+1) \Delta_i \\ 
    & = \sum_{i:\Delta_i>0} (\frac{2}{\Delta^2} \ln{2T}+1) \Delta_i \\ 
    & \leq \sum_{i:\Delta_i>0} ( \frac{2\Delta_i}{\Delta^2} \ln{2T} + \Delta_i) \\ 
    & \leq \sum_{i:\Delta_i>0} ( \frac{2}{\Delta^2} \ln{2T} +1) \ \ \ \text{(since the rewards are in $[0,1]$, we have $\Delta_i\leq 1$)} 
\end{align*}
\end{proof} 


\subsection{The original conjecture using ETC}
Consider the following instances where $\mu_1 >\mu_2$ and the distributions can be random (not deterministic): 
\begin{enumerate}
    \item A: run ETC with instance $(\mu_1, \mu_2)$
    \item B: run ETC with instance $(\mu_1, \mu_2, \mu_1)$
    \item C: run ETC with instance $(\mu_1, \mu_2, \mu_2)$
\end{enumerate}

What we want to prove as stronger version of conjecture:
For any $x \in [0,T]$ ,
\begin{align*}
    \Pr{R_A < x} \le \frac{\Pr{R_B < x} + \Pr{R_C < x}}{2}
\end{align*}

\begin{theorem}
    Using the above ETC algorithm then we have $R_A \leq \frac{R_B+R_C}{2}$ if the horizon $T\ge 2$. 
    \note{Seyed: the horizon must always have at least two rounds so this is not restrictive at all.}
\end{theorem}
\begin{proof}
Using Theorem \ref{th:ETC_main_th} we clearly have: 
\begin{align}
    R_A \leq (m+1) \Delta_2 = m\Delta_2 + \Delta_2 
\end{align}
Since the algorithm always does $m$ many exploration rounds per arm we immediately have:
\begin{align}
    & R_B \ge m \Delta_2  \\
    & R_C \ge 2 m \Delta_2 
\end{align}
\end{proof}
This implies that: 
\begin{align}
    \frac{R_B+R_C}{2} \ge \frac{3}{2} m \Delta_2 = m\Delta_2 + \frac{1}{2} m\Delta_2 \ge  m\Delta_2 + \Delta_2  \ge R_A
\end{align}
where $m\Delta_2 + \frac{1}{2} m\Delta_2 \ge  m\Delta_2 + \Delta_2$ holds if $m\ge 2$. Since $m=2 \ln(2T)$ and we have at least two rounds $T\ge 2$, then $m\ge 2$. 

\paragraph{Note:} What made the above result easy to obtain is that ETC has a deterministic sub-process where each arm is always pulled $m$ times during exploration. Further, the above version of ETC has $m$ without any dependence on the number of existing arms $k$. 


==> temp/icml-abstract.tex <==
%Revised version
We study a problem of designing replication-proof bandit mechanisms when agents strategically register or replicate their own arms to maximize their payoff. 
We consider Bayesian agents who are unaware of ex-post realization of their own arms' mean rewards, which is the first to study Bayesian extension of~\cite{shin2022multi}. 
This extension presents significant challenges in analyzing equilibrium, in contrast to the fully-informed setting by~\cite{shin2022multi} under which the problem simply reduces to a case where each agent only has a single arm.
With Bayesian agents, even in a single-agent setting, analyzing the replication-proofness of an algorithm becomes complicated.
Remarkably, we first show that the algorithm proposed by~\cite{shin2022multi}, defined H-UCB, is no longer replication-proof for any exploration parameters.
Then, we provide sufficient and necessary conditions for an algorithm to be replication-proof in the single-agent setting.
These results centers around several analytical results in comparing the expected regret of multiple bandit instances, which might be of independent interest. 
We further prove that exploration-then-commit (ETC) algorithm satisfies these properties, whereas UCB does not, which in fact leads to the failure of being replication-proof.
We expand this result to multi-agent setting, and provide a replication-proof algorithm for any problem instance.
The proof mainly relies on the single-agent result, as well as some structural properties of ETC and the novel introduction of a restarting round, which largely simplifies the analysis while maintaining the regret unchanged (up to polylogarithmic factor).
We finalize our result by proving its sublinear regret upper bound, which matches that of H-UCB.


%%%% Seyed Edits 
%We study the problem of designing replication-proof bandit mechanisms when agents strategically register, or even replicate, their own arms to maximize payoff.
%We consider Bayesian agents who is oblivious to the ex-post realization of their own arms, which is the first to study Bayesian extension of \cite{shin2022multi}.
%%This extension
%%Compared to the fully informed agent of \cite{shin2022multi}, the Bayesian agent cannot cherrypick its own best arm, but instead computes the expected rewards over the realization of rewards, and plays a strategy that maximizes ex-ante payoff \note{Seyed - previous sentence could be improved, maybe keep it high-level}.
%This extension introduces significant challenges in analyzing replication-proof algorithms, compared to the single-agent setting under which the problem simply reduces to the case where each agent only has a single arm.
%% \note{Seyed- change to something like even the single agent case in the Bayesian setting is not trivial as the problem cannot be reduced to to the case where each agent only has a single arm}
%Notably, analyzing the replication-proofness of an algorithm is not straightforward even in a single-agent setting.
%We first show that, surprisingly, H-UCB proposed by \cite{shin2022multi} is no longer replication-proof.
%On the positive side, we first provide sufficient conditions under which an algorithm is replication-proof for a single-agent setting, and further prove that exploration-then-commit (ETC) satisfies these properties.
%At the heart of this analysis, we provide several analytical results in comparing the expected regret of multiple bandit instances, which might be of independent interest.
%For the multi-agent setting, we introduce a variant of H-UCB, named \textsc{Hierarchy with Restart}, and prove its replication-proofness.
%Our proof is based on the algebraic properties of ETC as well as the introduction of restarting round which largely simplifies the analysis by removing the correlation between the rounds.
%
%For the multi-agent setting, we present a slightly stronger condition that makes it sufficient for any algorithm to be replication-proof, once it runs as a sub-module of a two-stage hierarchical algorithms with first-stage being ETC. \note{Seyed - previous sentence: I think that part (b) would effect thi sentence. I think it might be best to remove it.}
%We further show that such a hierarchical algorithm equipped with ETC and ETC essentially satisfies replication-proof, while maintaining sublinear regret. \note{Seyed - previous sentence: (1) I think you should give an idea of what hierarchical means. Say something like a Bandit alg is applied over the arms of each aget and another over the agents with the rewards of all of their pulled arms aggregated. (2) ``ETC and ETC'': I think it's not clear, maybe something like both levels of the heirachcal algorithm use ETC.}

%%%%% Original abstract 
% We study a problem of designing replication-proof bandit mechanism when agents strategically register, or even replicate, their own arms to maximize payoff, where each agent is oblivious the ex-post realization of its own arms' parameters.
% Compared to the fully informed agent of \cite{shin2022multi}, the Bayesian agent cannot cherrypick its own best arm, but instead computes the expected rewards over the realization of rewards, and plays a strategy that maximizes ex-ante payoff.
% This introduces significant challenges in analyzing replication-proof algorithm, compared to the single-agent setting under which the problem simply reduces to the case where each agent only has a single arm.
% Notably, analyzing a replication-proofness of an algorithm is not straightforward even in a single-agent setting.
% We first show that, surprisingly, H-UCB (and RH-UCB) proposed by \cite{shin2022multi} is no more replication-proof, due to UCB's deterministic and adaptive exploration, based on the observation that UCB is not replication-proof even in the single agent setting.
% On positive sides, we first provide sufficient conditions under which an algorithm is replication-proof for a single-agent setting, and further prove that exploration-then-commit (ETC) satisfies these properties.
% For the multi-agent setting, we present a slightly stronger condition that makes sufficient for an algorithm replication-proof, once it runs as a submodule of a two-stage hierarchical algorithms with first-stage being ETC.
% We further show that such a hierarchical algorithm equipped with ETC and ETC essentially satisfies replication-proof, while maintaining sublinear regret.
% At the heart of our analysis, we provide several analytical results in comparing the expected regret of multiple bandit instances, which might be of independent interest.





==> temp/icml-conclusion.tex <==
\section{Conclusion}
We study bandit mechanism design problem to disincentivize replication of arms, which is the first to study Bayesian extension of \cite{shin2022multi}.
Our extension brings significant challenges in analyzing equilibrium, even in the single-agent setting.
We first prove that H-UCB of \cite{shin2022multi} does not work.
We then characterize sufficient conditions for an algorithm to be replication-proof in the single-agent setting.
A special case of our analysis boils down to identify whether a bandit algorithm is robust against an adversary who replicates some arms uniformly-at-random given a bandit instance, which might be of independent interest.
Based on the single-agent result, we obtain the existence of replication-proof algorithm with sublinear regret, by introducing a restarting round and exploiting the structural property of exploration-then-commit algorithm.
We further provide a regret analysis of our replication-proof algorithm, which matches the regret of H-UCB.
Obtaining a lower bound of any replication-proof algorithm, improving the regret upper bound using more sophisticated algorithm possibly with adaptive exploration, and further investigating which algorithms satisfy truthfulness under random permutation remain as major open problems.


==> temp/icml-discussion.tex <==
\section{Discussions}
\subsection{algorithm}

\begin{algorithm} 
\SetAlgoLined
%$i \in \set{N}$, $\set{S} = \cup_{i \in \set{N}} \set{S}_i$\\

Initialize $R(i), N(i), r(a)$ and $n(a)$ at zero  
for all $i \in \set{N}$ and $a\in \cup_{i \in \set{N}} \set{S}_i$;

%Initialize $r(a) = n(a) = R(i)=N(i)=0$~$\forall a, i$;


 \For{$t=1,2,\ldots$}{
  \tcp{Phase 1 - agent selection}
  \eIf{Unexplored agent exists}{ 
    %\tcp{Agent initialization}
    Pick an unexplored $\hat{i}\in \{i \in \set{N}: N(i) = 0\} $; % an unexplored agent ;
  }{
    % $i^\star = \argmax_{i} \{R_i + \sqrt{2\ln t / N_i}\}$
    Pick $\hat{i} = \argmax_{i \in \set{N}} \left\{R(i) + \sqrt{\frac{2 \sqrt{t}}{N(i)}} \right\}$;
  }
  
  \tcp{Phase 2 - arm selection}
  \eIf{Unexplored arm exists in $\set{S}_{\hat{i}}$}{
    %\tcp{Arm initialization}
    Pick an unexplored $\hat{a} \in \{a \in \set{S}_{\hat{i}}: n(a) = 0\} $; % an unexplored agent
  }{
    % $a^\star = \argmax_{a \in \set{S}_{i^\star}} \{r(a) + \sqrt{2 \ln N_i / n(a)}\}$
    Pick $\hat{a} = \argmax_{a \in \set{S}_{\hat{i}}} 
    \left\{r(a) + \sqrt{\frac{2 \ln N(i)}{n(a)}} \right\}$;
  }
  
  Play $A_t = \hat{a}$ and receive reward $R_t$; \\
  Update statistics:
  $r(\hat{a}) \leftarrow \tfrac{r(\hat{a})n(\hat{a}) + R_t}{n(\hat{a})+1}; ~~
  R(\hat{i}) \leftarrow \tfrac{R(\hat{i})N(\hat{i}) + R_t}{N(\hat{i})+1};$
  
  $n(\hat{a}) \leftarrow n(\hat{a}) + 1; ~~ N(\hat{i}) \leftarrow N(\hat{i}) + 1;$
 }
 \caption{Hierarchical UCB (H-UCB) \label{alg:hucb}}
\end{algorithm}

The major bottleneck in analyzing incentive compatibility in Bayesian setting is that it is hard to show the following fact.
\begin{conjecture}
Consider Bernoulli arms.
\begin{enumerate}
    \item A: run UCB with instance $(0.1, 0.3)$
    \item B: run UCB with instance $(0.1, 0.3, 0.3)$
    \item C: run UCB with instance $(0.1, 0.1, 0.3)$
\end{enumerate}
Note that $0.1, 0.3$ can be replaced with any two different numbers.
Definitely in terms of regret, regret of $C > A > B$ (this can be easily proved using coupling technique of ~\cite{shin2022multi}).
Main question is, then, how can we prove that (average regret of B,C) is larger than (regret of A)?
I personally think that we should prove stochastic dominance of regret random variables, rather than comparison between expected regret, i.e., $R_B + R_C >= 2R_A$ where $>=$ is (first-order) stochastic dominance.
\end{conjecture}
This conjecture basically implies, although it needs to be generalized, that replicating one arm randomly does not give any incentive to the agent, in case of H-UCB in \cite{shin2022multi}.
To briefly see why, phase 2 is running UCB, and by conjecture, replicating arm only increases expected regret, however the agent should maximize the expected regret in phase 2 to be selected more in phase 1.

This was not happened in complete information setting, since complete information setting reduces to the single-arm-per-agent case which significantly simplifies the analysis of incentive compatibility.

\paragraph{ETC style algorithm}
Using exploration-then-commit (ETC) style of algorithm, we can directly compute the regret, as depicted by the failure probability in exploitation phase.
In this context, we've tried Algorithm~\ref{alg:agent_explore_comm} which we believed to be incentive compatible.

\begin{algorithm}
  \SetAlgoLined
  Parameter $N_0$; \\
  \For{$i=1,\ldots, K$}{
    Uniform randomly sort the arms of agent $i$; \\
  	Explore the arms total $N_0$ times in round-robin manner; \\
  } 
  Select empirically best arm and pull it for the remaining rounds
 \caption{Agentwise-Exploration-then-Commit}\label{alg:agent_explore_comm}
\end{algorithm}

However, suppose that there is an agent with only $0$ reward arm.
If this agent replicates as much as possible, so that during the entire exploration phase each replicated arm will be selected a single time, then it is hard to distinguish that this agent's arm is indeed bad.
This definitely gives incentive for this agent to replicate, which yields that this does not have DSIC.

\paragraph{hierarchical algorithm}
Next, we thought about hierarchical algorithm with phase 2 changed to ETC, as described by Algorithm~\ref{alg:hucb}.
For simplicity, I denote $0.1'$ the replicated arm of $0.1$.
In this case, we can at least (roughly) prove that  submitting $0.1,0.3,0.1',0.3'$ is worse than submitting $0.1,0.3$.
This is because in order to be selected more in phase 1, the agent should make the algorithm find arm with $0.3$ with higher probability.
Submitting more $0.1$ and $0.3$ only reduces this probability.
To see why, let the length of exploration phase be $4N$.
In the replicated case, call it an instance $X$, each $0.1,0.3,0.1',0.3'$ will be sampled $N$ times in the exploration phase.
In the truthful case, call it an instance $Y$, each $0.1,0.3$ will be sampled $2N$ times.
Suppose that the infinite tape of $0.1$ and infinite tape of $0.1'$ till round $t$ in problem $X$ is coupled to the infinite tape of $0.1$ till round $2t$ in problem $Y$ for any $t \in [T]$.
For example, at even round, $0.1$ in $Y$ is coupled with $0.1'$ in $X$, and at odd round, it is coupled with $0.1$ in $X$.
In such a coupling, joint probability measure over $N$ random variables of $0.1$ and $0.1'$ in problem $X$ exactly corresponds to probability measure over $2N$ random variables in problem $Y$, thus we can just compare the statistics in $X,Y$ by assuming that their random incidences are coupled in this manner.
Then, we can conclude, followed by some probability calculations, that the probability of false exploitation is higher for the replicated case.


Note however that in order for this argument to be held, the length of exploration phase should be some multiplies of the registered arm.
What even worse is that we cannot handle the case of single replication using these coupling techniques.
For example, if agent with two original arms replicate only one arm, there are two possible cases: when better arm is replicated and when worse arm is replicated. Hence, this strategy's payoff will be average of this one.
Indeed, the payoff exactly corresponds to the average regret of B,C in Conjecture 1.
Proving this conjecture seems not easy, so it will be interesting if one can prove this conjecture with some nice algorithms.

Secondly, we should derive a lower bound for any incentive-compatible algorithm.
Recall that Algorithm~\ref{alg:agent_explore_comm} does not work.
This gave us some general intuitions that some kinds of hierarchy is essential to make algorithm incentive-compatible.
Combined with the fact that Algorithm~\ref{alg:agent_explore_comm} has regret of $T^{2/3}$, we conjecture that any incentive-compatible algorithm suffers regret lower bound of $O(T^{3/4})$.


\paragraph{SPA style algorithm}
See~\cite{braverman2019multi}.
The analysis seems to again reduce to Conjecture 1.


% \subsection{lower bound}
% Known results: any non-adaptive exploration algorithm has regret lower bound of $T^{2/3}$.

% \todo{priority 2: Regret lower bound of any incentive-compatible algorithm is $T^{2/3}$.}

% \todo{conjecture: if the algorithm explores adaptively, then it has regret lower bound of $O(T^{3/4})$, then since non-adaptive exploration has lower bound of $O(T^{2/3})$, the proof will be done.}
% \suho{This does not work}




\begin{algorithm} 
\SetAlgoLined
%$i \in \set{N}$, $\set{S} = \cup_{i \in \set{N}} \set{S}_i$\\

Initialize $R(i), N(i), r(a)$ and $n(a)$ at zero  
for all $i \in \set{N}$ and $a\in \cup_{i \in \set{N}} \set{S}_i$;

%Initialize $r(a) = n(a) = R(i)=N(i)=0$~$\forall a, i$;


 \For{$t=1,2,\ldots$}{
  \tcp{Phase 1 - agent selection}
  
  \eIf{Unexplored agent exists}{ 
    %\tcp{Agent initialization}
    Pick an unexplored $\hat{i}\in \{i \in \set{N}: N(i) = 0\} $; % an unexplored agent ;
  }{
    % $i^\star = \argmax_{i} \{R_i + \sqrt{2\ln t / N_i}\}$
    Pick $\hat{i} = \argmax_{i \in \set{N}} \left\{R(i) + \sqrt{\frac{2 \sqrt{t}}{N(i)}} \right\}$;
  }
  
  \tcp{Phase 2 - arm selection}
  If $N(i) \le 1/2T^{1/3} \log(T)^{1/3}$, round-robin exploration of arms in $\set{S}_i$;\\
  Else, commit $\hat{a} = \argmax_{a \in \set{S}_{\hat{i}}} 
    \left\{r(a) \right\}$
  Play $A_t = \hat{a}$ and receive reward $R_t$; \\
  Update statistics:
  $r(\hat{a}) \leftarrow \tfrac{r(\hat{a})n(\hat{a}) + R_t}{n(\hat{a})+1}; ~~
  R(\hat{i}) \leftarrow \tfrac{R(\hat{i})N(\hat{i}) + R_t}{N(\hat{i})+1};$
  
  $n(\hat{a}) \leftarrow n(\hat{a}) + 1; ~~ N(\hat{i}) \leftarrow N(\hat{i}) + 1;$
 }
 \caption{Hierarchy(UCB, Exploration-then-Commit) \label{alg:hucb}}
\end{algorithm}




\section{Byproducts in some trials}
	\note{Below - attempt to show it with sth between EPF and SPF.}
	\begin{assumption}
		For any strategy $\cS$, we have $\Ex{\Gamma_i^{\cO}\Ind{\Gamma_i^{\cO} \le x}} \le \Ex{\Gamma_i^{\cS}\Ind{\Gamma_i^{\cS} \le x}}$ for any $x \in [0,1]$. 	
	\end{assumption}
	
	\begin{claim}
		Let $p= (p_i)_{i \in [l]}$, $q = (q_i)_{i \in [l]}$ and $q' = (q'_i)_{i \in [l]}$ be sequences of real values such that $p$ is monotone increasing, $q$ and $q'$ are monotone decreasing, and $q$ majorizes $q'$ in an inverse order, \ie $\sum_{i=1}^k q_{n-i+1} \ge \sum_{i=1}^k q'_{n-i+1}$ for any $k \in [n]$.
		Then, we have $\sum_{i \in [l]}p_iq_i \ge \sum_{i \in [l]}p_iq'_i$.
	\end{claim}
	\begin{proof}
		Some algebra
	\end{proof}
	
	By assumption we have
	\begin{align*}
		\sum_{y \le x}\sum_{\sigma \in S_l} q_i^{\cS'}(y,v)	
		\ge
		\sum_{y \le x}\sum_{\sigma \in S_l} q_i^{\cS'}(y,v),
	\end{align*}
	for any $x \in [0,1]$.
	Hence, by the claim we obtain
	\begin{align*}
		\sum_{y \in [0,1]}
		p_i^{\cO}(y,v)
		\parans{
		\sum_{\sigma \in S_l}
		q_i^{\cO}(y,v)
		}
		\ge
		\sum_{y \in [0,1]}
		p_i^{\cS}(y,v)
		\parans{
		\sum_{\sigma \in S_l}
		q_i^{\cS}(y,v)
		},
	\end{align*}
	and it completes the proof.


==> temp/icml-dynamic.tex <==
\section{Dynamic Setting with Online Arrivals}\label{sec:dynamic}
\note{Not quite sure to add this section or not.}
In this section, we discuss how our model and corresponding results can be extended to beyond the simultaneous game setup.
We mainly discuss that our model accommodates a \emph{dynamic game} version of interpretation.
Instead of considering simultaneous game between the agents, we consider an online arrival of agents.
At each time step $t$,

suppose that at each time step $t$, an agent $t$ with $\cO_t$ arrives and decide which (sub)set of arms to register in the platform.
\note{Make it more formal}
The arms registered in the system are cumulated over the rounds, and the algorithm runs from the initial round with no contents.
The agents may have partial information on the other arms exist in the system, \eg by observing some statistics of the system or directly exploring the contents, or may have no information at all.
In any case, our notion of dominant strategy effectively allows us to guarantee an \emph{anytime truthfulness} of our algorithm, \ie regardless of arrival time, own prior distribution and information on other agents, any agent will play truthful strategy.
We will discuss this more formally in Section~\ref{sec:dynamic}.


==> temp/icml-intro.tex <==
\section{Introduction}\label{sec:intro}
Multi-armed bandit (MAB) algorithms are an important paradigm for interactive learning that focuses on quantifying the trade-off between exploration and exploitation \citep{slivkins2019introduction}. They are used to model various practical applications where there is a set of actions (arms) to be selected (pulled) over a collection of rounds. Pulling an arm yields a reward sampled from its distribution which is generally different from the other arms' distributions. The objective is to maximize the sum of rewards accumulated through the rounds or equivalently minimize the \emph{regret} with respect to the optimal clairvoyant arm choice. The main difficulty of the problem stems from the fact that the distributions are unknown and have to be learned by pulling the arms over a collection of rounds. Due to its significant usefulness, the MAB model has been used in various applications such as recommender systems  \citep{barraza2020introduction,tang2014ensemble}, dynamic pricing by \citep{badanidiyuru2018bandits,badanidiyuru2014resourceful}, and clinical trials by \citep{djallel2019survey} to name a few.
%Clearly, algorithms with low regret (good performance) minimize the pulls of all sub-optimal arms. 

In deploying MAB algorithms in real-world applications, however, the rewards are often not coming from stochastic distributions, but from a collection of rational individuals (agents) who seek to maximize their own payoff.
Consequently, there has been a surge of interest in bandit mechanism design, which studies MAB algorithms which induces a good outcome with respect to agents' strategic behavior, while maintaining its efficiency.
Examples of such settings include two-sided matching markets, where agents learn their preferences through sequential interactions \citep{liu2021bandit,liu2020competing}, and learning in environments where agents can strategically modify the realized rewards of their arms \citep{braverman2019multi,feng2020intrinsic}.
%In the meantime, MAB algorithms are being exceedingly applied in game theoretic settings where there are a collection of individuals (agents) interested in maximizing their utility, and thus there has been a surge of interest in bandit mechanism design. In words, MAB algorithms that take agents' incentives into account and achieve good performance. Examples include two-sided matching markets where agents learn their preferences thorugh sequential interactions \citep{liu2021bandit,liu2020competing} and learning in settings where agents can strategically modify the realized rewards of their arms \citep{braverman2019multi,feng2020intrinsic}. 

Recently, \cite{shin2022multi} considered a problem where agents register arms to a platform that uses a MAB algorithm to minimize regret. 
Each agent has an original set of arms, and the mean reward of each arm is known to him a priori, \ie agents are \emph{fully-informed}.
Each agent receives a fixed constant portion of the reward whenever its arm is pulled, and tries to maximize cumulative reward.
Importantly, each agent can potentially register the same arm \emph{more than once} (replication), which possibly ruins the exploration-exploitation balance of the bandit algorithm, where the replicated arm has exactly the same are with the original arm.
Indeed, \cite{shin2022multi} show that ``ordinary'' algorithms such as upper-confidence-bound (UCB) or $\eps$-greedy induce rational agents to replicate infinitely many times, and thus the algorithm suffers linear regret.
To address this problem, \cite{shin2022multi} introduce a novel problem of designing \emph{replication-proof} bandit mechanism where any agents' dominant strategy is to not replicate.
They propose a hierarchical algorithm that consists of two phases, where the first phase determines agent and the second one decides the arm to select within the selected agent.

Although the replication-proof mechanism of \cite{shin2022multi} is remarkable, the assumptions that each agent is fully informed about its own arms is very strong, both in terms of theoretical and practical perspective.
Intuitively, if an agent knows all of its own arms' mean rewards, there exists no reason for the agent to consider suboptimal arms.
Indeed, this assumption significantly simplifies the equilibrium analysis so that the problem simply reduces to the case under which each agent only has a \emph{single arm}.
Then, it is straightforward to check that any bandit algorithm is replication-proof under a single-agent setting, and their contribution lies on introducing a hierarchical structure to maintain replication-proofness with multiple agents.
Moreover, in practice, it is more reasonable to assume that each agent only has partial information regarding its own arm.
For instance, in an online content platform, each content provider usually does not know the quality of each content that has not been posted yet, but only can guess its outcome, based on the data possibly acquired from the previous contents he/she may have.

In this context, we study a \emph{Bayesian extension}\footnote{We remark that our notion of Bayesian differs from that of Bayesian mechanism design or Bayesian game in the literature. In those settings, each agent usually computes ex-interim payoff given the \emph{incomplete} information regarding others' types. In this paper, however, we aim to develop an \emph{incentive-compatible} mechanism under which each agent truthfully register all the arms without regard to others' actions, when he/she faces uncertainty on their own arms and computes ex-ante payoff over such uncertainty.} of the replication-proof bandit mechanism design problem, where each agent only knows such a distribution from which its own arm's mean reward is sampled.\footnote{To practically motivate our problem setup, in creator economy like Youtube, a content creator typically does exactly know about each content's quality in advance, but only has some historical information on the qualities of his/her previous content. Historical information can be thought of as a prior distribution of the agent in our setting. The setting by Shin et al. can be interpreted as a scenario in which all the agents know the exact quality of their contents. In this case, the agent does not have any ambiguity in registering/replicating which arms, since he/she knows own best arm, which might be a bit impractical.}
Given the prior distribution, each agent computes its own ex-ante payoff by taking expectation over all the possible realization of its own arms, and commits to a strategy that maximizes the payoff.
Importantly, we aim to obtain an \emph{dominant strategy incentive-compatible} (DSIC) mechanism such that each agent has no incentive to deviate from its truthful strategy, \ie submitting all the original arms without any replication, regardless of the others' strategies.

Our extension brings significant challenges in analyzing an algorithm's equilibrium compared to the fully-informed agent setting.
Notably, even in a single-agent case, it is not trivial to obtain a replication-proof algorithm.
This is in stark contrast to fully-informed setting by~\cite{shin2022multi} under which any bandit algorithm trivially satisfies replication-proofness.
The question of designing replication-proofness in the single-agent setting spawns an intriguing question of \emph{comparing expected regret of multiple bandit instances}, which we will elaborate more shortly.

\paragraph{Outline of the paper}
In the two subsequent subsections, we present our main contributions and related works.
Section~\ref{sec:model} introduces formal problem setup and preliminary.
The failure of H-UCB and its implication is provided in Section~\ref{sec:fail}.
Section~\ref{sec:single} develops our main intuition on constructing replication-proof algorithm by investigating single-agent setting, and Section~\ref{sec:multi} extends this result and provide our main result on the replication-proof algorithm with sublinear regret.

\subsection{Contributions and techniques}
Overall, our main results towards replication-proof algorithms are presented in a step-by-step manner.
We start with investigating the previous algorithm suggested by~\cite{shin2022multi}, which mainly builds upon standard UCB\footnote{We focus our attention on a structured class of UCB algorithms with index $\muhat_a + f(t,n_a)$ where $\muhat_a$ denotes empirical average reward, $t$ is current round, and $n_a$ denotes the number of pulls of arm $a$. Note that standard UCB1~\cite{auer2002finite} has a form of $f(t,n_a) = \sqrt{\log(t)/n_a}$.} along with the idea of hierarchical structure.
Unlike from the fully-informed setting under which any bandit algorithm is replication-proof in the single-agent setting, we reveal that the standard UCB algorithm fails to be replication-proof even with single-agent, regardless of the exploration parameter $f$.
Mainly, we show that UCB does not satisfy a property called \emph{truthful under random permutation} which will be elaborated shortly, via construction of worst-case problem instance that exploits structural properties of UCB which adaptively and deterministically (up to tie-break) select the arms.
This phenomenon carries over to the multi-agent setting, so that UCB equipped with hierarchical structure, namely H-UCB by~\cite{shin2022multi}, fails to be replication-proof, regardless of the number of agents.

To tackle this challenge, we first thoroughly investigate the single-agent setting, and characterize necessary and sufficient conditions for an algorithm to be replication-proof.
Let us provide a simple example to explain the main technical challenges one would face in analyzing equilibriums.
\begin{example}
	Consider a single agent whose prior distribution is $Bern(0.5)$. 
	The agent has two original arms, say arm $a$ and $b$.
	There exist three cases in terms of the pair of realized rewards $(\mu_a, \mu_b)$: (i) $(1,1)$ with probability (w.p.) $0.25$ (ii) $(1,0)$ w.p. $0.25$, (iii) $(0,1)$ w.p. $0.25$, (iv) $(0,0)$ w.p. $0.25$.
	Suppose that the agent decides replicate only arm $a$, without observing the ex-post realization of the mean rewards, say the replicated arm $a'$.
	For cases (i) and (iv), the replicated arm has no effect since all the arms have the same mean rewards, \ie pulling any arm yields the same expected reward, so let's focus on case (ii) and (iii).
	In case (ii), the resulting bandit instance from the agent's strategy will be $\cI_A: (\mu_a, \mu_{a'},\mu_b) = (1,1,0)$ whereas in case (iii), it will be $\cI_B: (1,0,0)$
	Hence, compared to the strategy with no replication, the agent's gain from replicating arm $a$ is equal to the gain from the average of expected payoff in case (ii) and (iii), compared to the case in which the algorithm runs with bandit instance $\cI_O: (1,0)$.
	Hence, if the agent has no incentive to replicate arm $a$ once, the expected regret under $\cI_O$ should be at most the average of that under $\cI_A$ and $\cI_B$.
\end{example}
%
%We observe that the problem of designing a replication-proof algorithm even under this simple case (single agent, Bernoulli arms) boils down to the following question.
%\begin{example}
%    Consider a bandit instance $\cI_A$ with two Bernoulli arms with mean rewards $0.1$ and $0.5$. Consider Bernoulli bandit instances $\cI_B$ and $\cI_C$ each equipped with three Bernoulli arms such that $B$'s arms have mean rewards $0.1, 0.1$ and $0.5$ and $\cI_C$'s arms have $0.1, 0.5$ and $0.5$. 
%    Given some standard bandit algorithms, would the expected regret under $\cI_A$ be larger than the average of expected regret under $\cI_B$ and $\cI_C$?
%\end{example}
Even under simplistic and standard algorithms such as UCB, it is not straightforward to answer the above question.
Intuitively, instance $\cI_A$ will incur smaller regret as the number of optimal arm increases, but the instance $\cI_B$ will have larger regret due to more suboptimal arms with mean reward $0.1$.\footnote{Note that this can be shown using a coupling-like argument between random reward tapes of the arms, combined with a regret decomposition lemma. See~\cite{shin2022multi} for more details.}
Thus, the question is whether the loss from $\cI_B$ will be larger than the gain from $\cI_A$ in average, compared to $\cI_O$.

More formally, we can refine the above observation as the following fundamental question in comparing the expected regret of multiple bandit instances.
\begin{center}
	\emph{Given an arbitrary stochastic bandit problem, consider an adversary who uniformly randomly selects an arm and replicates. Which bandit algorithms guarantee that the regret does not increase against the adversary? What if it randomly replicates multiple arms possibly at different times?}
\end{center}
We affirmatively answer this question by proving that, there exists an algorithm that satisfies the above questions for \emph{any} bandit instance under some mild assumptions.
To this end, we introduce a notion of \emph{random-permutation regret}, which captures the average regret of an agent's strategy with replication without observing the ex-post realization.
We show that if an algorithm satisfies that the random-permutation regret does not increase with respect to replication (called, truthfulness under random permutation - TRP), and is permutation invariant between the arm indices, then it is replication-proof under single-agent setting.
We refer to Section~\ref{sec:single} for precise definitions.
We further prove that the conditions presented above are indeed necessary for any algorithm to be replication-proof.
In fact, the failure of UCB comes from violating TRP.
Meanwhile, we prove that exploration-then-commit (henceforth ETC) satisfies these properties, thus replication-proof in the single-agent setting.

With the goal of designing a replication-proof algorithm for any number of agents, we combine several techniques upon the observation above.
First, we borrow the hierarchical structure of~\cite{shin2022multi}, and analyze hierarchical algorithm with each phase running ETC, which effectively decomposes each agent's payoff from each other.
Moreover, our analysis heavily depends on the non-adaptivity and decoupled nature of ETC.
It remains as a major open problem whether it is necessary for the algorithm to have non-adaptive exploration structure in order to satisfy TRP.
In addition, we introduce a restarting round in the second phase at the beginning of the exploitation rounds in the first rounds.
This largely simplifies the analysis of the selected agent in the exploitation rounds in the first phase, since the second phase simply reduces to the single-agent case with that selected agent with the highest empirical average reward.
We cement our result by proving that our algorithm has sublinear regret, thereby achieving both of robustness and efficiency.


%%Then, we extend it to replication-proof algorithm in the multi-agent setting by adopting the hierarchical structure of \cite{shin2022multi} while introducing a novel device of \emph{restarting} and largely exploiting the \emph{non-adaptive} and \emph{decoupled} structural nature of ETC algorithm.
%We cement our result by proving that our algorithm has sublinear regret, thereby achieving both of robustness and efficiency.


%
%We develop a replication-proof algorithm based on this single-agent analysis, which captures the both rabbits of efficiency and robustness.
%To this end, we begin with analyzing H-UCB presented by \cite{shin2022multi}.
%Surprisingly, however, we observe that it is no more replication-proof with Bayesian agents.
%This mainly stems from the fact that UCB itself is \emph{not replication-proof} even in the single-agent setting, and thereby H-UCB is \emph{not replication-proof} in the multi-agent setting.
%Thus, UCB is not the algorithm that answers the above question positively.
%To overcome the limitation of H-UCB, we first thoroughly investigate the single-agent setting, and characterize \emph{sufficient conditions} under which an algorithm becomes replication-proof.
%This analysis eventually spawns the question presented above, which might be of independent interest in \emph{comparing regrets of multiple bandit instances}.
%Notably, we prove that exploration-then-commit (henceforth ETC) satisfies these properties, thus replication-proof in the single-agent setting.
%Then, we extend it to replication-proof algorithm in the multi-agent setting by adopting the hierarchical structure of \cite{shin2022multi} while introducing a novel device of \emph{restarting} and largely exploiting the \emph{non-adaptive} and \emph{decoupled} structural nature of ETC algorithm.
%We cement our result by proving that our algorithm has sublinear regret, thereby achieving both of robustness and efficiency.
%
%
%
%
%
%We reveal that 
% and show that it fails to be replication-proof even in the single-agent setting.
%Subsequently, we characterize necessary and sufficient conditions for an algorithm to be replication in the single-agent setting, and prove that exploration-then-commit (ETC) satisfies this property, whereas UCB does not.
%Built upon it, we present a hierarchical algorithm with ETC, equipped with a restarting technique that re-initializes every parameters in the second phase (arm selection phase), and analyze its replication-proofness.
%We complement this result by providing its sublinear regret upper bound, thereby capturing the both rabbits of robustness and efficiency.
%
%
%As noted thus far, our main result starts with the failure of H-UCB.
%
%Indeed, we observe that the analysis of designing a replication-proof algorithm even under a very simple case (two Bernoulli arms, single agent) boils down to the following question.
%\begin{example}
%    Consider a Bernoulli bandit instance $\cI_A$ with two arms with mean rewards $0.1$ and $0.5$. Consider Bernoulli bandit instances $\cI_B$ and $\cI_C$ each equipped with three arms such that $B$'s arms have mean rewards $0.1, 0.1$ and $0.5$ and $\cI_C$'s arms have $0.1, 0.5$ and $0.5$. 
%    Given some standard bandit algorithms, would the expected regret under $\cI_A$ be larger than the average of expected regret under $\cI_B$ and $\cI_C$?
%\end{example}
%Even under simplistic and standard algorithms such as exploration-then-commit (ETC) or UCB, it is not straightforward to answer the above question.
%Obviously, instance $C$ will incur smaller regret, but the instance will have larger regret.\footnote{Note that this can be shown using a coupling-like argument between random reward tapes of the arms, combined with a regret decomposition lemma. See~\cite{shin2022multi} for more details.}
%Thus, the question is whether the loss from $B$ will be larger than the gain from $C$, compared to $A$ respectively.
%
%More formally, in its simplest form, a single-agent analysis case of our objective to construct replication-proof algorithm spawns to the fundamental question of comparing the expected regret of multiple bandit instances, presented as follows.
%\begin{center}
%	\emph{Given an arbitrary stochastic bandit problem, consider an adversary who uniformly randomly selects an arm and replicates. Which bandit algorithms guarantee that the regret does not increase against the adversary? What if it randomly replicates multiple arms possibly at different times?}
%\end{center}
%We affirmatively answer this question by proving that, there exists an algorithm that satisfies the above questions for \emph{any} bandit instance under some mild assumptions.
%We develop a replication-proof algorithm based on this single-agent analysis, which captures the both rabbits of efficiency and robustness.
%To this end, we begin with analyzing H-UCB presented by \cite{shin2022multi}.
%Surprisingly, however, we observe that it is no more replication-proof with Bayesian agents.
%This mainly stems from the fact that UCB itself is \emph{not replication-proof} even in the single-agent setting, and thereby H-UCB is \emph{not replication-proof} in the multi-agent setting.
%Thus, UCB is not the algorithm that answers the above question positively.
%To overcome the limitation of H-UCB, we first thoroughly investigate the single-agent setting, and characterize \emph{sufficient conditions} under which an algorithm becomes replication-proof.
%This analysis eventually spawns the question presented above, which might be of independent interest in \emph{comparing regrets of multiple bandit instances}.
%Notably, we prove that exploration-then-commit (henceforth ETC) satisfies these properties, thus replication-proof in the single-agent setting.
%Then, we extend it to replication-proof algorithm in the multi-agent setting by adopting the hierarchical structure of \cite{shin2022multi} while introducing a novel device of \emph{restarting} and largely exploiting the \emph{non-adaptive} and \emph{decoupled} structural nature of ETC algorithm.
%We cement our result by proving that our algorithm has sublinear regret, thereby achieving both of robustness and efficiency.


% In Section~\ref{sec:model}, we introduce our model and further preliminaries.
% We then provide negative result of UCB and H-UCB in Section~\ref{sec:fail}.
% Positive results for the single-agent setting is presented in Section~\ref{sec:single}.
% Finally in Section~\ref{sec:multi}, we present our main results of replication-proof algorithm along with its regret analysis.
% All the proofs are deferred to the appendix due to space constraints.

%In this context, we study a Bayesian extension of \cite{shin2022multi}, where each agent only knows such a distribution.

%it is inadequate to apply in various applications where --more realistically-- an agent's knowledge about the means of his arms is imperfect. Specifically, an agent in general does not know the mean of each arm but rather has a Bayesian prior over the mean of the arm, e.g. an arm may have mean $0.7$ with probability $\frac{1}{4}$ and $0.3$ with probability $\frac{3}{4}$. 
%
%
%This Bayesian modification of the setting holds for many real life applications. For example, consider an online video sharing platform such as YouTube. An agent can have a collection of videos which he may be able to upload more than once, however he may only posses uncertain knowledge (Bayesian prior) about the quality (mean reward) of a video before it is registered to the platform and viewed by the users. Similarly, one can consider an e-commerce website such a eBay or Airbnb \note{Seyed - the issue with both of these is that unlike a video the resource can be consumed, i.e. if someone rents a place you cannot replicate it, similarly if someone wants to buy an item you cannot replicate it as well}   
%
%While the modification to the model is simple it introduces non-trivial implications. Specifically, we show that \note{text needs to flow better with what is before and after}   

%
%\subsection{Our contributions and techniques}
%Our negative result on H-UCB of \cite{shin2022multi} mainly relies on the deterministic nature of UCB along with its adaptive exploration.
%This
%
%
%\note{Emphasize that our problem basically  boils down to the problem of comparing the expected regret of multiple bandit instances.}
%
%\note{Also emphasize that our results directly carry over to the dynamic setting in which at each round an agent arrives with some arms and try to register their contents, since we are essentially dealing with "incentive-compatible".}



\subsection{Related work}
There exists a growing literature at the intersection of multi-armed bandits and game theory. The work of \cite{braverman2019multi} considers a setting where the arms are agents. When an arm (agent) is pulled a reward is realized. The agent can take part of the reward and only report the remaining reward to the principal. The paper's major contribution is showing that there exists instances where the agents can engage in collusion and deliver only a sublinear amount of cumulative rewards to the principle. The work of \cite{feng2020intrinsic} is closely related to \cite{braverman2019multi} in that the agents are still arms that can modify their rewards. However, in \cite{feng2020intrinsic} an agent's utility equals the total number of pulls and are not related to the rewards. Further, the reward modifications are not real but rather fake and not adding to the principal's utility. Their main contribution is showing that under such a setting standard MAB algorithms like UCB and $\eps$-greedy can still achieve sublinear regret if the modifications are sublinear. 
\cite{esmaeili2023robust} introduce a further extension of~\cite{braverman2019multi} in which the agent can either take the rewards or increase the rewards at costly efforts.
\cite{ghosh2013learning} consider a setting where each arm (agent) gains higher utility with more pulls. The arm can increase its mean at some cost and they show that if the horizon is large enough, then a Nash equilibrium exists where all agents contribute the highest possible mean. 
\cite{hajiaghayi2023regret} study a bandit variant of the delegated choice problem by~\cite{kleinberg2018delegated} where a strategic agent decides which arm to commit while the principal can either accept or reject based on its reward afterward.
While the above works share some connections to our model in their perspective of \emph{bandit mechanism design against strategic agents}, the problem setups are very different from ours.

Initiated by \cite{kremer2014implementing} and \cite{che2018recommender}, there exists a line of works studying \emph{incentivized exploration} to design a mechanism that incentivizes myopic agents to explore the arms.
At each round, a myopic agent arrives and select an arm based on the signal sent by the bandit algorithm.
If the signaling scheme is not incentive-compatible, the agent will not follow the algorithm's recommendation, but rather exploits the empirically best arm.
Thus, the principal needs to design a mechanism to induce myopic agents to explore the arms.
To this end, the principal may exploit the information asymmetry arises from the principal's information design scheme~\citep{mansour2015bayesian, immorlica2018incentivizing, sellke2021price} or may compensate the myopic users~\citep{frazier2014incentivizing, han2015incentivizing, chen2018incentivizing}.
These works, however, focus on agents who are delegated to \emph{select} the arms based on the information available at hand, whereas our problem focuses on agents who are delegated to \emph{design} the bandit instance by selecting which arms to register in the system.
A long line of works \citep{banerjee1992simple, bala1998learning, smith2000pathological, lazer2007network, banihashem2023bandit} has been asking a similar question of \emph{learning dynamics} under a presence of myopic agents pulling the arms. Since these works mostly aim to characterize regimes under which the social learning succeeds or fail, \ie not in a mechanism design perspective, so we do not discuss more in details.


% There also exists a growing literature at the intersection of matching and multi-armed bandits where the agents preferences are learned through sequential interactions in centralized \citep{liu2020competing,jagadeesan2021learning} as well as decentralized settings \citep{liu2021bandit,basu2021beyond}. 
% \suho{we can add SODA paper, and some more papers, if we will discuss matching and bandit. But not quite sure whether this topic is worth discussing}
% \suho{explain a bit about bandit algorithm against infinite number of arms, refer to SHIN.}
% \suho{discuss incentivized exploration literature as well}

% While the above works share some connections to our work in their perspective of bandit mechanism design against strategic agents, the models are very different from ours. 
Most closely related to this paper is the work of \cite{shin2022multi}. 
In particular, similar to our work agents have a collection of arms which they can register to the platform and are capable of replicating an unbounded number of times. 
The main contribution is to construct an incentive-compatible mechanism, named hierarchical UCB (H-UCB), under which each agent does not replicate, but registers only the arm with the highest mean.
Their equilibrium analysis is relatively simple due to the fact that the agents are aware of the ex-post realization of their own arms' mean rewards, \ie \emph{fully informed}.
% The main contribution is showing that a hierarchical UCB algorithm (H-UCB) that leads to an incentive-compatible mechanism where each agent's dominant strategy is to only register the arm with the highest mean. 
Despite the close connection to our work, in our setting the agent's knowledge of the arms' means is not complete (deterministic) but rather imperfect and modelled by Bayesian priors. 
While the modification itself looks simple, its consequences are challenging. In fact, we show that H-UCB fails in this setting. 
Further, while our solution shares some features with \cite{shin2022multi} in that we still use a hierarchical structure, the details of our solution differ greatly and require new ideas and analysis.

Finally, a number of works~\citep{manyarmed:berry, manyarmed:carpentier, manyarmed:wang, manyarmed:zhu} study a bandit algorithm when there exists infinite number of arms in the system or the arms arrive over the time. 
While these works focus on designing a robust algorithm to adapt to infinite number of arms with some structural assumptions on the proportion of optimal arms or their arrival time, our work takes a perspective of algorithmic scheme to \emph{prevent} such many arms in advance.
We remark that preventing such an overload in advance is typically more desirable, \eg  saving computational resources.


==> temp/icml-model.tex <==
% !TEX root =  main.tex
\section{Model}\label{sec:model}
% We consider a mechanism design approach for the standard stochastic bandit problem in which the set of arms registered in the bandit instance are determined by the algorithm itself.
We consider a simultaneous game between a set of agents $[n] = \{1,2,\ldots, n\}$ and a principal.
Each agent $i \in \set{N}$ has a set of original arms $\set{O}_i = \{o_{i,1},\ldots, o_{i,l_i}\}$ given a constant $l_i \in \N$.
Each agent $i$ is equipped with a cumulative distribution $F_i$ from which each original arm $o_{i,k}$'s mean reward $\mu(o_{i,k})$ is sampled for $k \in [l_i]$.
Each arm $o_{i,k}$ further follows a reward distribution $G_{i,k}$ with the mean reward sampled as noted above.
We use $f_i$ and $g_{i,k}$ to denote the density function of $F_i$ and $G_{i,k}$,\footnote{We assume the existence of density function for ease of exposition, but all the results will easily be generalized.} and we assume that all the distributions are supported on $[0,1]$.
%Each arm $o_{i,k}$ has a 
%Let $f_i$ denotes the density function of $F_i$,\footnote{We assume that $f_i$ exists for ease of exposition, but all the results will easily be generalized.} and we assume it has bounded support on $[0,1]$.
We further assume that $F_i$ is independent from $F_j$ for $i \neq j \in [n]$.
For instance, $F_i$ might be a uniform distribution over $[0,1]$, and each arm $a \in \cO_i$ has a Bernoulli reward distribution with the mean sampled from $F_i$.
%Precisely, arm $a \in \set{O}_i$ is parameterized by its mean reward $\mu(a)$, which is sampled from the cumulative distribution $F_i$ with density function $f_i$ supported on $[0,1]$.
%We assume $F_i$ is independent between the agents $i \in [n]$.
%For instance, $\cF_i$ can be a family of Bernoulli distributions with mean rewards sampled from $[0,1]$, or even simply can be a family of distributions having a singleton support on the mean reward.
%We assume that this sampling of mean reward is independent across the agents.
%This assumption is innocuous because a creation of contents (arms) is usually independent of what other content providers are creating simultaneously.
We often deal with a \emph{single agent} setting with $n=1$.

\paragraph{Bayesian agents}
Importantly, we consider a \emph{Bayesian scenario} in which each agent is only aware of its own distribution $F_i$, but not the exact realization of $\mu_a$ for $a \in \set{O}_i$.
We note that such assumption is indeed practical since content providers (agents) in contents platform typically only have a partial information on how much their contents may attract the users, \eg based on his/her previous contents and outcomes therein.
This is in stark contrast to the setting of~\cite{shin2022multi} in which they assume \emph{fully-informed} agents such that any strategic agent does not have any incentive to register the arms except the best one reducing the problem into the single-arm case, which is not practical in many real-world scenarios.
We highlight that the equilibrium analysis in the fully-informed setting simply boils down to the case under which each agent only has a single original arm and decides how much to replicate that unique arm, whereas our extension significantly complicates the analysis of equilibrium, as will be elaborated shortly.
%Compared to their model, our setting of Bayesian agents brings a substantial amount of technical challenges in both designing and analyzing equilibrium of algorithms, where we elaborate more in subsequent sections.

%\paragraph{Agent's strategy}
\paragraph{Agent's strategy and mechainsm procedure}
Given the prior distribution $F_i$, the set of original $O_{i,k}$ and the principal's algorithm $\fA$, each agent $i$ decides how many times to replicate arm $k$, including $0$ of no replication, for each $k \in [l_i]$.
Precisely, agent $i$ commits to a set $\set{S}_i = \{s_{i,k}^{(c)}:c \in [c_{i,k}], k \in [l_i]\}$ in a strategic manner, where $c_{i,k}$ denotes the total number of replica for arm $o_{i,k}$.
The replicated arm $s_{i,k}^{(c)}$ has the same mean reward to the original arm, \ie $\mu(s_{i,k}^{(c)}) = \mu(o_{i,k})$ for any $i \in [n]$ and $k \in [l_i]$.
We often use $s_{i,k}^{(0)}$ to denote $o_{i,k}$ for simplicity.
Define $\cS = (\cS_1, \ldots, \cS_n)$ and $\cO = (\cO_1, \ldots, \cO_n)$.
Given all the agents' strategies $\set{S}$, the bandit algorithm $\fA$ runs and corresponding rewards are realized.
%Importantly, we assume that a constant portion $\alpha \in (0,1)$, which is exogenous to the mechanism, of the rewards are transferred from to each agent whenever the agent's arm is selected.

The overall mechanism proceeds as follows: (i) The principal commits to a bandit algorithm (mechanism), (ii) Each agent $i \in \set{N}$  decides an action $\set{S}_i$ to register given $\mathfrak{A}$ to maximize own payoff, (iii) The mean rewards $\mu_a$ for each $a \in \set{O}$ are sampled, (iv) The bandit algorithm $\mathfrak{A}$ runs and rewards are realized, (v) The principal and the agent realize their own utility.\footnote{Note that if all the agents do not strategize and simply register $\set{O}_i$ in step (ii), our problem reduces to the standard stochastic multi-armed bandit problem, where standard bandit algorithms would work well.}
% \begin{enumerate}[(i)]
% \item The principal commits to a bandit algorithm $\mathfrak{A}$.
% \item Each agent $i \in \set{N}$  decides an action $\set{S}_i$ to register given $\mathfrak{A}$ to maximize own payoff.
% \item The mean rewards $\mu_a$ for each $a \in \set{O}$ are sampled.
% \item The bandit algorithm $\mathfrak{A}$ runs and rewards are realized.
% \item The principal and the agent realize their own utility.
% \end{enumerate} 


\paragraph{Agent's payoff}
%The most remarkable difference from the perfect information model is that the exact mean reward in $\set{S}_i$ is determined after the selection of the strategy.
%Therefore, each agent should basically select the strategy set in ex-ante manner so that its expected payoff becomes larger in regards of the randomness in realization of $\mu_a$ for $a \in \set{O}_i$.
%Alternatively, this procedure can be interpreted as (i) sampling $\mu_a$ for $a \in \set{O}_i$ from $D_i$ and then (ii) randomly permuting the realized mean reward over the set of arms $o_{i,1},\ldots, o_{i,l(i)}$.
%This interpretation will particularly be useful in defining the expected payoff of each agent.
%\note{Suho - TBD - No need to interpret like this here. Just present the expectation, and later provide some intuitions when we define replication proof or results.}
Once an arm is selected by $\fA$, a fixed portion $\alpha \in (0,1)$ of the reward is paid to the agent who registers the arm.
We write $\muvec_i$ to denote $(\mu_{i,1}, \mu_{i,2}, \ldots, \mu_{i,l_i})$, \ie the vector of agent $i$'s (realized) mean rewards of the arms.
Let $E_{i}(\muvec_i)$ be an event that the mean reward of agent $i$'s arms are realized to be $\muvec_{i}$.
Recall that $E_i(\cdot)$ are mutually independent for for $i \in [n]$.
We often abuse $E_{i}$ to denote $E_i(\muvec_i)$ if the realization $\muvec_i$ is clear from the context.
% and write $E_{-i}(\muvec_{-i})$ to denote the realization of the other agents' mean rewards of the arms, \ie an event that for $\cN \ni j \neq i$, agent $j$'s arms' mean rewards are sampled to be $\muvec_j$.
We also write $\cS_{-i}$ to denote $(\cS_1, \ldots, \cS_{i-1}, \cS_{i+1}, \ldots, \cS_n)$, and $E(\muvec)$ for $\muvec = (\muvec_1,\muvec_2, \ldots, \muvec_n)$ to denote the event such that $\cap_{i \in [n]}E_i(\muvec_i)$.

We further introduce some notations given the principal's algorithm $\fA$.
Conditioned on the $E_{i}(\muvec_i)$, agent $i$'s \emph{ex-post payoff} of selecting strategy $\set{S}_i$ given the others' strategies is defined as
\begin{align*}
U_i(\set{S}_i, \set{S}_{-i} ;E(\muvec)) = \alpha \sum_{t=1}^T R_t\Ind{I^{(t)} \in \set{S}_i},
\end{align*}
where  $R_t$ refers to the reward at round $t$ and $I_t$ denotes the arm selected at round $t$.

Given the ex-post utility, each agent computes its \emph{ex-ante payoff} by marginalizing over the realization of its own arms' mean rewards, defined as follows
\begin{align*}
	u_i(\set{S}_i, \set{S}_{-i}) = \Ex{U_i(\set{S}_i, \set{S}_{-i};E(\muvec))},
\end{align*}
where the randomness in the expectation comes from $E(\muvec)$, i.e. the realization of the mean rewards, and possibly from the random bits of the algorithm $\fA$.
In words, each agent is rational \emph{expected utility maximizer} who maximizes its expected payoff.
%We denote $U_i(\set{S}_i, \set{S}_{-i};E_{i})$ by \emph{ex-post} utility, and $u_i(\set{S}_i, \set{S}_{-i})$ by \emph{ex-ante} utility.
% We often overwrite $u_i(\set{S}_i, \set{S}_{-i})$ by $u_i(\set{S}_i)$ when $\set{S}_{-i}$ is clear from the context.

\paragraph{Information and desiderata}
We now describe the information structure of the mechanism, and how each agent decides its own strategy based on its ex-ante payoff.
We first assume that the principal does not have any information regarding the agents' distributions, nor the number of original arms.
This is often called \emph{prior-independent mechanism} in the mechanism design, \cf \cite{hartline2013bayesian}.
In addition, we assume that the agent does not have any information regarding the others.
Instead, our objective is to construct a \emph{incentive-compatible} mechanism such that each agent's \emph{dominant strategy} is to register the arms without any replication, without regard to what others may have proposed.
To this end, we first define a dominant strategy as follows.
\begin{definition}[Dominant Strategy]
Agent $i$'s strategy $\set{S}_i$ is dominant strategy if $u_i(\cS_i \cup \set{S}_{-i}) \ge  u_i(\set{S}'_i \cup \cS_{-i})$ for any $\set{S}'_i$ and $\set{S}_{-i}$.
\end{definition}
Correspondingly, we introduce the following notion of \emph{dominant strategy equilibrium}.
\begin{definition}[Equilibrium]
An algorithm $\mathfrak{A}$ has dominant strategy equilibrium	(DSE) if there exists a set of agent strategies $\set{S} = \{\set{S}_i\}_{i \in [n]}$ such that $\set{S}_i$ is dominant strategy for any agent $i \in [n]$.
\end{definition}
As per the definition, the total ordering of the agent's payoff with respect to its own strategy should remain the same regardless of the others' strategies $\cS_{-i}$.
Thus, we often omit the parameter $\cS_{-i}$ in denoting agent $i$'s payoff, \eg $u_i(\cS_i)$ instead of $u_i(\cS_i, \cS_{-i})$.
Note, however, that the realization of the other agents' mean rewards may affect the actual quantity of $u_i(\cS_i)$, although it does not affect which strategy agent $i$ will eventually commit to.
Since we are interested only in how the agents will "behave", the absolute amount of the payoff is beyond our interest, and thus it does not lose any generality.

We finally introduce incentive compatibility of an algorithm as follows.
\begin{definition}[Replication-proof]
An algorithm $\mathfrak{A}$ is \emph{replication-proof} if it has a dominant strategy equilibrium $\{\set{O}_i\}_{i \in [n]}$ for any $T \in \N$.
\end{definition}
Replication-proofness is desirable as the agents are not motivated to replicate their own arms, thereby reducing the number of arms that a bandit algorithm faces.
Since the regret upper bound of a standard bandit algorithm usually depends on the number of arms, maintaining a smaller number of suboptimal arms in the system affects the eventual learning efficiency of the algorithm.
% it narrows down a set of identical arms into a single arm, therefore reduces the exploration burden in which the algorithm should have faced to identify that they indeed are equal arms.
We often say that the algorithm is \emph{incentive-compatible} or \emph{truthful} to denote the replication-proofness, as in the literature, \cf \cite{nisan2007algorithmic}.

%In short, our objective is to construct a \emph{prior-independent} \emph{incentive-compatible} mechanism.



%Importantly, we do not impose any assumption on the information structure of an agent regarding others, \ie each agent does not know about the realization of the others' mean rewards nor their prior distributions.
%This allows some agents to be aware of other agents' prior distributions so that they may strategize over such a knowledge, while also admitting other agents to be fully oblivious to others' information.
%
%Instead, the principal's objective here is to construct an \emph{dominant-strategy incentive-compatible mechanism} under which each agent has no incentive to deviate from its truthful strategy, with "no" regards to what others do.
%\begin{definition}[Dominant Strategy]
%Agent $i$'s strategy $\set{S}_i$ is dominant strategy if $u_i(\cS_i \cup \set{S}_{-i}) \ge  u_i(\set{S}'_i \cup \cS_{-i})$ for any $\set{S}'_i$ and $\set{S}_{-i}$.
%\end{definition}
%
%Correspondingly, we introduce the following notion of \emph{dominant strategy equilibrium}.
%\begin{definition}[Equilibrium]
%An algorithm $\mathfrak{A}$ has dominant strategy equilibrium	(DSE) if there exists a set of agent strategies $\set{S} = \{\set{S}_i\}_{i \in [n]}$ such that $\set{S}_i$ is dominant strategy for any agent $i \in [n]$.
%\end{definition}
%
%We emphasize that such a mechanism with dominant strategy equilibrium indeed allows each agent to have arbitrary information regarding other agents in deciding its own strategy, since the inequality above holds for any choice of $\cS_{-i}$.
%Hence, with focus on obtaining dominant strategy, we can simply write $u_i(\cS_i)$ to denote $u_i(\cS_i, \cS_{-i})$.
%Note, however, that the realization of the other agents' mean rewards may affect the actual quantity of $u_i(\cS_i)$, although it does not affect what agent $i$ will eventually "choose" as a strategy.
%Since we are interested only in how the agents will "behave", the absolute amount of the payoff is beyond our interest, and thus it does not lose any generality.
%
%Finally, we assume that the principal has no information on the agents' prior distributions.
%This is often called \emph{prior-independent mechanism} in the mechanism design (\cite{hartline2013bayesian}).

%For example, given two agents $a$ and $b$, suppose that agent $a$ has an incomplete information and thus knows the prior distribution of agent $b$ and its number of arms, and agent $b$ has no information regarding $a$ at all.
%In this case, agent $a$ may decide its own strategy based on marginalizing all the possible outcomes of $\muvec$, while assuming that agent $b$ will play
%On the contrary, agent $b$ may play maxmin strategy,


%Then, we can define agent $i$'s \emph{expected payoff} of choosing action $\set{S}$ to be
%\begin{align*}
%u_i(\set{S}_i, \set{S}_{-i}) = \Exu{\mu_{\set{O}_i}}{\Ex{v_i(\set{S}_i, \set{S}_{-i};\mu_{\set{O}_i})} | \mu_{\set{O}_i}},	
%\end{align*}
%
%This is mainly because each agent does not know the realization of the rewards $\mu_a$ for own arm $a \in \set{O}_i$, the strategy itself may include a randomness arisen from choosing which arms to replicate or register.
%For example, suppose that agent $i$ decides to register only a single arm among $\set{O}_i = \{o_{i,1},o_{i,2}\}$ where $\mu_{o_{i,1}} > \mu_{o_{i,2}}$.
%Since he does not know the exact realization of the mean rewards $\mu_{o_{i,1}}$ and $\mu_{o_{i,2}}$, the only possible action would be to choose any single arm and register it, which yields the probability $50\%$ of registering high-reward arm and another $50\%$ of registering low-reward arm.
%Alternatively, this procedure can be interpreted as (i) given the prior distribution $D_i$, agent $i$ selects own action


%Importantly, we consider a \emph{Bayesian information} of agents in which each agent $i$ only has a partial information on its own arms $\set{O}_i$.
%More precisely, each agent $i$ only knows a distribution $D_i$ with support on $[0,1]$ from which the expected reward of arm $a$ is drawn independently and identically for the original arms $a \in \set{O}_i$.




%\paragraph{Learning efficiency}
On top of designing \emph{prior-independent} \emph{incentive-compatible} mechanism, we are also interested in a learning efficiency, \ie learning the reward distribution in a sample-efficient manner.
In the online learning and bandit literature, this is usually described as a notion of cumulative regret, defined as follows.
\begin{definition}[Regret]
	Given time horizon $T$, strategy $\set{S}$ and the event $E(\muvec)$, the ex-post regret of algorithm $\mathfrak{A}$ is 
	\[\reg(\mathfrak{A}, T ; \set{S}, E(\muvec)) = \parans{\max_{a \in \cup_{i \in \cN} \cO_i}\sum_{t=1}^T \mu(a)} -\sum_{t=1}^T \mu(I_t),\]
	where $I_t$ denotes the arm selected by $\mathfrak{A}$ at round $t$.
\end{definition}
\sscomment{Clarify ex-post, but its expected regret, and define it w.r.t. expectation, and expand as above}
We emphasize that the optimal benchmark is selected from $\cup_{i \in \set{N}}\set{O}_i$, not from the registered set of arms $\cup_{i \in \set{S}}\set{S}_i$.
This benchmark is indeed important since the principal should incentivize the agents to decide an action that contains own best arm to maintain larger utility.
For example, if an algorithm motivates an agent to not register all the arms, then there might be a constant probability that the omitted arm has the largest mean reward, which essentially yields sublinear regret with respect to the regret defined above.
More formally, our notion of regret implicitly implies that any sublinear regret algorithm incentivizes all the agents to register all their original arms at least once.
%Note that this definition of regret is based on the ex-post realization of the arms' parameters.
%We can also define a version of Bayesian regret by marginalizing over the realization of the arms' parameters, but we will focus on obtaining a good performance based on our definition presented above.
%Note that any analysis of the regret upper bound based on our definition easily carries over to the Bayesian regret by simply marginalizing over the priors.
We also remark that although the arms' mean rewards are sampled from prior distributions, which is often referred to Bayesian bandits (\eg see Ch.3 of \cite{slivkins2019introduction}), we deal with ex-post regret, \eg as does in \cite{agrawal2012analysis} which analyzes the ex-post regret of Thompson Sampling in Bayesian bandits.
Obviously, ex-post regret upper bound \emph{implies} the Bayesian regret upper bound by simply taking an expectation over the prior distributions.
%We also emphasize that the optimal benchmark $a^\star$ is selected from $\cup_{i \in \set{N}}\set{O}_i$, not from the registered set of arms $\cup_{i \in \set{S}}\set{S}_i$.
%This benchmark is indeed important since the principal should incentivize the agents to decide an action that contains own best arm to maintain larger utility.



%\paragraph{Negative result for standard algorithms}
%Note, however, that it is not obvious how much the algorithm could be worsen even if it does not satisfy replication-proofness.
%This is because even though an algorithm is not replication-proof, if it only allows a small number of replication, then the standard algorithm would still enjoy sublinear regret assuming that the agents only replicate sublinear number of times.
%In \cite{shin2022multi}, the authors define the following notion of replication-proneness to show that the standard algorithms indeed incurs a bad outcome.
%\begin{definition}[Replication-prone]
%An algorithm $\mathfrak{A}$ is replication-prone (RP) if for any strategy $\set{S}_i$ of agent $i$, there exists a strategy $\set{S}'_i$ such that $\set{S}_i \subset \set{S}'_i$ and $u_i(\set{S}_i \cup \set{S}_{-i}) < u_i(\set{S}'_i \cup \set{S}_{-i})$ for any $\set{S}_{-i}$.
%\end{definition}
%They formally prove that the standard algorithm such as UCB suffers replication-proneness based on a coupling technique.
%This essentially implies that the number of arms registered in the system can be arbitrarily large if the agents behavior in a strategic manner.
%Since our model accommodates the setup of \cite{shin2022multi} as a special case with prior distributions having singleton support, since their model is essentially reduced to each agent having a single arm, this negative result carries over to our model as well.
%\begin{proposition}
%	UCB suffers replication-proneness.
%\end{proposition}
%
%This would be the worst possible property that any algorithm may have, since any rational agent under such algorithm would infinitely replicate its own arms to maximize the expected payoff, and thus the it cannot guarantee the sublinear regret anymore since UCB has regret of $O(\sqrt{KT\log T})$ in the worst case where $K\to \infty$ denotes the number of arms registered in the system.
%
%\paragraph{Precluding partial replication}
%Finally, we note that it is always bad strategy for agent $i$ to register only a proper subset of $\cO$.
%Suppose that agent $i$ plays $\cS_i \subset \cO_i$ and $\cS_i \neq \cO_i$.
%Then, there exists an arm $a \in \cO_i$ which is not contained in $\cS_i$.
%Due to the nature of sampling process of arms' mean rewards, with constant probability of at least $1/|\cO_i|$, arm $a$ has the largest (or equal) mean reward.
%In this realization, excluding $a$ always induce linear regret of $\Theta(t)$ in terms of agent $i$'s utility until agent $i$ is selected $t$ rounds, and thus incurs constant probability times $\Theta(t)$ regret in expectation.
%Therefore, we only consider a strategy $\cO_i \subset \cS_i$ without loss of generality.
%This can be formalized as follows, where the proof is deferred to Appendix~\ref{app:subset}.
%\begin{proposition}\label{prop:subset}
%	For any algorithm that achieves sublinear-regret in any problem instance, for any $T$ and agent $i \in [n]$, playing $\cS_i \subset \cO_i$ such that $\cS_i \neq \cO_i$ is not dominant strategy, unless agent $i$'s distribution only has a strictly positive measure on a singleton support.
%\end{proposition}

%
%\subsection{Preliminary}
%We now discuss 
%
%\note{Suho - TBD - discuss previous algorithms/analysis, and discuss why bayesian setting makes it challenging}
%
%\note{It might be good to motivate both the single/multi agent setting.}
%
%\note{Also, briefly argue that if the agent excludes some arms, then it is always bad strategy, so without loss of generality, we only consider a strategy that replicates some arms from $\cO$.}


==> temp/icml-multi-agent.tex <==
\section{Towards Replication-proof Algorithm}\label{sec:multi}

%
%In the proof of Theorem~\ref{thm:hucb_negative} for the multiple agent case, we essentially observe that agent $i$ will play a strategy that maintains the random variable $R(i)$ as large as possible at every round in order to maximize the change of being selected.
%In this context, for an algorithm to be intuitively replication-proof given the hierarchical structure, we need to construct an algorithm such that truthful registration yields the random variable $R(i)$ largest possible for each agent $i$, regardless of the others' strategies.
%
%=========================
%
Now we turn our attention to the more general setting with multiple agents.
Basically, we start by reusing the machinery of \emph{hierarchical structure} by \cite{shin2022multi} 

%This effectively separates Phase 2 from each agent and motivates the agents to increase their chance of being selected in Phase 1, which will in turn imply the replication-proofness equipped with some good choices of $\alg_1$ and $\alg_2$.

% \vspace{-1mm}
\begin{algorithm} 
\SetAlgoLined
%$i \in \set{N}$, $\set{S} = \cup_{i \in \set{N}} \set{S}_i$\\
\textbf{Input}: Tie-breaking rule, agent set $\cN$, arm set $\cS_i$ for $i \in \cN$, restarting round $\tau \in [T]$\\
Let $\muhat_i \gets 0$, $n_i\gets 0$, $\muhat_{i,a} \gets 0$, $n_{i,a} \gets 0$ for $i \in \cN$ and $a \in \cS_i$\\


 \For{$t=1,2,\ldots,M$}{
  \If{$t = \tau+1$}
  {
  $\muhat_{i,a} \gets 0; ~ n_{i,a} \gets 0$ for $\forall a \in \cS_i$, $\forall i \in \cN$
  }
  \If{$n_i < M$ for some $i \in \cN$}
  {
  	$\hat{i} \gets i$
  }
  \Else{$\hat{i} \gets \argmax_{i \in \cN}\muhat_{i}$}
  
  \If{$n_{\hat{i},a} < m$ for some $a \in \cS_{\hat{i}}$}
  {
  	$\hat{a} \gets a$
  }
  \Else{$\hat{a} \gets \argmax_{a \in \cS_{\hat{i}}}\muhat_{\hat{i},a}$}  
%  If $N(i) \le 1/2T^{1/3} \log(T)^{1/3}$, round-robin exploration of arms in $\set{S}_i$;\\
%  Else, commit $\hat{a} = \argmax_{a \in \set{S}_{\hat{i}}} 
%    \left\{r(a) \right\}$
  Pull $\hat{a}$ of agent $\hat{i}$ and obtain reward $R_t$\\
  Update statistics:
  $\muhat_{\hat{i},\hat{a}} \leftarrow \tfrac{\muhat_{\hat{i},\hat{a}}n_{\hat{i}, \hat{a}} + R_t}{n_{\hat{i}, \hat{a}}+1}; ~
  \muhat_{\hat{i}} \leftarrow \tfrac{\muhat_{\hat{i}}n_{\hat{i}} + R_t}{n_{\hat{i}}+1};~ n_{\hat{i}, \hat{a}} \leftarrow n_{\hat{i}, \hat{a}} + 1; ~~ n_{\hat{i}} \leftarrow n_{\hat{i}} + 1;$
 }
 \caption{Hierarchical ETC with Restarting ($\hbb$)\label{alg:hbb}}
\end{algorithm}
% \vspace{-1mm}

A direct implication of Theorem~\ref{thm:single_pf_rp} is that if we run a variant of H-UCB such that the first phase runs a simple uniform-random selection algorithm, and the second phase runs some arbitrary TRP and PI algorithms, then the resulting algorithm is replication-proof.
To formally see this why, let $\set{S}_i$ be the strategy of agent $i$.
Define $\Gamma_i(\set{S}_i)$ be the agent $i$'s utility under the single-agent setting with agent $i$, \ie when there are no other agents other than $i$.
Due to the uniformly random selection nature in the first phase, the expected utility of any agent $i$ can be simply written $u_i(\cS_i, \cS_{-i}) = {\Gamma_i(\set{S}_i)}/{n}$.
Note that the dynamic of the algorithm purely reduces to the dynamic of the second phase algorithm if there's only a single agent.
Hence, by Theorem~\ref{thm:single_pf_rp} and due to the TRP and PI of the second phase algorithm, we conclude that truthful registration is a dominant strategy for any agent $i$, and thus the result follows.
%\begin{theorem}\label{thm:multi_rp_uniform}
%	The algorithm constructed as above is replication-proof
%\end{theorem}
%\begin{proof}
%	Let $\set{S}_i$ be the strategy of agent $i$.
%	Define $\Gamma_i(\set{S}_i)$ be the agent $i$'s utility under the single-agent setting with agent $i$, \ie when there are no other agents other than $i$.
%	Due to the uniformly random selection nature of $\alg_1$, the expected utility of any agent $i$ can be simply written $u_i(\cS_i, \cS_{-i}) = \nicefrac{\Gamma_i(\set{S}_i)}{n}$.
%	Note that the dynamic of $\hbb$ reduces to the dynamic of $\alg_2$ if there's only a single agent.
%	Hence, by Theorem~\ref{thm:single_pf_rp} and due to the TRP and PI of $\alg_2$, we conclude that truthful registration is a dominant strategy for any agent $i$, and it completes the proof.
%\end{proof}
%Note, however, that
%The main takeaway of Theorem~\ref{thm:multi_rp_uniform} is that the use of hierarchical structure effectively decouples the agent-wise exploration.
Note, however, that if we deploy uniform random selection algorithm in $\alg_1$, it essentially suffers \emph{linear regret} since it always choose any suboptimal agent with constant probability at every rounds.



To capture the both rabbits of sublinear regret and replication-proofness, we need more carefully tailored algorithm with sublinear regret in the first phase.
To this end, we present $\hbb$ presented in Algorithm~\ref{alg:hbb}, which adopts ETC in both phases along with additional device of \emph{restarting round}.
Similar to H-UCB, this consists of two phases each running ETC agent-wise and arm-wise manner, respectively.
To analyze the replication-proofness, we pose a minor assumption on the arms.
We say that the set of arms belong to \emph{stochastically ordered family} if two arms $a$ and $b$ satisfy $\mu_a \ge \mu_b$, then the reward distribution of arm $a$ is (first-order) stochastic dominant over that of $b$, \ie $\Pr{r_a \ge x} \ge \Pr{r_b \ge x}$ for any $x\ge 0$, where $r_i$ denotes arm $i$'s reward random variable.\footnote{Note that Bernoulli arms and Gaussian arms parameterized by mean rewards, belongs to this family. We also refer to~\cite{yu2009stochastic} for more examples in exponential family.}
Further, define $L = \max_{i \in [n]}l_i$.
Then, our main result can be presented as follows.
\begin{theorem}\label{thm:spf_rp}
	Consider a stochastically ordered family of arms, and discrete support of prior distributions.
	Consider $\hbb$ with $M \ge mL$ and $m = \frac{2}{\Delta^2} L\ln (2T)$, and $\tau = Mn$
	Then, $\hbb$ is replication-proof under any number of agents.\footnote{Similar to what we discussed in Theorem~\ref{thm:single-refine1}, we can refine this results and make the algorithm truly prior-independent, at the cost of some other assumptions. We omit these details as it goes beyond our main interest/takeaway.}
\end{theorem}
We provide a brief proof sketch.
\sscomment{revise sketches}
The proof mainly relies on the single-agent result in Theorem~\ref{thm:single_pf_rp} along with a number of algebraic manipulations which heavily relies on the nature of ETC and the restarting round.
Let us focus on agent $i$.
We can decompose agent $i$'s total expected utility to be (i) exploitation phase utility and (ii) exploration phase utility.
In terms of the infinite reward tapes, remark that the utility from (i) and (ii) is independent due to the nature of ETC.
Since (i) simply reduces to running single-agent ETC for each agent, we can compare (i) of two strategies using the single-agent result, thus truthful strategy is at least better for (i).

For (ii), if agent $i$ is not selected in the exploitation phase, it is simply zero, so we can only focus on the case when agent $i$ is selected in the exploitation phase.
Thus, its expected utility from (ii) can be written as multiplication of (a) probability that agent $i$ has the largest empirical average reward and (b) the expected utility by being pulled over the exploitation rounds.
For (b), since our choice of $\tau$ \emph{restarts} Phase 2 for any agent exactly at the beginning of exploitation phase of Phase 1, the expected utility therein simply reduces to the expected utility of single-agent setting with agent $i$ given the time horizon $T-Mn$.
Thus, again by our single-agent result of Theorem~\ref{thm:single_pf_rp}, the truthful strategy yields larger (or equal) quantity for (b) as well.
Finally, by carefully using a series of concentration inequalities, we bound the difference from (a) between the truthful strategy and any other strategy is relatively smaller and by doing so, loss from (a) cannot make up the gains from (b) and (i), which eventually implies the dominance of truthful strategy.

% To accommodate the case under which the algorithm does not know $l_i$ for $i \in [n]$, one can effectively replace each $l_i$ with some superconstant function on $T$, \eg $\log T$, and run the same algorithm.
% This will eventually incur the same regret bound (up to polylogarithmic factor) assuming that $l(i) = O(1)$ for $i \in [n]$.
% The detailed analysis of this technique have been presented in \cite{shin2022multi}.


We finalize our results by presenting regret upper bound of the $\hbb$ with ETC and ETC,  which concludes that it achieves sublinear regret as well as replication-proofness.
\begin{theorem}\label{thm:regret}
	Set $\alg_1$ be ETC with $M = \max(mL, \sqrt{T\ln T})$, and $\alg_2$ be ETC with $m =\nicefrac{2}{\Delta^2}\cdot L\ln(2T)$.
	Then, $\hbb$ has expected regret of $O(\frac{nL^3\sqrt{T \ln T}}{\Delta^3})$.
\end{theorem}
The regret analysis is based on a construction of clean event on each agent under which the agent's empirical average reward becomes close enough to his own optimal arm's mean reward.
The deviation probability of this clean event can be obtained using tail bounds along with the regret analysis of ETC, which essentially implies the necessity of having $\alg_1$'s exploration length polynomial.
The regret bound then easily follows from obtaining the probability that all the clean event holds.
The full proof for the regret analysis is deferred to Appendix~\ref{apd:thm:regret}.

\sscomment{discussion 1: obtaining instance-independent regret bound}

\sscomment{discussion 2: comparing the regret bound to Shin et al.}

Finally, we remark that the algorithm's dependency on the problem parameters can be weakened analogous to Theorem~\ref{thm:single-refine1}, but we omit the details as it goes beyond our interest.

\subsection{Proof of Theorem~\ref{thm:spf_rp}}
\begin{proof}
	\sscomment{proofread again, and structurize}
	First, note that our $\hbb$ is well-defined since our choice of $M$ and $m$ ensures that the exploitation phase of the first phase starts after the exploitation of the second phase ends.
	For simplicity, denote the first phase ETC by $\alg_1$ and the second phase ETC by $\alg_2$.
	Pick an agent $i$ with arms $\{o_{i,1}, \ldots, o_{i,l}\}$, let $\cS_i$ be agent $i$'s arbitrary strategy which replicates arm $o_{i,j}$ of $r_{i,j} \in \N_0$ times for each $j \in [l_i]$.
	Let $r_i = (r_{i,1},\ldots, r_{i,l_i})$, and denote by $v_i = (v_{i,1}, \ldots, v_{i,l_i})$ the realization of agent $i$'s original arms' mean rewards.
	Fix strategies of all the other agents $j \neq i$ by $\cS_{-i}$, and fix a realization $v_{-i}$ of all the other agents' arms' mean rewards.
	Henceforth, we will omit $\cS_{-i}$ and $v_{-i}$ from the arguments in the notations presented hereafter, unless confusion arises.
	In addition, we assume that all the prior distributions do not have point mass for simplicity, but it can easily be generalized as discussed in the proof of Theorem~\ref{thm:single_pf_rp}.
	
	Let $i^*$ denote the agent selected at the exploitation phase of $\alg_1$, and $l_i$ to denote agent $i$'s number of arms.
	We further write $\muhat_i(M)$ to denote the empirical average reward of agent $i$ when agent $i$ is selected $M$ times,
	and $\muhat_{i,a}(m)$ to denote the empirical average reward of agent $i$'s arm $a$ when it's selected $m$ times.
	Then, given $v_i$ and $r_i$, recall that the bandit instance agent $i$ submits can be presented as $\bigtimes_{i \in [l]}(v_a: r_a)$.
	
	Now, similar to the proof of Theorem~\ref{thm:single_pf_rp}, we first write agent $i$'s expected utility as follows.
	\begin{align}
		u_i(\cS_i)
		=
		\int_{\mu_{i,1} = v_{i,1}} \int_{\mu_{i,2} = v_{i,2} < v_{i,1}}\ldots \int_{\mu_{i,l_i} = v_{i,l_i}< v_{i,l_i-1}} 
		\sum_{\sigma \in \cP_{l_i}}\Ex{U_i(\cS_i)\ |\ \bigtimes_{a \in [l_i]}(v_{i,\sigma(a)}: r_{i,a})}g(v_i)dv_i.\label{eq:04262152}
	\end{align}
%	Now, we fix a realization of agent $i$'s arms' parameters to be $v = (v_1,v_2,\ldots, v_l)$, and focus on the integrand.
%	Since we fix the realization of the parameters, we simply write $\sigma(v)$ to denote the event $\{\mu_1 = \sigma(v)_1,\ldots, \mu_l = \sigma(v)_l\}$, \ie
%	\begin{align*}
%		\Ex{U_i(\cS)\ |\ \sigma(v)_1,\ldots, \sigma(v)_l}
%		=
%		\CEx{U(\cS)}{\sigma(v)},
%	\end{align*}
%	unless confusion arises.
	
	We first characterize the expected utility of agent $i$ based on its utility under the single agent setting with agent $i$.
	To this end, we introduce several notations.
	Write $\Gamma_i^{\cS_i}(t, \sigma(v_i))$ to denote agent $i$'s utility when he is selected $t$ times under the single agent setting in $\alg_2$ when its arms' mean rewards are realized to be $\sigma(v_i)$, and he plays strategy $\cS_i$ with replication vector $r_i$.
	Given $M$, $m$, and $\cS_i$, define an event
	\[
	C^{\cS_i}_i(y,\sigma(v)) = \{\max_{\cN \ni j\neq i}\parans{\muhat_j(M) }= y \ | \ \bigtimes_{a \in [l_i]}(v_{i, \sigma(a)}:r_{i,a})\},
	\]
	\ie the event that agents other than $i$ have maximal agent-wise empirical average reward $y$ at the end of the exploration phase in $\alg_1$.
	Again given $M$, $m$, and $\cS_i$, we further define following two quantities:
	\begin{align*}
		p^{\cS_i}_i(y, \sigma(v_i)) &= \CPr{C_i(y)}{\bigtimes_{a \in [l_i]}(v_{i, \sigma(a)}:r_{i,a})}
		\\
		q^{\cS_i}_i(y,\sigma(v_i)) &= \CPr{\muhat_i(M) \ge y}{\bigtimes_{a \in [l_i]}(v_{i, \sigma(a)}:r_{i,a})}.
	\end{align*}
	Remark that all the quantities above are conditioned on the event that $v_{-i}$ is realized and the other agents are playing $\cS_{-i}$.

	The following claim essentially characterizes the expected utility of agent $i$ under strategy $\cS$.
	\begin{claim}
		Agent $i$'s expected utility can be written as follows.
		\begin{align}
			\CEx{U_i(\cS_i)}{\bigtimes_{a \in [l_i]}(v_{i, \sigma(a)}:r_{i,a}}
			&=
			\Ex{\Gamma_i^{\cS_i}(M,\sigma(v_i))}  \nonumber
			\\
			&~~~+ \Ex{\Gamma_i^{\cS_i}(T-Mn,\sigma(v_i))} \int_0^1p_i^{\cS_i}(y,\sigma(v_i))q_i^{\cS_i}(y,\sigma(v_i))dy.\label{eq:04271231}	
		\end{align}
	\end{claim}
	\begin{proof}[Proof of the claim]
		Since $\hbb$ is running with the first phase being ETC, the expected utility of agent $i$ can be decomposed as (i) expected utility in the exploration phase and (ii) expected utility in the exploitation phase.
		Note that (i) essentially coincides with the expectation of $\Gamma_i^{\cS_i}(M, \sigma(v_i))$ since it chooses agent $i$ exactly $M$ times regardless of the random rewards.
		Moreover, due to our restarting at time $\tau = Mn$, when the exploitation phase of $\alg_1$ starts, all the parameters of $\alg_2$ is initialized.
		Thus, conditioned on the event that agent $i$ has the largest empirical average reward at round $\tau = Mn$, its expected utility in the exploitation phase again coincides with the single agent case expected utility $\Gamma_i^{\cS_i}(T-Mn, \sigma(v_i))$.
		Otherwise, if agent $i$ has not been selected as the empirically best agent, then its conditional expected utility is simply zero.
		Note that the probability of agent $i$ being the empirically best agent can be written as follows,\footnote{To be precise, we need to take account for the tie-breaking rule and the event that tie happens, but we omit the detail as it can be easily handled and is beyond of our interest.}
		\begin{align*}
			\Pr{\text{agent $i$ is the empirically best agent at round $\tau = Mn$}}
			&=
			\int_{0}^1 \Pr{\muhat_i(M) \ge y}\Pr{C_i(y)}
			\\
			&=
			\int_0^1p_i^{\cS_i}(y,\sigma(v_i))q_i^{\cS_i}(y,\sigma(v_i))dy,
		\end{align*}
		and we finish the proof of the claim.
	\end{proof}
	Using the claim above, for any strategy $\cS_i$, we can further expand its conditional expected utility $\sum_{\sigma \in \cP_{l_i}} \CEx{u_i(\cS_i)}{\bigtimes_{a \in [l_i]}(v_{i, \sigma(a)}:r_{i,a})}$ as follows.
	\begin{align}
		\sum_{\sigma \in \cP_{l_i}}
		& 
		\CEx{U_i(\cS_i)}{\bigtimes_{a \in [l_i]}(v_{i, \sigma(a)}:r_{i,a})}\nonumber
		\\
		&=
		\sum_{\sigma \in \cP_{l_i}}
		\parans{
		\Ex{\Gamma_i^{\cS_i}(M,\sigma(v_i))} + \Ex{\Gamma_i^{\cS_i}(T-Mn,\sigma(v_i))} \int_0^1p_i^{\cS_i}(y,\sigma(v))q_i^{\cS_i}(y,\sigma(v_i))dy
		}
		\nonumber
		\\
		&=
		\parans{
		\sum_{\sigma \in \cP_{l_i}}
		\Ex{\Gamma_i^{\cS}(M,\sigma(v_i))}
		}
		+
		\sum_{\sigma \in \cP_{l_i}}
		\parans{
		\Ex{\Gamma_i^{\cS_i}(T-Mn,\sigma(v_i))}
		\int_{0}^1p_i^{\cS_i}(y,\sigma(v_i))q_i^{\cS_i}(y,\sigma(v_i))dy
		}
		\nonumber
		\\
		&=
		\parans{
		\sum_{\sigma \in \cP_{l_i}}
		\Ex{\Gamma_i^{\cS_i}(M,\sigma(v_i))}
		}
		+
		\int_{0}^1
		\parans{\sum_{\sigma \in \cP_{l_i}}
		\Ex{\Gamma_i^{\cS_i}(T-Mn,\sigma(v_i))}
		p_i^{\cS_i}(y,\sigma(v_i))q_i^{\cS_i}(y,\sigma(v_i))}dy
		\nonumber
		\\
		&=
		\parans{
		\sum_{\sigma \in \cP_{l_i}}
		\Ex{\Gamma_i^{\cS_i}(M,\sigma(v_i))}
		}
		+
		\int_{0}^1
		p_i^{\cS_i}(y,\sigma(v_i))
		\parans{
		\sum_{\sigma \in \cP_{l_i}}
		\Ex{\Gamma_i^{\cS_i}(T-Mn,\sigma(v_i))}
		q_i^{\cS_i}(y,\sigma(v_i))
		}dy,\label{eq:04271244}
	\end{align}
	where the third equality follows from Fubini's theorem, and the last inequality holds since $p_i^{\cS_i}(y,\sigma(v_i))$ is independent from $\sigma$.
	
	In case of the truthful strategy $\cO_i$, since any permutation $\sigma$ yields the same problem instance, all the terms inside \eqref{eq:04271244} remains the same.
	Thus,
	\begin{align}
		\sum_{\sigma \in \cP_{l_i}} &
		\CEx{U_i(\cO_i)}{\bigtimes_{a \in [l_i]}(v_{i, \sigma(a)}:r_{i,a})}\nonumber
		\\
		&~~~~~~=
		|\cP_{l_i}| 
		\parans{
		\Ex{\Gamma_i^{\cO_i}(M,
		v_i)}
		+
		\Ex{\Gamma_i^{\cO_i}(T-Mn,v_i)}
		\int_{0}^1p_i^{\cO_i}(y,v_i)q_i^{\cO_i}(y,v_i)dy
		}.\label{eq:05082325}
	\end{align}
	Now it suffices to prove that the RHS of \eqref{eq:05082325} is at least that of \eqref{eq:04271244}.
	
	We first observe that the first term can effectively compared based on our result on the single-agent setting.
	\begin{claim}\label{cl:reduc_to_single}
		For any strategy $\cS_i$, we have
		\begin{align*}
			\sum_{\sigma \in \cP_{l_i}}\Ex{\Gamma_i^{\cO_i}(M, \sigma(v_i))}	
			\ge
			\sum_{\sigma \in \cP_{l_i}}\Ex{\Gamma_i^{\cS_i}(M, \sigma(v_i))}.
		\end{align*}
	\end{claim}
	\begin{proof}
		Note that $\Gamma_i^{\cO_i}(M, \sigma(v_i))$ denotes the agent $i$'s utility at round $M$ under the single agent setting.
		Thus, the claim directly follows from Theorem~\ref{thm:single_rp} since we run ETC with $m = 2l/\Delta^2 \ln (2T)$ as Phase 2 algorithm.
	\end{proof}
	Thus, it remains to compare the latter term that involves the integral.
	Given $v_i \in \R_{\ge 0}^{l_i}$, for $a \in [l_i]$, write $Y_{i,a}$ to denote the event that the arm with mean $v_a$ of agent $i$ is selected in the exploitation rounds of $\alg_2$ for agent $i$, \ie having the largest empirical average reward at the end of the exploration rounds in $\alg_2$ for agent $i$.
%	Let $Z_{i,a}$ denote the event that arm with mean $v_a$ in agent $i$ has the largest empirical average reward at the end of the exploration rounds in $\alg_2$.
	
	\sscomment{Proofread}
	Further, similar to the definition of $\Gamma_i^{\cS_i}(\cdot, \cdot)$, we analogously define $\Gamma_{i,a}^{\cS_i}(\cdot, \cdot)$ to be the random cumulative rewards when there exists only agent $i$ and only arm $a$ under $\alg_2$.
	That is, $\Gamma_{i,a}^{\cS_i}(t, \sigma(v_i))$ is just a summation of $t$ random variables where each random variable follows the agent $i$'s arm's reward distribution parameterized by the mean reward $\sigma(v_i)$.
	Note that our construction in equation~\eqref{eq:04262152} verifies $v_{i,1} \ge v_{i,2} \ge \ldots \ge v_{i,l_i}$.
	Define $\delta_{i,a} = v_{i,1} - v_{i,a}$ for $a \in [l_i]$.
	
	We now construct a lower bound of $q_i^{\cO_i}(y,v_i)$ in the following. \sscomment{$o_i$ and $o$ are both used. Also, make consistent $\sigma(v)$ or $v$.}
	\begin{claim}\label{cl:tail_lower}
		For any $y \in [0,1]$, and $\sigma \in \cP_{l_i}$, consider arbitrary $v_i \in [0,1]^{l_i}$ such that $v_{i,1} \ge v_{i,2} \ge \ldots \ge v_{i,l_i}$.
		 Then, we have
		\begin{align*}
			q_i^{\cO_i}(y, v_i)
			\ge
			\Pr{\Gamma_{i,1}^{\cO_i}(M,v_i) \ge My} \parans{1 - 2\sum_{a=2}^{l_i} \exp(-\frac{\delta_{i,a}^2 m }{2})}
		\end{align*}

	\end{claim}
	\begin{proof}[Proof of the claim]
		Due to the independence of rewards from arm $a$ at exploitation phase and the random variable $\Ind{Y_{i,a}}$, we can rewrite $q_i^{\cO}(y,\sigma(v))$ as follows.
		\sscomment{FIXING...}
		\begin{align}
%			q_i^{\cO}(y,\sigma(v))
%			=
			q_i^{\cO_i}(y,v_i)
			&=
			\Pr{
			\sum_{a=1}^{l_i}
			\parans{
			\Gamma_{i,a}^{\cO_i}(m,v)
			+
			\Ind{Y_{i,a}}\Gamma_{i,a}^{\cO_i}(M-l_im, v_i)
			}
			\ge My
			}
			\nonumber
			\\
			&=
			\sum_{a=1}^{l_i}
			\CPr{
			\sum_{a=1}^{l_i} 
			\parans{
			\Gamma_{i,a}^\cO(m,v)
			+
			\Ind{Y_{i,a}}\Gamma_{i,a}^{\cO}(M-l_im, v)
			}
			\ge My
			}{Y_{i,a}}\Pr{Y_{i,a}}
			\nonumber
			\\
			&=
			\sum_{a=1}^{l_i}
			\CPr{
			\parans{
			\sum_{a=1}^{l_i} 
			\Gamma_{i,a}^\cO(m,v)
			}
			+
			\Gamma_{i,a}^{\cO}(M-l_im, v)
			\ge My
			}{Y_{i,a}}\Pr{Y_{i,a}}
			\nonumber
			\\
			&\ge
			\CPr{
			\parans{
			\sum_{a=1}^{l_i} 
			\Gamma_{i,1}^\cO(m,v)
			}
			+
			\Gamma_{i,1}^{\cO}(M-l_im, v)
			\ge My
			}{Y_{i,1}}\Pr{Y_{i,1}}
%			\nonumber
%			\\
%			&=
%			\sum_{a=1}^{l_i}
%			\CPr{
%			\Gamma_{i,a}^\cO(M,v) \ge l_iMy
%			}{Z_{i,a}}\Pr{Z_{i,a}}
%			\tag{Definition of $\Gamma_{i,a}^{\cO}$}
%			\\
%			&=
%			\sum_{a=1}^{l_i}
%			\Pr{
%			\Gamma_{i,a}^\cO(M,v) \ge l_iMy
%			}\Pr{Z_{i,a}}
%			\tag{Independence of $\Gamma_{i,a}^{\cO}$ and $Z_{i,a}$}
%			\\
%			&\ge
%			\Pr{\Gamma_{i,1}^\cO(M,v) \ge l_iMy}\Pr{Z_{i,a}},
%			\label{ineq:05090246}
			\nonumber
		\end{align}
		
		Note further that due to the positive correlation between the event $Y_{i,1}$ and the tail event, it follows that
		\begin{align*}
			\CPr{
			\parans{
			\sum_{a=1}^{l_i} 
			\Gamma_{i,1}^{\cO_i}(m,v)
			}
			+
			\Gamma_{i,1}^{\cO_i}(M-l_im, v)
			\ge My
			}{Y_{i,1}}
			\ge
			\Pr{
			\parans{
			\sum_{a=1}^{l_i} 
			\Gamma_{i,1}^{\cO_i}(m,v)
			}
			+
			\Gamma_{i,1}^{\cO_i}(M-l_im, v)
			\ge My
			}.
		\end{align*}
		
		Let us write
		\begin{align*}
			\psi_i(M, y, v) 
			= \Pr{
			\parans{
			\sum_{a=1}^{l_i} 
			\Gamma_{i,1}^{\cO_i}(m,v)
			}
			+
			\Gamma_{i,1}^{\cO_i}(M-l_im, v)
			\ge My
			},
		\end{align*}
		then we have
		\begin{align}
			q_i^{\cO_i}(y,v_i) \ge \psi_i(M, y,v)\Pr{Y_{i,1}}
			\label{ineq:05090246}
		\end{align}
		
		Since $Z_{i,1}$ is the complement of $\cup_{a=2}^l Z_{i,a}$, observe that
		\begin{align*}
			\Pr{Z_{i,1}^c}
			&=
			\Pr{\cup_{a=2}^l Z_{i,a}}
			\\
			&\le
			\sum_{a=2}^l\Pr{Z_{i,a}}
			\tag{Union bound}
			\\
			&\le
			\sum_{a=2}^l\Pr{\muhat_{i,1}(m) \le \muhat_{1,a}(m)}
			\tag{Definition of $Z_{i,a}$}
			\\
			&\le
			\sum_{a=2}^l 2\exp(-\frac{\delta_{i,a}^2 m}{2}).
			\tag{Claim~\ref{cl:concen}}
		\end{align*}
		
		Hence, we obtain
		\begin{align*}
			q_i^{\cO}(y,\sigma(v))
			\ge
			\psi_i(M, y, v)  \parans{1 - 2\sum_{a=2}^l \exp(-\frac{\delta_{i,a}^2 m }{2})},
		\end{align*}
		and it proves the claim.
	\end{proof}
	
%	\begin{lemma}
%		Let $X_1,X_2,\ldots, X_n$ be random variables supported on $ S\subset\R_{\ge 0}$ such that $X_i$ stochastically dominates $X_j$ for $i,j \in [n]$ such that $i \le j$.
%		Then, the following holds for any $x \in \R_{\ge 0}$ and $i < j$:
%		\begin{align*}
%			\Pr{\sum_{k \in [n]}X_k \ge x, X_i = \max_{k \in [n]}X_k} \ge \Pr{\sum_{k \in [n]}X_k \ge x, X_j = \max_{k \in [n]}X_k}.
%		\end{align*}
%	\end{lemma}
%	\begin{proof}[Proof of the lemma]
%		Let the random variables be discrete random variables with finite support for simplicity. Note that the arguments easily extend to the continuous case.
%		Write $S = \{s_1,s_2,\ldots, s_m\}$ and $X_{-i,-j}$ to denote the vector of random variables $X_k$ or $k \in [n]$ such that $k \neq i,j$, \ie
%		\begin{align*}
%			X_{-i,-j} = (X_1,\ldots, X_{i-1},X_{i+1}, \ldots, X_{j-1},X_{j+1}, \ldots, X_n).
%		\end{align*}
%		Note that LHS can be decomposed as follows.
%		\begin{align}
%			\Pr{\sum_{k \in [n]}X_k \ge x, X_i = \max_{k \in [n]}X_k}
%			&= \sum_{z \in S^{n-2}}\Pr{\sum_{k \in [n]}X_k \ge x, X_i = \max_{k \in [n]}X_k, X_{-i,-j} = z}.\label{eq:12231632}
%		\end{align}
%		Fix any realization $z \in S^{n-2}$ of $X_{-i,-j}$, and we can rewrite each term in RHS as follows.
%		\begin{align*}
%			\Pr{\sum_{k \in [n]}X_k \ge x, X_i = \max_{k \in [n]}X_k, X_{-i,-j} = z}
%			&= \Pr{X_i + X_j \ge x - \abs{z}_1, X_i \ge \max(\abs{z}_{\infty}, X_j)}\Pr{X_{-i,-j} = z},
%		\end{align*}
%		where $\abs{\cdot}_1$ and $\abs{\cdot}_\infty$ denote $\ell_1$ and $\ell_{\infty}$ norm respectively.
%		We can further expand
%		\begin{align*}
%			\Pr{X_i + X_j \ge x - \abs{z}_1, X_i \ge \max(\abs{z}_{\infty}, X_j)} = \sum_{k \in [m]}\Pr{ X_i \ge \max(x - \abs{z}_1 - s_k,\abs{z}_{\infty}, s_k)}\Pr{X_j = s_k}.
%		\end{align*}
%		Given $z$, define $f_k = \max(x-\abs{z}_1 - s_k, \abs{z}_\infty, s_k)$, then RHS can be written as
%		\begin{align*}
%			\sum_{k \in [m]}\Pr{X_i \ge f_k}\Pr{X_j = s_k}.	
%		\end{align*}
%		Note that $f_k$ is monotone increasing over $k$.
%		By Abel's transformation
%		\begin{align*}
%			\sum_{k \in [m]}\Pr{X_i \ge f_k}\Pr{X_j = s_k}
%			&= \Pr{X_i = f_m} - \sum_{k=1}^{m-1}\Pr{X_j \le s_k}\Pr{X_i = f_{k+1}} \\
%			&\ge \Pr{X_i = f_m} - \sum_{k=1}^{m-1}\Pr{X_i \le s_k}\Pr{X_i = f_{k+1}} \\
%			&= \sum_{k \in [m]}\Pr{X_i \ge f_k}\Pr{X_i = s_k} \\
%			&\ge \sum_{k \in [m]}\Pr{X_j \ge f_k}\Pr{X_i = s_k}.
%		\end{align*}
%		Hence we obtain
%		\begin{align*}
%			\Pr{\sum_{k \in [n]}X_k \ge x, X_i = \max_{k \in [n]}X_k, X_{-i,-j} = z}
%			&= \sum_{k \in [m]}\Pr{X_i \ge f_k}\Pr{X_j = s_k} \\
%			&\ge \sum_{k \in [m]}\Pr{X_j \ge f_k}\Pr{X_i = s_k} \\
%			&= \Pr{\sum_{k \in [n]}X_k \ge x, X_j = \max_{k \in [n]}X_k, X_{-i,-j} = z}.
%		\end{align*}
%		Plugging into~\eqref{eq:12231632} we finish the proof.
%	\end{proof}
%	\begin{lemma}
%		Let $X_1,X_2,\ldots, X_n$ be random variables supported on $ S\subset\R_{\ge 0}$ such that $X_i$ stochastically dominates $X_j$ for $i,j \in [n]$ such that $i \le j$.
%		Then, the following holds for any $x \in \R_{\ge 0}$:
%		\begin{align*}
%			\CPr{\sum_{k \in [n]}X_k \ge x}{X_1 = \max_{k \in [n]}X_k} \ge \Pr{\sum_{k \in [n]}X_k \ge x}
%		\end{align*}
%	\end{lemma}
%	\begin{proof}
%		Note that
%		\begin{align*}
%			\Pr{\sum_{k \in [n]}X_k \ge x} 
%			&= \sum_{i \in [n]}\Pr{\sum_{k \in [n]}X_k \ge x, X_i = \max_{k \in [n]}X_k} \\
%			&\le n\cdot\Pr{\sum_{k \in [n]}X_k \ge x, X_1 = \max_{k \in [n]}X_k}
%		\end{align*}
%	
%	\end{proof}
%
%
%	
%	To lower bound the difference between $q_i^\cO(y,\sigma(v))$ and $q_i^\cS(y,\sigma(v))$, we use the following rough upper bound for $q_i^\cS(y,\sigma(v))$.
%	\begin{claim}\label{cl:tail_upper}[New Claim]
%		For any strategy $\cS_i$, $\sigma \in S_{l_i}$, $y \in [0,1]$ and $v \in [0,1]^{l_i}$, we have 
%		\begin{align*}
%			q_i^{\cS_i}(y, \sigma(v))	 
%			\le 
%			\CPr{asd \ge y}{Y_{i,1}}\Pr{Y_{i,1}} + 1-\Pr{Y_{i,1}}.
%		\end{align*}
%	\end{claim}
	\begin{claim}\label{cl:tail_upper}
		For any strategy $\cS_i$, $\sigma \in S_{l_i}$, $y \in [0,1]$ and $v \in [0,1]^{l_i}$, we have 
		\begin{align*}
			q_i^{\cS_i}(y, \sigma(v))	 
			\le 
			\psi_i(M, y, v)
%			\Pr{\Gamma_{i,1}^{\cS}(M,\sigma(v)) \ge y}
%			=
%			\Pr{\Gamma_{i,1}^{\cO}(M,\sigma(v)) \ge y}
		\end{align*}
	\end{claim}
	\begin{proof}[Proof of the claim]
		This easily follows from the fact that in the probability $\psi(M,y,v)$, the exploration phase runs with the original $l_i$ arms for $m$ times each and then the exploration phase runs with the optimal arm $(i,1)$, whereas in the probability $q_i^{\cS_i}(y, \sigma(v))$, the exploration runs with the original $l_i$ arms upon the replicated arm for $m$ times each, and then exploitation runs with the empirically best arm.
		That is, we can couple the first $l_i \cdot m$ rounds for the exploration phase of the original $l_i$ arms, and then the exploitation is dominant for $\psi(M,y,v)$ due to the stochastic dominance of the arm $(i,1)$ over the other arms.
		
%		We can expand
%		\begin{align*}
%			q_i^{\cS}(y,\sigma(v))
%			&=
%			\Pr{
%			\sum_{a=1}^{l_i}
%			\parans{
%			\Gamma_{i,a}^\cS(m,\sigma(v))
%			+
%			\Ind{Y_{i,a}}\Gamma_{i,a}^{\cS}(M-lm, \sigma(v))
%			}
%			\ge y
%			}
%			\\
%			&=
%			\sum_{a=1}^{l_i}
%			\CPr{
%			\Gamma_{i,a}^\cS(M,\sigma(v)) \ge y
%			}{Z_{i,a}}\Pr{Z_{i,a}}
%			\\
%			&=
%			\sum_{a=1}^{l_i}
%			\Pr{
%			\Gamma_{i,a}^\cS(M,\sigma(v)) \ge y
%			}\Pr{Z_{i,a}}.
%		\end{align*}
%		Note further that $\Pr{\Gamma_{i,a}^\cS(M,\sigma(v)) \ge y} \le \Pr{\Gamma_{i,1}^\cS(M,\sigma(v)) \ge y}$ due to the stochastic dominance of the arm with mean $v_1$ over the arm with mean $v_a$, for any $a \in [l_i]$.
%		Thus, we have
%		\begin{align*}
%			q_i^{\cS}(y,\sigma(v))
%			&\le
%			\sum_{a=1}^{l_i}
%			\Pr{
%			\Gamma_{i,1}^\cS(M,\sigma(v)) \ge y
%			}\Pr{Z_{i,a}}
%			\\
%			&=
%			\Pr{\Gamma_{i,1}^\cS(M,\sigma(v)) \ge y}.
%		\end{align*}
%		In addition, observe that 
%		\begin{align*}
%			\Pr{\Gamma_{i,1}^{\cS}(y,\sigma(v)) \ge y}
%			=
%			\Pr{\Gamma_{i,1}^{\cO}(y,\sigma(v)) \ge y}	
%		\end{align*}
%		follows from the fact that $\Gamma_{i,1}^{\cS}(y,\sigma(v)) = \Gamma_{i,1}^{\cO}(y,\sigma(v))$ since both are random rewards when there is only arm with mean rewards $v_1$ of agent $i$.
	\end{proof}

	Now, combining Claim~\ref{cl:tail_lower} and~\ref{cl:tail_upper}, we obtain
	\begin{align}
		q_i^{\cO}(y, \sigma(v)) - q_i^{\cS}(y,\sigma(v))
		&\ge
		-2
		\psi_i(M, y, v)
%		\Pr{\Gamma_{i,1}^\cO(M,\sigma(v)) \ge y}
		\parans{\sum_{a=2}^{l_i} \exp(-\frac{\delta_{i,a}^2 m }{2})}
		\nonumber
		\\
		&\ge
		-2l_i 
		\psi_i(M, y, v)
%		\Pr{\Gamma_{i,1}^\cO(M,\sigma(v)) \ge y}
		\parans{\exp(-\frac{\Delta^2 m }{2})}
		\tag{Due to $\delta_{i,a} \ge \Delta$}
		\\
		&\ge
		-2l_i \cdot \frac{q_i^{\cO}(y, v)}{\Pr{Y_{i,1}}} \cdot
		\parans{\exp(-\frac{\Delta^2 m }{2})}\tag{Due to ineq. \eqref{ineq:05090246}}
		\\
		&\ge
		-2l_i \cdot \frac{q_i^{\cO}(y, v)}{1 - \sum_{a=2}^{l_i} 2\exp(-\frac{\delta_i^2 m}{2})} \cdot
		\parans{\exp(-\frac{\Delta^2 m }{2})}
		\nonumber
		\\
		&\ge
		-2l_i
		\cdot 
		\frac{q_i^{\cO}(y, v)}{1 - 2l_i\exp(-\frac{\Delta^2 m}{2})} \cdot
		\parans{\exp(-\frac{\Delta^2 m }{2})},
		\label{ineq:05090213}
	\end{align}
	where the fourth inequality follows from the concentration on $Z_{i,1}$ in the proof of Claim~\ref{cl:tail_lower}.

	Now we consider two cases regarding $\sigma$: (i) when $\sigma(1) = 1$ and (ii) otherwise.
	
%	\paragraph{case (i): $\sigma(1) = 1$}
%	This means that there exists a suboptimal arm with at least one replication.
%	In this case, as per the proof of 
%	
%	\paragraph{case (ii): $\sigma(1) \neq 1$}
	
	Recall that it suffices to prove that the RHS of \eqref{eq:05082325} is at least that of \eqref{eq:04271244}.
	Due to Claim~\ref{cl:reduc_to_single}, it suffices to prove the following inequality.
	\begin{align}
		\int_{0}^1
		&p_i^{\cS}(y,\sigma(v))
		\parans{
		\sum_{\sigma \in S_l}\underbrace{\paranm{\Ex{\Gamma_i^{\cO}(T-Mn,\sigma(v))}
		q_i^{\cO}(y,\sigma(v))
		-
		\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		q_i^{\cS}(y,\sigma(v))}}_{\Theta(\sigma, v)}
		}dy 
		\ge 
		0.
		\label{eq:05090205}
	\end{align}
%	Now we prove the following positive correlation.
%	\begin{claim}
%		For any $\sigma_1,\sigma_2 \in S_l$, 
%		it satisfies $q_i^{\cS}(y,\sigma_1(v)) \ge 	q_i^{\cS}(y,\sigma_2(v))$ iff the following holds.
%		\begin{align*}
%			\Ex{\Gamma_i^{\cS}(T-Mn,\sigma_1(v))} \ge \Ex{\Gamma_i^{\cS}(T-Mn,\sigma_2(v))}	
%		\end{align*}
%	\end{claim}
%	\begin{proof}
%		\note{TBD - Intuitive}
%	\end{proof}
%	Thus, by Chebyshev's sum inequality, we have
%	
%
%
%
%	
%	=========2nd=========
	
	
	Note that the term inside the summation can be decomposed as follows.
	\begin{align*}
		\Theta(\sigma, v)
		=
		\paranm{\Ex{\Gamma_i^{\cO}(T-Mn,\sigma(v))} - \Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}}q_i^{\cO}(y,\sigma(v))
		\\
		+
		\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		\paranm{q_i^\cO(y,\sigma(v)) - q_i^{\cS}(y,\sigma(v))}.
	\end{align*}
	
	Due to \eqref{ineq:05090213}, we further obtain
	\begin{align*}
		\Theta(\sigma, v) 
		&\ge 
		\underbrace{\paranm{\Ex{\Gamma_i^{\cO}(T-Mn,\sigma(v))} - \Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}}q_i^{\cO}(y,\sigma(v))}_{\Theta_1(\sigma, v)}
		\\
		&-
		\underbrace{2\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		\cdot l_i\cdot \frac{q_i^{\cO}(y, v)}{1 - 2l_i\exp(-\frac{\Delta^2 m}{2})} \cdot
		\parans{\exp(-\frac{\Delta^2 m }{2})}}_{\Theta_{2}(\sigma, v)} 
		.
	\end{align*}
	By summing over $\sigma \in S_{l_i}$, for $\Theta_1(\sigma, v)$, we have
	\begin{align*}
		\sum_{\sigma \in S_l} \Theta_1(\sigma, v)	
		&=
		\sum_{\sigma \in S_l}\paranm{\Ex{\Gamma_i^{\cO}(T-Mn,\sigma(v))} - \Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}}q_i^{\cO}(y,\sigma(v))
		\\
		&=
		q_i^{\cO}(y,\sigma(v)) \cdot \sum_{\sigma \in S_{l_i}}\paranm{\Ex{\Gamma_i^{\cO}(T-Mn,\sigma(v))} - \Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}}
	\end{align*}
	
	From inequality~\eqref{ineq:05090221} and \eqref{ineq:05090222} we know that
	\begin{align*}
		\sum_{\sigma \in S_{l_i}}\paranm{\Ex{\Gamma_i^{\cO}(T-Mn,\sigma(v))} - \Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}}
		&\ge
		\sum_{a \in [l_i]} \delta_{i,a} (\frac{m}{l_i} - 1)
		\\
		&\ge
		\sum_{a \in [l_i]} \delta_{i,a} (\frac{2l_i \ln 2T / \Delta^2}{l_i} - 1)
		\\
		&= 
		\sum_{a \in [l_i]} \delta_{i,a} (\frac{\ln 2T}{\Delta^2} - 1),
	\end{align*}
	which implies
	\begin{align*}
		\sum_{\sigma \in S_l} \Theta_1(\sigma, v)
		&\ge
		q_i^{\cO}(y,\sigma(v)) 
		\cdot \sum_{i \in [l]} \delta_{i,a} (\frac{\ln 2T}{\Delta^2} - 1).
	\end{align*}
	
	Putting $m = 4 \cdot \frac{2}{\Delta^2} (\max_i l_i) \ln(2T)$, observe that the following holds.
	\begin{align*}
		\exp(-\frac{\Delta^2 m}{2}) \le \frac{1}{4l_iT}	
	\end{align*}

	Hence, for $\Theta_2(\sigma,v)$, we further obtain
	\begin{align*}
		\sum_{\sigma \in S_{l_i}}\Theta_2(\sigma,v)
		&=
		2\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		\cdot l_i\cdot \frac{q_i^{\cO}(y, v)}{1 - 2l_i\exp(-\frac{\Delta^2 m}{2})} \cdot
		\parans{\exp(-\frac{\Delta^2 m }{2})}
		\\
		&\le
		4\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		\cdot l_i\cdot q_i^\cO(y,v)\cdot \frac{1}{4l_iT}
		\\
		&=
		\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))}
		 q_i^\cO(y,v)\frac{1}{4T}
		\\
		&\le
		\frac{q_i^{\cO}(y,v)}{4}\tag{Since $\Ex{\Gamma_i^{\cS}(T-Mn,\sigma(v))} \le T$}
	\end{align*}
	
	Combining the above observations, for $\Theta(\sigma, v)$, we obtain
	\begin{align*}
		\sum_{\sigma \in S_{l_i}}\Theta(\sigma, v)
		&\ge
		q_i^{\cO}(y,v)
		\parans{
		\sum_{a \in [l_i]} \delta_{i,a} (\frac{\ln 2T}{\Delta^2} - 1)
		-
		\frac{1}{4}
		}
		\\
		&\ge
		q_i^{\cO}(y,v)
		\parans{
		\sum_{a \in [l_i]}  (\frac{\ln 2T}{\Delta} - 1)
		-
		\frac{1}{4}
		}
		\\
		&=
		q_i^{\cO}(y,v)\parans{l_i \cdot \ln(2T) - l_i -\frac{1}{4}} 
		\\
		&\ge 0,
	\end{align*}
	where the last inequality follows from $T \ge 1$ and $q_i^\cO(y,v) \ge 0$.
	Thus, inequality \eqref{eq:05090205} is true, and it finishes the proof.

	
%	===========	===========	===========	===========	===========	===========
%
%	
%	Let $\cS$ be agent $i$'s strategy with replication vector $r = (r_1,r_2,\ldots, r_l)$, with at least one coordinate being strictly positive.
%	Without loss of generality, suppose $r_1 \ge r_2 \ge \ldots \ge r_l$, then we have $r_1 \ge 1$.
%	This indeed brings no difference since the expected payoff is marginalized over all the possible permutations, as we see thus far.
%	Let $\Omega_1$ be a set of permutation $\sigma \in S_l$ such that arm $\sigma(1) = 1$, \ie the best arm is replicated the most times, and define $\Omega_2 = S_l \setminus \Omega_1$.
%	We handle case $\omega \in \Omega_1$ and $\omega \in \Omega_2$ separately.
	
	

%
%	
%	Since our $alg_2$ is stochastically schur-concave, if two strategies $\cS$ and $\cS'$ with replication vector $r$ and $r'$ satisfy $r' \succ r$, then we can obtain
%	\begin{align*}
%		\sum_{\sigma \in S_l}
%		q_i^{\cS}(y,\sigma(v))
%		\ge
%		\sum_{\sigma \in S_l}
%		q_i^{\cS'}(y,\sigma(v)).
%	\end{align*}
%	Furthermore, the following easily follows from the fact that $\alg_2$ is SPF.
%	\begin{claim}
%		Given that $\alg_2$ is SPF, for any $v$ and $t$, we have $\Ex{\Gamma_i^{\cS}(t,v)}\ge \Ex{\Gamma_i^{\cS'}(t,v)}$.
%	\end{claim}
%	\begin{proof}
%		It is easy to check that SPF implies EPF.
%		Then, the claim directly follows from the single-agent characterization in  Theorem~\ref{thm:single_pf_rp}.
%	\end{proof}
%	
%	Combining the above facts, we can obtain
%	\begin{align*}
%		\sum_{\sigma \in S_l} 
%		\CEx{U_i(\cS)}{\sigma, v}
%		\ge
%		\sum_{\sigma \in S_l} 
%		\CEx{U_i(\cS')}{\sigma, v}.
%	\end{align*}

%	Thus, putting back to \eqref{eq:04262152} completes the proof.	
\end{proof}





==> temp/icml-positive_lemma.tex <==
\section{Towards Replication-Proof Mechanism}
The following notation will play a crucial role in analyzing replication-proofness of an algorithm.
\begin{definition}[Permutation-free]
	Consider any single-agent bandit instance $\cI$ with mean rewards $\mu_1\ge \mu_2 \ge \ldots \ge \mu_k$.
	Let $\cI_i$ be a bandit instance in which arm $i$ is replicated once from $\cI$.
	We say that an algorithm is permutation-free if the following holds for any $T \ge 1$,
	\begin{align*}
		\reg_{\cI}(T) \le \frac{\sum_{i=1}^k\reg_{\cI_i}(T)}{k}.
	\end{align*}
\end{definition}

\begin{theorem}[Permutation-free yields replication-proof under a single agent]\label{thm:single_pf_rp}
	Under a single-agent setting, if an algorithm is permutation-free, then it is replication-proof.
\end{theorem}
\begin{proof}
	
	\begin{lemma}
		Consider a permutation-free algorithm $\alg$ under a single-agent instance $\cI$ with mean rewards $\mu_1 \ge \mu_2 \ge \ldots \ge \mu_k$.
		Let $R$ be a random variable that chooses $l$ indices from $[k]$ uniformly at random, allowing the repetition.
		Let $\cI'$ be any bandit instance in which the corresponding $l$ arms are selected according to the index sampled from $R$.
		Then, the following holds for any $T \ge 1$,
		\begin{align*}
			\reg_{\cI}(T) \le \reg_{\cI'}(T).
		\end{align*}
	\end{lemma}
	\begin{proof}[Proof of the lemma]
	\note{Suho - TBD}
	\end{proof}
	
	\begin{lemma}
		Given two strategies
		Let $R_{\alg}(i)$ be the agent-wise random variable of agent $i$ under $\alg$, and $R_{\alg'}(i)$ be that under $\alg'$.
		
	\end{lemma}
	\note{Suho - TBD}
\end{proof}



\begin{algorithm} 
\SetAlgoLined
%$i \in \set{N}$, $\set{S} = \cup_{i \in \set{N}} \set{S}_i$\\
Parameter $\alg_1$, $\alg_2$
;\\
Initialize $R(i), N(i), r(a)$ and $n(a)$ at zero  
for all $i \in \set{N}$ and $a\in \cup_{i \in \set{N}} \set{S}_i$;


 \For{$t=1,2,\ldots$}{
  \tcp{Phase 1 - agent selection}
  Run $\alg_1$ with agent-wise parameters $R(i)$, $N(i)$, and round index $t$;\\
  Let $\hat{i}$ be the selected agent;\\
  \tcp{Phase 2 - arm selection}
  Run $\alg_2$ within agent $\hat{i}$ with parameters $r(a)$, $n(a)$, and round index $N(i)$ for $a \in \set{S}_i$;\\
  Let $\hat{a}$ be the selected arm;\\
%  
%  If $N(i) \le 1/2T^{1/3} \log(T)^{1/3}$, round-robin exploration of arms in $\set{S}_i$;\\
%  Else, commit $\hat{a} = \argmax_{a \in \set{S}_{\hat{i}}} 
%    \left\{r(a) \right\}$
  Play $A_t = \hat{a}$ and receive reward $R_t$; \\
  Update statistics:
  $r(\hat{a}) \leftarrow \tfrac{r(\hat{a})n(\hat{a}) + R_t}{n(\hat{a})+1}; ~~
  R(\hat{i}) \leftarrow \tfrac{R(\hat{i})N(\hat{i}) + R_t}{N(\hat{i})+1};$
  
  $n(\hat{a}) \leftarrow n(\hat{a}) + 1; ~~ N(\hat{i}) \leftarrow N(\hat{i}) + 1;$
 }
 \caption{\hbb\label{alg:hbb}}
\end{algorithm}

A direct implication of Theorem~\ref{thm:single_pf_rp} is that H-BlackBox with a simple of $\alg_1$ and $\alg_2$ yields 
\begin{theorem}
	Let $\alg_1$ denote a uniform random selection algorithm.
	Then, for any permutation-free  $\alg_2$, $\hbb$ with $\alg_1$ and $\alg_2$ is replication-proof.
\end{theorem}
\begin{proof}
	\note{Suho - TBD - Easily follow, but make it formal}	
\end{proof}

Together with Theorem [That shows permutation-free example], the above theorem implies the existence of the replication-proof algorithm.
Note however that if we deploy uniform random selection algorithm in $\alg_1$, it essentially suffers linear regret since it always choose any suboptimal agent with constant probability at every rounds.
To capture the both rabbits of sublinear regret and replication-proofness, we need more carefully tailored algorithm with sublinear regret in $\alg_1$.

\begin{conjecture}[Hierarchical algorithm with permutation free submodule suffices]
	Given permutation-free algorithms $\alg_1$ and $\alg_2$, suppose that $\alg_1$ satisfies STH.
	Then,
	H-BlackBox $\alg_1$ and $\alg_2$ is replication-proof.
	\note{What should be STH? - Thompson sampling would be a natural choice, since each choice prob. is naturally proportional to the mean empirical reward of the agent.}
\end{conjecture}


==> temp/icml-single-agent.tex <==
\section{Warm-up: Single-agent Setting}\label{sec:single}
As noted thus far, UCB is not replication-proof even in the single agent setting.
Indeed, as per Theorem~\ref{thm:ucb_negative}, it is not obvious to verify which algorithm would satisfy replication-proofness even in the single-agent setting.
%Inferring from the worst-case problem instance we present in Theorem~\ref{thm:ucb_negative}, one can essentially observe that an algorithm should \emph{necessarily} be robust to partial replication.
%Indeed, it is not easy to verify which algorithms would satisfy replication-proofness even in the single agent setting.
In this section, we step towards in constructing replication-proof algorithm, by carefully investigating the single-agent setting first.
We present a set of conditions which is sufficient for an algorithm to be replication-proof in the single-agent setting, and then, as an example, will prove that exploration-then-commit (ETC) will satisfy these properties.
As we restrict our attention to single-agent setting in this section, we often omit the agent index $i$ in the notations.

To this end, we first introduce several notations.
For any natural number $l$, let $\cP_l$ be a set of all possible permutations $\sigma:[l] \mapsto [l]$.
Now we introduce a dictionary form of bandit instance $\cI$.
Given the realization of the arms' mean rewards, suppose that the set of mean rewards constitute a sorted sequence $\{1 \ge \mu_1 > \mu_2 > \ldots > \mu_l  > 0\}$, where some arms may share the same mean reward.
For each $\mu_a$ for $a \in [l]$, we count the number of arms which have mean reward $\mu_a$, and denote the count by $c_a$.
Then, our bandit instance $\cI$ can essentially presented as tuples of the mappings $\bigtimes_{a\in[l]}(\mu_a:c_a)$, which we say dictionary form of the bandit instance $\cI$.

Suppose that we have a standard multi-armed bandit instance $\cI$ with dictionary form $(\mu_a:c_a)_{a \in [l]}$.
Then, we define a \emph{permuted bandit instance} $\cI_\sigma$ to be a bandit instance with dictionary form of $\bigtimes_{a\in[l]}(\mu_a: c_{\sigma(a)})$, \ie arms with mean reward $\mu_i$ appears $c_{\sigma(a)}$ times.
For instance, given the original bandit instance $\cI = (0.5: 1, 0.7: 2)$, consider a permutation $\sigma$ such that $\sigma(1) = 2$ and $\sigma(2)=1$ correspondingly.
Then, one can easily verify that $\cI_\sigma = (0.5:2, 0.7:1)$.


Now, we introduce the following refinement of the standard regret.
\begin{definition}[Random permutation regret]
	Given a single-agent bandit instance $\cI$ with $l$ arms, we define an algorithm $\fA$'s \emph{random permutation regret} (RP-Regret) as follows.
	\begin{align}
		\rpreg(\fA, T) 
		&= 
		\Exu{\sigma \in \cP_l}{\reg_{I_{\sigma}}(\fA, T)}
		\nonumber
		\\
		&=
		\frac{1}{|\cP_l|} \cdot \parans{\sum_{\sigma \in \cP_l}\reg_{I_{\sigma}}(\fA, T)}.\label{eq:epf}
	\end{align}
\end{definition}
Given the random permutation regret, we define the following property of algorithm, which will play an essential role in obtaining truthful algorithm in the single-agent setting.
\begin{definition}[Truthful under random permutation]
	Given an arbitrary single-agent bandit instance $\cI$ with $l$ arms,
	consider a truthful strategy $\cO$ and arbitrary strategy $\cS$.
	We say that an algorithm $\fA$ is \emph{truthful under random permutation} (TRP) if
	\begin{align*}
		\rpreg(\fA,T;\cO) 
		\le 	
		\rpreg(\fA,T;\cS).
	\end{align*}
\end{definition}
Note that TRP requires the inequality to holds for arbitrary bandit instance $\cI$.
The foundation of these notions essentially builds upon the observation from our counterexample provided in Theorem~\ref{thm:ucb_negative}.
To elaborate more, 
consider a strategy $\cS$ that only replicates the first arm given a bandit instance $\mu_1\ge \mu_2 \ge \ldots \ge \mu_l$.
Then, we can observe that any permutation $\sigma \in \cP_l$ results in a bandit instance that belongs to the following family of bandit instances: define $\cI^* = \cup_{i \in [l]}\cI_i$ such that
\begin{align*}
    \cI_1 = \{\underbrace{\mu_1, \mu_1}_{replicated}, \mu_2, \mu_3, \ldots, \mu_l\}, \cI_2 = \{\mu_1, \underbrace{\mu_2,\mu_2}_{replicated}, \mu_3, \ldots, \mu_l\}, \ldots,  \cI_l = \{\mu_1, \underbrace{\mu_2,\mu_2}_{replicated}, \mu_3, \ldots, \mu_l\}
\end{align*}
% \begin{itemize}
% 	\item $\cI_1 = \{\underbrace{\mu_1, \mu_1}_{replicated}, \mu_2, \mu_3, \ldots, \mu_l\}, \cI_2 = \{\mu_1, \underbrace{\mu_2,\mu_2}_{replicated}, \mu_3, \ldots, \mu_l\}, \cI_2 = \{\mu_1, \underbrace{\mu_2,\mu_2}_{replicated}, \mu_3, \ldots, \mu_l\}$
% 	\item $\cI_2 = \{\mu_1, \underbrace{\mu_2,\mu_2}_{replicated}, \mu_3, \ldots, \mu_l\}$
% 	\\ $\vdots$\\
% 	\item $\cI_l = \{\mu_1, \mu_2, \mu_3, \ldots, \underbrace{\mu_l, \mu_l}_{replicated}\}$.
% \end{itemize}
In words, $\cI_i$ denotes the case that the strategy $\cS$ replicates the arm with $i$-th highest reward.
For example, suppose that $\sigma \in \cP_l$ satisfies $\sigma(1) = i$ for some $i \in [l]$.
Since $\cS$ replicates the first arm, under the permutation $\sigma$, the arm with parameter $\mu_i$ is replicated, and thus it corresponds to $\cI_i$.
Then, our notion of TRP essentialy asks what is an algorithm that makes the expected regret of $\cI$ smaller than (or equal to) the average of expected regret of $\cI_1,\dots, \cI_l$.
Put it differently, TRP essentially asks the following fundamental question, which corresponds to the one that we discuss in Section~\ref{sec:intro}.
\begin{center}
	\emph{Given a bandit instance, does ``uniform randomly'' replicate one arm increase the expected regret?}
\end{center}
This foundation of truthfulness under random permutation will play an essential role in constructing replication-proof algorithm in both the single-agent and the multi-agent setting, as can be seen shortly.
Indeed, one can verify that UCB does not satisfy the above question, and thus fails to be replication-proof, from our proof of Theorem~\ref{thm:ucb_negative}.


We finally introduce a permutation invariant of a bandit algorithm.
\begin{definition}[Permutation invariance]
	An algorithm is \emph{permutation invariant} (PI) if given the random bits of the algorithm and the arms, the choice of which arms to pull remains the same (up to tie-breaking) when the index of the arms are permuted.
\end{definition}
Note that the permutation-invariance essentially requires the algorithm to be agnostic to the index of the arms, \ie does not use the arm index to choose the arm, possibly except the tie-breaking case.
One can easily verify that it holds for a broad class canonical algorithms including the ETC, UCB, $\eps$-greedy, etc.

Our main result on the single-agent setting can be presented as follows.

\begin{theorem}\label{thm:single_pf_rp}
	Under the single-agent setting, if an algorithm is truthful under random permutation and permutation-invariant, then it is replication-proof.
\end{theorem}
The proof essentially follows from the observation that the algorithm's ex-ante regret can be partitioned into a disjoint set of random permutation regret, with respect to the ex-post realization of the mean rewards.
Based on this disjoint partition, we can effectively marginalize over the priors while maintaining the partition, and thus conclude that the dominance over the partition yields the overall dominance, where each partition corresponds to a set of randomly permuted bandit instances.
\begin{proof}[Proof of Theorem~\ref{thm:single_pf_rp}]
	Let $\fA$ be an algorithm with symmetry and TRP.
	Given a single agent problem instance $\cI$ with original set $\cO$ with $l$ arms, let $\cS$ be a truthful strategy that registers $\cO$.
	Consider any non-truthful strategy $\cS$ such that it replicates $r_i \in \Z_0$ times for arm $a$ for $a \in [l]$, where $\Z_0 =  \{0,1,2,\ldots\}$ denotes the set of nonnegative integers.
	Note that since $\cS$ is non-truthful strategy, at least one $r_a$ has to be strictly positive for some $a \in [l]$.
	We abuse $r_a=0$ to say that arm $a$ is only registered once without any replication, and write $r = (r_1,\ldots, r_l)$.
	For $v = (v_1,\ldots, v_l) \in \R_{\ge 0}^l$, we write $g(v)$ to denote the density of the mean rewards of arms having $v$, \ie $g(v) = \prod_{a=1}^l f(v_a)$, where $\R_{\ge 0}^l$ denotes the set of $l$-dimensional nonnegative real vectors.
	For simplicity, we assume that the prior distribution of the agent has probability density function, and does not have any point mass.\footnote{This assumption is for ease of exposition, and does not restrict any of our results. For instance, if there exists point mass so that two arms may realize the same mean reward with strictly positive probability, then we can essentially unionize those two arms and consider it as a single arm. In this way, one can verify that all the analysis carry over.}
	We further write $dv$ to denote $dv_1 dv_2 \ldots dv_l$.
	We use $\reg_{v, r}$ to denote the regret of problem instance such that the arms' mean rewards are realized to be $v$ and each arm $i$ is replicated $r_i$ times.
	We finally write $\sigma(v)$ to the permuted vector given a permutation $\sigma \in S^l$, and $\sigma(v)_i$ to denote $i$-coordinate of $\sigma(v)$.
	
%	The following claim easily follows from our definition of permutation-freeness.
	
	Observe that the expected utility in playing the strategy $\cS$ can be written as follows.
	\begin{align*}
		u(\cS) 
		&= 
%		\int_{\mu_1 = v_1}\ldots \int_{\mu_l = v_l} \Ex{U(\cS)\ |\ v_1,\ldots, v_l}g(v)dv
		\int_{\mu_1 = v_1}\ldots \int_{\mu_l = v_l} \Ex{U(\cS)\ |\ \bigtimes_{i \in [l]}(v_a: r_a)}g(v)dv
		\\
		&=
%		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 < v_1}\ldots \int_{\mu_k = v_l< v_{l-1}} 
%		\sum_{\sigma \in \cP_l}\Ex{U(\cS)\ |\ \sigma(v)_1,\ldots, \sigma(v)_l}g(v)dv
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 < v_1}\ldots \int_{\mu_k = v_l< v_{l-1}} 
		\sum_{\sigma \in \cP_l}\Ex{U(\cS)\ |\ \bigtimes_{i \in [l]}(v_{\sigma(a)}: r_a)}g(v)dv
		\\
		&=
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 < v_1}\ldots \int_{\mu_k = v_l< v_{l-1}} 
%		\sum_{\sigma \in \cP_l}\Ex{v_1T - \reg_{\sigma(v),r}(T) \ |\ \sigma(v)_1,\ldots, \sigma(v)_l}g(v)dv.
		\sum_{\sigma \in \cP_l}\Ex{v_1T - \reg_{\sigma(v),r}(T) \ |\ \bigtimes_{i \in [l]}(v_a: r_a)}g(v)dv,
	\end{align*}
	where in the last equation, we condition on $\bigtimes_{i \in [n]}(v_i:r_i)$ since $\reg_{\sigma(v),r}(T)$ already accounts for the permuted bandit instance.
	Further, due to the permutation invariance of the algorithm, applying $\sigma^{-1}$ to all the arm indices does not change the expected regret, and thus we can further expand it to be
	\begin{align}
		u(\cS)
		&=
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 <v_1}\ldots \int_{\mu_l = v_l< v_{l-1}} 
%		\sum_{\sigma \in \cP_l}\Ex{v_1T - \reg_{v,\sigma(r)}(T) \ |\ v_1, \ldots, v_l}g(v)dv.
		\sum_{\sigma \in \cP_l}\Ex{v_1T - \reg_{v,\sigma(r)}(T) \ |\ \bigtimes_{a \in [l]}(v_a: r_a)}g(v)dv.
		\label{ineq:05131256}
	\end{align}
	Let $\vec{0}_l$ denote the $l$-dimensional zero vector.
%	, and the inequality easily follows from the fact that $(0,0,\ldots,0) \prec_m r$ and the algorithm is TRP.
	We now prove the following claim.
	\begin{claim}
		For any $v \in R_{\ge 0}^l$, $\sigma \in \cP_l$, and $r \in \Z_{\ge 0}^l$, we have
		\begin{align*}
			\sum_{\sigma \in \cP_l}\Ex{\reg_{v,\sigma(\vec{0}_l)}(T)} 
			\le 
			\sum_{\sigma \in \cP_l}
			\Ex{\reg_{v,\sigma(r)}(T)}.
		\end{align*}
	\end{claim}
	\begin{proof}
		This directly follows from our definition of TRP.
		More formally,
		\begin{align*}
			\sum_{\sigma \in \cP_l}\Ex{\reg_{v,\sigma(\vec{0}_l)}(T)} 
			\tag{def. of RP-Regtret}
			&=
			\frac{\rpreg(\fA,T;\cO)}{|\cP_l|}
			\\
			&\le
			\frac{\rpreg(\fA,T;\cS) }{|\cP_l|}
			\tag{since $\fA$ is TRP}
			\\
			&=
			\sum_{\sigma \in \cP_l}
			\Ex{\reg_{v,\sigma(r)}(T)}.
			\tag{def. of RP-Regret}
		\end{align*}
		It completes the proof.
	\end{proof}
	By the claim, we can further expand from \eqref{ineq:05131256} as follows.
	\begin{align*}
		u(\cS)
		&\le
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 < v_1}\ldots \int_{\mu_l = v_l< v_{l-1}} 
		\sum_{\sigma \in \cP_l}\Ex{v_1T - \reg_{v,\sigma(\vec{0}_l)}(T) \ |\ \bigtimes_{a \in [l]}(v_a: r_a)}g(v)dv,	
	\end{align*}

	

	Since $\reg_{v, \sigma(\vec{0}_l)}$ is equivalent to the regret of the truthful strategy $\cO$ given the ex-post realization $v$, we obtain
	\begin{align*}
		u(\cS)
		&\le
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 < v_1}\ldots \int_{\mu_l = v_l< v_{l-1}} 
		\sum_{\sigma \in \cP_l}\Ex{v_1T - \reg_{\cI}(T) \ |\ \bigtimes_{a \in [l]}(v_a: r_a)}g(v)dv
		\\
		&=
		\int_{\mu_1 = v_1} \int_{\mu_2 = v_2 }\ldots \int_{\mu_l = v_l} 
		\Ex{U(\cO)\ |\ \bigtimes_{a \in [l]}(v_a: r_a)}g(v)dv
		\\
		&=
%		\int_{\mu_1 = v_1}\ldots \int_{\mu_l = v_l} \Ex{U(\cO)\ |\ v_1,\ldots, v_l}g(v)dv		
%		=
		u(\set{O}),
	\end{align*}
	and thus the truthful registration $\set{O}$ is a dominant strategy.
\end{proof}

Furthermore, we observe that TRP is indeed a necessary condition for an algorithm to be replication-proof in the single-agent setting.
\begin{theorem}
	If an algorithm is not truthful under random permutation, then it is not replication-proof.
\end{theorem}
\begin{proof}
	Consider a single-agent setting.
	Since the algorithm $\fA$ does not satisfy TRP, there exists a problem instance with original arms $\cO$ and the agent's strategy $\cS$, time horizon $T$ such that 
	\begin{align*}
		\rpreg(\fA,T;\cO) 
		\le 	
		\rpreg(\fA,T;\cS).
	\end{align*}
	As observed in the proof of Theorem~\ref{thm:single_pf_rp}, the expected utility of the strategies $\cO$ and $\cS$ can be compared using $\rpreg(\fA,T;\cO)$ and $\rpreg(\fA,T;\cS)$, so the result follows.
    \sscomment{double check}
\end{proof}

\begin{discussion}
	One may wonder if PI can be violated for any replication-proof algorithm.
	This is indeed true.
	For example, one can consider a black-box algorithm that first randomly selects an agent, and runs a bandit algorithm within the agent.
	Further consider a very artificial agent-selection process which does not uniform randomly select the agents, but asymmetrically favors some agent indices with higher probability.
	Such an algorithm indeed is not permutation invariant, since the permutation of agent index would lead to a different outcome given the bandit instance.
	In perspective of the agents, however, each agent only needs to care about the secondary arm selection phase after the agent selection since they cannot change the probability to be selected in the agent selection phase.
	Using these observations, one can observe that such an algorithm is indeed replication-proof, but not permutation invariant.
	One may refine the notion of PI to be restricted within each agent, but we do not argue any more details as it is beyond of our interest and main takeaway.
\end{discussion}



\paragraph{Constructing TRP algorithm}
We now present an algorithm that satisfies TRP.
In what follows, we mainly prove that exploration-then-commit (ETC) satisfies TRP once equipped with a proper parameter.
Its pseudocode is presented in Algorithm~\ref{alg:ETC} for completeness.
We suppose that the algorithm breaks tie in a uniform random manner.\footnote{As can be seen in the proof, any tie-breaking rule does not hurt our analysis.}
ETC essentially decouples the exploration phase and the exploitation phase very explicitly, and thus brings a significant advantage in comparing its expected regret under several problem instances.


\begin{algorithm}
\textbf{Input}: exploration length $m$, tie-breaking rule\\
Play each arm for $m$ rounds.\\
Play the arm with the highest empirical mean for all remaining rounds
\caption{\textsc{ETC}}\label{alg:ETC}
\end{algorithm}

For analytical tractability, we pose some \emph{assumptions} on the support of the prior distributions.
Namely, for any agent $i$, $F_i$ has a discrete support over $[0,1]$ for $i \in \cN$.
Further, we define $\Delta_i$ be the minimum gap between any two possible outcomes from $F_i$, and let $\Delta = \min_{i \in \cN}\Delta$.
Furthermore, the algorithm knows this gap $\Delta$.
\begin{discussion}
	We discuss how one can weaken these assumptions at the end of Section~\ref{sec:single}, possibly at the cost of polylogarithmic blowup in the regret rate or another assumptions.
	We also remark that such assumptions, especially that the algorithm knows the minimum gap, often appear in the literature, \cf \cite{auer2002finite,audibert2010best,garivier2016explore}.
	Moreover, in practice, we believe that it is quite plausible in real-world applications. 
	For example in content platforms, suppose that a content creator comes up with several contents and is about to register. 
	Assume the reward of each content is just the number of views. 
	Typically, the content creator does not exactly know the reward of each content but has historical data on its previous contents. 
	The historical data can be used to structure a prior distribution of the quality of his/her contents. 
	In this case, since usually each content creator has a very small number of original contents compared to the recommendation algorithm's time scale (one for each traffic), this prior distribution may consist of a fairly limited number of samples, thereby having discrete support with a few number of points.
\end{discussion}


Then, our main result in the single-agent setting can be written as follows.
\begin{theorem}\label{thm:single_rp}
	ETC with exploration length $m \ge \frac{2}{\Delta^2} l \ln (2T)$ is TRP in the single-agent setting.
        Further, it has regret of
        \begin{align*}
            \sum_{a\in [l]} \Big( \frac{2\delta_a l\ln{(2T)}}{\Delta^2} + 1 \Big),
        \end{align*}
        where $l$ denotes the number of arms and $\delta_a$ denotes the gap of the mean rewards between optimal arm and arm $a$, of the single agent.
\end{theorem}
The proof essentially follows from the standard regret analysis of ETC along with carefully chosen $m$.
By setting $m$ sufficiently large, we can essentially decrease the probability that a suboptimal arm is chosen to be $o(1/T)$.
This will guarantee that the expected number of rounds the suboptimal arm is chosen is smaller than $1$, whereas any replicating strategy incurs a simple regret lower bound larger than this quantity.
Together with Theorem~\ref{thm:single_pf_rp} and the fact that ETC is permutation invariant (which is straightforward to verify), it follows that ETC is replication-proof in the single-agent setting.

\begin{proof}[Proof of Theorem~\ref{thm:single_rp}]
	Recall that we will deal with a single agent.
	Consider a bandit instance $\cI$ in which there exists $l$ arms with parameters $v_1 \ge v_2 \ge \ldots \ge v_l$, and the time horizon is $T$.
	Let $n_a(t)$ be the number of rounds that arm $a$ is pulled and $\muhat_a(t)$ be the empirical average reward, at the end of round $t$, and define $\delta_a = v_1 - v_a$ for $a \in [l]$.
	
	Our proof mainly relies on the following lemma.
	\begin{lemma}\label{th:ETC_main_th}
		Suppose that the realization of the arms's mean rewards is given, and let $a^*$ be the arm the largest mean reward.
		If $m \ge \frac{2 l}{\Delta^2} \ln{2T}$, then for a sub-optimal arm we have:
		\begin{align*}
			\Ex{n_a(T)} \leq m+1.
		\end{align*}
		Especially for $m = \frac{2}{\Delta^2} l \ln (2T)$, the expected regret is upper bounded by:
		\begin{align*}
    		\reg(T) 
    		\leq 
    		\sum_{a\in [l]} (m+1) \Delta_i 
    		\leq 
    		\sum_{a\in [l]} \Big( \frac{2\delta_a l\ln{(2T)}}{\Delta^2} + 1 \Big).
		\end{align*}	
	\end{lemma}
	\begin{proof}[Proof of the lemma]
		Due to the structural nature of ETC, for any sub-optimal arm $a$ we have
		\begin{align*}
    		\Ex{n_a(T)} \leq m + (T-mk) \Pr{\hat{\mu}_a(m) \ge \hat{\mu}_{a^*}(m)} 
    	\end{align*}
    	Now we focus on upper bounding $\Pr{\hat{\mu}_a(m) \ge \hat{\mu}_{a^*}(m)}$.
    	\begin{claim}\label{cl:concen}
    		For any arm $a \neq a^*$, the following holds.
    		\begin{align*}
    			\Pr{\hat{\mu}_a(m) \ge \hat{\mu}_{a^*}(m)} 
    			\le 
    			2\exp(-\frac{\delta_a^2 m}{2})
    		\end{align*}
    	\end{claim}
    	\begin{proof}[Proof of the claim]
    		We can expand the inequality as follows.
    		\begin{align*}
    			\Pr{\hat{\mu}_a(m) \ge \hat{\mu}_{a^*}(m)} &= \Pr{(\hat{\mu}_a(m) -v_a) + (v_{a^*} - \hat{\mu}_{a^*}(m)) \ge \delta_a}
    			\\ 
    	    	&\leq 
    	    	\Pr{(\hat{\mu}_a(m) -v_a) \ge \frac{\delta_a}{2}} + \Pr{(v_{a^*} - \hat{\mu}_{a^*}(m)) \ge \frac{\delta_a}{2}}
    	    	\\ 
    	    	&\leq 
    	    	2 \exp(- \frac{\delta_a^2}{4} \frac{1}{2} \frac{1}{\frac{1}{4m}}) \tag{Hoeffding's inequality} \\
    	    	& \leq 2\exp(- \frac{\delta_a^2 m}{2}),
			\end{align*}
			which finishes the proof.
			Note that we use the following well-known type of Hoeffding's inequality.
			\begin{theorem}
				Let $X_1,\ldots, X_n$ be independent random variables such that $a_i \le X_i \le b_i$ almost surely.
				Define $S_n = X_1 + \ldots X_n$.
				For any $t >0$,
				\begin{align*}
					\Pr{|S_n - \Ex{S_n}| \ge t}
					\le 
					2\exp\parans{-\frac{2t^2}{\sum_{i=1}^n (b_i - a_i)^2}}.	
				\end{align*}
			\end{theorem}
    	\end{proof}
		Using the claim above, we can further expand,
		\begin{align*}
       		\Ex{n_a(T)} 
       		&\leq
       		m + (T-mk) \Pr{\hat{\mu}_a(m) \ge \hat{\mu}_{a^*}(m)} 
       		\\
       		&\leq 
       		m + 2T\exp(- \frac{\delta_a^2 m}{2})
       		\tag{Claim~\ref{cl:concen} $\&$ $T-mk \le T$}
      		\\
       		&\leq
       		m + 2T  \exp(- \Big(\frac{\delta_a}{\Delta}\Big)^2 \ln{2T})
       		\tag{$m\ge 2/\Delta^2 \ln(2T)$}
       		\\
       		&\leq 
       		m+ 2T  \exp(- \ln{2T})
       		\tag{Since $\frac{\delta_a}{\Delta} \ge 1$} 
       		\\
       		&=
       		m + 1.
		\end{align*}
		This proves the upper bound on $\Ex{n_a(T)}$.
		To obtain the upper bound on the regret, one can use the following well-known regret decomposition lemma.
		\begin{lemma}[Regret decomposition]
			The regret can be writtten as
			$\reg(T) = \sum_{a \in [l]} \Ex{n_i(T)\delta_a}$.
		\end{lemma}

		From this, the regret bound easily follows as below
		\begin{align*}
    		\reg(T)
    		&\leq 
    		\sum_{a\in [l]} (m+1) \delta_a 
    		\\
    		&= 
    		\sum_{a\in [l]} (\frac{2l}{\Delta^2} \ln{2T}+1) \delta_a 
    		\\ 
    		&\leq 
    		\sum_{a\in [l]} ( \frac{2l\delta_a}{\Delta^2} \ln{2T} +1).
    		\tag{Since $\Delta_a\leq 1$} 
		\end{align*}
		This completes the proof.
	\end{proof}
	
	Now, consider a strategy $\cS \neq \cO$ of which the replication vector is $r = (r_1,\ldots, r_l)$ (as defined in the proof of Theorem~\ref{thm:single_pf_rp}), and at least one coordinate being strictly positive.
	Consider a realization $v \in \R_{\ge 0}^l$, and a permutation $\sigma(v)$.
	Let $\cI_{\sigma}$ be a bandit instance in which the arms are permuted by $\sigma$ from $\cI$.

	
	
	Given $v_1 \ge \ldots \ge v_l$, let $\cI_{\sigma,v}$ be the instance in which $i$-th arm has mean reward $v_{\sigma(a)}$ for $a \in [l]$, \ie $\cI_{\sigma, v} = \bigtimes_{a \in [l]}(v_{\sigma(a)}: r_a)$.
	Denote the expected regret under $\cI_{\sigma,v}$ by $\reg_{I_{\sigma,v}}$.
	
	From the regret decomposition lemma, we have
	\begin{align*}
		\reg_{I_{\sigma,v}}(T) = \sum_{a\in [l]}	\Ex{n_{\sigma(a),t}}\delta_{\sigma(a)} \parans{r_a + 1}.
	\end{align*}
	Due to the initial exploration phase of ETC, obviously $\Ex{n_{\sigma(a),t}} \ge m$.
	Hence we obtain
	\begin{align*}
		\reg_{I_{\sigma,v}}(T) 
		&\ge
		\sum_{a\in [l]} m \cdot \delta_{\sigma(a)}(r_a + 1).
	\end{align*}
%	\note{Notation for $reg$ suddenly changes}
	Now, RHS in the random permutation regret \eqref{eq:epf} can be written as follows.
	\begin{align}
		\sum_{\sigma \in \cP_l}\reg_{\cI_{\sigma,v}}(T)/|\cP_l|
		&\geq
		\frac{\sum_{\sigma \in \cP_l}\sum_{a\in [l]} m \cdot \delta_{\sigma(a)}(r_a + 1)}{l!}
		\nonumber
		\\
		&\geq
		\frac{\sum_{a\in [l]} \sum_{\sigma \in \cP_l} m \cdot \delta_{\sigma(a)}(r_a + 1)}{l!}
		\nonumber
		\tag{Change order of summation}
		\\
		&=
		\frac{\sum_{a\in [l]} \sum_{\sigma \in \cP_l} m \cdot \delta_{a}(r_{\sigma(a)} + 1)}{l!}
		\nonumber
		\tag{Sum over $\sigma$ equals that over $\sigma^{-1}$}
		\\
		&=
		\frac{\sum_{a\in [l]} m \cdot \delta_a(l-1)!\sum_{j=1}^l (r_{j}+1)}{l!}
		\nonumber
		\tag{fix $\sigma(a) = j$ and sum over $\sigma \in \cP_l$	}
		\\
		&=
		\frac{\sum_{a\in [l]} m \cdot \delta_a (\norm{r}_1+l)}{l}\label{ineq:05090221}
	\end{align}
	Due to our construction of $r$, we have $\norm{r}_1 \ge 1$, and finally we obtain
	\begin{align}
		\reg_\cI(T) 
		&\le
		\sum_{a\in [l]} (m+1) \delta_a 
		\label{ineq:05090222}
		\\
		&\le
		\sum_{a\in [l]} m\delta_a \frac{l+1}{l},
		\nonumber
		\tag{$m = \frac{2l}{\Delta^2}\ln 2T \ge l$}
		\\
		&\le
		\frac{\sum_{a\in [l]} m \cdot \delta_a\sum_{j=1}^l (r_{j}+1)}{l}
		\tag{$\norm{r}_1 \ge 1$}
		\nonumber
		\\
		&\le
		\sum_{\sigma \in \cP_l}\reg_{\cI_{\sigma,v}}(T)/|\cP_l|,
		\nonumber
	\end{align}
	where the last inequality follows from the inequality~\eqref{ineq:05090221}.
	Note further that $\reg_\cI(T)$ is $\rpreg$ of truthful strategy $\cO$ given the realization $v$, and RHS denotes that of a strategy $\cS$ whose replication vector is $r$.
	Thus,
	\begin{align*}
		\rpreg(\fA, T, \cO) \le \rpreg(\fA, T, \cS),	
	\end{align*}
	for $\fA$ being ETC, and it concludes that ETC is TRP.
\end{proof}


%\begin{discussion}
Note that the proof of Theorem~\ref{thm:single_rp} heavily relies on the fact that the algorithm can observe $\Delta$ in advance and set the exploration length correspondingly.
Thus, despite we aim to obtain a \emph{prior-independent} algorithm that does not require any knowledge in the agent's prior distributions, it is not \emph{truly} prior-independent in an algorithmic manner since it requires some problem parameters to operate the algorithm.
We discuss several ways to refine such restrictions, thereby suggesting a road for truly prior-independent algorithm.
First, assume $\Delta$ is constant but not known to the algorithm.
In this case, one may replace $\Delta$ in the algorithm to be some increasing functions $f(T) = \omega(1)$, and it is straightforward to verify that Theorem~\ref{thm:single_rp} still holds, but in an asymptotical regime.
Similarly, one can effectively wipe out the dependency on the total number of original arms $l$ by assuming that $l = O(1)$ and replacing it with some increasing functions.
Furthermore, the knowledge on $T$ can be wiped out by the standard doubling trick, \cf see Chapter 1 in ~\cite{slivkins2019introduction}, without sacrificing any other guarantees on the truthfulness.
In short, the guarantees can remain the same even without knowing the problem parameters, with sacrifice on the analysis being held only in an asymptotic manner.
Remark that all these refinements only introduce polylogarithmic blowup in the regret upper bound.
%We do not provide more formal discussions as this goes beyond our main takeaway.
%\end{discussion}
The following theorem spells out these arguments, whose formal proof is deferred to Appendix~\ref{apd:thm:single-refine1}.
\begin{theorem}\label{thm:single-refine1}
	Assume $l = O(1),\Delta = \Omega(1)$.
	Then, there is a prior-independent algorithm, which does not require any information on problem parameters, satisfying TRP and PI in the single-agent setting for sufficiently large $T$.
\end{theorem}

\begin{discussion}
	One may ask if we can fully remove the assumption on $\Delta$ without sacrificing regret at all.
	This, in fact, is impossible using a variant of ETC as discussed by~\cite{garivier2016explore}.
	Instead, \cite{garivier2016explore} propose a variant of ETC via considering a best arm identification algorithm in the exploration phase, in the two-armed bandit setting.
	This approach indeed wipes out the dependency of $\Delta$ in the algorithm description, however, such successive elimination style of algorithms, that shrinks the set of active arms gradually based on some stopping rules, significantly complicates the analysis of truthfulness.
	This is because we need to account for every probability that a single arm is deactivated at certain rounds, and this event is highly correlated with the reward tape of the other arms as well as its own.
	The non-adaptive structure of ETC largely simplifies such an analysis as we observe, and it remains as major open problems whether any adaptively exploring algorithm can be made replication-proof in the single-agent setting.
\end{discussion}

%Now that we obtain truly prior-independent algorithm, this is still not satisfactory since the assumption that all the prior distributions have discrete support and $\Delta = O(1)$ may look restrictive.
%Indeed, the assumption of $\Delta$ being constant, however, is more crucial.
%For example, if $\Delta$ can be arbitrarily small, \eg $\Delta = 1/\sqrt{T}$, then our theorem statement specifies that exploration length needs to be set $O(T \ln T)$, which obviously yields a linear regret.
%Indeed, our proof essentially relies on the inequality~\eqref{ineq:05090222},\footnote{This in fact can be loosened by $\reg(\cI) \le \sum_{a \in [l]} (m+m/l)\delta_a$, but it does not change our arguments thereafter.} and this cannot be made true if $\Delta$ is not sufficiently large.
%For example, if $\Delta$ is very small, \eg $O(1/\sqrt{T})$, the quantity $n_a(T)$ in Lemma~\ref{th:ETC_main_th} cannot be upper bounded by $m+c$ for some positive constant $c$.
%
%Instead, one can tackle this assumption as what we describe follows so that our argument carries over even to prior distributions with continuous support.
%Take a sufficiently small positive real number $d$.
%For any two different arms $a \neq a' \in \cO$, define an event $\clean_{a,a'}$ such that the realized quantities $\mu_{a}$ and $\mu_{a'}$ satisfies $|\mu_{a} - \mu_{a'}| \ge d$.
%Further define $\clean = \cap_{a\neq a' \in \cO} \clean_{a,a'}$, and one can compute the deviation probability such that $\clean$ does not occur.
%In upper bounding the number of pulls for suboptimal arms, we can decompose $\Ex{n_a(T)}$ as follows.
%\begin{align*}
%	\Ex{n_a(T)} = \CEx{n_a(T)}{\clean}\Pr{\clean} + \CEx{n_a(T)}{\clean^c}\Pr{\clean^c}.
%\end{align*}
%The first term can be analogously upper bounded to the proof of Theorem~\ref{thm:single_rp}.
%For the latter term, note that $\Pr{\clean^c}$ can equivalently presented as $\Pr{\min_{a \neq a' \in \cO} |\mu_a - \mu_{a'}| < d}$.
%Therefore, if one can essentially compute $\Ex{\min_{a \neq a' \in \cO} |\mu_a - \mu_{a'}|}$, one may upper bound the latter term using some concentration inequalities using a proper amount of deviation.
%Hence, we may only need some reasonable assumptions on  the quantity $\Ex{\min_{a \neq a' \in \cO} |\mu_a - \mu_{a'}|}$.
%Formalizing this argument, we obtain the following theorem.
%\begin{theorem}\label{thm:single-refine2}
%	Let $Z:= \min_{a \neq a' \in \cO} |\mu_a - \mu_{a'}|$.
%\end{theorem}
%
%Remark that
%\begin{theorem}\label{thm:single-refine2}
%	Suppose that $F_i(x) = x$ for $x \in [0,1]$, \ie all the prior distributions	follow $U[0,1]$.
%	Then, there exists an algorithm satisfying TRP and PI in the single-agent setting.
%\end{theorem}

%\note{discuss that this can be further generalized}
%
%\note{discuss why it is hard to fully remove the assumption on $\Delta$}
%
%\note{See also Double Explore-then-Commit: Asymptotic Optimality and Beyond}
%
%\note{See also Garivier, and see if we can remove this assumption. This also argued that if gap is unknown, fixed-interval ETC cannot have logarithmic regret.}

% and for the latter term, one can essentially use some anti-concentration arguments to obtain a upper bound.
%More detailedly, we need to compute a deviation probability
%
%This anti-concentration argument, however, entails a computation of
%
%We provide a formal 



%Next, we tackle the assumption that $\Delta$ is constant, which further requires that all the prior distributions have discrete support.



% \begin{corollary}
% 	ETC is replication-proof in the single agent setting.
% \end{corollary}


%\paragraph{Note:} The algorithm assumes knowledge of the minimum gap between the arms $\min_{i \in [k]} \Delta_i$. 

%\paragraph{Note:} Any algorithm which assumes knowledge of the minimum gap must also imply that the prior over the means is over a discrete support. For example, the prior has non-zero probability only over the set  over $\{0,0.2,0.4,0.6,0.8,1.0\} \subset [0,1]$. If that is not the case and we deal with continuous distributions instead, then it is possible in general to have two means such that the gap between them is arbitrarily small. 


==> temp/icml-ucb.tex <==
\section{Negative Results: Failure of UCB and H-UCB}\label{sec:fail}
We start by presenting negative results on the replication-proof algorithms proposed by \cite{shin2022multi} in our setting.
To this end, we first provide a brief explanation on the algorithms presented by~\cite{shin2022multi}.
They mainly propose hierarchical UCB (H-UCB), which is a variant of the standard UCB by~\cite{auer2002finite}.
We provide the formal pseudocode of both UCB and H-UCB in Algorithm~\ref{alg:UCB} and~\ref{alg:hucb} respectively, to make the paper self-contained.


\begin{algorithm}
\SetAlgoLined
\textbf{Input}: Tie-breaking rule $\tau$, arm set $A$\\
%\textbf{Input}: exploration function $f:\N^2\mapsto \R_{\ge 0}$, tie-break rule $\tau$, arm set $A$\\
Let $\muhat_a \gets 0$ and $n_a \gets 0$ for $a \in A$\\
\For{$t=1,2, \ldots$}
{
	\If{$n_{a} = 0$ for some $a \in A$}{Let $a^* \gets a$}
	\Else
	{
		Compute $s_a \gets \muhat_a + \sqrt{2\ln t/n_a}$\\
		Let $\hat{a} \gets \argmax_{a \in A} s_a$\\
	}
}
Pull $\hat{a}$ and obtain reward $R_t$\\
Update statistics: $\muhat_{\hat{a}} \gets \tfrac{n_{\hat{a}} \muhat_{\hat{a}} + R_t}{n_{\hat{a}} + 1}$;~ $n_{\hat{a}} \gets n_{\hat{a}} + 1$
\caption{\textsc{UCB} [\cite{auer2002finite}]}\label{alg:UCB}
\end{algorithm}


H-UCB mainly consists of two phases: (i) in the first phase, it runs UCB1 by considering each agent as a single arm and selects one agent at each round, and (ii) in the second phase, it runs UCB within the selected agent.
Precisely, it maintains two types of statistics: (i) agent-wise empirical average reward $\muhat_i$, number of pulls per agent $n_i$, and (ii) arm-wise empirical average reward $\muhat_{i,a}$ and number of pulls per arm $n_{i,a}$.
% Such a hierarchical structure effectively decomposes each agent's utility from each other in the fully-informed agent setting.

They prove that H-UCB admits replication-proofness while maintaining sublinear regret.
Their analysis is largely based on the observation that fully-informed agents \emph{do not} have any incentive to register \emph{suboptimal arms}.
Therefore, their setting essentially reduces to the case under which each agent is equipped with only a \emph{single arm}, and its only choice is to determine how many times to replicate the optimal arm.
This observation largely simplifies the equilibrium analysis since replicating the same arm does not change the expected rewards of the agent due to the hierarchical structure therein.
For example, if one uses uniform-random selection in Phase 1, each agent's expected utility is totally independent from each other.
Thus, it suffices to show truthfulness under single-agent setting.
Especially, if there is only a single agent, \emph{any standard sublinear regret algorithm} would achieve replication-proofness due to the observation above.
Hence, it follows that the pair of uniform-random selection algorithm in the first phase and any standard bandit algorithm in the second phase would achieve replication-proofness.

Furthermore, this observation significantly simplifies the regret analysis as well.
This is because given that each agent is equipped with a single original arm, replication of this arm does not change the regret of the algorithms due to the hierarchical structure of H-UCB.
Thus, the regret analysis exactly becomes the same as that of UCB since one can essentially view the (possibly) multiple arms in the second phase as a single arm.
These two facts imply that H-UCB incurs sublinear regret and replication-proofness, if all the agents are fully strategic.
They refine this result by considering additional types of agents who arbitrarily replicate or truthfully register all their arms.
This complicates the regret analysis since one cannot view the second phase as each agent having a single arm.
They propose RH-UCB which slightly varies the exploration parameter in the first phase, along with an arm subsampling phase, and provide its regret analysis.

%Interestingly, 
%
%In particular, since the replication of a single arm
%
%Especially, since the replication
% although one needs more sophisticated algorithm in Phase 1 to obtain sublinear regret.


%In this section, we present a negative result on H-UCB introduced by \cite{shin2022multi}.
% \footnote{They also consider a variant called RH-UCB, which adopts arm-subsampling procedure upon with larger phase 1 exploration parameters, but we do not discuss in detail since it easily follows from our analysis that RH-UCB also fails to be replication-proof in our model.}
%H-UCB mainly consists of two phases: (i) in Phase 1, it runs UCB by considering each agent as a single arm and selects one agent at each round, and (ii) in Phase 2, it runs UCB within the selected agent.
% Such a hierarchical structure effectively decomposes each agent's utility from each other in the fully-informed agent setting.


\begin{algorithm} 
\SetAlgoLined
%$i \in \set{N}$, $\set{S} = \cup_{i \in \set{N}} \set{S}_i$\\
\textbf{Input}: Tie-break rule, agent set $\cN$, arm set $\cS_i$ for $i \in \cN$\\
Let $\muhat_i \gets 0$, $n_i\gets 0$, $\muhat_{i,a} \gets 0$, $n_{i,a} \gets 0$ for $i \in \cN$ and $a \in \cS_i$\\
%Initialize $r(a) = n(a) = R(i)=N(i)=0$~$\forall a, i$;


 \For{$t=1,2,\ldots$}{
%  \tcp{Phase 1 - agent selection}  
  \eIf{$n_i = 0$ for some $i \in \cN$}{ 
    %\tcp{Agent initialization}
    Let $\hat{i} \gets i$
%    Pick an unexplored $\hat{i}\in \{i \in \set{N}: N(i) = 0\} $; % an unexplored agent ;
  }{
    % $i^\star = \argmax_{i} \{R_i + \sqrt{2\ln t / N_i}\}$
    Compute $s_i = \muhat_i + \sqrt{2\ln(t)/n_i}$\\
    Let $\hat{i} \gets \argmax_{i \in \cN} s_i$
%    Pick $\hat{i} = \argmax_{i \in \set{N}} \left\{R(i) + \sqrt{\frac{f(t)}{N(i)}} \right\}$;
  }
%  
%  \tcp{Phase 2 - arm selection}
  \eIf{$n_{\hat{i},a} = 0$ for some $a \in \cS_{\hat{i}}$}{ 
    %\tcp{Agent initialization}
    Let $\hat{a} \gets a$
%    Pick an unexplored $\hat{a}\in \{a \in \set{S}_i: n(a) = 0\} $; % an unexplored agent ;
  }{
  	Compute $s_{\hat{i}, a} \gets \muhat_{\hat{i}, a} + \sqrt{2\ln (n_i)/n_{a,t}}$
%  	Compute $s_{\hat{i}, a} \gets \muhat_{\hat{i}, a} + g(n_{\hat{i},a}, n_{\hat{i}})$
%    Pick $\hat{a} = \argmax_{a \in \set{S}_i} \left\{r(a) + \sqrt{\frac{g(N(i))}{n(a)}} \right\}$;
  }
%  
%  If $N(i) \le 1/2T^{1/3} \log(T)^{1/3}$, round-robin exploration of arms in $\set{S}_i$;\\
%  Else, commit $\hat{a} = \argmax_{a \in \set{S}_{\hat{i}}} 
%    \left\{r(a) \right\}$
  Pull $\hat{a}$ of agent $\hat{i}$ and obtain reward $R_t$\\
  Update statistics:
  $\muhat_{\hat{i},\hat{a}} \leftarrow \tfrac{\muhat_{\hat{i},\hat{a}}n_{\hat{i}, \hat{a}} + R_t}{n_{\hat{i}, \hat{a}}+1}; ~
  \muhat_{\hat{i}} \leftarrow \tfrac{\muhat_{\hat{i}}n_{\hat{i}} + R_t}{n_{\hat{i}}+1};~ n_{\hat{i}, \hat{a}} \leftarrow n_{\hat{i}, \hat{a}} + 1; ~~ n_{\hat{i}} \leftarrow n_{\hat{i}} + 1;$
 }
 \caption{H-UCB [\cite{shin2022multi}]\label{alg:hucb}}
\end{algorithm}


%They prove that H-UCB admits replication-proofness while maintaining sublinear regret.
%Their analysis is largely based on the observation that fully informed agents \emph{do not} have any incentive to register \emph{suboptimal arms}.
%Therefore, fully-informed setting effectively reduces to the case under which each agent is equipped with only a \emph{single arm}, and its only choice is to determine how many times to replicate the optimal arm.
%This observation largely simplifies the analysis of equilibrium since replicating the same arm does not change the expected rewards of the agent due to the hierarchical structure therein.
%For example, they argue that if one uses uniformly random selection algorithm is Phase 1, each agent's expected utility is totally independent from each other.
%Thus, it suffices to show truthfulness under single-agent setting, and thereby any standard bandit algorithm in Phase 2 would work, although we need more sophisticated algorithm in Phase 1 to maintain sublinear regret.
%Especially, if there is only a single agent, any standard sublinear regret algorithm would achieve replication-proofness.

In our setting, however, the agents only know about the prior distributions from which the arms' mean rewards are drawn, and they are oblivious to which original arm will have the highest mean reward.
This motivates each agent to register multiple arms possibly with some replications. 
This indeed significantly complicates the analysis of equilibrium.
For example, it is not trivial to identify which algorithm is replication-proof even under the \emph{single agent setting}.

Interestingly, we show that UCB is not replication-proof even in the single-agent setting.
%To this end, we consider a structured class of UCB algorithms presented in Algorithm~\ref{alg:UCB}, where the exploration parameter $f(\cdot, \cdot)$ governs the amount of pure exploration for each arm.
%\note{would it be worth making it generic?}
%In particular, we are interested in a class of exploration functions $f$ such that it is a monotone decreasing on $n_a$ given $t$, and a monotone increasing on $t$ given $n_a$.
%Further, we assume that $f(\cdot, t) \to \infty$ as $t \to \infty$ and $f(n_a, n_a+c) \to 0$ as $n_a \to \infty$ for any constant $c \in \N$, \ie it decreases more rapidly on $n_a$ than it increases from $t$.
%We denote a function satisfying the above by \emph{doubly monotone}.
%Note that the classical UCB1~\cite{auer2002finite} that corresponds to $f(n_a, t) = \sqrt{\log(t)/n_a}$ is doubly monotone.
\begin{theorem}[Single-agent failure]\label{thm:ucb_negative}
	There exists a problem instance such that UCB1 is not replication-proof in the single-agent setting.
%	UCB with arbitrary positive exploration parameter is not replication-proof in the single agent setting.\footnote{All the proofs are deferred to the appendix due to space constraints.}
\end{theorem}
The proof relies on a construction of bad problem instance which exploits the deterministic and adaptively exploring nature UCB.
To briefly explain the proof, we consider an agent with two Bernoulli arms whose prior distribution is supported on $\{0,1\}$, where it samples mean $0$ and $1$ equally likely.
Let's focus on a realization in which one arm has mean $0$, and the other has $1$.
Observe that replicating one arm essentially yields one of the following two bandit instances: (i) arms with mean rewards $(1,1,0)$\footnote{We write $(x,y,z)$ to denote bandit instance with three arms  mean rewards $1,1,0$.} or (ii) arms with mean rewards $(1,0,0)$.
Note that, intuitively, (i) yields a lower expected regret, but higher in (ii), compared to the original instance with $(0,1)$.
Thus, our analysis mainly reduces to show that the loss from (ii) is larger than the gains from (i).
This can be made indeed true since after observing the dynamics of instance (ii), we can essentially set the time horizon to be exactly right \emph{before} the two arms with mean rewards zero are \emph{consecutively} chosen.
In this way, the loss from (ii) can be made smaller while the gains from (i) is moderately large, which implies the dominance of replicating strategy.


%Then, we compare the truthful strategy with a strategy that replicates only a single arm, and construct a time horizon that the average expected regret of replicating one arm becomes strictly smaller.

%Note that we can focus on the realization where one arm has mean reward of $0$, and the other has $1$.
%Due to the deterministic nature of UCB and the rewards, we can exactly compute the dynamics of UCB for any rounds.
%Since UCB chooses optimal and suboptimal arm in an adaptive manner, these deterministic process incurs a dynamic in which one arm is consecutively chosen, and the other arm is consecutively chosen, and then repeated.
%If we consider a strategy that replicates only a single arm, then, we can essentially select a time horizon that


%Regardless of the UCB's parameter, it is obvious that UCB will determine the arms in a deterministic manner due to deterministic rewards.
%In addition, the arm with mean $1$ will be consecutively chosen some rounds, and then $0$ will be chosen, and this will be repeated.
%If the agent replicates one arm, with probability half this can be $1$, or it will be $0$ otherwise.
%If the agent happens to replicate the arm with mean $1$,



Furthermore, even in the multi-agent setting, we can prove that H-UCB cannot be made replication-proof with any choice of algorithm parameters, thereby showing that the suggested algorithms cannot be made replication-proof for any number of agents.
\begin{theorem}[Multi-agent failure]\label{thm:hucb_negative}
	For any number of agents $n \ge 1$, there exists a problem instance such that H-UCB is not replication-proof.
\end{theorem}
The proof is essentially based on the fact that its Phase 2 does not guarantee replication-proofness within the chosen agent due to Theorem~\ref{thm:ucb_negative}, along with carefully chosen problem parameters to propagate this phenomenon to Phase 1 so as to increase the agent's expected utility under replication.

\begin{discussion}
	We further note that the above two theorems can be easily generalized by parameterizing the exploration parameters $f(n_i, t) = \sqrt{2 \ln(t) / n_i}$ or $g(n_{a,t}, n_i) = \sqrt{2 \ln(n_i)/n_{a,t}}$.
	For example, consider a class of exploration functions $f$ such that it is a monotone decreasing on $n_a$ given $t$, and a monotone increasing on $t$ given $n_a$.
	Further, assume that $f(\cdot, t) \to \infty$ as $t \to \infty$ and $f(n_a, n_a+c) \to 0$ as $n_a \to \infty$ for any constant $c \in \N$, \ie it decreases more rapidly on $n_a$ than it increases from $t$.
	Then, one can check that the both results carry over.
\end{discussion}




\subsection{Proof of Theorem~\ref{thm:ucb_negative} and~\ref{thm:hucb_negative}}
\begin{proof}[Proof of Theorem~\ref{thm:ucb_negative}]
	\sscomment{Add figures}
%	Denote the exploration parameter by function $f(t):\N \mapsto \R_{\ge 0}$.
	Consider a single agent with two arms indexed by $1$ and $2$ from distribution $D$ in which each arm's mean reward is $1$ with probability $1/2$ and $0$ with probability $1/2$.
	Consider a truthful strategy $\set{O}$ and strategy $\set{S}$ that replicates arm $1$.
	There exists four possible cases regarding the realization of the arms parameters: (i) both the arms have mean reward $1$, (ii) only arm $1$ has mean reward $1$, (iii) only arm $2$ has mean reward $1$, and (iv) both the arms have mean reward $0$.
	Denote each cases by $X_i$ for $i =1,2,3,4$.
%	
%	\begin{lemma}[Ex-post to ex-ante dominance]
%		For any two strategies $\set{S}$ and $\set{S}'$, suppose that agent $i$'s ex-post utility under $\set{S}$ is larger than or equal to that under $\set{S}'$ for any measurable set $E_i$ of agent $i$'s arms' realization.
%		Then, $\set{S}$ is dominant strategy over $\set{S}'$.
%		Furthermore, if the equality does not hold for some measurable $E_i$ with strictly positive probability, then $\set{S}$ is strictly dominant strategy over $\set{S}'$.
%	\end{lemma}
%	\begin{proof}
%		\note{Suho - TBD - straightforward but will spell it out}
%	\end{proof}
	For $X_1$ and $X_4$, note that there exists no difference in the agent's ex-post utility.
	For $X_2$ and $X_3$, we show that there exists a time horizon $T$ such that the average ex-post regret is minimized for strategy $\set{S}$.
	
	\begin{figure}[t]
	\includegraphics[width=0.7\textwidth]{Figures/single.jpg}
	\centering
	\caption{Bad instance for UCB in Theorem~\ref{thm:ucb_negative}. 
	Each node denotes the sequence of the bandit algorithm's selection for each instance.
	Blue node denotes the original arm with mean reward $1$, and green one is the replica of it.
	Red nodes the original arm with mean reward $0$, and yellow node is the replica of it.
	Note that at round $t = s_1+s_2+2$, instance $A$ realizes reward $0$ two times, whereas $B$ and $C$ realizes three times, thus having $1.5$ times in average.}
	\label{fig:single-bad}
	\end{figure}
	
	Consider the following list of bandit problem instances with Bernoulli arms.
	\begin{itemize}
		\item Let $A$ be a bandit instance with $\cI_A = (1,0)$.
		\item Let $B$ be a bandit instance with $\cI_B = (1,1',0)$.
		\item Let $C$ be a bandit instance with $\cI_C = (1,0,0')$.
	\end{itemize}
	Each element in $\cI$ denotes the sequence of mean reward of Bernoulli arms, where we write $1'$ and $0'$ to distinguish the arms with same mean.
	Importantly, observe that $A$ denotes the ex-post problem instance that the algorithm faces against strategy $\set{O}$ under $X_2$ or $X_3$.
	Furthermore, $B$ denotes the ex-post problem instance against $\set{S}$ under $X_2$, and $C$ denotes that against $\set{S}$ under $X_3$.
	
	We now show the following claim.
	\begin{claim}\label{cl:neg_ucb}
		Suppose that we run UCB with exploration parameter $f(\cdot)$ for all the problem instances $A,B$, and $C$.
		Then, there exists a time horizon $T$ such that $\reg_A(T) > \nicefrac{(\reg_B(T) + \reg_C(T))}{2}$.
	\end{claim}
	\begin{proof}[Proof of the claim]	
	Define $s_1 = 1$.
	For any integer $i \ge 2$, let $s_i$ denote the minimum integer satisfying
%	\begin{align*}
%		1 + f(s_i + i, s_i) < 0 + f(s_i + i, i)	
%	\end{align*}
	\begin{align*}
		1 + \sqrt{\frac{\ln(s_i + i)}{s_i}} 
		< 0 + \sqrt{\frac{\ln(s_i + i)}{i}}.
	\end{align*}
	Such $s_i$ exists for any $i \ge 2$ since LHS is a decreasing function of $s_i$ which goes to $1$ as $s_i$ increases and RHS is an increasing function of $s_i$ which goes to $\infty$ as $s_i$ increases, and putting $s_i = i$ yields that LHS is larger than RHS.
	Further, it is easy to check that $s_i > s_j$ if $i > j$ and $s_i \ge i$.
	
	Due to our construction of the sequence $s_i$, in $A$, arm with mean $1$ is selected exactly $s_i$ times and then arm with mean $0$ is selected for a single round, and it repeats for $i=1,2,\ldots$.
	Figure~\ref{fig:single-bad} illustrates this bandit instances.
	As can be seen in the figure, the bandit process in $A$ can be described as
	\begin{align*}
		(1:s_1, 0:1, 1:s_2, 0:1, 1:s_3, 0:1, \ldots),
	\end{align*}
	where in each element of $x:y$ denotes that arm with mean $x$ is selected $y$ times.
	Likewise, in $B$, we have
	\begin{align*}
		(1:s_1, 1':s_1, 0:1, [1:s_2, 1':s_2], 0:1, [1:s_3, 1':s_3], 0:1, \ldots),
	\end{align*}
	where for each element in $[\cdot]$, we ignore the orders how $1$ and $1'$ are selected, but aggregate them to only present the total number of times each one is selected before getting to the arm $0$.
	For $C$, we have
	\begin{align*}
		(1:s_1, [0:1, 0':1], 1:s_2, [0:1, 0':1], 1:s_3, [0:1, 0':1], \ldots).
	\end{align*}
	Set $T = s_1 + 2 + s_2$.
	Given $T$, in $A$, the arm $0$ is selected twice.
	In $B$, the arm $0$ is selected once.
	In $C$, the arm $0$ is selected once, and also $0'$ is selected once.
	Hence, at round $t=T$, $\reg_A(T) = 2 > \frac{1+ 2}{2} = \frac{\reg_B(T) + \reg_C(T)}{2}$,
	and it completes the proof.
	\end{proof}
	Set $T$ as defined in the claim above.
	% In the single-agent setting, given any realization $E = (\mu_1, \mu_2)$ with $\mu_1 \ge \mu_2$, note that an agent's ex-ante utility can be easily derived from his ex-post regret as follows.
	% \begin{align*}
	% 	U(\set{S};E) = \mu_1 N_1(T) + \mu_2 N_2(T) = 
	% 	\mu_1 T - (\mu_1 - \mu_2)N_2(T) =  \max_{a \in E}\mu_a \cdot T - \reg_E(T).
	% \end{align*}
	Finally, we can decompose the agent's ex-ante utility as follows.
	\begin{align*}
		u(\set{O}) 
		= 
		\frac{1}{4}\parans{\sum_{i=1}^4U(\set{O};E_i)}
		&=
		\frac{1}{4}\parans{\sum_{i=1,4}U(\set{O};E_i)} + \frac{1}{4}\parans{\sum_{i=2,3}U(\set{S};E_i)}
		\\
		&=
		\frac{1}{4}\parans{\sum_{i=1,4} \parans{\max_{a \in E_i}\mu_a \cdot T - \reg_{E_i}(T)}}
		+
		\frac{1}{4}\parans{\sum_{i=2,3} \parans{\max_{a \in E_i}\mu_a \cdot T - \reg_{E_i}(T)}}
		\\
		&=
            \frac{T - \reg_A(T)}{2}
		\\
		&<
		\frac{T - (\reg_B(T) + \reg_C(T))/2}{2}
		\\
		&=
		\frac{1}{4}\parans{\sum_{i=1,4}U(\set{S};E_i)} + \frac{1}{4}\parans{\sum_{i=2,3}U(\set{S};E_i)}
		\\
		&= u(\set{S}),
	\end{align*}
	and thus $\set{S}$ yields the strictly larger ex-ante utility, and it concludes the proof.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:hucb_negative}]
	If there exists only a single agent, it is easy to see that the dynamics of the algorithm reduces to standard UCB1.
	Thus, by Theorem~\ref{thm:ucb_negative}, H-UCB is not replication-proof.
	Now we consider multiple agents with $n \ge 2$.
	We only show for the case $n=2$ since it easily extends to the cases with $n \ge 3$.
	Without loss of generality, we assume that the algorithm breaks tie uniformly at random in both phases $1$ and $2$.
	Suppose that agent $1$ has two deterministic arms sampled from $D$ in which the mean reward is $c \in [0,1]$ with probability $0.5$, and $0$ otherwise, for some $c>0$.
	We further assume that agent $2$ is equipped with a deterministic prior $D_i$ supported on $\mu$, and the arm also deterministically outputs reward $\mu$.
	Our choice of $\mu$ will be determined later, which will be selected in order to propagate the single-agent failure to the two-agent cases.
	Especially, we will focus on the round that agent $1$ is selected exactly $s_1+s_2+2$ times, as defined in the proof of Theorem~\ref{thm:ucb_negative}.
	Note that the bandit process is deterministic for any realization of the arms' parameters.
	
	We consider a truthful strategy $\cO$ of registering both arms, and another strategy $\cS$ of replicating only a single arm, and focus on the difference on the agent's expected utility between two strategies.
	If the agent samples $c$ or $0$ both the arms, then the rewards of the bandit process and the agent's ex-post utility therein will be indifferent.
	Thus, we only focus on the remaining case.
	Suppose that agent $1$ samples $c$ for one arm and $0$ for the other, which occurs with probability $1/2$.
	Similar to the proof of Claim~\ref{cl:neg_ucb}, we consnider the following list of bandit problem instances with deterministic arms.
	\begin{itemize}
		\item Let $A$ be a bandit instance with $\cI_A = (c,0)$.
		\item Let $B$ be a bandit instance with $\cI_B = (c,c',0)$.
		\item Let $C$ be a bandit instance with $\cI_C = (c,0,0')$.
	\end{itemize}
	% \note{Some figure may help}
	Each element in $\cI$ denotes the sequence of mean reward of Bernoulli arms, where we write $c'$ and $0'$ to distinguish the arms with same mean.
	We simply say arm $c$ and arm $0$ to denote the arm with the corresponding parameter $c$ and $0$, respectively.
	Then, the realization of the agent $1$'s arms in playing strategy $\cS$ corresponds to either of bandit instance $B$ or $C$, and strategy $\cO$ corresponds to the bandit instance $A$.
	Let us abuse the notation of $s_1,s_2,\ldots$ defined in the proof of Claim~\ref{cl:neg_ucb}, so that it denotes the number of rounds that arm $c$ is selected consecutively before arm $0$ is sampled $i$-th time, in problem instance $A$.
	Also, we use $R_t(i)$ and $N_t(i)$ to denote the quantity of $R(i)$ and $N(i)$ at round $t$.
	
	Given the random bits of the tie-breaking rule used by the algorithm, let $\tau^{i}_1,\tau^i_2,\ldots, \tau^i_{k}, \ldots$ be the rounds that agent $1$ is sampled $k$ times when the mean rewards of the agent $1$'s arms are realized to be $i= A,B,C$.
	It is straightforward to check that $\tau^{B}_t \le \tau^{A}_t \le \tau^{C}_t$\footnote{This can  be shown using the coupling technique introduced in \cite{shin2022multi}.}.
	Let $k = s_1+s_2+2$, and following the argument of Claim~\ref{cl:neg_ucb}, we observe that at round $\tau^{B}_k$, agent $1$'s empirical mean rewards by playing $\cS$ will be either of (i) $\frac{c(s_1+s_2)}{s_1+s_2+2}$ or (ii) $\frac{c(s_1+s_2+1)}{s_1+s_2+2}$ based on whether the arms are realized to be instance $B$ or $C$.
	By playing $\cO$, agent $1$ simply has empirical mean reward of $\frac{c(s_1+s_2)}{s_1+s_2+2}$ at round $\tau^{A}_k$.
	Furthermore, if $\tau^{B}_k < \tau^{A}_k$, then in problem instance $A$, it means that the agents' parameters at round $\tau^{B}_k$ satisfy
	\begin{align*}
		R_{\tau^B_k}(1) + \sqrt{\frac{2\ln(t)}{k-1}}
		<
		R_{\tau^B_k}(2) + \sqrt{\frac{2\ln(t)}{\tau^B_k - k}},
	\end{align*}
	where $R_t(i)$ denotes the empirical average reward of agent $i$ at round $t$,  $R_{\tau^B_k}(1) = \frac{c(s_1+s_2)}{s_1+s_2+2}$ and $R_{\tau^B_k}(2) = \mu$.
	However, from our construction of the variables and the fact that H-UCB selects agent $1$ at round $\tau^{B}_k$ in $B$, we know that
	\begin{align*}
		\frac{c(s_1+s_2)}{s_1+s_2+2} + \sqrt{\frac{2\ln(t)}{k-1}}
		\ge
		\mu + \sqrt{\frac{2\ln(t)}{\tau^B_k - k}},
	\end{align*}
	and thus $\tau^A_k$ and $\tau^B_k$ needs to be exactly equivalent.
	Similarly, for instance $C$, since arm $c$ and $c'$ are selected the same number of times at the beginning of round $\tau^B_k$, we conclude that $\tau^i_k$ are equivalent for $i=A,B,C$.
	
	Now define $\theta = \sqrt{\frac{2\ln(t)}{k}} - \sqrt{\frac{2\ln(t)}{\tau^B_k-k}}$ and we pick any $\mu \in (\frac{c(s_1+s_2)}{s_1+s_2+2} + \theta,\frac{c(s_1+s_2+1)}{s_1+s_2+2} + \theta)$.
%	We claim that there exists a choice of parameters $c$ that such $\mu$ always exist.
%	\begin{claim}
%		There exists  $c>0$ such that the interval $\mu \in (\frac{c(s_1+s_2)}{s_1+s_2+2} + C_1,\frac{c(s_1+s_2+1)}{s_1+s_2+2} + C_2)$ is well-defined.
%	\end{claim}
%	\begin{proof}
%		It suffices to show that 
%		\begin{align*}
%			\sqrt{\frac{f(t)}{k-1}} - \sqrt{\frac{f(t)}{k}} < \frac{c}{s_1+s_2+2}.
%		\end{align*}
%		Note that all $k = s_1+s_2+2$,$s_1$ and $s_2$ are in fact functions of $c$.
%		Define $s = s_1+s_2$ and rearrange the inequality, we obtain 
%		\begin{align*}
%			\sqrt{f(t)}\parans{\frac{\sqrt{s+2} - \sqrt{s+1}}{\sqrt{(s+1)(s+2)}}}
%			<
%			\frac{c}{s+2}.
%		\end{align*}
%		Define $x = \sqrt{s+1}$ and rearrange again, it suffices to show that
%		\begin{align*}
%			\sqrt{f(t)}\parans{x+\frac{1}{x}-1} \le c,
%		\end{align*}
%		for some $c$.
%		Since LHS is at most 
%		
%
%
%		
%		When we increase the value of $c$, it is easy to see that  
%		
%		By making $c$ sufficiently large, we
%
%	\end{proof}

	
	Then, at round $\tau^B_k+1$, for bandit instance $A$ and $C$, we observe that agent $2$ will be selected since
	\begin{align*}
		R_{\tau^B_k+1}(2) + \sqrt{\frac{2\ln(t)}{N_{\tau^B_k}(2)}}
		&=
		\mu + \sqrt{\frac{2\ln(t)}{\tau^B_k - k}}
		\\
		&>
		\frac{s_1+s_2}{s_1+s_2+2} + \theta + \sqrt{\frac{2\ln(t)}{\tau^B_k - k}}
		\\
		&=
		\frac{s_1+s_2}{s_1+s_2+2} + \sqrt{\frac{2\ln(t)}{k}}
		= 
		R_{\tau^B_k+1}(1) + \sqrt{\frac{2\ln(t)}{N_{\tau^B_k}(1)}}.
	\end{align*}
	For bandit instance $C$, however, observe that
	\begin{align*}
		R_{\tau^C_k+1}(2) + \sqrt{\frac{2\ln(t)}{N_{\tau^C_k}(2)}}
		&=
		\mu + \sqrt{\frac{2\ln(t)}{\tau^C_k - k}}
		\\
		&<
		\frac{s_1+s_2+1}{s_1+s_2+2} + \theta + \sqrt{\frac{2\ln(t)}{\tau^C_k - k}}
		\\
		&=
		\frac{s_1+s_2+1}{s_1+s_2+2} + \sqrt{\frac{2\ln(t)}{k}} 
		=
		R_{\tau^C_k+1}(1) + \sqrt{\frac{2\ln(t)}{N_{\tau^C_k}(1)}},
	\end{align*}
	and thus arm $1$ is selected.
	This essentially implies that by setting $T = \tau_k^A+1$, agent $1$ is selected at round $T$ with probability $1/4$ if he plays $\cS$, is never selected if he plays $\cO$, where the probability $1/4$ comes from the fact that problem instance $C$ is realized with probability $1/4$.
	Thus, agent $1$'s expected utility becomes larger for such $T$ by replicating one of its arm, and we finish the proof.
%
%
%	
%	Note that each $\tau_i$ depends on agent $2$'s reward $\mu$.
%	Define the sequence $s_1,s_2,\ldots$ and the problem instance $A,B$, and $C$ as we did in the proof of Claim~\ref{cl:neg_ucb}.
%	Following the argument of Claim~\ref{cl:neg_ucb}, we observe that at round $\tau_i$ with $i = s_1+2+s_2$, agent $1$'s ex-post regret is strictly larger on problem instance $A$, compared to the average of that of $B$ and $C$.
%	This essentially implies that at round $\tau_i$, agent $1$'s empirical mean reward becomes exactly larger in strategy $\cS'$.
%	
%	Now we pick any $\mu \in (\frac{s_1+s_2}{s_1+s_2+2},\frac{s_1+s_2+1}{s_1+s_2+2})$.
%	Then, in problem instance $A$, at round $\tau$
	
%	
%	\note{Suho - TBD - need to be fixed}
%	
%	Consider two symmetric agents $a$ and $b$ with two deterministic arms of $1$ and $\eps$.
%	Denote the agent $a$'s arm by $1_a$ and $\eps_a$, and similarly for agent $b$.
%	Let $(s_i)_{i\in \N}$ be the sequence defined in the proof of Theorem~\ref{thm:ucb_negative}.
%	Set $T = 2(s_1+2+s_2) + 1$.
%	Suppose that both the agents truthfully register.
%	Up to round $t=T-1$, due to the deterministic nature of the arms, both agents are selected $s_1+2+s_2$ times, and their agent-wise average rewards are $R(a) = R(b) = 1 - \frac{2\eps}{s_1+2+s_2}$.
%	Thus, at round $t=T$, the selected agent will be based on the tie-breaking rule of H-UCB.
%	On the other hand, suppose that agent $a$ replicates one of the arms randomly.
%	Then, by the observation in the proof of Theorem~\ref{thm:ucb_negative}, the average reward of agent $a$ at round $t=T-1$ will be $R(a) = 1 - \frac{\eps}{s_1+2+s_2}$ if arm $1$ is replicated.
%	Otherwise if arm $\eps$ is replicated, then $R(a) = 1 - \frac{2\eps}{s_1+2+s_2}$.
%	In the former case, agent $a$ will be deterministically selected as it satisfies $R(a) > R(b)$.
%	In the latter case, the tie-breaking rule determines whom to select.
%	This implies that the average reward of replicating both arms is larger, and thus $H-UCB$ is not replication-proof.
\end{proof}
	






==> ucb.tex <==
\section{Negative Results: Failure of UCB and H-UCB}\label{sec:fail}
We start by presenting negative results on the replication-proof algorithms proposed by \cite{shin2022multi} in our setting.
To this end, we first provide a brief explanation on the algorithms presented by~\cite{shin2022multi}.
They mainly propose hierarchical UCB (H-UCB), which is a variant of the standard UCB by~\cite{auer2002finite}.
We provide the formal pseudocode of both UCB and H-UCB in Algorithm~\ref{alg:UCB} and~\ref{alg:hucb} respectively, to make the paper self-contained.


\begin{algorithm}
\SetAlgoLined
\textbf{Input}: Tie-breaking rule $\tau$, arm set $A$\\
%\textbf{Input}: exploration function $f:\N^2\mapsto \R_{\ge 0}$, tie-break rule $\tau$, arm set $A$\\
Let $\muhat_a \gets 0$ and $n_a \gets 0$ for $a \in A$\\
\For{$t=1,2, \ldots$}
{
	\If{$n_{a} = 0$ for some $a \in A$}{Let $a^* \gets a$}
	\Else
	{
		Compute $s_a \gets \muhat_a + \sqrt{2\ln t/n_a}$\\
		Let $\hat{a} \gets \argmax_{a \in A} s_a$\\
	}
}
Pull $\hat{a}$ and obtain reward $R_t$\\
Update statistics: $\muhat_{\hat{a}} \gets \tfrac{n_{\hat{a}} \muhat_{\hat{a}} + R_t}{n_{\hat{a}} + 1}$;~ $n_{\hat{a}} \gets n_{\hat{a}} + 1$
\caption{\textsc{UCB} [\cite{auer2002finite}]}\label{alg:UCB}
\end{algorithm}


H-UCB mainly consists of two phases: (i) in the first phase, it runs UCB1 by considering each agent as a single arm and selects one agent at each round, and (ii) in the second phase, it runs UCB within the selected agent.
Precisely, it maintains two types of statistics: (i) agent-wise empirical average reward $\muhat_i$, number of pulls per agent $n_i$, and (ii) arm-wise empirical average reward $\muhat_{i,a}$ and number of pulls per arm $n_{i,a}$.
% Such a hierarchical structure effectively decomposes each agent's utility from each other in the fully-informed agent setting.

They prove that H-UCB admits replication-proofness while maintaining sublinear regret.
Their analysis is largely based on the observation that fully-informed agents \emph{do not} have any incentive to register \emph{suboptimal arms}.
Therefore, their setting essentially reduces to the case under which each agent is equipped with only a \emph{single arm}, and its only choice is to determine how many times to replicate the optimal arm.
This observation largely simplifies the equilibrium analysis since replicating the same arm does not change the expected rewards of the agent due to the hierarchical structure therein.
For example, if one uses uniform-random selection in Phase 1, each agent's expected utility is totally independent from each other.
Thus, it suffices to show truthfulness under single-agent setting.
Especially, if there is only a single agent, \emph{any standard sublinear regret algorithm} would achieve replication-proofness due to the observation above.
Hence, it follows that the pair of uniform-random selection algorithm in the first phase and any standard bandit algorithm in the second phase would achieve replication-proofness.

Furthermore, this observation significantly simplifies the regret analysis as well.
This is because given that each agent is equipped with a single original arm, replication of this arm does not change the regret of the algorithms due to the hierarchical structure of H-UCB.
Thus, the regret analysis exactly becomes the same as that of UCB since one can essentially view the (possibly) multiple arms in the second phase as a single arm.
These two facts imply that H-UCB incurs sublinear regret and replication-proofness, if all the agents are fully strategic.
They refine this result by considering additional types of agents who arbitrarily replicate or truthfully register all their arms.
This complicates the regret analysis since one cannot view the second phase as each agent having a single arm.
They propose RH-UCB which slightly varies the exploration parameter in the first phase, along with an arm subsampling phase, and provide its regret analysis.

%Interestingly, 
%
%In particular, since the replication of a single arm
%
%Especially, since the replication
% although one needs more sophisticated algorithm in Phase 1 to obtain sublinear regret.


%In this section, we present a negative result on H-UCB introduced by \cite{shin2022multi}.
% \footnote{They also consider a variant called RH-UCB, which adopts arm-subsampling procedure upon with larger phase 1 exploration parameters, but we do not discuss in detail since it easily follows from our analysis that RH-UCB also fails to be replication-proof in our model.}
%H-UCB mainly consists of two phases: (i) in Phase 1, it runs UCB by considering each agent as a single arm and selects one agent at each round, and (ii) in Phase 2, it runs UCB within the selected agent.
% Such a hierarchical structure effectively decomposes each agent's utility from each other in the fully-informed agent setting.


\begin{algorithm} 
\SetAlgoLined
%$i \in \set{N}$, $\set{S} = \cup_{i \in \set{N}} \set{S}_i$\\
\textbf{Input}: Tie-break rule, agent set $\cN$, arm set $\cS_i$ for $i \in \cN$\\
Let $\muhat_i \gets 0$, $n_i\gets 0$, $\muhat_{i,a} \gets 0$, $n_{i,a} \gets 0$ for $i \in \cN$ and $a \in \cS_i$\\
%Initialize $r(a) = n(a) = R(i)=N(i)=0$~$\forall a, i$;


 \For{$t=1,2,\ldots$}{
%  \tcp{Phase 1 - agent selection}  
  \eIf{$n_i = 0$ for some $i \in \cN$}{ 
    %\tcp{Agent initialization}
    Let $\hat{i} \gets i$
%    Pick an unexplored $\hat{i}\in \{i \in \set{N}: N(i) = 0\} $; % an unexplored agent ;
  }{
    % $i^\star = \argmax_{i} \{R_i + \sqrt{2\ln t / N_i}\}$
    Compute $s_i = \muhat_i + \sqrt{2\ln(t)/n_i}$\\
    Let $\hat{i} \gets \argmax_{i \in \cN} s_i$
%    Pick $\hat{i} = \argmax_{i \in \set{N}} \left\{R(i) + \sqrt{\frac{f(t)}{N(i)}} \right\}$;
  }
%  
%  \tcp{Phase 2 - arm selection}
  \eIf{$n_{\hat{i},a} = 0$ for some $a \in \cS_{\hat{i}}$}{ 
    %\tcp{Agent initialization}
    Let $\hat{a} \gets a$
%    Pick an unexplored $\hat{a}\in \{a \in \set{S}_i: n(a) = 0\} $; % an unexplored agent ;
  }{
  	Compute $s_{\hat{i}, a} \gets \muhat_{\hat{i}, a} + \sqrt{2\ln (n_i)/n_{a,t}}$
%  	Compute $s_{\hat{i}, a} \gets \muhat_{\hat{i}, a} + g(n_{\hat{i},a}, n_{\hat{i}})$
%    Pick $\hat{a} = \argmax_{a \in \set{S}_i} \left\{r(a) + \sqrt{\frac{g(N(i))}{n(a)}} \right\}$;
  }
%  
%  If $N(i) \le 1/2T^{1/3} \log(T)^{1/3}$, round-robin exploration of arms in $\set{S}_i$;\\
%  Else, commit $\hat{a} = \argmax_{a \in \set{S}_{\hat{i}}} 
%    \left\{r(a) \right\}$
  Pull $\hat{a}$ of agent $\hat{i}$ and obtain reward $R_t$\\
  Update statistics:
  $\muhat_{\hat{i},\hat{a}} \leftarrow \tfrac{\muhat_{\hat{i},\hat{a}}n_{\hat{i}, \hat{a}} + R_t}{n_{\hat{i}, \hat{a}}+1}; ~
  \muhat_{\hat{i}} \leftarrow \tfrac{\muhat_{\hat{i}}n_{\hat{i}} + R_t}{n_{\hat{i}}+1};~ n_{\hat{i}, \hat{a}} \leftarrow n_{\hat{i}, \hat{a}} + 1; ~~ n_{\hat{i}} \leftarrow n_{\hat{i}} + 1;$
 }
 \caption{H-UCB [\cite{shin2022multi}]\label{alg:hucb}}
\end{algorithm}


%They prove that H-UCB admits replication-proofness while maintaining sublinear regret.
%Their analysis is largely based on the observation that fully informed agents \emph{do not} have any incentive to register \emph{suboptimal arms}.
%Therefore, fully-informed setting effectively reduces to the case under which each agent is equipped with only a \emph{single arm}, and its only choice is to determine how many times to replicate the optimal arm.
%This observation largely simplifies the analysis of equilibrium since replicating the same arm does not change the expected rewards of the agent due to the hierarchical structure therein.
%For example, they argue that if one uses uniformly random selection algorithm is Phase 1, each agent's expected utility is totally independent from each other.
%Thus, it suffices to show truthfulness under single-agent setting, and thereby any standard bandit algorithm in Phase 2 would work, although we need more sophisticated algorithm in Phase 1 to maintain sublinear regret.
%Especially, if there is only a single agent, any standard sublinear regret algorithm would achieve replication-proofness.

In our setting, however, the agents only know about the prior distributions from which the arms' mean rewards are drawn, and they are oblivious to which original arm will have the highest mean reward.
This motivates each agent to register multiple arms possibly with some replications. 
This indeed significantly complicates the analysis of equilibrium.
For example, it is not trivial to identify which algorithm is replication-proof even under the \emph{single agent setting}.

Interestingly, we show that UCB is not replication-proof even in the single-agent setting.
%To this end, we consider a structured class of UCB algorithms presented in Algorithm~\ref{alg:UCB}, where the exploration parameter $f(\cdot, \cdot)$ governs the amount of pure exploration for each arm.
%\note{would it be worth making it generic?}
%In particular, we are interested in a class of exploration functions $f$ such that it is a monotone decreasing on $n_a$ given $t$, and a monotone increasing on $t$ given $n_a$.
%Further, we assume that $f(\cdot, t) \to \infty$ as $t \to \infty$ and $f(n_a, n_a+c) \to 0$ as $n_a \to \infty$ for any constant $c \in \N$, \ie it decreases more rapidly on $n_a$ than it increases from $t$.
%We denote a function satisfying the above by \emph{doubly monotone}.
%Note that the classical UCB1~\cite{auer2002finite} that corresponds to $f(n_a, t) = \sqrt{\log(t)/n_a}$ is doubly monotone.
\begin{theorem}[Single-agent failure]\label{thm:ucb_negative}
	There exists a problem instance such that UCB1 is not replication-proof in the single-agent setting.
%	UCB with arbitrary positive exploration parameter is not replication-proof in the single agent setting.\footnote{All the proofs are deferred to the appendix due to space constraints.}
\end{theorem}
The proof relies on a construction of bad problem instance which exploits the deterministic and adaptively exploring nature UCB.
To briefly explain the proof, we consider an agent with two Bernoulli arms whose prior distribution is supported on $\{0,1\}$, where it samples mean $0$ and $1$ equally likely.
Let's focus on a realization in which one arm has mean $0$, and the other has $1$.
Observe that replicating one arm essentially yields one of the following two bandit instances: (i) arms with mean rewards $(1,1,0)$\footnote{We write $(x,y,z)$ to denote bandit instance with three arms  mean rewards $1,1,0$.} or (ii) arms with mean rewards $(1,0,0)$.
Note that, intuitively, (i) yields a lower expected regret, but higher in (ii), compared to the original instance with $(0,1)$.
Thus, our analysis mainly reduces to show that the loss from (ii) is larger than the gains from (i).
This can be made indeed true since after observing the dynamics of instance (ii), we can essentially set the time horizon to be exactly right \emph{before} the two arms with mean rewards zero are \emph{consecutively} chosen.
In this way, the loss from (ii) can be made smaller while the gains from (i) is moderately large, which implies the dominance of replicating strategy.


%Then, we compare the truthful strategy with a strategy that replicates only a single arm, and construct a time horizon that the average expected regret of replicating one arm becomes strictly smaller.

%Note that we can focus on the realization where one arm has mean reward of $0$, and the other has $1$.
%Due to the deterministic nature of UCB and the rewards, we can exactly compute the dynamics of UCB for any rounds.
%Since UCB chooses optimal and suboptimal arm in an adaptive manner, these deterministic process incurs a dynamic in which one arm is consecutively chosen, and the other arm is consecutively chosen, and then repeated.
%If we consider a strategy that replicates only a single arm, then, we can essentially select a time horizon that


%Regardless of the UCB's parameter, it is obvious that UCB will determine the arms in a deterministic manner due to deterministic rewards.
%In addition, the arm with mean $1$ will be consecutively chosen some rounds, and then $0$ will be chosen, and this will be repeated.
%If the agent replicates one arm, with probability half this can be $1$, or it will be $0$ otherwise.
%If the agent happens to replicate the arm with mean $1$,



Furthermore, even in the multi-agent setting, we can prove that H-UCB cannot be made replication-proof with any choice of algorithm parameters, thereby showing that the suggested algorithms cannot be made replication-proof for any number of agents.
\begin{theorem}[Multi-agent failure]\label{thm:hucb_negative}
	For any number of agents $n \ge 1$, there exists a problem instance such that H-UCB is not replication-proof.
\end{theorem}
The proof is essentially based on the fact that its Phase 2 does not guarantee replication-proofness within the chosen agent due to Theorem~\ref{thm:ucb_negative}, along with carefully chosen problem parameters to propagate this phenomenon to Phase 1 so as to increase the agent's expected utility under replication.

\begin{discussion}
	We further note that the above two theorems can be easily generalized by parameterizing the exploration parameters $f(n_i, t) = \sqrt{2 \ln(t) / n_i}$ or $g(n_{a,t}, n_i) = \sqrt{2 \ln(n_i)/n_{a,t}}$.
	For example, consider a class of exploration functions $f$ such that it is a monotone decreasing on $n_a$ given $t$, and a monotone increasing on $t$ given $n_a$.
	Further, assume that $f(\cdot, t) \to \infty$ as $t \to \infty$ and $f(n_a, n_a+c) \to 0$ as $n_a \to \infty$ for any constant $c \in \N$, \ie it decreases more rapidly on $n_a$ than it increases from $t$.
	Then, one can check that the both results carry over.
\end{discussion}




\subsection{Proof of Theorem~\ref{thm:ucb_negative} and~\ref{thm:hucb_negative}}
\begin{proof}[Proof of Theorem~\ref{thm:ucb_negative}]
	\sscomment{Add figures}
%	Denote the exploration parameter by function $f(t):\N \mapsto \R_{\ge 0}$.
	Consider a single agent with two arms indexed by $1$ and $2$ from distribution $D$ in which each arm's mean reward is $1$ with probability $1/2$ and $0$ with probability $1/2$.
	Consider a truthful strategy $\set{O}$ and strategy $\set{S}$ that replicates arm $1$.
	There exists four possible cases regarding the realization of the arms parameters: (i) both the arms have mean reward $1$, (ii) only arm $1$ has mean reward $1$, (iii) only arm $2$ has mean reward $1$, and (iv) both the arms have mean reward $0$.
	Denote each cases by $X_i$ for $i =1,2,3,4$.
%	
%	\begin{lemma}[Ex-post to ex-ante dominance]
%		For any two strategies $\set{S}$ and $\set{S}'$, suppose that agent $i$'s ex-post utility under $\set{S}$ is larger than or equal to that under $\set{S}'$ for any measurable set $E_i$ of agent $i$'s arms' realization.
%		Then, $\set{S}$ is dominant strategy over $\set{S}'$.
%		Furthermore, if the equality does not hold for some measurable $E_i$ with strictly positive probability, then $\set{S}$ is strictly dominant strategy over $\set{S}'$.
%	\end{lemma}
%	\begin{proof}
%		\note{Suho - TBD - straightforward but will spell it out}
%	\end{proof}
	For $X_1$ and $X_4$, note that there exists no difference in the agent's ex-post utility.
	For $X_2$ and $X_3$, we show that there exists a time horizon $T$ such that the average ex-post regret is minimized for strategy $\set{S}$.
	
	\begin{figure}[t]
	\includegraphics[width=0.7\textwidth]{Figures/single.jpg}
	\centering
	\caption{Bad instance for UCB in Theorem~\ref{thm:ucb_negative}. 
	Each node denotes the sequence of the bandit algorithm's selection for each instance.
	Blue node denotes the original arm with mean reward $1$, and green one is the replica of it.
	Red nodes the original arm with mean reward $0$, and yellow node is the replica of it.
	Note that at round $t = s_1+s_2+2$, instance $A$ realizes reward $0$ two times, whereas $B$ and $C$ realizes three times, thus having $1.5$ times in average.}
	\label{fig:single-bad}
	\end{figure}
	
	Consider the following list of bandit problem instances with Bernoulli arms.
	\begin{itemize}
		\item Let $A$ be a bandit instance with $\cI_A = (1,0)$.
		\item Let $B$ be a bandit instance with $\cI_B = (1,1',0)$.
		\item Let $C$ be a bandit instance with $\cI_C = (1,0,0')$.
	\end{itemize}
	Each element in $\cI$ denotes the sequence of mean reward of Bernoulli arms, where we write $1'$ and $0'$ to distinguish the arms with same mean.
	Importantly, observe that $A$ denotes the ex-post problem instance that the algorithm faces against strategy $\set{O}$ under $X_2$ or $X_3$.
	Furthermore, $B$ denotes the ex-post problem instance against $\set{S}$ under $X_2$, and $C$ denotes that against $\set{S}$ under $X_3$.
	
	We now show the following claim.
	\begin{claim}\label{cl:neg_ucb}
		Suppose that we run UCB with exploration parameter $f(\cdot)$ for all the problem instances $A,B$, and $C$.
		Then, there exists a time horizon $T$ such that $\reg_A(T) > \nicefrac{(\reg_B(T) + \reg_C(T))}{2}$.
	\end{claim}
	\begin{proof}[Proof of the claim]	
	Define $s_1 = 1$.
	For any integer $i \ge 2$, let $s_i$ denote the minimum integer satisfying
%	\begin{align*}
%		1 + f(s_i + i, s_i) < 0 + f(s_i + i, i)	
%	\end{align*}
	\begin{align*}
		1 + \sqrt{\frac{\ln(s_i + i)}{s_i}} 
		< 0 + \sqrt{\frac{\ln(s_i + i)}{i}}.
	\end{align*}
	Such $s_i$ exists for any $i \ge 2$ since LHS is a decreasing function of $s_i$ which goes to $1$ as $s_i$ increases and RHS is an increasing function of $s_i$ which goes to $\infty$ as $s_i$ increases, and putting $s_i = i$ yields that LHS is larger than RHS.
	Further, it is easy to check that $s_i > s_j$ if $i > j$ and $s_i \ge i$.
	
	Due to our construction of the sequence $s_i$, in $A$, arm with mean $1$ is selected exactly $s_i$ times and then arm with mean $0$ is selected for a single round, and it repeats for $i=1,2,\ldots$.
	Figure~\ref{fig:single-bad} illustrates this bandit instances.
	As can be seen in the figure, the bandit process in $A$ can be described as
	\begin{align*}
		(1:s_1, 0:1, 1:s_2, 0:1, 1:s_3, 0:1, \ldots),
	\end{align*}
	where in each element of $x:y$ denotes that arm with mean $x$ is selected $y$ times.
	Likewise, in $B$, we have
	\begin{align*}
		(1:s_1, 1':s_1, 0:1, [1:s_2, 1':s_2], 0:1, [1:s_3, 1':s_3], 0:1, \ldots),
	\end{align*}
	where for each element in $[\cdot]$, we ignore the orders how $1$ and $1'$ are selected, but aggregate them to only present the total number of times each one is selected before getting to the arm $0$.
	For $C$, we have
	\begin{align*}
		(1:s_1, [0:1, 0':1], 1:s_2, [0:1, 0':1], 1:s_3, [0:1, 0':1], \ldots).
	\end{align*}
	Set $T = s_1 + 2 + s_2$.
	Given $T$, in $A$, the arm $0$ is selected twice.
	In $B$, the arm $0$ is selected once.
	In $C$, the arm $0$ is selected once, and also $0'$ is selected once.
	Hence, at round $t=T$, $\reg_A(T) = 2 > \frac{1+ 2}{2} = \frac{\reg_B(T) + \reg_C(T)}{2}$,
	and it completes the proof.
	\end{proof}
	Set $T$ as defined in the claim above.
	% In the single-agent setting, given any realization $E = (\mu_1, \mu_2)$ with $\mu_1 \ge \mu_2$, note that an agent's ex-ante utility can be easily derived from his ex-post regret as follows.
	% \begin{align*}
	% 	U(\set{S};E) = \mu_1 N_1(T) + \mu_2 N_2(T) = 
	% 	\mu_1 T - (\mu_1 - \mu_2)N_2(T) =  \max_{a \in E}\mu_a \cdot T - \reg_E(T).
	% \end{align*}
	Finally, we can decompose the agent's ex-ante utility as follows.
	\begin{align*}
		u(\set{O}) 
		= 
		\frac{1}{4}\parans{\sum_{i=1}^4U(\set{O};E_i)}
		&=
		\frac{1}{4}\parans{\sum_{i=1,4}U(\set{O};E_i)} + \frac{1}{4}\parans{\sum_{i=2,3}U(\set{S};E_i)}
		\\
		&=
		\frac{1}{4}\parans{\sum_{i=1,4} \parans{\max_{a \in E_i}\mu_a \cdot T - \reg_{E_i}(T)}}
		+
		\frac{1}{4}\parans{\sum_{i=2,3} \parans{\max_{a \in E_i}\mu_a \cdot T - \reg_{E_i}(T)}}
		\\
		&=
            \frac{T - \reg_A(T)}{2}
		\\
		&<
		\frac{T - (\reg_B(T) + \reg_C(T))/2}{2}
		\\
		&=
		\frac{1}{4}\parans{\sum_{i=1,4}U(\set{S};E_i)} + \frac{1}{4}\parans{\sum_{i=2,3}U(\set{S};E_i)}
		\\
		&= u(\set{S}),
	\end{align*}
	and thus $\set{S}$ yields the strictly larger ex-ante utility, and it concludes the proof.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:hucb_negative}]
	If there exists only a single agent, it is easy to see that the dynamics of the algorithm reduces to standard UCB1.
	Thus, by Theorem~\ref{thm:ucb_negative}, H-UCB is not replication-proof.
	Now we consider multiple agents with $n \ge 2$.
	We only show for the case $n=2$ since it easily extends to the cases with $n \ge 3$.
	Without loss of generality, we assume that the algorithm breaks tie uniformly at random in both phases $1$ and $2$.
	Suppose that agent $1$ has two deterministic arms sampled from $D$ in which the mean reward is $c \in [0,1]$ with probability $0.5$, and $0$ otherwise, for some $c>0$.
	We further assume that agent $2$ is equipped with a deterministic prior $D_i$ supported on $\mu$, and the arm also deterministically outputs reward $\mu$.
	Our choice of $\mu$ will be determined later, which will be selected in order to propagate the single-agent failure to the two-agent cases.
	Especially, we will focus on the round that agent $1$ is selected exactly $s_1+s_2+2$ times, as defined in the proof of Theorem~\ref{thm:ucb_negative}.
	Note that the bandit process is deterministic for any realization of the arms' parameters.
	
	We consider a truthful strategy $\cO$ of registering both arms, and another strategy $\cS$ of replicating only a single arm, and focus on the difference on the agent's expected utility between two strategies.
	If the agent samples $c$ or $0$ both the arms, then the rewards of the bandit process and the agent's ex-post utility therein will be indifferent.
	Thus, we only focus on the remaining case.
	Suppose that agent $1$ samples $c$ for one arm and $0$ for the other, which occurs with probability $1/2$.
	Similar to the proof of Claim~\ref{cl:neg_ucb}, we consnider the following list of bandit problem instances with deterministic arms.
	\begin{itemize}
		\item Let $A$ be a bandit instance with $\cI_A = (c,0)$.
		\item Let $B$ be a bandit instance with $\cI_B = (c,c',0)$.
		\item Let $C$ be a bandit instance with $\cI_C = (c,0,0')$.
	\end{itemize}
	% \note{Some figure may help}
	Each element in $\cI$ denotes the sequence of mean reward of Bernoulli arms, where we write $c'$ and $0'$ to distinguish the arms with same mean.
	We simply say arm $c$ and arm $0$ to denote the arm with the corresponding parameter $c$ and $0$, respectively.
	Then, the realization of the agent $1$'s arms in playing strategy $\cS$ corresponds to either of bandit instance $B$ or $C$, and strategy $\cO$ corresponds to the bandit instance $A$.
	Let us abuse the notation of $s_1,s_2,\ldots$ defined in the proof of Claim~\ref{cl:neg_ucb}, so that it denotes the number of rounds that arm $c$ is selected consecutively before arm $0$ is sampled $i$-th time, in problem instance $A$.
	Also, we use $R_t(i)$ and $N_t(i)$ to denote the quantity of $R(i)$ and $N(i)$ at round $t$.
	
	Given the random bits of the tie-breaking rule used by the algorithm, let $\tau^{i}_1,\tau^i_2,\ldots, \tau^i_{k}, \ldots$ be the rounds that agent $1$ is sampled $k$ times when the mean rewards of the agent $1$'s arms are realized to be $i= A,B,C$.
	It is straightforward to check that $\tau^{B}_t \le \tau^{A}_t \le \tau^{C}_t$\footnote{This can  be shown using the coupling technique introduced in \cite{shin2022multi}.}.
	Let $k = s_1+s_2+2$, and following the argument of Claim~\ref{cl:neg_ucb}, we observe that at round $\tau^{B}_k$, agent $1$'s empirical mean rewards by playing $\cS$ will be either of (i) $\frac{c(s_1+s_2)}{s_1+s_2+2}$ or (ii) $\frac{c(s_1+s_2+1)}{s_1+s_2+2}$ based on whether the arms are realized to be instance $B$ or $C$.
	By playing $\cO$, agent $1$ simply has empirical mean reward of $\frac{c(s_1+s_2)}{s_1+s_2+2}$ at round $\tau^{A}_k$.
	Furthermore, if $\tau^{B}_k < \tau^{A}_k$, then in problem instance $A$, it means that the agents' parameters at round $\tau^{B}_k$ satisfy
	\begin{align*}
		R_{\tau^B_k}(1) + \sqrt{\frac{2\ln(t)}{k-1}}
		<
		R_{\tau^B_k}(2) + \sqrt{\frac{2\ln(t)}{\tau^B_k - k}},
	\end{align*}
	where $R_t(i)$ denotes the empirical average reward of agent $i$ at round $t$,  $R_{\tau^B_k}(1) = \frac{c(s_1+s_2)}{s_1+s_2+2}$ and $R_{\tau^B_k}(2) = \mu$.
	However, from our construction of the variables and the fact that H-UCB selects agent $1$ at round $\tau^{B}_k$ in $B$, we know that
	\begin{align*}
		\frac{c(s_1+s_2)}{s_1+s_2+2} + \sqrt{\frac{2\ln(t)}{k-1}}
		\ge
		\mu + \sqrt{\frac{2\ln(t)}{\tau^B_k - k}},
	\end{align*}
	and thus $\tau^A_k$ and $\tau^B_k$ needs to be exactly equivalent.
	Similarly, for instance $C$, since arm $c$ and $c'$ are selected the same number of times at the beginning of round $\tau^B_k$, we conclude that $\tau^i_k$ are equivalent for $i=A,B,C$.
	
	Now define $\theta = \sqrt{\frac{2\ln(t)}{k}} - \sqrt{\frac{2\ln(t)}{\tau^B_k-k}}$ and we pick any $\mu \in (\frac{c(s_1+s_2)}{s_1+s_2+2} + \theta,\frac{c(s_1+s_2+1)}{s_1+s_2+2} + \theta)$.
%	We claim that there exists a choice of parameters $c$ that such $\mu$ always exist.
%	\begin{claim}
%		There exists  $c>0$ such that the interval $\mu \in (\frac{c(s_1+s_2)}{s_1+s_2+2} + C_1,\frac{c(s_1+s_2+1)}{s_1+s_2+2} + C_2)$ is well-defined.
%	\end{claim}
%	\begin{proof}
%		It suffices to show that 
%		\begin{align*}
%			\sqrt{\frac{f(t)}{k-1}} - \sqrt{\frac{f(t)}{k}} < \frac{c}{s_1+s_2+2}.
%		\end{align*}
%		Note that all $k = s_1+s_2+2$,$s_1$ and $s_2$ are in fact functions of $c$.
%		Define $s = s_1+s_2$ and rearrange the inequality, we obtain 
%		\begin{align*}
%			\sqrt{f(t)}\parans{\frac{\sqrt{s+2} - \sqrt{s+1}}{\sqrt{(s+1)(s+2)}}}
%			<
%			\frac{c}{s+2}.
%		\end{align*}
%		Define $x = \sqrt{s+1}$ and rearrange again, it suffices to show that
%		\begin{align*}
%			\sqrt{f(t)}\parans{x+\frac{1}{x}-1} \le c,
%		\end{align*}
%		for some $c$.
%		Since LHS is at most 
%		
%
%
%		
%		When we increase the value of $c$, it is easy to see that  
%		
%		By making $c$ sufficiently large, we
%
%	\end{proof}

	
	Then, at round $\tau^B_k+1$, for bandit instance $A$ and $C$, we observe that agent $2$ will be selected since
	\begin{align*}
		R_{\tau^B_k+1}(2) + \sqrt{\frac{2\ln(t)}{N_{\tau^B_k}(2)}}
		&=
		\mu + \sqrt{\frac{2\ln(t)}{\tau^B_k - k}}
		\\
		&>
		\frac{s_1+s_2}{s_1+s_2+2} + \theta + \sqrt{\frac{2\ln(t)}{\tau^B_k - k}}
		\\
		&=
		\frac{s_1+s_2}{s_1+s_2+2} + \sqrt{\frac{2\ln(t)}{k}}
		= 
		R_{\tau^B_k+1}(1) + \sqrt{\frac{2\ln(t)}{N_{\tau^B_k}(1)}}.
	\end{align*}
	For bandit instance $C$, however, observe that
	\begin{align*}
		R_{\tau^C_k+1}(2) + \sqrt{\frac{2\ln(t)}{N_{\tau^C_k}(2)}}
		&=
		\mu + \sqrt{\frac{2\ln(t)}{\tau^C_k - k}}
		\\
		&<
		\frac{s_1+s_2+1}{s_1+s_2+2} + \theta + \sqrt{\frac{2\ln(t)}{\tau^C_k - k}}
		\\
		&=
		\frac{s_1+s_2+1}{s_1+s_2+2} + \sqrt{\frac{2\ln(t)}{k}} 
		=
		R_{\tau^C_k+1}(1) + \sqrt{\frac{2\ln(t)}{N_{\tau^C_k}(1)}},
	\end{align*}
	and thus arm $1$ is selected.
	This essentially implies that by setting $T = \tau_k^A+1$, agent $1$ is selected at round $T$ with probability $1/4$ if he plays $\cS$, is never selected if he plays $\cO$, where the probability $1/4$ comes from the fact that problem instance $C$ is realized with probability $1/4$.
	Thus, agent $1$'s expected utility becomes larger for such $T$ by replicating one of its arm, and we finish the proof.
%
%
%	
%	Note that each $\tau_i$ depends on agent $2$'s reward $\mu$.
%	Define the sequence $s_1,s_2,\ldots$ and the problem instance $A,B$, and $C$ as we did in the proof of Claim~\ref{cl:neg_ucb}.
%	Following the argument of Claim~\ref{cl:neg_ucb}, we observe that at round $\tau_i$ with $i = s_1+2+s_2$, agent $1$'s ex-post regret is strictly larger on problem instance $A$, compared to the average of that of $B$ and $C$.
%	This essentially implies that at round $\tau_i$, agent $1$'s empirical mean reward becomes exactly larger in strategy $\cS'$.
%	
%	Now we pick any $\mu \in (\frac{s_1+s_2}{s_1+s_2+2},\frac{s_1+s_2+1}{s_1+s_2+2})$.
%	Then, in problem instance $A$, at round $\tau$
	
%	
%	\note{Suho - TBD - need to be fixed}
%	
%	Consider two symmetric agents $a$ and $b$ with two deterministic arms of $1$ and $\eps$.
%	Denote the agent $a$'s arm by $1_a$ and $\eps_a$, and similarly for agent $b$.
%	Let $(s_i)_{i\in \N}$ be the sequence defined in the proof of Theorem~\ref{thm:ucb_negative}.
%	Set $T = 2(s_1+2+s_2) + 1$.
%	Suppose that both the agents truthfully register.
%	Up to round $t=T-1$, due to the deterministic nature of the arms, both agents are selected $s_1+2+s_2$ times, and their agent-wise average rewards are $R(a) = R(b) = 1 - \frac{2\eps}{s_1+2+s_2}$.
%	Thus, at round $t=T$, the selected agent will be based on the tie-breaking rule of H-UCB.
%	On the other hand, suppose that agent $a$ replicates one of the arms randomly.
%	Then, by the observation in the proof of Theorem~\ref{thm:ucb_negative}, the average reward of agent $a$ at round $t=T-1$ will be $R(a) = 1 - \frac{\eps}{s_1+2+s_2}$ if arm $1$ is replicated.
%	Otherwise if arm $\eps$ is replicated, then $R(a) = 1 - \frac{2\eps}{s_1+2+s_2}$.
%	In the former case, agent $a$ will be deterministically selected as it satisfies $R(a) > R(b)$.
%	In the latter case, the tie-breaking rule determines whom to select.
%	This implies that the average reward of replicating both arms is larger, and thus $H-UCB$ is not replication-proof.
\end{proof}
	





